The Panchromatic Hubble Andromeda Treasury: Triangulum Extended Region (PHATTER). III. The Mass Function of Young Star Clusters in M33

We measure the star cluster mass function for the Local Group galaxy M33. We use the catalog of stellar clusters selected from the Panchromatic Hubble Andromeda Treasury: Triangulum Extended Region (PHATTER) survey. We analyze 711 clusters in M33 with $\rm 7.0 < log(Age/yr) < 8.5$, and log($M/M_{\odot}$) $>$ 3.0 as determined from color-magnitude diagram fits to individual stars. The M33 cluster mass function is best described by a Schechter function with power law slope $\alpha = -2.06^{+0.14}_{-0.13}$, and truncation mass log($M_c/M_{\odot}$) $= 4.24^{+0.16}_{-0.13}$. The data show strong evidence for a high-mass truncation, thus strongly favoring a Schechter function fit over a pure power law. M33's truncation mass is consistent with the previously identified linear trend between $M_c$, and star formation rate surface density, \SigSFR. We also explore the effect that individual cluster mass uncertainties have on derived mass function parameters, and find evidence to suggest that large cluster mass uncertainties have the potential to bias the truncation mass of fitted mass functions on the one sigma level.

==> Tables/Catalog_to_go_in_paper.tex <==
\begin{table}
\begin{tabular}{ccccccccccccccc}
ID & NMS & Exclude_Flag & Age_16 & Age_50 & Age_84 & Bestfit_Age & Mass_16 & Mass_50 & Mass_84 & Bestfit_Mass & AV_16 & AV_50 & AV_84 & Bestfit_AV \\
1 & 293 & 0.0 & 8.009605023529451 & 8.03894250474452 & 8.078837471018483 & 8.0 & 3.755490064962947 & 3.7735059910493742 & 3.7915219171358014 & 3.7631452770987077 & 0.1077875279437066 & 0.12488001090737118 & 0.14197249387103575 & 0.1 \\
2 & 796 & 0.0 & 8.12003348271561 & 8.220472794448611 & 8.288588953455283 & 8.1 & 3.5551047880787787 & 3.5866532510375784 & 3.6275382575798503 & 3.56258769120407 & 0.2966299782098811 & 0.3410278006717265 & 0.4331018898437723 & 0.4 \\
3 & 796 & 0.0 & 8.341324241591872 & 8.377786452208865 & 8.41877879775763 & 8.4 & 3.4082436792720787 & 3.4298474366502414 & 3.456246227678518 & 3.447964687303943 & 0.2630721136739471 & 0.29241519036929575 & 0.3378525726373925 & 0.3 \\
4 & 530 & 0.0 & 8.90798297704941 & 8.924989867291316 & 8.941996757533222 & 8.95 & 4.054306400657874 & 4.088231275409505 & 4.129060449734598 & 4.094061959212958 & 0.11900014180141993 & 0.23651489023928157 & 0.2996692713096015 & 0.2 \\
5 & 587 & 0.0 & 8.30815295603286 & 8.325492850068072 & 8.342832744103285 & 8.3 & 4.159840243866336 & 4.180786301771877 & 4.207473943764834 & 4.191499485146169 & 0.5599672025777305 & 0.581189857294868 & 0.6597281758171524 & 0.6 \\
\end{tabular}
\end{table}


==> references.tex <==
%Dummy call for Catalog paper XXX Fix Later XXX
@article{johnson_catalog_2022,
	title = {The {Panchromatic} {Hubble} {Andromeda} {Treasury}: {Triangulum} {Extended} {Region} ({PHATTER}) {IV}. {Local} {Group} {Cluster} {Search} {Star} {Cluster} {Catalog}},
	journal = {submitted to AAS Journals},
	author = {Johnson, L. Clifton and Wainer, Tobin M. and TorresVillanueva, Estephani E. and Seth, Anil C. and Dalcanton, Julianne J. and Williams, Benjamin F.},
	year = {2022}
}

@article{messa_looking_2021,
	title = {Looking for {Obscured} {Young} {Star} {Clusters} in {NGC} 1313},
	volume = {909},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2021ApJ...909..121M},
	doi = {10.3847/1538-4357/abe0b5},
	abstract = {Using recently acquired Hubble Space Telescope NIR observations (J, Pa$\beta$, and H bands) of the nearby galaxy NGC 1313, we investigate the timescales required by a young star cluster to emerge from its natal cloud. We search for extincted star clusters, potentially embedded in their natal cloud as either (1) compact sources in regions with high H$\alpha$/Pa$\beta$ extinctions or (2) compact H II regions that appear as point-like sources in the Pa$\beta$ emission map. The NUV-optical-NIR photometry of the candidate clusters is used to derive their ages, masses, and extinctions via a least-$\chi$2 spectral energy distribution broad- and narrowband fitting process. The 100 clusters in the final samples have masses in the range \$\{{\textbackslash}mathrm\{log\}\}\_\{10\}(M/\{M\}\_\{{\textbackslash}odot \})=2.5{\textbackslash}mbox\{--\}3.5\$ and moderate extinctions, E(B - V) ? 1.0 mag. Focusing on the young clusters (0-6 Myr), we derive a weak correlation between extinction and age of the clusters. Almost half of the clusters have low extinctions, E(B - V) {\textless} 0.25 mag, already at very young ages (<=3 Myr), suggesting that dust is quickly removed from clusters. A stronger correlation is found between the morphology of the nebular emission (compact, partial or absent, both in H$\alpha$ and Pa$\beta$) and cluster age. Relative fractions of clusters associated with a specific nebular morphology are used to estimate the typical timescales for clearing the natal gas cloud, resulting in between 3 and 5 Myr, \~{}1 Myr older than what was estimated from NUV-optical-based cluster studies. This difference hints at a bias for optical-only-based studies, which James Webb Space Telescope will address in the coming years.},
	urldate = {2022-02-01},
	journal = {The Astrophysical Journal},
	author = {Messa, Matteo and Calzetti, Daniela and Adamo, Angela and Grasha, Kathryn and Johnson, Kelsey E. and Sabbi, Elena and Smith, Linda J. and Bajaj, Varun and Finn, Molly K. and Lin, Zesen},
	month = mar,
	year = {2021},
	note = {ADS Bibcode: 2021ApJ...909..121M},
	keywords = {1560, 1569, 1833, 286, 837, Astrophysics - Astrophysics of Galaxies, Compact H II region, Interstellar dust extinction, Spiral galaxies, Star formation, Young star clusters},
	pages = {121},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/2TZQD4UY/Messa et al. - 2021 - Looking for Obscured Young Star Clusters in NGC 13.pdf:application/pdf},
}

@article{lieberz_origin_2017,
	title = {On the origin of the {Schechter}-like mass function of young star clusters in disc galaxies},
	volume = {465},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.3775L},
	doi = {10.1093/mnras/stw2953},
	abstract = {The mass function of freshly formed star clusters is empirically often described as a power law. However, the cluster mass function of populations of young clusters over the scale of a galaxy has been found to be described by a Schechter-function. Here we address this apparent discrepancy. We assume that in an annulus of an isolated self-regulated radially exponential axially symmetric disc galaxy, the local mass function of very young (embedded) clusters is a power law with an upper mass limit which depends on the local star formation rate density. Radial integration of this mass function yields a galaxy-wide embedded cluster mass function. This integrated embedded cluster mass function has a Schechter-type form, which results from the addition of many low-mass clusters forming at all galactocentric distances and rarer massive clusters only forming close to the centre of the galaxy.},
	urldate = {2022-01-19},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Lieberz, P. and Kroupa, P.},
	month = mar,
	year = {2017},
	note = {ADS Bibcode: 2017MNRAS.465.3775L},
	keywords = {galaxies: star clusters: general, galaxies: stellar content, mass function, stars: formation, stars: luminosity function, stars: statistics},
	pages = {3775--3783},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/CXT9LF9F/Lieberz and Kroupa - 2017 - On the origin of the Schechter-like mass function .pdf:application/pdf},
}

@article{u_new_2009,
	title = {A {New} {Distance} to {M33} {Using} {Blue} {Supergiants} and the {FGLR} {Method}},
	volume = {704},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2009ApJ...704.1120U},
	doi = {10.1088/0004-637X/704/2/1120},
	abstract = {The quantitative spectral analysis of medium resolution optical spectra of A and B supergiants obtained with DEIMOS and ESI at the Keck Telescopes is used to determine a distance modulus of 24.93 {\textpm} 0.11 mag (968 {\textpm} 50 kpc) for the Triangulum Galaxy M33. The analysis yields stellar effective temperatures, gravities, interstellar reddening, and extinction, the combination of which provides a distance estimate via the flux-weighted gravity-luminosity relationship (FGLR). This result is based on an FGLR calibration that is continually being polished. An average reddening of langE(B - V)rang {\textasciitilde} 0.08 mag is found, with a large variation ranging from 0.01 to 0.16 mag, however, demonstrating the importance of accurate individual reddening measurements for stellar distance indicators in galaxies with evident signatures of interstellar absorption. The large-distance modulus found is in good agreement with recent work on eclipsing binaries, planetary nebulae, long-period variables, RR Lyrae stars, and also with Hubble Space Telescope (HST) observations of Cepheids, if reasonable reddening assumptions are made for the Cepheids. Since distances based on the tip of the red giant branch (TRGB) method found in the literature give conflicting results, we have used HST Advanced Camera for Surveys V- and I-band images of outer regions of M33 to determine a TRGB distance of 24.84 {\textpm} 0.10 mag, in basic agreement with the FGLR result. We have also determined stellar metallicities and discussed the metallicity gradient in the disk of M33. We find metallicity of Z sun at the center and 0.3 Z sun in the outskirts at a distance of one isophotal radius. The average logarithmic metallicity gradient is -0.07 {\textpm} 0.01 dex kpc-1. However, there is a large scatter around this average value, very similar to what has been found for the H II regions in M33.},
	urldate = {2022-01-07},
	journal = {The Astrophysical Journal},
	author = {U, Vivian and Urbaneja, Miguel A. and Kudritzki, Rolf-Peter and Jacobs, Bradley A. and Bresolin, Fabio and Przybilla, Norbert},
	month = oct,
	year = {2009},
	note = {ADS Bibcode: 2009ApJ...704.1120U},
	keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, galaxies: distances and redshifts, galaxies: individual: M33, stars: abundances, stars: early-type, supergiants},
	pages = {1120--1134},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/3PZVVZ2S/U et al. - 2009 - A New Distance to M33 Using Blue Supergiants and t.pdf:application/pdf},
}

@article{kass_bayes_1995,
	title = {Bayes {Factors}},
	volume = {90},
	issn = {0162-1459},
	url = {https://www.jstor.org/stable/2291091},
	doi = {10.2307/2291091},
	abstract = {In a 1935 paper and in his book Theory of probability, Jeffresy developed a methodology for quantifying the evidence in favor of a scientific theory. The centerpies was a number, now called the Bayes factor, which is the posterior odds of the null hypothesis when the prior probability on the null is one-half. Although there has been much discussion of Bayesian hypothesis testing in the context of criticism of P-values, less attention has been given to the Bayes as a practical tool of applied statistics. In this article we review and discuss the uses of Bayes factors in the context of five scientific applications in genetics, sports, ecology, sociology, and psychology. We emphasize the following points: From Jeffrey's Bayesian viewpoint, the purpose of hypothesis testing is to evaluate the evidence in favor of a scientific theory. Bayes factors offer a way of evaluating evidence in favor of a null hypothesis. Bayes factors provide a way of incorporating external information into the evaluation of evidence about a hypothesis. Bayes factors are very general and do not require alternative models to be nested. Several techniques are available for computing Bayes factors, including asymptotic approximations that are easy to compute using the output from standard packages that maximize likelihoods. In "non-Bayesian significance tests. The Schwarz criterion (or BIC) gives a rough approximation to the logarithm of the Bayes factor, which is easy to use and does not require evaluation of prior distributions. When one is interested in estimation or prediction, Bayes factors may be converted to weights to be attached to various models so that a composite estimate or prediction may be obtained that takes account of structural or model uncertainty. Algorithms have been proposed that allow model uncertainty to be taken into account when the class of models initially considered is very large. Bayes factors are useful for guiding an evolutionary model-building process. It is important, and feasible, to assess the sensitivity of conclusions to the prior distributions used.},
	number = {430},
	urldate = {2022-01-05},
	journal = {Journal of the American Statistical Association},
	author = {Kass, Robert E. and Raftery, Adrian E.},
	year = {1995},
	note = {Publisher: [American Statistical Association, Taylor \& Francis, Ltd.]},
	pages = {773--795},
}

@article{whitmore_legus_2020,
	title = {{LEGUS} and {H$\alpha$}-{LEGUS} {Observations} of {Star} {Clusters} in {NGC} 4449: {Improved} {Ages} and the {Fraction} of {Light} in {Clusters} as a {Function} of {Age}},
	volume = {889},
	issn = {0004-637X},
	shorttitle = {{LEGUS} and {H$\alpha$}-{LEGUS} {Observations} of {Star} {Clusters} in {NGC} 4449},
	url = {https://ui.adsabs.harvard.edu/abs/2020ApJ...889..154W},
	doi = {10.3847/1538-4357/ab59e5},
	abstract = {We present a new catalog and results for the cluster system of the starburst galaxy NGC 4449, based on multiband imaging observations taken as part of the LEGUS and H$\alpha$-LEGUS surveys. We improve the spectral energy fitting method used to estimate cluster ages, and find that the results, particularly for older clusters, are in better agreement with those from spectroscopy. The inclusion of H$\alpha$ measurements, the role of stochasticity for low-mass clusters, the assumptions about reddening, and the choices of SSP model and metallicity all have important impacts on the age dating of clusters. A comparison with ages derived from stellar color-magnitude diagrams for partially resolved clusters shows reasonable agreement, but large scatter in some cases. The fraction of light found in clusters relative to the total light (I.e., TL) in the U, B, and V filters in 25 different ? kiloparsec-size regions throughout NGC 4449 correlates with both the specific region luminosity, RL, and the dominant age of the underlying stellar population in each region. The observed cluster age distribution is found to decline over time as dN/d$\tau$ ? $\tau$$\gamma$, with $\gamma$ = -0.85 {\textpm} 0.15, independent of cluster mass, and is consistent with strong, early cluster disruption. The mass functions of the clusters can be described by a power law with dN/dM ? M$\beta$ and $\beta$ = -1.86 {\textpm} 0.2, independent of cluster age. The mass and age distributions are quite resilient to differences in age-dating methods. There is tentative evidence for a factor of 2-3 enhancement in both the star and cluster formation rate ?100-300 Myr ago, indicating that cluster formation tracks star formation generally. The enhancement is probably associated with an earlier interaction event.},
	urldate = {2021-12-09},
	journal = {The Astrophysical Journal},
	author = {Whitmore, Bradley C. and Chandar, Rupali and Lee, Janice and Ubeda, Leonardo and Adamo, Angela and Aloisi, Alessandra and Calzetti, Daniela and Cignoni, Michele and Cook, David and Dale, Daniel and Elmegreen, B. G. and Gouliermis, Dimitrios and Grebel, Eva K. and Grasha, Kathryn and Johnson, Kelsey E. and Kim, Hwihyun and Sacchi, Elena and Smith, Linda J. and Tosi, Monica and Wofford, Aida},
	month = feb,
	year = {2020},
	note = {ADS Bibcode: 2020ApJ...889..154W},
	keywords = {1567, 2049, 417, 621, 656, Astrophysics - Astrophysics of Galaxies},
	pages = {154},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/BIN3BD53/Whitmore et al. - 2020 - LEGUS and H$\alpha$-LEGUS Observations of Star Clusters i.pdf:application/pdf},
}

@article{berg_chaos_2015,
	title = {{CHAOS} {I}. {Direct} {Chemical} {Abundances} for {H} {II} {Regions} in {NGC} 628},
	volume = {806},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806...16B},
	doi = {10.1088/0004-637X/806/1/16},
	abstract = {The CHemical Abundances of Spirals (CHAOS) project leverages the combined power of the Large Binocular Telescope (LBT) with the broad spectral range and sensitivity of the Multi Object Double Spectrograph (MODS) to measure {\textquotedblleft}direct{\textquotedblright} abundances (based on observations of the temperature-sensitive auroral lines) in large samples of H ii regions in spiral galaxies. We present LBT MODS observations of 62 H ii regions in the nearby spiral galaxy NGC 628, with an unprecedentedly large number of auroral lines measurements (18 [O iii] $\lambda$4363, 29 [N ii] $\lambda$5755, 40 [S iii]$\lambda$6312, and 40 [O ii] $\lambda$$\lambda$7320, 7330 detections) in 45 H ii regions. Comparing derived temperatures from multiple auroral line measurements, we find: (1) a strong correlation between temperatures based on [S iii] $\lambda$6312 and [N ii] $\lambda$5755 and (2) large discrepancies for some temperatures based on [O ii] $\lambda$$\lambda$7320, 7330 and [O iii] $\lambda$4363. Both of these trends are consistent with other observations in the literature, yet, given the widespread use and acceptance of [O iii] $\lambda$4363 as a temperature determinant, the magnitude of the T[O iii] discrepancies still came as a surprise. Based on these results, we conduct a uniform abundance analysis prioritizing the temperatures derived from [S iii] $\lambda$6312 and [N ii] $\lambda$5755, and report the gas-phase abundance gradients for NGC 628. Relative abundances of S/O, Ne/O, and Ar/O are constant across the galaxy, consistent with no systematic change in the upper IMF over the sampled range in metallicity. These alpha-element ratios, along with N/O, all show small dispersions ($\sigma$ \~{} 0.1 dex) over 70\% of the azimuthally averaged radius. We interpret these results as an indication that, at a given radius, the interstellar medium in NGC 628 is chemically well-mixed. Unlike the gradients in the nearly temperature-independent relative abundances, O/H abundances have a larger intrinsic dispersion of \~{}0.165 dex. We posit that this dispersion represents an upper limit to the true dispersion in O/H at a given radius and that some of that dispersion is due to systematic uncertainties arising from temperature measurements.},
	urldate = {2021-10-29},
	journal = {The Astrophysical Journal},
	author = {Berg, Danielle A. and Skillman, Evan D. and Croxall, Kevin V. and Pogge, Richard W. and Moustakas, John and Johnson-Groh, Mara},
	month = jun,
	year = {2015},
	note = {ADS Bibcode: 2015ApJ...806...16B},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: abundances, galaxies: evolution, galaxies: individual: NGC 628, galaxies: ISM, galaxies: spiral, ISM: lines and bands},
	pages = {16},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/CDPK7TX8/Berg et al. - 2015 - CHAOS I. Direct Chemical Abundances for H II Regio.pdf:application/pdf},
}


@article{mok_constraints_2019,
	title = {Constraints on {Upper} {Cutoffs} in the {Mass} {Functions} of {Young} {Star} {Clusters}},
	volume = {872},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872...93M},
	doi = {10.3847/1538-4357/aaf6ea},
	abstract = {We test claims that the power-law mass functions of young star clusters (ages ? few {\texttimes} 108 yr) have physical upper cutoffs at \{M\}* \~{} \{10\}5 \{M\}? . Specifically, we perform maximum likelihood fits of the Schechter function, {\textbackslash}psi (M)=\{dN\}/\{dM\}{\textbackslash}propto \{M\}$\beta$ {\textbackslash}exp (-M/\{M\}* ), to the observed cluster masses in eight well-studied galaxies (LMC, SMC, NGC 4214, NGC 4449, M83, M51, Antennae, and NGC 3256). In most cases, we find that a wide range of cutoff masses is permitted (\{10\}5 \{M\}? ? \{M\}* {\textless} $\infty$ ). We find a weak detection at \{M\}* \~{} \{10\}5 \{M\}? in one case (M51) and strong evidence against this value in two cases. However, when we include realistic errors in cluster masses in our analysis, the constraints on M * become weaker and there are no significant detections (even for M51). Our data are generally consistent with much larger cutoffs, at \{M\}* \~{} \{few\}{\texttimes} \{10\}6 \{M\}? . This is the predicted cutoff from dynamical models in which old globular clusters and young clusters observed today formed by similar physical processes with similar initial mass functions.},
	urldate = {2021-10-27},
	journal = {The Astrophysical Journal},
	author = {Mok, Angus and Chandar, Rupali and Fall, S. Michael},
	month = feb,
	year = {2019},
	note = {ADS Bibcode: 2019ApJ...872...93M},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star clusters: general, stars: formation},
	pages = {93},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/XLAEJEVL/Mok et al. - 2019 - Constraints on Upper Cutoffs in the Mass Functions.pdf:application/pdf},
}

@article{longmore_formation_2014,
	address = {eprint: arXiv:1401.4175},
	title = {The {Formation} and {Early} {Evolution} of {Young} {Massive} {Clusters}},
	url = {https://ui.adsabs.harvard.edu/abs/2014prpl.conf..291L},
	abstract = {We review the formation and early evolution of the most massive ({\textgreater} few 104 M?) and dense (radius of a few parsecs) young stellar clusters, focusing on the role that studies of these objects in our Galaxy can play in our understanding of star and planet formation as a whole. Comparing the demographics of young massive cluster (YMC) progenitor clouds and YMCs across the Galaxy shows that gas in the Galactic Center can accumulate to a high enough density that molecular clouds already satisfy the criteria used to define YMCs, without forming stars. In this case formation can proceed in situ {\textemdash} i.e., the stars form at protostellar densities close to the final stellar density. Conversely, in the disk, the gas either begins forming stars while it is being accumulated to high density, in a "conveyor belt" mode, or the timescale to accumulate the gas to such high densities must be much shorter than the star-formation timescale. The distinction between the formation regimes in the two environments is consistent with the predictions of environmentally dependent density thresholds for star formation. This implies that stars in YMCs of similar total mass and radius can have formed at widely different initial protostellar densities. The fact that no strong, systematic variations in fundamental properties (such as the IMF) are observed between YMCs in the disk and Galactic Center suggests that, statistically speaking, stellar mass assembly is not affected by the initial protostellar density. We then review recent theoretical advances and summarize the debate on three key open questions: the initial (proto)stellar distribution, infant (im)mortality, and age spreads within YMCs. We conclude that (1) the initial protostellar distribution is likely hierarchical, (2) YMCs likely experienced a formation history that was dominated by gas exhaustion rather than gas expulsion, (3) YMCs are dynamically stable from a young age, and (4) YMCs have age spreads much smaller than their mean age. Finally, we show that it is plausible that metal-rich globular clusters may have formed in a similar way to YMCs in nearby galaxies. In summary, the study of YMC formation bridges star/planet formation in the solar neighborhood to the oldest structures in the local universe.},
	urldate = {2021-10-19},
	author = {Longmore, S. N. and Kruijssen, J. M. D. and Bastian, N. and Bally, J. and Rathborne, J. and Testi, L. and Stolte, A. and Dale, J. and Bressert, E. and Alves, J.},
	month = jan,
	year = {2014},
	note = {Conference Name: Protostars and Planets VI
Pages: 291
ADS Bibcode: 2014prpl.conf..291L},
	keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/XGIAA9RS/Longmore et al. - 2014 - The Formation and Early Evolution of Young Massive.pdf:application/pdf},
}

@article{portegies_zwart_young_2010,
	title = {Young {Massive} {Star} {Clusters}},
	volume = {48},
	issn = {0066-4146},
	url = {https://ui.adsabs.harvard.edu/abs/2010ARA%26A..48..431P/abstract},
	doi = {10.1146/annurev-astro-081309-130834},
	abstract = {Young massive clusters (YMCs) are dense aggregates of young stars that form the fundamental building blocks of galaxies. Several examples exist in the Milky Way Galaxy and the Local Group, but they are particularly abundant in starburst and interacting galaxies. The few YMCs that are close enough to resolve are of prime interest for studying the stellar mass function and the ecological interplay between stellar evolution and stellar dynamics. The distant unresolved clusters may be effectively used to study the star-cluster mass function, and they provide excellent constraints on the formation mechanisms of young cluster populations. YMCs are expected to be the nurseries for many unusual objects, including a wide range of exotic stars and binaries. So far only a few such objects have been found in YMCs, although their older cousins, the globular clusters, are unusually rich in stellar exotica. In this review, we focus on star clusters younger than \~{}100 Myr, more than a few current crossing times old, and more massive than \~{}10{\textless}SUP{\textgreater}4{\textless}/SUP{\textgreater}M{\textless}SUB{\textgreater}?{\textless}/SUB{\textgreater}; the size of the cluster and its environment are considered less relevant as distinguishing parameters. We describe the global properties of the currently known young massive star clusters in the Local Group and beyond, and discuss the state of the art in observations and dynamical modeling of these systems. In order to make this review readable by observers, theorists, and computational astrophysicists, we also review the cross-disciplinary terminology.},
	language = {en},
	urldate = {2021-10-19},
	journal = {Annual Review of Astronomy and Astrophysics, vol. 48, p.431-493},
	author = {Portegies Zwart, Simon F. and McMillan, Stephen L. W. and Gieles, Mark},
	month = sep,
	year = {2010},
	pages = {431},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/IJNA73BD/Portegies Zwart et al. - 2010 - Young Massive Star Clusters.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/PHIXJZWV/abstract.html:text/html},
}

@article{aniyan_resolving_2018,
	title = {Resolving the disc-halo degeneracy - {I}: a look at {NGC} 628},
	volume = {476},
	issn = {0035-8711},
	shorttitle = {Resolving the disc-halo degeneracy - {I}},
	url = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.1909A},
	doi = {10.1093/mnras/sty310},
	abstract = {The decomposition of the rotation curve of galaxies into contribution from the disc and dark halo remains uncertain and depends on the adopted mass-to-light ratio (M/L) of the disc. Given the vertical velocity dispersion of stars and disc scale height, the disc surface mass density and hence the M/L can be estimated. We address a conceptual problem with previous measurements of the scale height and dispersion. When using this method, the dispersion and scale height must refer to the same population of stars. The scale height is obtained from near-infrared (IR) studies of edge-on galaxies and is weighted towards older kinematically hotter stars, whereas the dispersion obtained from integrated light in the optical bands includes stars of all ages. We aim to extract the dispersion for the hotter stars, so that it can then be used with the correct scale height to obtain the disc surface mass density. We use a sample of planetary nebulae (PNe) as dynamical tracers in the face-on galaxy NGC 628. We extract two different dispersions from its velocity histogram - representing the older and younger PNe. We also present complementary stellar absorption spectra in the inner regions of this galaxy and use a direct pixel fitting technique to extract the two components. Our analysis concludes that previous studies, which do not take account of the young disc, underestimate the disc surface mass density by a factor of \~{}2. This is sufficient to make a maximal disc for NGC 628 appear like a submaximal disc.},
	urldate = {2021-10-03},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Aniyan, S. and Freeman, K. C. and Arnaboldi, M. and Gerhard, O. E. and Coccato, L. and Fabricius, M. and Kuijken, K. and Merrifield, M. and Ponomareva, A. A.},
	month = may,
	year = {2018},
	note = {ADS Bibcode: 2018MNRAS.476.1909A},
	keywords = {Astrophysics - Astrophysics of Galaxies, dark matter, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: spiral},
	pages = {1909--1930},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7N4399WC/Aniyan et al. - 2018 - Resolving the disc-halo degeneracy - I a look at .pdf:application/pdf},
}


@article{cook_spitzer_2014,
	title = {Spitzer {Local} {Volume} {Legacy} ({LVL}) {SEDs} and physical properties},
	volume = {445},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.445..899C},
	doi = {10.1093/mnras/stu1787},
	abstract = {We present the panchromatic spectral energy distributions (SEDs) of the Local Volume Legacy (LVL) survey which consists of 258 nearby galaxies (D {\textless} 11 Mpc). The wavelength coverage spans the ultraviolet to the infrared (1500 {\r A}-24 $\mu$m) which is utilized to derive global physical properties (i.e. star formation rate, stellar mass, internal extinction due to dust). With these data, we find colour-colour relationships and correlated trends between observed and physical properties (i.e. optical magnitudes and dust properties, optical colour and specific star formation rate, and ultraviolet-infrared colour and metallicity). The SEDs are binned by different galaxy properties to reveal how each property affects the observed shape of these SEDs. In addition, due to the volume-limited nature of LVL, we utilize the dwarf-dominated galaxy sample to test star formation relationships established with higher mass galaxy samples. We find good agreement with the star-forming `main-sequence' relationship, but find a systematic deviation in the infrared `main sequence' at low luminosities. This deviation is attributed to suppressed polycyclic aromatic hydrocarbon (PAH) formation in low-metallicity environments and/or the destruction of PAHs in more intense radiation fields occurring near a suggested threshold in star formation rates (sSFR) at a value of log(sSFR) \~{} -10.2.},
	urldate = {2021-10-03},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Cook, David O. and Dale, Daniel A. and Johnson, Benjamin D. and Van Zee, Liese and Lee, Janice C. and Kennicutt, Robert C. and Calzetti, Daniela and Staudaher, Shawn M. and Engelbracht, Charles W.},
	month = nov,
	year = {2014},
	note = {ADS Bibcode: 2014MNRAS.445..899C},
	keywords = {Astrophysics - Astrophysics of Galaxies, dust, extinction, galaxies: dwarf, galaxies: ISM, galaxies: spiral, galaxies: star formation, Local Group},
	pages = {899--912},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/I24YZR23/Cook et al. - 2014 - Spitzer Local Volume Legacy (LVL) SEDs and physica.pdf:application/pdf},
}

@article{adamo_formation_2020,
	title = {Star cluster formation in the most extreme environments: insights from the {HiPEEC} survey},
	volume = {499},
	issn = {0035-8711},
	shorttitle = {Star cluster formation in the most extreme environments},
	url = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.3267A},
	doi = {10.1093/mnras/staa2380},
	abstract = {We present the Hubble imaging Probe of Extreme Environments and Clusters (HiPEEC) survey. We fit HST NUV to NIR broad-band and H $\alpha$ fluxes to derive star cluster ages, masses, and extinctions and determine the star formation rate (SFR) of six merging galaxies. These systems are excellent laboratories to trace cluster formation under extreme gas physical conditions, rare in the local Universe, but typical for star-forming galaxies at cosmic noon. We detect clusters with ages of 1-500 Myr and masses that exceed 107 M?. The recent cluster formation history and their distribution within the host galaxies suggest that systems such as NGC 34, NGC 1614, and NGC 4194 are close to their final coalescing phase, while NGC 3256, NGC 3690, and NGC 6052 are at an earlier/intermediate stage. A Bayesian analysis of the cluster mass function in the age interval 1-100 Myr provides strong evidence in four of the six galaxies that an exponentially truncated power law better describes the observed mass distributions. For two galaxies, the fits are inconclusive due to low number statistics. We determine power-law slopes $\beta$ \~{} -1.5 to -2.0 and truncation masses, Mc, between 106 and a few times 107 M?, among the highest values reported in the literature. Advanced mergers have higher Mc than early/intermediate merger stage galaxies, suggesting rapid changes in the dense gas conditions during the merger. We compare the total stellar mass in clusters to the SFR of the galaxy, finding that these systems are among the most efficient environments to form star clusters in the local Universe.},
	urldate = {2021-09-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Adamo, A. and Hollyhead, K. and Messa, M. and Ryon, J. E. and Bajaj, V. and Runnholm, A. and Aalto, S. and Calzetti, D. and Gallagher, J. S. and Hayes, M. J. and Kruijssen, J. M. D. and K{\"o}nig, S. and Larsen, S. S. and Melinder, J. and Sabbi, E. and Smith, L. J. and {\"O}stlin, G.},
	month = dec,
	year = {2020},
	note = {ADS Bibcode: 2020MNRAS.499.3267A},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: interactions, galaxies: star clusters: general, galaxies: starburst, star clusters: statistics},
	pages = {3267--3294},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/DAW8WVE3/Adamo et al. - 2020 - Star cluster formation in the most extreme environ.pdf:application/pdf},
}


@article{kruijssen_formation_2019,
	title = {The formation and assembly history of the {Milky} {Way} revealed by its globular cluster population},
	volume = {486},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.3180K},
	doi = {10.1093/mnras/sty1609},
	abstract = {We use the age-metallicity distribution of 96 Galactic globular clusters (GCs) to infer the formation and assembly history of the Milky Way (MW), culminating in the reconstruction of its merger tree. Based on a quantitative comparison of the Galactic GC population to the 25 cosmological zoom-in simulations of MW-mass galaxies in the E-MOSAICS project, which self-consistently model the formation and evolution of GC populations in a cosmological context, we find that the MW assembled quickly for its mass, reaching \{25, 50\} per cent of its present-day halo mass already at z = \{3, 1.5\} and half of its present-day stellar mass at z = 1.2. We reconstruct the MW's merger tree from its GC age-metallicity distribution, inferring the number of mergers as a function of mass ratio and redshift. These statistics place the MW's assembly rate among the 72th-94th percentile of the E-MOSAICS galaxies, whereas its integrated properties (e.g. number of mergers, halo concentration) match the median of the simulations. We conclude that the MW has experienced no major mergers (mass ratios {\textgreater}1:4) since z \~{} 4, sharpening previous limits of z \~{} 2. We identify three massive satellite progenitors and constrain their mass growth and enrichment histories. Two are proposed to correspond to Sagittarius (a few 108 M?) and the GCs formerly associated with Canis Major (\~{} 10{\textasciicircum}9 M\_?). The third satellite has no known associated relic and was likely accreted between z = 0.6 and 1.3. We name this enigmatic galaxy Kraken and propose that it is the most massive satellite (M\_*\~{} 2{\texttimes} 10{\textasciicircum}9 M\_?) ever accreted by the MW. We predict that \~{}40 per cent of the Galactic GCs formed ex situ (in galaxies with masses M* = 2 {\texttimes} 107-2{\texttimes} 10{\textasciicircum}9 M\_?), with 6 {\textpm} 1 being former nuclear clusters.},
	urldate = {2021-09-20},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kruijssen, J. M. Diederik and Pfeffer, Joel L. and Reina-Campos, Marta and Crain, Robert A. and Bastian, Nate},
	month = jul,
	year = {2019},
	note = {ADS Bibcode: 2019MNRAS.486.3180K},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star formation, Galaxy: evolution, Galaxy: formation, Galaxy: halo, Galaxy: stellar content, globular clusters: general},
	pages = {3180--3202},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/3UC8BBWK/Kruijssen et al. - 2019 - The formation and assembly history of the Milky Wa.pdf:application/pdf},
}

@article{leroy_star_2008,
	title = {The {Star} {Formation} {Efficiency} in {Nearby} {Galaxies}: {Measuring} {Where} {Gas} {Forms} {Stars} {Effectively}},
	volume = {136},
	issn = {0004-6256},
	shorttitle = {The {Star} {Formation} {Efficiency} in {Nearby} {Galaxies}},
	url = {https://ui.adsabs.harvard.edu/abs/2008AJ....136.2782L},
	doi = {10.1088/0004-6256/136/6/2782},
	abstract = {We measure the star formation efficiency (SFE), the star formation rate (SFR) per unit of gas, in 23 nearby galaxies and compare it with expectations from proposed star formation laws and thresholds. We use H I maps from The H I Nearby Galaxy Survey (THINGS) and derive H2 maps of CO measured by HERA CO-Line Extragalactic Survey and Berkeley-Illinois-Maryland Association Survey of Nearby Galaxies. We estimate the SFR by combining Galaxy Evolution Explorer (GALEX) far-ultraviolet maps and the Spitzer Infrared Nearby Galaxies Survey (SINGS) 24 $\mu$m maps, infer stellar surface density profiles from SINGS 3.6 $\mu$m data, and use kinematics from THINGS. We measure the SFE as a function of the free fall and orbital timescales, midplane gas pressure, stability of the gas disk to collapse (including the effects of stars), the ability of perturbations to grow despite shear, and the ability of a cold phase to form. In spirals, the SFE of H2 alone is nearly constant at (5.25 {\textpm} 2.5) {\texttimes} 10-10 yr-1 (equivalent to an H2 depletion time of 1.9 {\texttimes} 109 yr) as a function of all of these variables at our 800 pc resolution. Where the interstellar medium (ISM) is mostly H I, however, the SFE decreases with increasing radius in both spiral and dwarf galaxies, a decline reasonably described by an exponential with scale length 0.2r 25-0.25r 25. We interpret this decline as a strong dependence of giant molecular cloud (GMC) formation on environment. The ratio of molecular-to-atomic gas appears to be a smooth function of radius, stellar surface density, and pressure spanning from the H2-dominated to H I-dominated ISM. The radial decline in SFE is too steep to be reproduced only by increases in the free-fall time or orbital time. Thresholds for large-scale instability suggest that our disks are stable or marginally stable and do not show a clear link to the declining SFE. We suggest that ISM physics below the scales that we observe{\textemdash}phase balance in the H I, H2 formation and destruction, and stellar feedback{\textemdash}governs the formation of GMCs from H I.},
	urldate = {2021-09-17},
	journal = {The Astronomical Journal},
	author = {Leroy, Adam K. and Walter, Fabian and Brinks, Elias and Bigiel, Frank and de Blok, W. J. G. and Madore, Barry and Thornley, M. D.},
	month = dec,
	year = {2008},
	note = {ADS Bibcode: 2008AJ....136.2782L},
	keywords = {Astrophysics, galaxies: ISM, stars: formation, galaxies: evolution, radio lines: galaxies},
	pages = {2782--2845},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/C7VTPVZM/Leroy et al. - 2008 - The Star Formation Efficiency in Nearby Galaxies .pdf:application/pdf},
}

@book{smith_ralph_c_uncertainty_2014,
	title = {Uncertainty quantification : theory, implementation, and applications},
	isbn = {978-1-61197-321-1},
	publisher = {SIAM},
	author = {{Smith, Ralph C.}},
	year = {2014},
}

@article{hogg_data_2010,
	title = {Data analysis recipes: {Fitting} a model to data},
	shorttitle = {Data analysis recipes},
	url = {https://arxiv.org/abs/1008.4686v1},
	abstract = {We go through the many considerations involved in fitting a model to data,
using as an example the fit of a straight line to a set of points in a
two-dimensional plane. Standard weighted least-squares fitting is only
appropriate when there is a dimension along which the data points have
negligible uncertainties, and another along which all the uncertainties can be
described by Gaussians of known variance; these conditions are rarely met in
practice. We consider cases of general, heterogeneous, and arbitrarily
covariant two-dimensional uncertainties, and situations in which there are bad
data (large outliers), unknown uncertainties, and unknown but expected
intrinsic scatter in the linear relationship being fit. Above all we emphasize
the importance of having a "generative model" for the data, even an approximate
one. Once there is a generative model, the subsequent fitting is non-arbitrary
because the model permits direct computation of the likelihood of the
parameters or the posterior probability distribution. Construction of a
posterior probability distribution is indispensible if there are "nuisance
parameters" to marginalize away.},
	language = {en},
	urldate = {2020-05-20},
	author = {Hogg, David W. and Bovy, Jo and Lang, Dustin},
	month = aug,
	year = {2010},
	file = {Snapshot:/Users/Tobin/Zotero/storage/TDJNV8U8/1008.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/83ZJG9PY/Hogg et al. - 2010 - Data analysis recipes Fitting a model to data.pdf:application/pdf},
}

@incollection{ivezic_bayesian_2020,
	edition = {REV - Revised},
	series = {A {Practical} {Python} {Guide} for the {Analysis} of {Survey} {Data}, {Updated} {Edition}},
	title = {Bayesian {Statistical} {Inference}},
	isbn = {978-0-691-19830-9},
	url = {https://www.jstor.org/stable/j.ctvrxk1hs.8},
	abstract = {We have already addressed the main philosophical differences between classical and Bayesian statistical inferences in {\textsection} 4.1. In this chapter, we introduce the most important aspects of Bayesian statistical inference and techniques for performing such calculations in practice. We first review the basic steps in Bayesian inference in {\textsection}5.1{\textendash}5.4, and then illustrate them with several examples in {\textsection}5.6{\textendash}5.7. Numerical techniques for solving complex problems are discussed in {\textsection}5.8, and the last section provides a summary of pros and cons for classical and Bayesian methods.  Let us briefly note a few historical facts. The Reverend Thomas Bayes (1702{\textendash}1761)},
	urldate = {2020-05-20},
	booktitle = {Statistics, {Data} {Mining}, and {Machine} {Learning} in {Astronomy}},
	publisher = {Princeton University Press},
	author = {Ivezi{\'c}, {\v Z}eljko and Connolly, Andrew J. and VanderPlas, Jacob T. and Gray, Alexander},
	year = {2020},
	doi = {10.2307/j.ctvrxk1hs.8},
	pages = {165--240},
}

@article{jordan_acs_2007,
	title = {The {ACS} {Virgo} {Cluster} {Survey}. {XII}. {The} {Luminosity} {Function} of {Globular} {Clusters} in {Early} {Type} {Galaxies}},
	volume = {171},
	issn = {0067-0049, 1538-4365},
	url = {http://arxiv.org/abs/astro-ph/0702496},
	doi = {10.1086/516840},
	abstract = {We analyze the luminosity function of the globular clusters (GCs) belonging to the early-type galaxies observed in the ACS Virgo Cluster Survey. We have obtained estimates for a Gaussian representation of the GC luminosity function (GCLF) for 89 galaxies. We have also fit the GCLFs with an "evolved Schechter function", which is meant to reflect the preferential depletion of low-mass GCs, primarily by evaporation due to two-body relaxation, from an initial Schechter mass function similar to that of young massive clusters. We find a significant trend of the GCLF dispersion with galaxy luminosity, in the sense that smaller galaxies have narrower GCLFs. We show that this narrowing of the GCLF in a Gaussian description is driven by a steepening of the GC mass function above the turnover mass, as one moves to smaller host galaxies. We argue that this behavior at the high-mass end of the GC mass function is most likely a consequence of systematic variations of the initial cluster mass function. The GCLF turnover mass M\_TO is roughly constant, at {\textasciitilde} 2.2 x 10{\textasciicircum}5 M\_sun in bright galaxies, but it decreases slightly in dwarfs with M\_B {\textgreater}{\textasciitilde} -18. We show that part of the variation could arise from the shorter dynamical friction timescales in smaller galaxies. We probe the variation of the GCLF to projected galactocentric radii of 20-35 kpc in the Virgo giants M49 and M87, finding that M\_TO is essentially constant over these spatial scales. Our fits of evolved Schechter functions imply average dynamical mass losses (Delta) over a Hubble time that fall in the range 2 x 10{\textasciicircum}5 {\textless}{\textasciitilde} (Delta/M\_sun) {\textless} 10{\textasciicircum}6 per GC. We agree with previous suggestions that if the full GCLF is to be understood in more detail GCLF models will have to include self-consistent treatments of dynamical evolution inside time-dependent galaxy potentials. (Abridged)},
	number = {1},
	urldate = {2020-05-19},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Jordan, Andres and McLaughlin, Dean E. and Cote, Patrick and Ferrarese, Laura and Peng, Eric W. and Mei, Simona and Villegas, Daniela and Merritt, David and Tonry, John L. and West, Michael J.},
	month = jul,
	year = {2007},
	note = {arXiv: astro-ph/0702496},
	keywords = {Astrophysics},
	pages = {101--145},
	file = {arXiv.org Snapshot:/Users/Tobin/Zotero/storage/G3B4QZJ5/0702496.html:text/html;arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/BU43H3YY/Jordan et al. - 2007 - The ACS Virgo Cluster Survey. XII. The Luminosity .pdf:application/pdf},
}

@article{larsen_mass_2009,
	title = {The mass function of young star clusters in spiral galaxies},
	volume = {494},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2009A%26A...494..539L},
	doi = {10.1051/0004-6361:200811212},
	abstract = {Aims: The initial cluster mass function (ICMF) in spiral discs is constrained and compared with data for old globular clusters and young clusters in starbursts. Methods: For a given absolute magnitude, the cluster age distribution depends on the ICMF. Here, the behaviour of the median age-magnitude relation is analysed in detail for Schechter ICMFs with various cut-off masses, M\_c. The calculated relations are compared with observations of the brightest clusters in spiral galaxies. Schechter functions are also fitted directly to observed mass functions (MFs). Results: A single Schechter ICMF with an Mc of a few times 105 M? can reproduce the observed ages and luminosities of the brightest (and 5th brightest) clusters in the spirals if disruption of optically visible clusters is dominated by relatively slow secular evolution. A Schechter function fit to the combined cluster MF for all spirals in the sample yields Mc = (2.1{\textpm}0.4){\texttimes}105 M?. The MFs in
cluster-poor and cluster-rich spirals are statistically
indistinguishable. An Mc = 2.1{\texttimes}105
M? Schechter function also fits the MF of young clusters in the Large Magellanic Cloud. If the same ICMF applies in the Milky Way, a bound cluster with M {\textgreater} 105 M? will
form about once every 107 years, while an M {\textgreater}
106 M? cluster will form only once every 50 Gyr. Luminosity functions (LFs) of model cluster populations drawn from an Mc = 2.1{\texttimes}105 M? Schechter
ICMF generally agree with LFs observed in spiral galaxies. Conclusions: The ICMF in present-day spiral discs can be modelled as a Schechter function with Mc ? 2{\texttimes}105
M?. However, the presence of significant numbers of M {\textgreater} 106 M? (and even M {\textgreater} 107
M?) clusters in some starburst galaxies makes it unlikely that the Mc value derived for spirals is universal. In high-pressure environments, such as those created by complex gas kinematics and feedback in mergers, Mc can shift to higher masses than in quiescent discs.},
	urldate = {2020-05-06},
	journal = {Astronomy and Astrophysics},
	author = {Larsen, S. S.},
	month = feb,
	year = {2009},
	keywords = {galaxies: spiral, galaxies: star clusters, Galaxy: open clusters and associations: general},
	pages = {539--551},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/RDLSXYSI/Larsen - 2009 - The mass function of young star clusters in spiral.pdf:application/pdf},
}

@article{gonzalez-lopezlira_gas_2012,
	title = {Gas {Surface} {Density}, {Star} {Formation} {Rate} {Surface} {Density}, and the {Maximum} {Mass} of {Young} {Star} {Clusters} in a {Disk} {Galaxy}. {I}. {The} {Flocculent} {Galaxy} {M} 33},
	volume = {761},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2012ApJ...761..124G},
	doi = {10.1088/0004-637X/761/2/124},
	abstract = {We analyze the relationship between maximum cluster mass M 
max and surface densities of total gas
($\Sigma$gas), molecular gas ({\textbackslash}Sigma \_H\_2), and star formation
rate ($\Sigma$SFR) in the flocculent galaxy M 33, using
published gas data and a catalog of more than 600 young star clusters in
its disk. By comparing the radial distributions of gas and most massive
cluster masses, we find that M maxvprop$\Sigma$4.7
{\textpm} 0.4 gas, M maxvprop$\Sigma$1.3
{\textpm} 0.1 H2 , and M
maxvprop$\Sigma$1.0 {\textpm} 0.1 SFR. We
rule out that these correlations result from the size of the sample;
hence, the change of the maximum cluster mass must be due to physical
causes.},
	urldate = {2020-05-06},
	journal = {The Astrophysical Journal},
	author = {Gonz{\'a}lez-L{\'o}pezlira, Rosa A. and Pflamm-Altenburg, Jan and Kroupa, Pavel},
	month = dec,
	year = {2012},
	keywords = {galaxies: spiral, galaxies: ISM, galaxies: star clusters: individual: M 33 NGC 598, stars: formation},
	pages = {124},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7NHZ5X8W/Gonz{\'a}lez-L{\'o}pezlira et al. - 2012 - Gas Surface Density, Star Formation Rate Surface D.pdf:application/pdf},
}

@article{fall_dynamical_2001,
	title = {Dynamical {Evolution} of the {Mass} {Function} of {Globular} {Star} {Clusters}},
	volume = {561},
	issn = {0004-637X},
	url = {https://doi.org/10.1086%2F323358},
	doi = {10.1086/323358},
	abstract = {We present a series of simple, largely analytical models to compute the effects of disruption on the mass function of star clusters. Our calculations include evaporation by two-body relaxation and gravitational shocks and mass loss by stellar evolution. We find that, for a wide variety of initial conditions, the mass function develops a turnover or peak and that, after 12 Gyr, this is remarkably close to the observed peak for globular clusters, at Mp ? 2 {\texttimes} 105 M?. Below the peak, the evolution is dominated by two-body relaxation, and the mass function always develops a tail of the form $\psi$(M) = const, reflecting that the masses of tidally limited clusters decrease linearly with time just before they are destroyed. This also agrees well with the empirical mass function of globular clusters in the Milky Way. Above the peak, the evolution is dominated by stellar evolution at early times and by gravitational shocks at late times. These processes shift the mass function to lower masses, while nearly preserving its shape. The radial variation of the mass function within a galaxy depends on the initial position-velocity distribution of the clusters. We find that some radial anisotropy in the initial velocity distribution, especially when this increases outward, is needed to account for the observed near-uniformity of the mass functions of globular clusters. This may be consistent with the observed near-isotropy of the present velocity distributions, because clusters on elongated orbits are preferentially destroyed. These results are based on models with static, spherical galactic potentials. We point out that there would be even more radial mixing of the orbits and hence more uniformity of the mass function if the galactic potentials were time-dependent and/or nonspherical.},
	language = {en},
	number = {2},
	urldate = {2020-04-30},
	journal = {The Astrophysical Journal},
	author = {Fall, S. Michael and Zhang, Qing},
	month = nov,
	year = {2001},
	note = {Publisher: IOP Publishing},
	pages = {751--765},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/HYLJUGPP/Fall and Zhang - 2001 - Dynamical Evolution of the Mass Function of Globul.pdf:application/pdf},
}

@article{boutloukos_star_2003,
	title = {Star cluster formation and disruption time-scales - {I}. {An} empirical determination of the disruption time of star clusters in four galaxies},
	volume = {338},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2003MNRAS.338..717B},
	doi = {10.1046/j.1365-8711.2003.06083.x},
	abstract = {We have derived the disruption times of star clusters from cluster 
samples of four galaxies, M51, M33, the Small Magellanic Cloud (SMC) and
the solar neighbourhood. If the disruption time of clusters in a galaxy
depends only on their initial mass as tdis(yr)
=t4dis(Mcl/104
Msolar)$\gamma$, and if the cluster formation rate
is constant, then the mass and age distributions of the observed
clusters will each be given by double power-law relations. For clusters
of low mass or young age the power law depends on the fading of the
clusters below the detection limit due to the evolution of the stars.
For clusters of high mass and old age the power law depends on the
disruption time of the clusters. The samples of clusters in M51 and M33,
observed with HST-WFPC2, indeed show the predicted double power-law
relations in both their mass and age distributions. The values of
tdis4 and $\gamma$ can be derived from
these relations. For the cluster samples of the SMC and the solar
neighbourhood, taken from the literature, only the age distribution is
known. This also shows the characteristic double power-law behaviour,
which allows the determination of tdis4
and $\gamma$ in these galaxies. The values of $\gamma$ are the same in the
four galaxies within the uncertainty, and the mean value is $\gamma$=
0.62 +/- 0.06. However, the disruption time
tdis4 of a cluster of 104
Msolar is very different in the different galaxies. The
clusters in the SMC have the longest disruption time,
tdis4{\textasciitilde}= 8 {\texttimes} 109 yr,
and the clusters at 1-3 kpc from the nucleus of M51 have the shortest
disruption time of tdis4{\textasciitilde}= 4 {\texttimes}
107 yr. The disruption time of clusters 1-5 kpc from the
nucleus of M33 is tdis4{\textasciitilde}= 1.3 {\texttimes}
108 yr and for clusters within 1 kpc from the Sun we find
tdis4{\textasciitilde}= 1.0 {\texttimes} 109 yr.},
	urldate = {2020-04-29},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Boutloukos, S. G. and Lamers, H. J. G. L. M.},
	month = jan,
	year = {2003},
	keywords = {galaxies: star clusters, galaxies: individual: M33, galaxies: individual: M51, Magellanic Clouds, open clusters and associations: general, solar neighbourhood},
	pages = {717--732},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/V6JRFGU5/Boutloukos and Lamers - 2003 - Star cluster formation and disruption time-scales .pdf:application/pdf},
}

@article{gieles_star_2005,
	title = {The star cluster population of {M} 51 - {III}. {Cluster} disruption and formation history},
	volume = {441},
	copyright = {{\textcopyright} ESO, 2005},
	issn = {0004-6361, 1432-0746},
	url = {https://www.aanda.org/articles/aa/abs/2005/39/aa2914-05/aa2914-05.html},
	doi = {10.1051/0004-6361:20052914},
	abstract = {In this work we concentrate on the evolution of the cluster population of the interacting galaxy M 51 (NGC 5194), more precisely the timescale of cluster disruption and possible variations in the cluster formation rate. We present a method to compare observed age vs. mass number density diagrams with predicted populations including various physical input parameters like the cluster initial mass function, cluster disruption, cluster formation rate and star bursts. If we assume that the cluster formation rate increases at the moments of the encounters with NGC 5195, we find an increase in the cluster formation rate of a factor of , combined with a disruption timescale which is slightly higher than when assuming a constant formation rate ( yr vs. yr). The measured cluster disruption time is a factor of 5 shorter than expected on theoretical grounds. This implies that the disk of M 51 is not a preferred location for survival of young globular clusters, since even clusters with masses on the order of will be destroyed within a few Gyr.},
	language = {en},
	number = {3},
	urldate = {2020-04-29},
	journal = {Astronomy \& Astrophysics},
	author = {Gieles, M. and Bastian, N. and Lamers, H. J. G. L. M. and Mout, J. N.},
	month = oct,
	year = {2005},
	note = {Number: 3
Publisher: EDP Sciences},
	pages = {949--960},
	file = {Snapshot:/Users/Tobin/Zotero/storage/UIBGDCFT/aa2914-05.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/MLJ8VFWF/Gieles et al. - 2005 - The star cluster population of M 51 - III. Cluster.pdf:application/pdf},
}

@article{chandar_fraction_2017,
	title = {The {Fraction} of {Stars} {That} {Form} in {Clusters} in {Different} {Galaxies}},
	volume = {849},
	issn = {0004-637X},
	url = {https://doi.org/10.3847%2F1538-4357%2Faa92ce},
	doi = {10.3847/1538-4357/aa92ce},
	abstract = {We estimate the fraction of stars that form in compact clusters (bound and unbound), , in a diverse sample of eight star-forming galaxies, including two irregulars, two dwarf starbursts, two spirals, and two mergers. The average value for our sample is . We also calculate the fraction of stars in clusters that survive to ages between and , denoted by , and find and , significantly lower than for the same galaxies. We do not find any systematic trends in or with the star formation rate (SFR), the SFR per unit area (), or the surface density of molecular gas () within the host galaxy. Our results are consistent with those found previously from the CMF/SFR statistic (where CMF is the cluster mass function), and with the quasi-universal model in which clusters in different galaxies form and disrupt in similar ways. Our results, however, contradict many previous claims that the fraction of stars in bound clusters increases strongly with and . We find that the previously reported trends are largely driven by comparisons that mixed and , where was systematically used for galaxies with higher and , and for galaxies with lower and .},
	language = {en},
	number = {2},
	urldate = {2020-04-29},
	journal = {The Astrophysical Journal},
	author = {Chandar, Rupali and Fall, S. Michael and Whitmore, Bradley C. and Mulia, Alexander J.},
	month = nov,
	year = {2017},
	note = {Publisher: American Astronomical Society},
	pages = {128},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/XWEYXVCG/Chandar et al. - 2017 - The Fraction of Stars That Form in Clusters in Dif.pdf:application/pdf},
}

@article{chandar_luminosity_2010,
	title = {{THE} {LUMINOSITY}, {MASS}, {AND} {AGE} {DISTRIBUTIONS} {OF} {COMPACT} {STAR} {CLUSTERS} {IN} {M83} {BASED} {ONHUBBLE} {SPACE} TEL{ESCOPE}/{WIDE} {FIELD} {CAMERA} 3 {OBSERVATIONS}},
	volume = {719},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F719%2F1%2F966},
	doi = {10.1088/0004-637X/719/1/966},
	abstract = {The newly installed Wide Field Camera 3 (WFC3) on the Hubble Space Telescope has been used to obtain multi-band images of the nearby spiral galaxy M83. These new observations are the deepest and highest resolution images ever taken of a grand-design spiral, particularly in the near-ultraviolet, and allow us to better differentiate compact star clusters from individual stars and to measure the luminosities of even faint clusters in the U band. We find that the luminosity function (LF) for clusters outside of the very crowded starburst nucleus can be approximated by a power law, dN/dL ? L $\alpha$, with $\alpha$ = {\textendash}2.04 {\textpm} 0.08, down to MV ? {\textendash}5.5. We test the sensitivity of the LF to different selection techniques, filters, binning, and aperture correction determinations, and find that none of these contribute significantly to uncertainties in $\alpha$. We estimate ages and masses for the clusters by comparing their measured UBVI, H$\alpha$ colors with predictions from single stellar population models. The age distribution of the clusters can be approximated by a power law, dN/d$\tau$ ? $\tau$$\gamma$, with $\gamma$ = {\textendash}0.9 {\textpm} 0.2, for M ? few {\texttimes} 103 M ? and $\tau$ ? 4 {\texttimes} 108 yr. This indicates that clusters are disrupted quickly, with ?80\%-90\% disrupted each decade in age over this time. The mass function of clusters over the same M-$\tau$ range is a power law, dN/dM ? M $\beta$, with $\beta$ = {\textendash}1.94 {\textpm} 0.16, and does not have bends or show curvature at either high or low masses. Therefore, we do not find evidence for a physical upper mass limit, MC , or for the earlier disruption of lower mass clusters when compared with higher mass clusters, i.e., mass-dependent disruption. We briefly discuss these implications for the formation and disruption of the clusters.},
	language = {en},
	number = {1},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Chandar, Rupali and Whitmore, Bradley C. and Kim, Hwihyun and Kaleida, Catherine and Mutchler, Max and Calzetti, Daniela and Saha, Abhijit and O{\textbackslash}textquotesingleConnell, Robert and Balick, Bruce and Bond, Howard and Carollo, Marcella and Disney, Michael and Dopita, Michael A. and Frogel, Jay A. and Hall, Donald and Holtzman, Jon A. and Kimble, Randy A. and McCarthy, Patrick and Paresce, Francesco and Silk, Joe and Trauger, John and Walker, Alistair R. and Windhorst, Rogier A. and Young, Erick},
	month = jul,
	year = {2010},
	note = {Publisher: IOP Publishing},
	pages = {966--978},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/CSVT5XMV/Chandar et al. - 2010 - THE LUMINOSITY, MASS, AND AGE DISTRIBUTIONS OF COM.pdf:application/pdf},
}

@article{elmegreen_disruption_2010,
	title = {{ON} {THE} {DISRUPTION} {OF} {STAR} {CLUSTERS} {IN} {A} {HIERARCHICAL} {INTERS}TEL{LAR} {MEDIUM}},
	volume = {712},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F712%2F1%2F604},
	doi = {10.1088/0004-637X/712/1/604},
	abstract = {The distribution of the number of clusters as a function of mass M and age T suggests that clusters get eroded or dispersed in a regular way over time, such that the cluster number decreases inversely as an approximate power law with T within each fixed interval of M. This power law is inconsistent with standard dispersal mechanisms such as cluster evaporation and cloud collisions. In the conventional interpretation, it requires the unlikely situation where diverse mechanisms stitch together over time in a way that is independent of environment or M. Here, we consider another model in which the large-scale distribution of gas in each star-forming region plays an important role. We note that star clusters form with positional and temporal correlations in giant cloud complexes, and suggest that these complexes dominate the tidal force and collisional influence on a cluster during its first several hundred million years. Because the cloud complex density decreases regularly with position from the cluster birth site, the harassment and collision rates between the cluster and the cloud pieces decrease regularly with age as the cluster drifts. This decrease is typically a power law of the form required to explain the mass-age distribution. We reproduce this distribution for a variety of cases, including rapid disruption, slow erosion, combinations of these two, cluster-cloud collisions, cluster disruption by hierarchical disassembly, and partial cluster disruption. We also consider apparent cluster mass loss by fading below the surface brightness limit of a survey. In all cases, the observed log M-log T diagram can be reproduced under reasonable assumptions.},
	language = {en},
	number = {1},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Elmegreen, Bruce G. and Hunter, Deidre A.},
	month = mar,
	year = {2010},
	note = {Publisher: IOP Publishing},
	pages = {604--623},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/B2WXZ7S8/Elmegreen and Hunter - 2010 - ON THE DISRUPTION OF STAR CLUSTERS IN A HIERARCHIC.pdf:application/pdf},
}

@article{lada_embedded_2003,
	title = {Embedded {Clusters} in {Molecular} {Clouds}},
	volume = {41},
	issn = {0066-4146},
	url = {http://adsabs.harvard.edu/abs/2003ARA%26A..41...57L},
	doi = {10.1146/annurev.astro.41.011802.094844},
	abstract = {Stellar clusters are born embedded within giant molecular clouds (GMCs) and during their formation and early evolution are often only visible at infrared wavelengths, being heavily obscured by dust. Over the past 15 years advances in infrared detection capabilities have enabled the first systematic studies of embedded clusters in galactic molecular clouds. In this article we review the current state of empirical knowledge
concerning these extremely young protocluster systems. From a survey of the literature we compile the first extensive catalog of galactic embedded clusters. We use the catalog to construct the mass function and estimate the birthrate for embedded clusters within 2 kpc of the sun. We find that the embedded cluster birthrate exceeds that of visible open clusters by an order of magnitude or more indicating a high infant mortality rate for protocluster systems. Less than 4-7\% of embedded clusters survive emergence from molecular clouds to become bound clusters of Pleiades age. The vast majority (90\%) of stars that form in embedded clusters form in rich clusters of 100 or more members with masses in excess of 50 M?. Moreover, observations of
nearby cloud complexes indicate that embedded clusters account for a significant (70-90\%) fraction of all stars formed in GMCs. We review the role of embedded clusters in investigating the nature of the initial mass function (IMF) that, in one nearby example, has been measured over the entire range of stellar and substellar mass, from OB stars to substellar objects near the deuterium burning limit. We also review the role embedded clusters play in the investigation of circumstellar disk evolution and the important constraints they provide for understanding the origin of planetary systems. Finally, we discuss current ideas concerning the origin and dynamical evolution of embedded clusters and the implications for the formation of bound open clusters.},
	urldate = {2020-04-28},
	journal = {Annual Review of Astronomy and Astrophysics},
	author = {Lada, Charles J. and Lada, Elizabeth A.},
	year = {2003},
	pages = {57--115},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/U36BZ7YL/Lada and Lada - 2003 - Embedded Clusters in Molecular Clouds.pdf:application/pdf},
}

@article{lamers_analytical_2005,
	title = {An analytical description of the disruption of star clusters in tidal fields with an application to {Galactic} open clusters},
	volume = {441},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2005A%26A...441..117L},
	doi = {10.1051/0004-6361:20042241},
	abstract = {We present a simple analytical description of the disruption of star 
clusters in a tidal field. The cluster disruption time, defined as
t\_dis= \{d ln M/dt\}-1, depends on the mass M of the cluster
as t\_dis=t\_0(M/M?)$\gamma$ with $\gamma$=0.62
for clusters in a tidal field, as shown by empirical studies of cluster
samples in different galaxies and by N-body simulations. Using this
simple description we derive an analytic expression for the way in which
the mass of a cluster decreases with time due to stellar evolution and
disruption. The result agrees very well with those of detailed N-body
simulations for clusters in the tidal field of our galaxy. The analytic
expression can be used to predict the mass and age histograms of
surviving clusters for any cluster initial mass function and any cluster
formation history. The method is applied to explain the age distribution
of the open clusters in the solar neighbourhood within 600 pc, based on
a new cluster sample that appears to be unbiased within a distance of
about 1 kpc. From a comparison between the observed and predicted age
distributions in the age range between 10 Myr to 3 Gyr we find the
following results: (1) The disruption time of a 104
M? cluster in the solar neighbourhood is about 1.3
{\textpm} 0.5 Gyr. This is a factor of 5 shorter than that derived from
N-body simulations of clusters in the tidal field of the galaxy.
Possible reasons for this discrepancy are discussed. (2) The present
star formation rate in bound clusters within 600 pc of the Sun is 5.9
{\textpm} 0.8 {\texttimes} 102 M? Myr-1,
which corresponds to a surface star formation rate of bound clusters of
5.2 {\textpm} 0.7 {\texttimes} 10-10 M?
yr-1 pc-2. (3) The age distribution of open
clusters shows a bump between 0.26 and 0.6 Gyr when the cluster
formation rate was 2.5 times higher than before and after. (4) The
present star formation rate in bound clusters is about half that derived
from the study of embedded clusters. The difference suggests that about
half of the clusters in the solar neighbourhood become unbound within
about 10 Myr. (5) The most massive clusters within 600 pc had an initial
mass of about 3{\texttimes} 104 M?. This is in
agreement with the statistically expected value based on a cluster
initial mass function with a slope of -2, even if the physical upper
mass limit for cluster formation is as high as 106
M?.},
	urldate = {2020-04-28},
	journal = {Astronomy and Astrophysics},
	author = {Lamers, H. J. G. L. M. and Gieles, M. and Bastian, N. and Baumgardt, H. and Kharchenko, N. V. and Portegies Zwart, S.},
	month = oct,
	year = {2005},
	keywords = {galaxies: star clusters, Galaxy: open clusters and associations: general, Galaxy: globular clusters: general, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: solar neighbourhood},
	pages = {117--129},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/C4KQ69T3/Lamers et al. - 2005 - An analytical description of the disruption of sta.pdf:application/pdf},
}

@article{adamo_legacy_2017,
	title = {Legacy {ExtraGalactic} {UV} {Survey} with {The} {Hubble} {Space} {Telescope}: {Stellar} {Cluster} {Catalogs} and {First} {Insights} {Into} {Cluster} {Formation} and {Evolution} in {NGC} 628},
	volume = {841},
	issn = {0004-637X},
	shorttitle = {Legacy {ExtraGalactic} {UV} {Survey} with {The} {Hubble} {Space} {Telescope}},
	url = {http://adsabs.harvard.edu/abs/2017ApJ...841..131A},
	doi = {10.3847/1538-4357/aa7132},
	abstract = {We report the large effort that is producing comprehensive high-level 
young star cluster (YSC) catalogs for a significant fraction of galaxies
observed with the Legacy ExtraGalactic UV Survey (LEGUS) Hubble treasury
program. We present the methodology developed to extract cluster
positions, verify their genuine nature, produce multiband photometry
(from NUV to NIR), and derive their physical properties via spectral
energy distribution fitting analyses. We use the nearby spiral galaxy
NGC 628 as a test case for demonstrating the impact that LEGUS will have
on our understanding of the formation and evolution of YSCs and compact
stellar associations within their host galaxy. Our analysis of the
cluster luminosity function from the UV to the NIR finds a steepening at
the bright end and at all wavelengths suggesting a dearth of luminous
clusters. The cluster mass function of NGC 628 is consistent with a
power-law distribution of slopes \~{} -2 and a truncation of a few
times 105 \{M\}? . After their formation, YSCs
and compact associations follow different evolutionary paths. YSCs
survive for a longer time frame, confirming their being potentially
bound systems. Associations disappear on timescales comparable to
hierarchically organized star-forming regions, suggesting that they are
expanding systems. We find mass-independent cluster disruption in the
inner region of NGC 628, while in the outer part of the galaxy there is
little or no disruption. We observe faster disruption rates for low mass
(<=104 \{M\}? ) clusters, suggesting that a
mass-dependent component is necessary to fully describe the YSC
disruption process in NGC 628.

Based on observations obtained with the NASA/ESA Hubble Space Telescope,
at the Space Telescope Science Institute, which is operated by the
Association of Universities for Research in Astronomy, Inc., under NASA
contract NAS 5-26555.},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Adamo, A. and Ryon, J. E. and Messa, M. and Kim, H. and Grasha, K. and Cook, D. O. and Calzetti, D. and Lee, J. C. and Whitmore, B. C. and Elmegreen, B. G. and Ubeda, L. and Smith, L. J. and Bright, S. N. and Runnholm, A. and Andrews, J. E. and Fumagalli, M. and Gouliermis, D. A. and Kahre, L. and Nair, P. and Thilker, D. and Walterbos, R. and Wofford, A. and Aloisi, A. and Ashworth, G. and Brown, T. M. and Chandar, R. and Christian, C. and Cignoni, M. and Clayton, G. C. and Dale, D. A. and de Mink, S. E. and Dobbs, C. and Elmegreen, D. M. and Evans, A. S. and Gallagher, III, J. S. and Grebel, E. K. and Herrero, A. and Hunter, D. A. and Johnson, K. E. and Kennicutt, R. C. and Krumholz, M. R. and Lennon, D. and Levay, K. and Martin, C. and Nota, A. and {\"O}stlin, G. and Pellerin, A. and Prieto, J. and Regan, M. W. and Sabbi, E. and Sacchi, E. and Schaerer, D. and Schiminovich, D. and Shabani, F. and Tosi, M. and Van Dyk, S. D. and Zackrisson, E.},
	month = jun,
	year = {2017},
	keywords = {stars: formation, galaxies: individual: NGC 628, galaxies: star clusters: general, galaxies: star formation, M74},
	pages = {131},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/Q9PNA9ST/Adamo et al. - 2017 - Legacy ExtraGalactic UV Survey with The Hubble Spa.pdf:application/pdf},
}

@article{lamb_sparsest_2010,
	title = {The {Sparsest} {Clusters} with {O} {Stars}},
	volume = {725},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2010ApJ...725.1886L},
	doi = {10.1088/0004-637X/725/2/1886},
	abstract = {There is much debate on how high-mass star formation varies with environment, and whether the sparsest star-forming environments are capable of forming massive stars. To address this issue, we have observed eight apparently isolated OB stars in the Small Magellanic Cloud (SMC) using Hubble Space Telescope's Advanced Camera for Surveys. Five of these objects appear as isolated stars, two of which are confirmed to be runaways. The remaining three objects are found to exist in sparse clusters, with lsim10 companion stars revealed, having masses of 1-4 M sun. Stochastic effects dominate in these sparse clusters, so we perform Monte Carlo simulations to explore how our observations fit within the framework of empirical, galactic cluster properties. We generate clusters using a simplistic -2 power-law distribution for either the number of stars per cluster (N *) or cluster mass (M cl). These clusters are then populated with stars randomly chosen from a Kroupa initial mass function (IMF). We find that simulations with cluster lower-mass limits of M
cl,lo {\textgreater}= 20 M sun and N *,lo {\textgreater}= 40 match best with observations of SMC and Galactic OB star populations. We examine the mass ratio of the second most massive and most massive stars m max,2/m max, finding that our observations all exist below the 20th percentile of our simulated clusters. However, all of our observed clusters lie within the parameter space spanned by the simulated clusters, although some are in the lowest 5th percentile frequency. These results suggest that clusters are built stochastically by randomly sampling stars from a universal IMF with a fixed stellar upper-mass limit. In particular, we see no evidence to suggest an m max-M cl relation. Our results may be more consistent with core accretion models of star formation than with competitive accretion models, and they are inconsistent with the proposed steepening of the integrated galactic stellar initial mass function (IGIMF).},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Lamb, J. B. and Oey, M. S. and Werk, J. K. and Ingleby, L. D.},
	month = dec,
	year = {2010},
	keywords = {stars: formation, Magellanic Clouds, galaxies: star clusters: general, galaxies: stellar content, stars: early-type},
	pages = {1886--1902},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/6H5FYXMH/Lamb et al. - 2010 - The Sparsest Clusters with O Stars.pdf:application/pdf},
}

@article{sun_star_2016,
	title = {The {Star} {Cluster} {Mass}-{Galactocentric} {Radius} {Relation}: {Implications} for {Cluster} {Formation}},
	volume = {816},
	issn = {0004-637X},
	shorttitle = {The {Star} {Cluster} {Mass}-{Galactocentric} {Radius} {Relation}},
	url = {http://adsabs.harvard.edu/abs/2016ApJ...816....9S},
	doi = {10.3847/0004-637X/816/1/9},
	abstract = {Whether or not the initial star cluster mass function is established 
through a universal, galactocentric-distance-independent stochastic
process, on the scales of individual galaxies, remains an unsolved
problem. This debate has recently gained new impetus through the
publication of a study that concluded that the maximum cluster mass in a
given population is not solely determined by size-of-sample effects.
Here, we revisit the evidence in favor and against stochastic cluster
formation by examining the young (? a few {\texttimes} \{10\}8
year old) star cluster mass-galactocentric radius relation in M33,
M51, M83, and the Large Magellanic Cloud. To eliminate size-of-sample
effects, we first adopt radial bin sizes containing constant numbers of
clusters, which we use to quantify the radial distribution of the first-
to fifth-ranked most massive clusters using ordinary least-squares
fitting. We supplement this analysis with an application of quantile
regression, a binless approach to rank-based regression taking an
absolute-value-distance penalty. Both methods yield, within the 1$\sigma$
to 3$\sigma$ uncertainties, near-zero slopes in the diagnostic plane,
largely irrespective of the maximum age or minimum mass imposed on our
sample selection, or of the radial bin size adopted. We conclude that,
at least in our four well-studied sample galaxies, star cluster
formation does not necessarily require an environment-dependent cluster
formation scenario, which thus supports the notion of stochastic star
cluster formation as the dominant star cluster-formation process within
a given galaxy.},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Sun, Weijia and de Grijs, Richard and Fan, Zhou and Cameron, Ewan},
	month = jan,
	year = {2016},
	keywords = {galaxies: individual: M33, galaxies: star clusters: general, galaxies: evolution, LMC, M51, M83},
	pages = {9},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/MLCZBLAC/Sun et al. - 2016 - The Star Cluster Mass-Galactocentric Radius Relati.pdf:application/pdf},
}

@article{pflamm-altenburg_galactocentric_2013,
	title = {The galactocentric radius dependent upper mass limit of young star clusters: stochastic star formation ruled out},
	volume = {435},
	issn = {0035-8711},
	shorttitle = {The galactocentric radius dependent upper mass limit of young star clusters},
	url = {http://adsabs.harvard.edu/abs/2013MNRAS.435.2604P},
	doi = {10.1093/mnras/stt1474},
	abstract = {It is widely accepted that the distribution function of the masses of 
young star clusters is universal and can be purely interpreted as a
probability density distribution function with a constant upper mass
limit. As a result of this picture the masses of the most massive
objects are exclusively determined by the size of the sample. Here we
show, with very high confidence, that the masses of the most massive
young star clusters in M33 decrease with increasing galactocentric
radius in contradiction to the expectations from a model of a randomly
sampled constant cluster mass function with a constant upper mass limit.
Pure stochastic star formation is thereby ruled out. We use this example
to elucidate how naive analysis of data can lead to unphysical
conclusions.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Pflamm-Altenburg, Jan and Gonz{\'a}lez-L{\'o}pezlira, Rosa A. and Kroupa, Pavel},
	month = nov,
	year = {2013},
	keywords = {stars: formation, galaxies: individual: M33, galaxies: star clusters: general},
	pages = {2604--2609},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/KU6U4RV8/Pflamm-Altenburg et al. - 2013 - The galactocentric radius dependent upper mass lim.pdf:application/pdf},
}

@article{gonzalez-lopezlira_gas_2012-1,
	title = {Gas {Surface} {Density}, {Star} {Formation} {Rate} {Surface} {Density}, and the {Maximum} {Mass} of {Young} {Star} {Clusters} in a {Disk} {Galaxy}. {I}. {The} {Flocculent} {Galaxy} {M} 33},
	volume = {761},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2012ApJ...761..124G},
	doi = {10.1088/0004-637X/761/2/124},
	abstract = {We analyze the relationship between maximum cluster mass M 
max and surface densities of total gas
($\Sigma$gas), molecular gas ({\textbackslash}Sigma \_H\_2), and star formation
rate ($\Sigma$SFR) in the flocculent galaxy M 33, using
published gas data and a catalog of more than 600 young star clusters in
its disk. By comparing the radial distributions of gas and most massive
cluster masses, we find that M maxvprop$\Sigma$4.7
{\textpm} 0.4 gas, M maxvprop$\Sigma$1.3
{\textpm} 0.1 H2 , and M
maxvprop$\Sigma$1.0 {\textpm} 0.1 SFR. We
rule out that these correlations result from the size of the sample;
hence, the change of the maximum cluster mass must be due to physical
causes.},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Gonz{\'a}lez-L{\'o}pezlira, Rosa A. and Pflamm-Altenburg, Jan and Kroupa, Pavel},
	month = dec,
	year = {2012},
	keywords = {galaxies: spiral, galaxies: ISM, galaxies: star clusters: individual: M 33 NGC 598, stars: formation},
	pages = {124},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/H7KW2GAF/Gonz{\'a}lez-L{\'o}pezlira et al. - 2012 - Gas Surface Density, Star Formation Rate Surface D.pdf:application/pdf},
}

@article{fall_similarities_2012,
	title = {Similarities in {Populations} of {Star} {Clusters}},
	volume = {752},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2012ApJ...752...96F},
	doi = {10.1088/0004-637X/752/2/96},
	abstract = {We compare the observed mass functions and age distributions of star clusters in six well-studied galaxies: the Milky Way, Magellanic Clouds, M83, M51, and Antennae. In combination, these distributions span wide ranges of mass and age: 102 {\textless}{\textasciitilde} M/M ?
{\textless}{\textasciitilde} 106 and 106 {\textless}{\textasciitilde} $\tau$/yr {\textless}{\textasciitilde}
109. We confirm that the distributions are well represented by power laws: dN/dMvpropM $\beta$ with $\beta$ ? -1.9
and dN/d$\tau$vprop$\tau$$\gamma$ with $\gamma$ ? -0.8.
The mass and age distributions are approximately independent of each other, ruling out simple models of mass-dependent disruption. As expected, there are minor differences among the exponents at a level close to the true uncertainties, epsilon$\beta$ {\textasciitilde}
epsilon$\gamma$ {\textasciitilde} 0.1-0.2. However, the overwhelming
impression is the similarity of the mass functions and age distributions of clusters in these different galaxies, including giant and dwarf, quiescent and interacting galaxies. This is an important empirical result, justifying terms such as "universal" or "quasi-universal." We provide a partial theoretical explanation for these observations in terms of physical processes operating during the formation and
disruption of the clusters, including star formation and feedback, subsequent stellar mass loss, and tidal interactions with passing molecular clouds. A full explanation will require additional information about the molecular clumps and star clusters in galaxies beyond the Milky Way.},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Fall, S. Michael and Chandar, Rupali},
	month = jun,
	year = {2012},
	keywords = {stars: formation, galaxies: star clusters: general, galaxies: individual: Magellanic Clouds Milky Way M51 M83 NGC 4038/39},
	pages = {96},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/AXDDHLR2/Fall and Chandar - 2012 - Similarities in Populations of Star Clusters.pdf:application/pdf},
}

@article{messa_young_2018,
	title = {The young star cluster population of {M51} with {LEGUS} - {I}. {A} comprehensive study of cluster formation and evolution},
	volume = {473},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2018MNRAS.473..996M},
	doi = {10.1093/mnras/stx2403},
	abstract = {Recently acquired WFC3 UV (F275W and F336W) imaging mosaics under the 
Legacy Extragalactic UV Survey (LEGUS), combined with archival ACS data
of M51, are used to study the young star cluster (YSC) population of
this interacting system. Our newly extracted source catalogue contains
2834 cluster candidates, morphologically classified to be compact and
uniform in colour, for which ages, masses and extinction are derived. In
this first work we study the main properties of the YSC population of
the whole galaxy, considering a mass-limited sample. Both luminosity and
mass functions follow a power-law shape with slope -2, but at high
luminosities and masses a dearth of sources is observed. The analysis of
the mass function suggests that it is best fitted by a Schechter
function with slope -2 and a truncation mass at 1.00 {\textpm} 0.12
{\texttimes} 105 M?. Through Monte Carlo
simulations, we confirm this result and link the shape of the luminosity
function to the presence of a truncation in the mass function. A mass
limited age function analysis, between 10 and 200 Myr, suggests that the
cluster population is undergoing only moderate disruption. We observe
little variation in the shape of the mass function at masses above 1
{\texttimes} 104 M? over this age range. The
fraction of star formation happening in the form of bound clusters in
M51 is \~{} 20 per cent in the age range 10-100 Myr and little
variation is observed over the whole range from 1 to 200 Myr.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Messa, M. and Adamo, A. and {\"O}stlin, G. and Calzetti, D. and Grasha, K. and Grebel, E. K. and Shabani, F. and Chandar, R. and Dale, D. A. and Dobbs, C. L. and Elmegreen, B. G. and Fumagalli, M. and Gouliermis, D. A. and Kim, H. and Smith, L. J. and Thilker, D. A. and Tosi, M. and Ubeda, L. and Walterbos, R. and Whitmore, B. C. and Fedorenko, K. and Mahadevan, S. and Andrews, J. E. and Bright, S. N. and Cook, D. O. and Kahre, L. and Nair, P. and Pellerin, A. and Ryon, J. E. and Ahmad, S. D. and Beale, L. P. and Brown, K. and Clarkson, D. A. and Guidarelli, G. C. and Parziale, R. and Turner, J. and Weber, M.},
	month = jan,
	year = {2018},
	keywords = {galaxies: individual: M51, galaxies: star clusters: general, galaxies: star formation, NGC 5194},
	pages = {996--1018},
	file = {Full Text:/Users/Tobin/Zotero/storage/8RHLXSWP/Messa et al. - 2018 - The young star cluster population of M51 with LEGU.pdf:application/pdf},
}

@article{chandar_age_2016,
	title = {The {Age}, {Mass}, and {Size} {Distributions} of {Star} {Clusters} in {M51}},
	volume = {824},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2016ApJ...824...71C},
	doi = {10.3847/0004-637X/824/2/71},
	abstract = {We present a new catalog of 3816 compact star clusters in the grand design spiral galaxy M51 based on observations taken with the Hubble Space Telescope. The age distribution of the clusters declines starting at very young ages, and can be represented by a power law, \{dN\}/d$\tau$ {\textbackslash}propto \{$\tau$ \}$\gamma$ , with $\gamma$ =-0.65+/- 0.15. No
significant changes in the shape of the age distribution at different masses is observed. The mass function of the clusters younger than $\tau$ ? 400 \{\{Myr\}\} can also be described by a power law, \{dN\}/\{dM\}{\textbackslash}propto \{M\}$\beta$ , with $\beta$ ? {\textbackslash}-2.1+/- 0.2. We compare these
distributions with the predictions from various cluster disruption models, and find that they are consistent with models where clusters disrupt approximately independent of their initial mass, but not with models where lower mass clusters are disrupted earlier than their higher mass counterparts. We find that the half-light radii of clusters more massive than M ? 3{\texttimes} \{10\}4 \{M\}? and
with ages between 100 and 400 \{\{Myr\}\} are larger by a factor of
?3-4 than their counterparts that are younger than
107 years old, suggesting that the clusters physically expand during their early life.},
	urldate = {2020-04-28},
	journal = {The Astrophysical Journal},
	author = {Chandar, Rupali and Whitmore, Bradley C. and Dinino, Daiana and Kennicutt, Robert C. and Chien, L.-H. and Schinnerer, Eva and Meidt, Sharon},
	month = jun,
	year = {2016},
	keywords = {stars: formation, galaxies: individual: M51, galaxies: star clusters: general, galaxies: starburst},
	pages = {71},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/G9MCGW7N/Chandar et al. - 2016 - The Age, Mass, and Size Distributions of Star Clus.pdf:application/pdf},
}

@article{adamo_probing_2015,
	title = {Probing the role of the galactic environment in the formation of stellar clusters, using {M83} as a test bench},
	volume = {452},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2015MNRAS.452..246A},
	doi = {10.1093/mnras/stv1203},
	abstract = {We present a study of the M83 cluster population, covering the disc of 
the galaxy between radii of 0.45 and 4.5 kpc. We aim to probe the
properties of the cluster population as a function of distance from the
galactic centre. We observe a net decline in cluster formation
efficiency ($\Gamma$, i.e. amount of star formation happening in bound
clusters) from about 26 per cent in the inner region to 8 per cent in
the outer part of the galaxy. The recovered $\Gamma$ values within
different regions of M83 follow the same $\Gamma$ versus star formation
rate density relation observed for entire galaxies. We also probe the
initial cluster mass function (ICMF) as a function of galactocentric
distance. We observe a significant steepening of the ICMF in the outer
regions (from -1.90 {\textpm} 0.11 to -2.70 {\textpm} 0.14) and for the
whole galactic cluster population (slope of -2.18 {\textpm} 0.07) of M83.
We show that this change of slope reflects a more fundamental change of
the `truncation mass' at the high-mass end of the distribution. This can
be modelled as a Schechter function of slope -2 with an exponential
cutoff mass (Mc) that decreases significantly from the inner
to the outer regions (from 4.00 to 0.25 {\texttimes} 105
M?) while the galactic Mc is ?1.60 {\texttimes}
105 M?. The trends in $\Gamma$ and ICMF are
consistent with the observed radial decrease of the
$\Sigma$(H2), hence in gas pressure. As gas pressure declines,
cluster formation becomes less efficient. We conclude that the host
galaxy environment appears to regulate (1) the fraction of stars locked
in clusters and (2) the upper mass limit of the ICMF, consistently
described by a near-universal slope -2 truncated at the high-mass end.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Adamo, A. and Kruijssen, J. M. D. and Bastian, N. and Silva-Villa, E. and Ryon, J.},
	month = sep,
	year = {2015},
	keywords = {galaxies: spiral, galaxies: star clusters, galaxies: star formation},
	pages = {246--260},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/ZP87WI2V/Adamo et al. - 2015 - Probing the role of the galactic environment in th.pdf:application/pdf},
}

@article{bastian_stellar_2012,
	title = {Stellar clusters in {M83}: formation, evolution, disruption and the influence of the environment},
	volume = {419},
	issn = {0035-8711},
	shorttitle = {Stellar clusters in {M83}},
	url = {http://adsabs.harvard.edu/abs/2012MNRAS.419.2606B},
	doi = {10.1111/j.1365-2966.2011.19909.x},
	abstract = {We study the stellar cluster population in two adjacent fields in the 
nearby, face-on spiral galaxy M83 using multiwavelength Wide Field
Camera 3/Hubble Space Telescope imaging. After automatic detection
procedures, the clusters are selected through visual inspection to be
centrally concentrated, symmetric, and resolved on the images, which
allows us to differentiate between clusters and likely unbound
associations. We compare our sample with previous studies and show that
the differences between the catalogues are largely due to the inclusion
of a large numbers of diffuse associations within previous catalogues as
well as the inclusion of the central starburst region, where the
completeness limit is significantly worse than in the surrounding
regions. We derive the size distribution of the clusters, which is well
described by a lognormal distribution with a peak at \~{}2.5 pc, and
find evidence for an expansion in the half-light radius of clusters with
age. The luminosity function of the clusters is well approximated by a
power law with an index of -2 over most of the observed range; however,
a steepening is seen at MV=-9.3 and -8.8 in the inner and
outer fields, respectively. Additionally, we show that the cluster
population is inconsistent with a pure power-law mass distribution, but
instead exhibits a truncation at the high-mass end. If described as a
Schechter function, the characteristic mass is 1.6 {\texttimes}
105 and 0.5 {\texttimes} 105 M? for the
inner and outer fields, respectively, in agreement with previous
estimates of other cluster populations in spiral galaxies. Comparing the
predictions of the mass-independent disruption (MID) and mass-dependent
disruption (MDD) scenarios with the observed distributions, we find that
both models can accurately fit the data. However, for the MID case, the
fraction of clusters destroyed (or mass lost) per decade in age is
dependent on the environment; hence, the age and mass distributions of
clusters are not universal. In the MDD case, the disruption time-scale
scales with galactocentric distance (being longer in the outer regions
of the galaxy) in agreement with analytic and numerical predictions.
Finally, we discuss the implications of our results on other
extragalactic surveys, focusing on the fraction of stars that form in
clusters and the need (or lack thereof) for infant mortality.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Bastian, N. and Adamo, A. and Gieles, M. and Silva-Villa, E. and Lamers, H. J. G. L. M. and Larsen, S. S. and Smith, L. J. and Konstantopoulos, I. S. and Zackrisson, E.},
	month = jan,
	year = {2012},
	keywords = {galaxies: star clusters: general, galaxies: individual: M83},
	pages = {2606--2622},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/JE6AD6GG/Bastian et al. - 2012 - Stellar clusters in M83 formation, evolution, dis.pdf:application/pdf},
}

@article{bastian_star_2008,
	title = {On the star formation rate - brightest cluster relation: estimating the peak star formation rate in post-merger galaxies},
	volume = {390},
	issn = {0035-8711},
	shorttitle = {On the star formation rate - brightest cluster relation},
	url = {http://adsabs.harvard.edu/abs/2008MNRAS.390..759B},
	doi = {10.1111/j.1365-2966.2008.13775.x},
	abstract = {We further the recent discussion on the relation between the star 
formation rate (SFR) of a galaxy and the luminosity of its brightest
star cluster (SFR versus MbrightestV). We first
show that the observed trend of SFR versus
MbrightestV is due to the brightest cluster in a
galaxy being preferentially young ({\textless}=15 Myr - for a constant SFR) and
hence a good tracer of the current SFR, although we give notable
exceptions to this rule. Archival Hubble Space Telescope (HST) imaging
of high-SFR galaxies, as well as additional galaxies/clusters from the
literature, is used to further confirm the observed trend. Using a
series of Monte Carlo simulations, we show that a pure power-law mass
function with index $\alpha$ = 2 is ruled out by the current data.
Instead, we find that a Schechter function (i.e. a power law with an
exponential truncation at the high-mass end) provides an excellent fit
to the data. Additionally, these simulations show that bound cluster
formation (in Msolaryr-1) represents only {\textasciitilde}8+/-3 per cent of
the total star formation within a galaxy, independent of the SFR. From
this, we conclude that there is only a single mode of cluster formation
which operates over at least 6 orders of magnitude in the SFR. We
provide a simple model of star/cluster formation feedback within dwarf
galaxies (and star-forming complexes within spirals) which highlights
the strong impact that a massive cluster can have on its surroundings.

Using this relation, we can extrapolate backwards in time in order to
estimate the peak SFR of major merger galaxies, such as NGC 7252,1316
and 3610. The derived SFRs for these galaxies are between a few hundred
and a few thousand solar masses per year. The inferred far-infrared
luminosity of the galaxies, from the extrapolated SFR, places them well
within the range of ultraluminous infrared galaxies (ULIRGs) and for NGC
7252 within the hyperluminous infrared galaxy (HLIRG) regime. Thus, we
provide evidence that these post-merger galaxies passed through a
ULIRG/HLIRG phase and are now evolving passively. Using the current and
extrapolated past SFR of NGC 34, we infer that the ULIRG phase of this
galaxy has lasted for at least 150 Myr.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Bastian, N.},
	month = oct,
	year = {2008},
	keywords = {galaxies: star clusters, galaxies: starburst},
	pages = {759--768},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/YGZNCQZA/Bastian - 2008 - On the star formation rate - brightest cluster rel.pdf:application/pdf},
}

@article{reina-campos_unified_2017,
	title = {A unified model for the maximum mass scales of molecular clouds, stellar clusters and high-redshift clumps},
	volume = {469},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2017MNRAS.469.1282R},
	doi = {10.1093/mnras/stx790},
	abstract = {We present a simple, self-consistent model to predict the maximum masses 
of giant molecular clouds (GMCs), stellar clusters and high-redshift
clumps as a function of the galactic environment. Recent works have
proposed that these maximum masses are set by shearing motions and
centrifugal forces, but we show that this idea is inconsistent with the
low masses observed across an important range of local-Universe
environments, such as low-surface density galaxies and galaxy outskirts.
Instead, we propose that feedback from young stars can disrupt clouds
before the global collapse of the shear-limited area is completed. We
develop a shear-feedback hybrid model that depends on three observable
quantities: the gas surface density, the epicylic frequency and the
Toomre parameter. The model is tested in four galactic environments: the
Milky Way, the Local Group galaxy M31, the spiral galaxy M83 and the
high-redshift galaxy zC406690. We demonstrate that our model
simultaneously reproduces the observed maximum masses of GMCs, clumps
and clusters in each of these environments. We find that clouds and
clusters in M31 and in the Milky Way are feedback-limited beyond radii
of 8.4 and 4 kpc, respectively, whereas the masses in M83 and zC406690
are shear-limited at all radii. In zC406690, the maximum cluster masses
decrease further due to their inspiral by dynamical friction. These
results illustrate that the maximum masses change from being
shear-limited to being feedback-limited as galaxies become less gas rich
and evolve towards low shear. This explains why high-redshift clumps are
more massive than GMCs in the local Universe.},
	urldate = {2020-04-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Reina-Campos, Marta and Kruijssen, J. M. Diederik},
	month = aug,
	year = {2017},
	keywords = {stars: formation, galaxies: star clusters: general, galaxies: evolution, galaxies: formation, globular clusters: general, ISM: clouds},
	pages = {1282--1298},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/ZAPGA5DN/Reina-Campos and Kruijssen - 2017 - A unified model for the maximum mass scales of mol.pdf:application/pdf},
}

@article{krumholz_star_2019,
	title = {Star {Clusters} {Across} {Cosmic} {Time}},
	volume = {57},
	issn = {0066-4146},
	url = {http://adsabs.harvard.edu/abs/2019ARA%26A..57..227K},
	doi = {10.1146/annurev-astro-091918-104430},
	abstract = {Star clusters stand at the intersection of much of modern astrophysics: the ISM, gravitational dynamics, stellar evolution, and cosmology. Here, we review observations and theoretical models for the formation, evolution, and eventual disruption of star clusters. Current literature suggests a picture of this life cycle including the following several phases: Clusters form in hierarchically structured, accreting molecular clouds that convert gas into stars at a low rate per dynamical time until feedback disperses the gas. The densest parts of the hierarchy resist gas removal long enough to reach high star-formation efficiency, becoming dynamically relaxed and well mixed. These remain bound after gas removal. In the first \~{}100 Myr after gas removal, clusters
disperse moderately fast, through a combination of mass loss and tidal shocks by dense molecular structures in the star-forming environment. After \~{}100 Myr, clusters lose mass via two-body relaxation and
shocks by giant molecular clouds, processes that preferentially affect low-mass clusters and cause a turnover in the cluster mass function to appear on \~{}1-10-Gyr timescales. Even after dispersal, some clusters remain coherent and thus detectable in chemical or action space for multiple galactic orbits.In the next decade, a new generation of space- and adaptive optics-assisted ground-based telescopes will enable us to test and refine this picture.},
	urldate = {2020-04-28},
	journal = {Annual Review of Astronomy and Astrophysics},
	author = {Krumholz, Mark R. and McKee, Christopher F. and Bland-Hawthorn, Joss},
	month = aug,
	year = {2019},
	pages = {227--303},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/229UVCKR/Krumholz et al. - 2019 - Star Clusters Across Cosmic Time.pdf:application/pdf},
}

@article{johnson_panchromatic_2017,
	title = {Panchromatic {Hubble} {Andromeda} {Treasury}. {XVIII}. {The} {High}-mass {Truncation} of the {Star} {Cluster} {Mass} {Function}},
	volume = {839},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2017ApJ...839...78J},
	doi = {10.3847/1538-4357/aa6a1f},
	abstract = {We measure the mass function for a sample of 840 young star clusters 
with ages between 10 and 300 Myr observed by the Panchromatic Hubble
Andromeda Treasury (PHAT) survey in M31. The data show clear evidence of
a high-mass truncation: only 15 clusters more massive than
\{10\}4 \{M\}? are observed, compared to the
\~{}100 expected for a canonical \{M\}-2 pure power-law mass
function with the same total number of clusters above the catalog
completeness limit. Adopting a Schechter function parameterization, we
fit a characteristic truncation mass of
\{M\}c=\{8.5\}-1.8+2.8{\texttimes}
\{10\}3 M ?. Although previous studies have
measured cluster mass function truncations, the characteristic
truncation mass we measure is the lowest ever reported. Combining this
M31 measurement with previous results, we find that the cluster mass
function truncation correlates strongly with the characteristic star
formation rate surface density of the host galaxy, where
\{M\}c{\textbackslash}propto {\textless} \{\{\{$\Sigma$ \}\}\}\{SFR\}\{\vphantom{\}}{\textgreater}
\vphantom{\{}\}\~{} 1.1. We also find evidence that suggests the observed
M c -\{\{\{$\Sigma$ \}\}\}\{SFR\} relation also applies to
globular clusters, linking the two populations via a common formation
pathway. If so, globular cluster mass functions could be useful tools
for constraining the star formation properties of their progenitor host
galaxies in the early universe.},
	urldate = {2020-04-06},
	journal = {The Astrophysical Journal},
	author = {Johnson, L. Clifton and Seth, Anil C. and Dalcanton, Julianne J. and Beerman, Lori C. and Fouesneau, Morgan and Weisz, Daniel R. and Bell, Timothy A. and Dolphin, Andrew E. and Sandstrom, Karin and Williams, Benjamin F.},
	month = apr,
	year = {2017},
	keywords = {galaxies: star clusters: general, galaxies: star formation, globular clusters: general, galaxies: individual: M31},
	pages = {78},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/XL9EVU6F/Johnson et al. - 2017 - Panchromatic Hubble Andromeda Treasury. XVIII. The.pdf:application/pdf},
}

@article{corbelli_molecules_2017,
	title = {From molecules to young stellar clusters: the star formation cycle across the disk of {M} 33},
	volume = {601},
	shorttitle = {From molecules to young stellar clusters},
	url = {https://ui.adsabs.harvard.edu/2017A&A...601A.146C/abstract},
	doi = {10.1051/0004-6361/201630034},
	abstract = {{\textless}BR /{\textgreater} Aims: We study the association between giant molecular clouds (GMCs) and young stellar cluster candidates (YSCCs) to shed light on the time evolution of local star formation episodes in the nearby galaxy M 33. {\textless}BR /{\textgreater} Methods: The CO (J = 2-1) IRAM all-disk survey was used to identify and classify 566 GMCs with masses between 2 {\texttimes} 10{\textless}SUP{\textgreater}4{\textless}/SUP{\textgreater} and 2 {\texttimes} 10{\textless}SUP{\textgreater}6{\textless}/SUP{\textgreater}M{\textless}SUB{\textgreater}?{\textless}/SUB{\textgreater} across the whole star-forming disk of M 33. In the same area, there are 630 YSCCs that we identified using Spitzer-24 $\mu$m data. Some YSCCs are embedded star-forming sites, while the majority have GALEX-UV and H$\alpha$ counterparts with estimated cluster masses and ages. {\textless}BR /{\textgreater} Results: The GMC classes correspond to different cloud evolutionary stages: inactive clouds are 32\% of the total and classified clouds with embedded and exposed star formation are 16\% and 52\% of the total, respectively. Across the regular southern spiral arm, inactive clouds are preferentially located in the inner part of the arm, possibly suggesting a triggering of star formation as the cloud crosses the arm. The spatial correlation between YSCCs and GMCs is extremely strong, with a typical separation of 17 pc. This is less than half the CO (2-1) beam size and illustrates the remarkable physical link between the two populations. GMCs and YSCCs follow the HI filaments, except in the outermost regions, where the survey finds fewer GMCs than YSCCs, which is most likely due to undetected clouds with low CO luminosity. The distribution of the non-embedded YSCC ages peaks around 5 Myr, with only a few being as old as 8-10 Myr. These age estimates together with the number of GMCs in the various evolutionary stages lead us to conclude that 14 Myr is the typical lifetime of a GMC in M 33 prior to cloud dispersal. The inactive and embedded phases are short, lasting about 4 and 2 Myr, respectively. This underlines that embedded YSCCs rapidly break out from the clouds and become partially visible in H$\alpha$ or UV long before cloud dispersal. Full Tables 5 and 6 are only available at the CDS via anonymous ftp to {\textless}A href="http://cdsarc.u-strasbg.fr"{\textgreater}http://cdsarc.u-strasbg.fr{\textless}/A{\textgreater} ({\textless}A href="http://130.79.128.5"{\textgreater}http://130.79.128.5{\textless}/A{\textgreater}) or via {\textless}A href="http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/601/A146"{\textgreater}http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/601/A146{\textless}/A{\textgreater}},
	language = {en},
	urldate = {2019-10-18},
	journal = {Astronomy and Astrophysics},
	author = {Corbelli, Edvige and Braine, Jonathan and Bandiera, Rino and Brouillet, Nathalie and Combes, Fran{\c c}oise and Druard, Cl{\'e}ment and Gratier, Pierre and Mata, Jimmy and Schuster, Karl and Xilouris, Manolis and Palla, Francesco},
	month = may,
	year = {2017},
	pages = {A146},
	file = {Snapshot:/Users/Tobin/Zotero/storage/QLRJNDVU/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/KPGJ9GBN/Corbelli et al. - 2017 - From molecules to young stellar clusters the star.pdf:application/pdf},
}

@article{sharma_population_2011,
	title = {The population of young stellar clusters throughout the disk of {M} 33},
	volume = {534},
	copyright = {{\textcopyright} ESO, 2011},
	issn = {0004-6361, 1432-0746},
	url = {https://www.aanda.org/articles/aa/abs/2011/10/aa17812-11/aa17812-11.html},
	doi = {10.1051/0004-6361/201117812},
	abstract = {{\textless}i{\textgreater}Aims.{\textless}i/{\textgreater} The properties of young stellar clusters (YSCs) in M 33, identified from the center out to about twice the size of the bright star-forming disk, are investigated to determine possible spatial and time variations of the star formation process in this Local Group blue galaxy.{\textless}i{\textgreater}Methods.{\textless}i/{\textgreater} 915 MIR sources have been extracted from the {\textless}i{\textgreater}Spitzer {\textless}i/{\textgreater}24 {\textless}i{\textgreater}$\mu${\textless}i/{\textgreater}m image. Upon inspection of H{\textless}i{\textgreater}$\alpha${\textless}i/{\textgreater} and GALEX images and exclusion of evolved AGB stars, a sample of 648 objects is selected as candidate YSCs and their luminosity function is examined. The spectral energy distribution of each object, based on aperture photometry, is compared with Starburst99 models to derive age, mass and {\textless}i{\textgreater}A{\textless}i/{\textgreater}{\textless}sub{\textgreater}V{\textless}sub/{\textgreater} of individual clusters. In the analysis we allow for different values of the upper mass cutoff of the stellar initial mass function (IMF), the porosity of the ISM, and the dustiness of HII regions. We also examine the influence of different dust models and include corrections for incompleteness of the IMF.{\textless}i{\textgreater}Results.{\textless}i/{\textgreater} We find discrete MIR sources as far as the extent of the warped HI disk, i.e. 16 kpc from the galaxy center. Their surface density has a steep radial decline beyond 4.5 kpc, and flattens out beyond the optical radius at 8.5 kpc. We are able to identify YSCs out to 12 kpc. At large galactocentric radii, the paucity of luminous clusters and the relevance of hot dust emission become evident from the analysis of the bolometric and MIR luminosity functions. The YSC mass and size are correlated with a log-log slope of 2.09 {\textpm} 0.01, similar to that measured for giant molecular clouds in M 33 and the Milky Way, which represent the protocluster environment. Most of the YSCs in our sample have {\textless}i{\textgreater}A{\textless}i/{\textgreater}{\textless}sub{\textgreater}V{\textless}sub/{\textgreater} {\textasciitilde} 0-1 mag and ages between 3 and 10 Myr. In the inner regions of M 33 the clusters span a wide range of mass (10{\textless}sup{\textgreater}2{\textless}sup/{\textgreater} {\textless} {\textless}i{\textgreater}M{\textless}i/{\textgreater} {\textless} 3 {\texttimes} 10{\textless}sup{\textgreater}5{\textless}sup/{\textgreater} {\textless}i{\textgreater}M{\textless}i/{\textgreater}{\textless}sub{\textgreater}?{\textless}sub/{\textgreater}) and luminosity (10{\textless}sup{\textgreater}38{\textless}sup/{\textgreater} {\textless} {\textless}i{\textgreater}L{\textless}i/{\textgreater}{\textless}sub{\textgreater}bol{\textless}sub/{\textgreater} {\textless} 3 {\texttimes} 10{\textless}sup{\textgreater}41{\textless}sup/{\textgreater} erg s{\textless}sup{\textgreater}-1{\textless}sup/{\textgreater}), while at galactocentric radii larger than {\textasciitilde}4 kpc we find a deficiency of massive clusters. Beyond 7 kpc, where the H{\textless}i{\textgreater}$\alpha${\textless}i/{\textgreater} surface brightness drops significantly, the dominant YSC population has {\textless}i{\textgreater}M{\textless}i/{\textgreater} {\textless} 10{\textless}sup{\textgreater}3{\textless}sup/{\textgreater} {\textless}i{\textgreater}M{\textless}i/{\textgreater}{\textless}sub{\textgreater}?{\textless}sub/{\textgreater} and a slightly older age (10 Myr). This implies the occurrence of star formation events about 10 Myr ago as far as 10-12 kpc from the center of M 33. The cluster {\textless}i{\textgreater}L{\textless}i/{\textgreater}{\textless}sub{\textgreater}FUV{\textless}sub/{\textgreater} vs. {\textless}i{\textgreater}L{\textless}i/{\textgreater}{\textless}sub{\textgreater}H{\textless}i{\textgreater}$\alpha${\textless}i/{\textgreater}{\textless}sub/{\textgreater} relation is non-linear for {\textless}i{\textgreater}L{\textless}i/{\textgreater}{\textless}sub{\textgreater}FUV{\textless}sub/{\textgreater} {\textless} 10{\textless}sup{\textgreater}39{\textless}sup/{\textgreater} erg s{\textless}sup{\textgreater}-1{\textless}sup/{\textgreater}, in agreement with randomly sampled models of the IMF which, furthermore, shows no appreciable variation throughout the M 33 disk.},
	language = {en},
	urldate = {2019-10-01},
	journal = {Astronomy \& Astrophysics},
	author = {Sharma, S. and Corbelli, E. and Giovanardi, C. and Hunt, L. K. and Palla, F.},
	month = oct,
	year = {2011},
	pages = {A96},
	file = {Snapshot:/Users/Tobin/Zotero/storage/JTUKN4IA/aa17812-11.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/8ECFCCNB/Sharma et al. - 2011 - The population of young stellar clusters throughou.pdf:application/pdf},
}

@article{johnson_phat_2012,
	title = {{PHAT} {S}TEL{LAR} {CLUSTER} {SURVEY}. {I}. {YEAR} 1 {CATALOG} {AND} {INTEGRATED} {PHOTOMETRY}},
	volume = {752},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F752%2F2%2F95},
	doi = {10.1088/0004-637X/752/2/95},
	abstract = {The Panchromatic Hubble Andromeda Treasury (PHAT) survey is an ongoing Hubble Space Telescope (HST) multi-cycle program to obtain high spatial resolution imaging of one-third of the M31 disk at ultraviolet through near-infrared wavelengths. In this paper, we present the first installment of the PHAT stellar cluster catalog. When completed, the PHAT cluster catalog will be among the largest and most comprehensive surveys of resolved star clusters in any galaxy. The exquisite spatial resolution achieved with HST has allowed us to identify hundreds of new clusters that were previously inaccessible with existing ground-based surveys. We identify 601 clusters in the Year 1 sample, representing more than a factor of four increase over previous catalogs within the current survey area (390 arcmin2). This work presents results derived from the first \~{}25\% of the survey data; we estimate that the final sample will include \~{}2500 clusters. For the Year 1 objects, we present a catalog with positions, radii, and six-band integrated photometry. Along with a general characterization of the cluster luminosities and colors, we discuss the cluster luminosity function, the cluster size distributions, and highlight a number of individually interesting clusters found in the Year 1 search.},
	language = {en},
	number = {2},
	urldate = {2019-09-25},
	journal = {The Astrophysical Journal},
	author = {Johnson, L. Clifton and Seth, Anil C. and Dalcanton, Julianne J. and Caldwell, Nelson and Fouesneau, Morgan and Gouliermis, Dimitrios A. and Hodge, Paul W. and Larsen, S{\o}ren S. and Olsen, Knut A. G. and Roman, Izaskun San and Sarajedini, Ata and Weisz, Daniel R. and Williams, Benjamin F. and Beerman, Lori C. and Bianchi, Luciana and Dolphin, Andrew E. and Girardi, L{\'e}o and Guhathakurta, Puragra and Kalirai, Jason and Lang, Dustin and Monachesi, Antonela and Nanda, Sanjay and Rix, Hans-Walter and Skillman, Evan D.},
	month = may,
	year = {2012},
	pages = {95},
}

@article{fouesneau_panchromatic_2014,
	title = {The {Panchromatic} {Hubble} {Andromeda} {Treasury} {V}: {Ages} and {Masses} of the {Year} 1 {Stellar} {Clusters}},
	volume = {786},
	issn = {0004-637X, 1538-4357},
	shorttitle = {The {Panchromatic} {Hubble} {Andromeda} {Treasury} {V}},
	url = {http://arxiv.org/abs/1402.7264},
	doi = {10.1088/0004-637X/786/2/117},
	abstract = {We present ages and masses for 601 star clusters in M31 from the analysis of the six filter integrated light measurements from near ultraviolet to near infrared wavelengths, made as part of the Panchromatic Hubble Andromeda Treasury (PHAT). We derive the ages and masses using a probabilistic technique, which accounts for the effects of stochastic sampling of the stellar initial mass function. Tests on synthetic data show that this method, in conjunction with the exquisite sensitivity of the PHAT observations and their broad wavelength baseline, provides robust age and mass recovery for clusters ranging from \~{} 102 - 2 {\texttimes} 106 M?. We find that the cluster age distribution is consistent with being uniform over the past 100 Myr, which suggests a weak effect of cluster disruption within M31. The age distribution of older ({\textgreater} 100 Myr) clusters fall towards old ages, consistent with a power-law decline of index -1, likely from a combination of fading and disruption of the clusters. We find that the mass distribution of the whole sample can be well-described by a single power-law with a spectral index of -1.9 {\textpm} 0.1 over the range of 103 - 3 {\texttimes} 105 M?. However, if we subdivide the sample by galactocentric radius, we find that the age distributions remain unchanged. However, the mass spectral index varies significantly, showing best fit values between -2.2 and -1.8, with the shallower slope in the highest star formation intensity regions. We explore the robustness of our study to potential systematics and conclude that the cluster mass function may vary with respect to environment.},
	language = {en},
	number = {2},
	urldate = {2019-09-24},
	journal = {The Astrophysical Journal},
	author = {Fouesneau, Morgan and Johnson, L. Clifton and Weisz, Daniel R. and Dalcanton, Julianne J. and Bell, Eric F. and Bianchi, Luciana and Caldwell, Nelson and Gouliermis, Dimitrios A. and Guhathakurta, Puragra and Kalirai, Jason and Larsen, S{\o}ren S. and Rix, Hans-Walter and Seth, Anil C. and Skillman, Evan D. and Williams, Benjamin F. and collaboration, PHAT},
	month = apr,
	year = {2014},
	note = {arXiv: 1402.7264},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {117},
	file = {Fouesneau et al. - 2014 - The Panchromatic Hubble Andromeda Treasury V Ages.pdf:/Users/Tobin/Zotero/storage/K97RS5KG/Fouesneau et al. - 2014 - The Panchromatic Hubble Andromeda Treasury V Ages.pdf:application/pdf},
}

@article{ashworth_exploring_2017,
	title = {Exploring the {IMF} of star clusters: a joint {SLUG} and {LEGUS} effort},
	volume = {469},
	issn = {0035-8711, 1365-2966},
	shorttitle = {Exploring the {IMF} of star clusters},
	url = {http://arxiv.org/abs/1705.02980},
	doi = {10.1093/mnras/stx935},
	abstract = {We present the implementation of a Bayesian formalism within the Stochastically Lighting Up Galaxies (SLUG) stellar population synthesis code, which is designed to investigate variations in the initial mass function (IMF) of star clusters. By comparing observed cluster photometry to large libraries of clusters simulated with a continuously varying IMF, our formalism yields the posterior probability distribution function (PDF) of the cluster mass, age, and extinction, jointly with the parameters describing the IMF. We apply this formalism to a sample of star clusters from the nearby galaxy NGC 628, for which broad-band photometry in five filters is available as part of the Legacy ExtraGalactic UV Survey (LEGUS). After allowing the upper-end slope of the IMF (\${\textbackslash}alpha\_3\$) to vary, we recover PDFs for the mass, age, and extinction that are broadly consistent with what is found when assuming an invariant Kroupa IMF. However, the posterior PDF for \${\textbackslash}alpha\_3\$ is very broad due to a strong degeneracy with the cluster mass, and it is found to be sensitive to the choice of priors, particularly on the cluster mass. We find only a modest improvement in the constraining power of \${\textbackslash}alpha\_3\$ when adding H\${\textbackslash}alpha\$ photometry from the companion H\${\textbackslash}alpha\$-LEGUS survey. Conversely, H\${\textbackslash}alpha\$ photometry significantly improves the age determination, reducing the frequency of multi-modal PDFs. With the aid of mock clusters we quantify the degeneracy between physical parameters, showing how constraints on the cluster mass that are independent of photometry can be used to pin down the IMF properties of star clusters.},
	number = {2},
	urldate = {2019-08-14},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Ashworth, G. and Fumagalli, M. and Krumholz, M. R. and Adamo, A. and Calzetti, D. and Chandar, R. and Cignoni, M. and Dale, D. and Elmegreen, B. G. and Gallagher III, J. S. and Gouliermis, D. A. and Grasha, K. and Grebel, E. K. and Johnson, K. E. and Lee, J. and Tosi, M. and Wofford, A.},
	month = aug,
	year = {2017},
	note = {arXiv: 1705.02980},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {2464--2480},
	file = {arXiv.org Snapshot:/Users/Tobin/Zotero/storage/3QK73KH7/1705.html:text/html;arXiv\:1705.02980 PDF:/Users/Tobin/Zotero/storage/HH74FVEP/Ashworth et al. - 2017 - Exploring the IMF of star clusters a joint SLUG a.pdf:application/pdf},
}

@article{land_galaxy_2008,
	title = {Galaxy {Zoo}: the large-scale spin statistics of spiral galaxies in the {Sloan} {Digital} {Sky} {Survey}},
	volume = {388},
	issn = {0035-8711},
	shorttitle = {Galaxy {Zoo}},
	url = {https://academic.oup.com/mnras/article/388/4/1686/981637},
	doi = {10.1111/j.1365-2966.2008.13490.x},
	abstract = {Abstract.  We re-examine the evidence for a violation of large-scale statistical isotropy in the distribution of projected spin vectors of spiral galaxies. We h},
	language = {en},
	number = {4},
	urldate = {2019-07-18},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Land, Kate and Slosar, An{\v z}e and Lintott, Chris and Andreescu, Dan and Bamford, Steven and Murray, Phil and Nichol, Robert and Raddick, M. Jordan and Schawinski, Kevin and Szalay, Alex and Thomas, Daniel and Vandenberg, Jan},
	month = aug,
	year = {2008},
	pages = {1686--1692},
	file = {1402.7264.pdf:/Users/Tobin/Zotero/storage/C7SQ838M/1402.7264.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/D7JHU8DX/981637.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/VL9AQ676/Land et al. - 2008 - Galaxy Zoo the large-scale spin statistics of spi.pdf:application/pdf},
}

@article{lintott_galaxy_2008,
	title = {Galaxy {Zoo}: morphologies derived from visual inspection of galaxies from the {Sloan} {Digital} {Sky} {Survey}},
	volume = {389},
	issn = {0035-8711},
	shorttitle = {Galaxy {Zoo}},
	url = {https://academic.oup.com/mnras/article/389/3/1179/1017183},
	doi = {10.1111/j.1365-2966.2008.13689.x},
	abstract = {Abstract.  In order to understand the formation and subsequent evolution of galaxies one must first distinguish between the two main morphological classes of ma},
	language = {en},
	number = {3},
	urldate = {2019-07-18},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Lintott, Chris J. and Schawinski, Kevin and Slosar, An{\v z}e and Land, Kate and Bamford, Steven and Thomas, Daniel and Raddick, M. Jordan and Nichol, Robert C. and Szalay, Alex and Andreescu, Dan and Murray, Phil and Vandenberg, Jan},
	month = sep,
	year = {2008},
	pages = {1179--1189},
	file = {Snapshot:/Users/Tobin/Zotero/storage/A4MIR9DS/1017183.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/2FK64YAX/Lintott et al. - 2008 - Galaxy Zoo morphologies derived from visual inspe.pdf:application/pdf},
}

@article{schwamb_planet_2012,
	title = {{PLANET} {HUNTERS}: {ASSESSING} {THEKEPLERINVENTORY} {OF} {SHORT}-{PERIOD} {PLANETS}},
	volume = {754},
	issn = {0004-637X},
	shorttitle = {{PLANET} {HUNTERS}},
	url = {https://doi.org/10.1088%2F0004-637x%2F754%2F2%2F129},
	doi = {10.1088/0004-637X/754/2/129},
	abstract = {We present the results from a search of data from the first 33.5 days of the Kepler science mission (Quarter 1) for exoplanet transits by the Planet Hunters citizen science project. Planet Hunters enlists members of the general public to visually identify transits in the publicly released Kepler light curves via the World Wide Web. Over 24,000 volunteers reviewed the Kepler Quarter 1 data set. We examine the abundance of ?2 R (+) planets on short-period ({\textless}15 days) orbits based on Planet Hunters detections. We present these results along with an analysis of the detection efficiency of human classifiers to identify planetary transits including a comparison to the Kepler inventory of planet candidates. Although performance drops rapidly for smaller radii, ?4 R (+) Planet Hunters ?85\% efficient at identifying transit signals for planets with periods less than 15 days for the Kepler sample of target stars. Our high efficiency rate for simulated transits along with recovery of the majority of Kepler ?4 R (+) planets suggests that the Kepler inventory of ?4 R (+) short-period planets is nearly complete.},
	language = {en},
	number = {2},
	urldate = {2019-07-18},
	journal = {The Astrophysical Journal},
	author = {Schwamb, Megan E. and Lintott, Chris J. and Fischer, Debra A. and Giguere, Matthew J. and Lynn, Stuart and Smith, Arfon M. and Brewer, John M. and Parrish, Michael and Schawinski, Kevin and Simpson, Robert J.},
	month = jul,
	year = {2012},
	pages = {129},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/CMFD5XA7/Schwamb et al. - 2012 - PLANET HUNTERS ASSESSING THEKEPLERINVENTORY OF SH.pdf:application/pdf},
}

@article{ma_metallicity_2004,
	title = {Metallicity estimates for old star clusters in {M} 33},
	volume = {413},
	issn = {0004-6361},
	doi = {10.1051/0004-6361:20031556},
	abstract = {Using the theoretical stellar population synthesis models of BC96, Kong et al. (2003) showed that some BATC colors and color indices could be used to disentangle the age and metallicity effect. They found that there is a very good relation between the flux ratio of L\_\{8510\}/L\_\{9170\} and the metallicity for stellar populations older than 1 Gyr. In this paper, based on the Kong et al. results and on the multicolor spectrophotometry of Ma et al. (2001, 2002a,b,c), we estimate the metallicities of 31 old star clusters in the nearby spiral galaxy M33, 23 of which are ``true'' globular clusters. The results show that most of these old clusters are metal poor. We also find that the ages and metal abundance for these old star clusters of M33 do not vary with deprojected radial position. Comment: Accepted for Publication in A\&A, 13 pages, 7 figures (1 figure of jpg)},
	language = {English},
	number = {2},
	journal = {Astronomy \& Astrophysics},
	author = {Ma, J. and Zhou, X. and Chen, Js},
	year = {2004},
	keywords = {Astrophysics;},
	pages = {563--570},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/VRM7RJW3/Ma et al. - 2004 - Metallicity estimates for old star clusters in M 3.pdf:application/pdf},
}

@article{de_meulenaer_deriving_2013,
	title = {Deriving physical parameters of unresolved star clusters. {I}. {Age}, mass, and extinction degeneracies},
	volume = {550},
	url = {https://ui.adsabs.harvard.edu/abs/2013A%26A...550A..20D/abstract},
	doi = {10.1051/0004-6361/201220674},
	abstract = {Context. Stochasticity and physical parameter degeneracy problems complicate the derivation of the parameters (age, mass, and extinction) of unresolved star clusters when using broad-band photometry. {\textless}BR /{\textgreater} Aims: We develop a method to simulate stochasticity and degeneracies and to investigate their influence on the accuracy of derived physical parameters. Then we apply it to star cluster samples of M 31 and M 33 galaxies. {\textless}BR /{\textgreater} Methods: Age, mass, and extinction of observed star clusters are derived by comparing their broad-band UBVRI integrated magnitudes to the magnitudes of a large grid of star cluster models with fixed metallicity Z = 0.008. Masses of stars for a cluster model are randomly sampled from the initial mass function. Models of star clusters from the model grid, which have all of their magnitudes located within 3 observational errors from the magnitudes of the observed cluster, are selected for computing their age, mass, and extinction. {\textless}BR /{\textgreater} Results: In the case of the M 31 galaxy, the extinction range is wide and the age-extinction degeneracy is strong for a fraction of its clusters. Because of a narrower extinction range, the age-extinction degeneracy is weaker for the M 33 clusters. By using artificial cluster sample, we show that age-extinction degeneracy can be reduced significantly if the range of intrinsic extinction within the host galaxy is narrow. Figures 6-8 are available in electronic form at {\textless}A href="http://www.aanda.org"{\textgreater}http://www.aanda.org{\textless}/A{\textgreater}},
	language = {en},
	urldate = {2019-07-18},
	journal = {Astronomy and Astrophysics},
	author = {de Meulenaer, P. and Narbutis, D. and Mineikis, T. and Vansevi{\v c}ius, V.},
	month = feb,
	year = {2013},
	pages = {A20},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/Z2V9DUWP/de Meulenaer et al. - 2013 - Deriving physical parameters of unresolved star cl.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/AGPF4UZV/abstract.html:text/html},
}

@article{de_meulenaer_deriving_2014,
	title = {Deriving physical parameters of unresolved star clusters. {II}. {The} degeneracies of age, mass, extinction, and metallicity},
	volume = {569},
	url = {https://ui.adsabs.harvard.edu/abs/2014A%26A...569A...4D/abstract},
	doi = {10.1051/0004-6361/201423988},
	abstract = {Context. This paper is the second of a series that investigates the stochasticity and degeneracy problems that hinder the derivation of the age, mass, extinction, and metallicity of unresolved star clusters in external galaxies when broad-band photometry is used. {\textless}BR /{\textgreater} Aims: While Paper I concentrated on deriving age, mass, and extinction of star clusters for one fixed metallicity, we here derive these parameters in case when metallicity is let free to vary. The results were obtained using several different filter systems (UBVRI, UBVRIJHK, GALEX+UBVRI), which allowed us to optimally reduce the different degeneracies between the cluster physical parameters. {\textless}BR /{\textgreater} Methods: The age, mass, and extinction of a sample of artificial star clusters were derived by comparing their broad-band integrated magnitudes with the magnitudes of a large grid of cluster models with various metallicities. {\textless}BR /{\textgreater} Results: A large collection of artificial clusters was studied to model the different degeneracies in the age, mass, extinction, and metallicity parameter space when stochasticity is taken into account in the cluster models. We show that, without prior knowledge on the metallicity, the optical bands (UBVRI) fail to allow a correct derivation of the age, mass, and extinction because of the strong degeneracies between models of different metallicities. Adding near-infrared information (UBVRI+JHK) slightly helps in improving the parameter derivation, except for the metallicity. Adding ultraviolet data (GALEX+UBVRI) helps significantly in deriving these parameters and allows constraining the metallicity when the photometric errors have a Gaussian distribution with standard deviations 0.05 mag for UBVRI and 0.15 mag for the GALEX bands.},
	language = {en},
	urldate = {2019-07-18},
	journal = {Astronomy and Astrophysics},
	author = {de Meulenaer, P. and Narbutis, D. and Mineikis, T. and Vansevi{\v c}ius, V.},
	month = sep,
	year = {2014},
	pages = {A4},
	file = {Snapshot:/Users/Tobin/Zotero/storage/GPEG27ET/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/JE2W9KX3/de Meulenaer et al. - 2014 - Deriving physical parameters of unresolved star cl.pdf:application/pdf},
}

@article{de_meulenaer_deriving_2015,
	title = {Deriving physical parameters of unresolved star clusters. {III}. {Application} to {M} 31 {PHAT} clusters},
	volume = {574},
	url = {https://ui.adsabs.harvard.edu/abs/2015A%26A...574A..66D/abstract},
	doi = {10.1051/0004-6361/201425121},
	abstract = {Context. This study is the third of a series that investigates the degeneracy and stochasticity problems present in the determination of physical parameters such as age, mass, extinction, and metallicity of partially resolved or unresolved star cluster populations situated in external galaxies when using broad-band photometry. {\textless}BR /{\textgreater} Aims: This work tests the derivation of parameters of artificial star clusters using models with fixed and free metallicity for the WFC3+ACS photometric system. Then the method is applied to derive parameters of a sample of 203 star clusters in the Andromeda galaxy observed with the HST. {\textless}BR /{\textgreater} Methods: Following Papers I and II, the star cluster parameters are derived using a large grid of stochastic models that are compared to the observed cluster broad-band integrated WFC3+ACS magnitudes. {\textless}BR /{\textgreater} Results: We derive the age, mass, and extinction of the sample of M 31 star clusters with one fixed metallicity in agreement with previous studies. Using artificial tests we demonstrate the ability of the WFC3+ACS photometric system to derive the metallicity of star clusters. We show that the metallicity derived using photometry of 36 massive M 31 star clusters is in a good agreement with the metallicity previously derived using spectroscopy taken from literature.},
	language = {en},
	urldate = {2019-07-18},
	journal = {Astronomy and Astrophysics},
	author = {de Meulenaer, P. and Narbutis, D. and Mineikis, T. and Vansevi{\v c}ius, V.},
	month = feb,
	year = {2015},
	pages = {A66},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/B8GPBIJI/de Meulenaer et al. - 2015 - Deriving physical parameters of unresolved star cl.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/ZUMEY2CU/abstract.html:text/html},
}

@article{meulenaer_deriving_2015,
	title = {Deriving physical parameters of unresolved star clusters - {IV}. {The} {M} 33 star cluster system},
	volume = {581},
	copyright = {{\textcopyright} ESO, 2015},
	issn = {0004-6361, 1432-0746},
	url = {https://www.aanda.org/articles/aa/abs/2015/09/aa26544-15/aa26544-15.html},
	doi = {10.1051/0004-6361/201526544},
	abstract = {{\textless}i{\textgreater}Context. {\textless}i/{\textgreater}When trying to derive the star cluster physical parameters of the M 33 galaxy using broad-band unresolved ground-based photometry, previous studies mainly made use of simple stellar population models, shown in the recent years to be oversimplified.{\textless}i{\textgreater}Aims. {\textless}i/{\textgreater}In this study, we aim to derive the star cluster physical parameters (age, mass, and extinction; metallicity is assumed to be LMC-like for clusters with age below 1 Gyr and left free for older clusters) of this galaxy using models that take stochastic dispersion of cluster integrated colors into account.{\textless}i{\textgreater}Methods. {\textless}i/{\textgreater}We use three recently published M 33 catalogs of cluster optical broad-band photometry in standard {\textless}i{\textgreater}UBVRI{\textless}i/{\textgreater} and in CFHT/MegaCam {\textless}i{\textgreater}u{\textless}i/{\textgreater}{\textless}sup{\textgreater}*{\textless}sup/{\textgreater}{\textless}i{\textgreater}g{\textless}i/{\textgreater}'{\textless}i{\textgreater}r{\textless}i/{\textgreater}'{\textless}i{\textgreater}i{\textless}i/{\textgreater}'{\textless}i{\textgreater}z{\textless}i/{\textgreater}' photometric systems. We also use near-infrared {\textless}i{\textgreater}JHK{\textless}i/{\textgreater} photometry that we derive from deep 2MASS images. We derive the cluster parameters using a method that takes into account the stochasticity problem, presented in previous papers of this series.{\textless}i{\textgreater}Results. {\textless}i/{\textgreater}The derived differential age distribution of the M 33 cluster population is composed of a two-slope profile indicating that the number of clusters decreases when age gets older. The first slope is interpreted as the evolutionary fading phase of the cluster magnitudes, and the second slope as the cluster disruption. The threshold between these two phases occurs at {\textasciitilde}300 Myr, comparable to what is observed in the M 31 galaxy. We also model by use of artificial clusters the ability of the cluster physical parameter derivation method to correctly derive the two-slope profile for different photometric systems tested.},
	language = {en},
	urldate = {2019-07-18},
	journal = {Astronomy \& Astrophysics},
	author = {Meulenaer, P. de and Narbutis, D. and Mineikis, T. and Vansevi{\v c}ius, V.},
	month = sep,
	year = {2015},
	pages = {A111},
	file = {Snapshot:/Users/Tobin/Zotero/storage/QXIIFUGW/aa26544-15.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/3YPDMNF4/Meulenaer et al. - 2015 - Deriving physical parameters of unresolved star cl.pdf:application/pdf},
}

@article{anders_stochastic_2013,
	title = {{STOCHASTIC} {S}TEL{LAR} {CLUSTER} {INITIAL} {MASS} {FUNCTIONS}: {MODELS} {AND} {IMPACT} {ON} {INTEGRATED} {CLUSTER} {PARAMETER} {DETERMINATION}},
	volume = {778},
	issn = {0004-637X},
	shorttitle = {{STOCHASTIC} {S}TEL{LAR} {CLUSTER} {INITIAL} {MASS} {FUNCTIONS}},
	url = {https://doi.org/10.1088%2F0004-637x%2F778%2F2%2F138},
	doi = {10.1088/0004-637X/778/2/138},
	abstract = {Stellar clusters are regularly used to study the evolution of their host galaxy. Except for a few nearby galaxies, these studies rely on the interpretation of integrated cluster properties, especially integrated photometry observed using multiple filters (i.e., the spectral energy distribution, SED). To allow interpretation of such observations, we present a large set of GALEV cluster models using the realistic approach of adopting stochastically sampled stellar initial mass functions. We provide models for a wide range of cluster masses (103-2 {\texttimes} 105 M ?), metallicities ({\textendash}2.3 ? [Fe/H] ? +0.18 dex), foreground extinction, and 184 regularly used filters. We analyze various sets of stochastic cluster SEDs by fitting them with non-stochastic models, which is the procedure commonly used in this field. We identify caveats and quantify the fitting uncertainties associated with this standard procedure. We show that this can yield highly unreliable fitting results, especially for low-mass clusters.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {The Astrophysical Journal},
	author = {Anders, P. and Kotulla, R. and Grijs, R. de and Wicker, J.},
	month = nov,
	year = {2013},
	pages = {138},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/RKNWFGSF/Anders et al. - 2013 - STOCHASTIC STELLAR CLUSTER INITIAL MASS FUNCTIONS M.pdf:application/pdf},
}

@article{johnson_panchromatic_2016,
	title = {{PANCHROMATIC} {HUBBLE} {ANDROMEDA} {TREASURY}. {XVI}. {STAR} {CLUSTER} {FORMATION} {EFFICIENCY} {AND} {THE} {CLUSTERED} {FRACTION} {OF} {YOUNG} {STARS}},
	volume = {827},
	issn = {0004-637X},
	url = {https://doi.org/10.3847%2F0004-637x%2F827%2F1%2F33},
	doi = {10.3847/0004-637X/827/1/33},
	abstract = {We use the Panchromatic Hubble Andromeda Treasury survey data set to perform spatially resolved measurements of star cluster formation efficiency ($\Gamma$), the fraction of stellar mass formed in long-lived star clusters. We use robust star formation history and cluster parameter constraints, obtained through color{\textendash}magnitude diagram analysis of resolved stellar populations, to study Andromeda{\textquoteright}s cluster and field populations over the last \~{}300 Myr. We measure $\Gamma$ of 4\%{\textendash}8\% for young, 10{\textendash}100 Myr-old populations in M31. We find that cluster formation efficiency varies systematically across the M31 disk, consistent with variations in mid-plane pressure. These $\Gamma$ measurements expand the range of well-studied galactic environments, providing precise constraints in an H i-dominated, low-intensity star formation environment. Spatially resolved results from M31 are broadly consistent with previous trends observed on galaxy-integrated scales, where $\Gamma$ increases with increasing star formation rate surface density ($\Sigma$SFR). However, we can explain observed scatter in the relation and attain better agreement between observations and theoretical models if we account for environmental variations in gas depletion time ($\tau$ dep) when modeling $\Gamma$, accounting for the qualitative shift in star formation behavior when transitioning from a H2-dominated to a H i-dominated interstellar medium. We also demonstrate that $\Gamma$ measurements in high $\Sigma$SFR starburst systems are well-explained by $\tau$ dep-dependent fiducial $\Gamma$ models.},
	language = {en},
	number = {1},
	urldate = {2019-07-16},
	journal = {The Astrophysical Journal},
	author = {Johnson, L. Clifton and Seth, Anil C. and Dalcanton, Julianne J. and Beerman, Lori C. and Fouesneau, Morgan and Lewis, Alexia R. and Weisz, Daniel R. and Williams, Benjamin F. and Bell, Eric F. and Dolphin, Andrew E. and Larsen, S{\o}ren S. and Sandstrom, Karin and Skillman, Evan D.},
	month = aug,
	year = {2016},
	pages = {33},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/EYQHYBW7/Johnson et al. - 2016 - PANCHROMATIC HUBBLE ANDROMEDA TREASURY. XVI. STAR .pdf:application/pdf},
}

@article{sarajedini_catalog_2007,
	title = {A {Catalog} of {Star} {Cluster} {Candidates} in {M33}},
	volume = {134},
	issn = {1538-3881},
	url = {https://iopscience.iop.org/article/10.1086/518835/meta},
	doi = {10.1086/518835},
	abstract = {We present a new catalog of star cluster candidates in the nearby spiral galaxy M33. It is based on eight existing catalogs wherein we have cross-referenced identifications and endeavored to resolve inconsistencies between them. Our catalog contains 451 candidates, of which 255 are confirmed clusters based on Hubble Space Telescope and high-resolution ground-based imaging. The catalog contains precise cluster positions (right ascension and declination), magnitudes and colors in the UBVRIJHKS filters, metallicities, radial velocities, masses and ages, where available, and galactocentric distances for each cluster. The color distribution of the M33 clusters appears to be similar to those in the Large Magellanic Cloud, with major peaks at (B - V)0 {\textasciitilde} 0.15 and (B - V)0 {\textasciitilde} 0.65. The intrinsic colors are correlated with cluster ages, which range from 107.5 to 1010.3 yr. The age distribution of the star clusters supports the notion of rapid cluster disruption with a slope of $\alpha$ = -1.09 {\textpm} 0.07 in the dNclus/d$\tau$ ? $\tau$$\alpha$ relation. In addition, comparison to theoretical single stellar population models suggests the presence of an age-metallicity relation among these clusters, with younger clusters being more metal-rich. Analysis of the radial distribution of the clusters yields some evidence that younger clusters (age lesssim1 Gyr) may be more concentrated toward the center of M33 than older ones. A similar comparison with the radial profile of the M33 field stars shows the clusters to be more centrally concentrated at the greater than 99.9\% confidence level. Possible reasons for this are presented and discussed; however, the overwhelming conclusion seems to be that a more complete and thorough cluster search is needed, covering at least 4 deg2 centered on M33.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {The Astronomical Journal},
	author = {Sarajedini, Ata and Mancone, Conor L.},
	month = jun,
	year = {2007},
	pages = {447},
	file = {Snapshot:/Users/Tobin/Zotero/storage/2ARGBSVA/518835.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/I7PJT79S/Sarajedini and Mancone - 2007 - A Catalog of Star Cluster Candidates in M33.pdf:application/pdf},
}

@article{ma_updated_2012,
	title = {{AN} {UPDATED} {CATALOG} {OF} {M33} {CLUSTERS} {AND} {CANDIDATES}:{UBVRIPHOTOMETRY} {AND} {SOME} {STATISTICAL} {RESULTS}},
	volume = {144},
	issn = {1538-3881},
	shorttitle = {{AN} {UPDATED} {CATALOG} {OF} {M33} {CLUSTERS} {AND} {CANDIDATES}},
	url = {https://doi.org/10.1088%2F0004-6256%2F144%2F2%2F41},
	doi = {10.1088/0004-6256/144/2/41},
	abstract = {We present UBVRI photometry for 392 star clusters and candidates in the field of M33, which are selected from the most recent star cluster catalog. In this catalog, the authors listed star clusters{\textquoteright} parameters such as cluster positions, magnitudes, colors in the UBVRIJHKs filters, and so on. However, a large fraction of objects in this catalog do not have previously published photometry. Photometry is performed using archival images from the Local Group Galaxies Survey, which covers 0.8 deg2 along the major axis of M33. Detailed comparisons show that, in general, our photometry is consistent with previous measurements. Positions (right ascension and declination) for some clusters are corrected here. Combined with previous literature, ours constitute a large sample of M33 star clusters. Based on this cluster sample, we present some statistical results: none of the youngest M33 clusters (\~{}107 yr) have masses approaching 105 M ?; roughly half the star clusters are consistent with the 104-105 M ? mass models; the continuous distribution of star clusters along the model line indicates that M33 star clusters have been formed continuously from the epoch of the first star cluster formation until recent times; and there are \~{}50 star clusters which are overlapped with the Galactic globular clusters on the color-color diagram, and these clusters are old globular cluster candidates in M33.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {The Astronomical Journal},
	author = {Ma, Jun},
	month = jun,
	year = {2012},
	pages = {41},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/KNNY4HVT/Ma - 2012 - AN UPDATED CATALOG OF M33 CLUSTERS AND CANDIDATES.pdf:application/pdf},
}

@article{san_roman_newly_2009,
	title = {{NEWLY} {IDENTIFIED} {STAR} {CLUSTERS} {IN} {M33}. {II}. {RADIALHUBBLE} {SPACE} TEL{ESCOPE}/{ADVANCED} {CAMERA} {FOR} {SURVEYS} {FIELDS}},
	volume = {699},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F699%2F1%2F839},
	doi = {10.1088/0004-637X/699/1/839},
	abstract = {We present integrated photometry and color-magnitude diagrams (CMDs) for 161 star clusters in M33, of which 115 were previously uncataloged, using the Advanced Camera For Surveys Wide Field Channel onboard the Hubble Space Telescope. The integrated V-band magnitudes of these clusters range from MV \~{}-9 to as faint as MV \~{}-4, extending the depth of the existing M33 cluster catalogs by \~{}1 mag. Comparisons of theoretical isochrones to the CMDs using the Padova models yield ages for 148 of these star clusters. The ages range from log(t) \~{} 7.0 to log(t) \~{} 9.0. Our CMDs are not sensitive to clusters older than \~{}1 Gyr. We find that the variation of the clusters' integrated colors and absolute magnitudes with age is consistent with the predictions of simple stellar population models. These same models suggest that the masses of the clusters in our sample range from 5 {\texttimes} 103 to 5 {\texttimes} 104 M ?.},
	language = {en},
	number = {1},
	urldate = {2019-07-16},
	journal = {The Astrophysical Journal},
	author = {San Roman, Izaskun and Sarajedini, Ata and Garnett, Donald R. and Holtzman, Jon A.},
	month = jun,
	year = {2009},
	pages = {839--849},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/RALJBNEY/Roman et al. - 2009 - NEWLY IDENTIFIED STAR CLUSTERS IN M33. II. RADIALH.pdf:application/pdf},
}

@article{krumholz_slug_2015,
	title = {{SLUG} {\textendash} stochastically lighting up galaxies {\textendash} {III}. {A} suite of tools for simulated photometry, spectroscopy, and {Bayesian} inference with stochastic stellar populations},
	volume = {452},
	issn = {0035-8711, 1365-2966},
	url = {https://academic.oup.com/mnras/article-lookup/doi/10.1093/mnras/stv1374},
	doi = {10.1093/mnras/stv1374},
	abstract = {Stellar population synthesis techniques for predicting the observable light emitted by a stellar population have extensive applications in numerous areas of astronomy. However, accurate predictions for small populations of young stars, such as those found in individual star clusters, star-forming dwarf galaxies, and small segments of spiral galaxies, require that the population be treated stochastically. Conversely, accurate deductions of the properties of such objects also require consideration of stochasticity. Here we describe a comprehensive suite of modular, open-source software tools for tackling these related problems. These include the following: a greatly-enhanced version of the SLUG code introduced by da Silva et al., which computes spectra and photometry for stochastically or deterministically sampled stellar populations with nearly arbitrary star formation histories, clustering properties, and initial mass functions; CLOUDY\_SLUG, a tool that automatically couples SLUG-computed spectra with the CLOUDY radiative transfer code in order to predict stochastic nebular emission; BAYESPHOT, a general-purpose tool for performing Bayesian inference on the physical properties of stellar systems based on unresolved photometry; and CLUSTER\_SLUG and SFR\_SLUG, a pair of tools that use BAYESPHOT on a library of SLUG models to compute the mass, age, and extinction of mono-age star clusters, and the star formation rate of galaxies, respectively. The latter two tools make use of an extensive library of pre-computed stellar population models, which are included in the software. The complete package is available at http://www.slugsps.com.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Krumholz, Mark R. and Fumagalli, Michele and da Silva, Robert L. and Rendahl, Theodore and Parra, Jonathan},
	month = sep,
	year = {2015},
	pages = {1447--1467},
	file = {Krumholz et al. - 2015 - SLUG {\textendash} stochastically lighting up galaxies {\textendash} III. .pdf:/Users/Tobin/Zotero/storage/J8ZZEDHS/Krumholz et al. - 2015 - SLUG {\textendash} stochastically lighting up galaxies {\textendash} III. .pdf:application/pdf},
}

@article{san_roman_photometric_2010,
	title = {{PHOTOMETRIC} {PROPERTIES} {OF} {THE} {M33} {STAR} {CLUSTER} {SYSTEM}},
	volume = {720},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F720%2F2%2F1674},
	doi = {10.1088/0004-637X/720/2/1674},
	abstract = {We present a catalog of 2990 extended sources in a 1{\textdegree} {\texttimes} 1{\textdegree} area centered on M33 using the MegaCam camera on the 3.6 m Canada-France-Hawaii Telescope. The catalog includes 599 new candidate stellar clusters, 204 previously confirmed clusters, 1969 likely background galaxies, and 218 unknown extended objects. We present ugriz integrated magnitudes of the candidates and confirmed star clusters (SCs) as well as the full width at half maximum, ellipticity, and stellarity. Based on the properties of the confirmed SCs, we select a sub-sample of highly probable clusters composed of 246 objects. The integrated photometry of the complete cluster catalog reveals a wide range of colors of {\textendash}0.4 {\textless} (g {\textendash} r) {\textless} 1.5 and {\textendash}1.0 {\textless} (r {\textendash} i) {\textless} 1.0 with no obvious cluster subpopulations. Comparisons with models of simple stellar populations suggest a large range of ages some as old as \~{}10 Gyr. In addition, we find a sequence in the color-color diagrams that deviates from the expected direction of evolution. This feature could be associated with very young clusters ({\textless}107 yr) possessing significant nebular emission. Analysis of the radial density distribution suggests that the cluster system of M33 has suffered from significant depletion possibly due to interactions with M31. We also detect a gap in the cluster distribution in the color-color diagram at (g {\textendash} r) ? 0.3 and (u {\textendash} g) ? 0.8. This gap could be interpreted as an evolutionary effect. This complete catalog provides promising targets for deep photometry and high-resolution spectroscopy to study the structure and star formation history of M33.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {The Astrophysical Journal},
	author = {San Roman, Izaskun and Sarajedini, Ata and Aparicio, Antonio},
	month = aug,
	year = {2010},
	pages = {1674--1683},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/S3EPA8C3/Roman et al. - 2010 - PHOTOMETRIC PROPERTIES OF THE M33 STAR CLUSTER SYS.pdf:application/pdf},
}

@article{fan_star_2014,
	title = {{STAR} {CLUSTERS} {IN} {M33}: {UPDATEDUBVRIPHOTOMETRY}, {AGES}, {METALLICITIES}, {AND} {MASSES}},
	volume = {211},
	issn = {0067-0049},
	shorttitle = {{STAR} {CLUSTERS} {IN} {M33}},
	url = {https://doi.org/10.1088%2F0067-0049%2F211%2F2%2F22},
	doi = {10.1088/0067-0049/211/2/22},
	abstract = {The photometric characterization of M33 star clusters is far from complete. In this paper, we present homogeneous UBVRI photometry of 708 star clusters and cluster candidates in M33 based on archival images from the Local Group Galaxies Survey, which covers 0.8 deg2 along the galaxy's major axis. Our photometry includes 387, 563, 616, 580, and 478 objects in the UBVRI bands, respectively, of which 276, 405, 430, 457, and 363 do not have previously published UBVRI photometry. Our photometry is consistent with previous measurements (where available) in all filters. We adopted Sloan Digital Sky Survey ugriz photometry for complementary purposes, as well as Two Micron All Sky Survey near-infrared JHK photometry where available. We fitted the spectral-energy distributions of 671 star clusters and candidates to derive their ages, metallicities, and masses based on the updated PARSEC simple stellar populations synthesis models. The results of our $\chi$2 minimization routines show that only 205 of the 671 clusters (31\%) are older than 2 Gyr, which represents a much smaller fraction of the cluster population than that in M31 (56\%), suggesting that M33 is dominated by young star clusters ({\textless}1 Gyr). We investigate the mass distributions of the star clusters{\textemdash}both open and globular clusters{\textemdash}in M33, M31, the Milky Way, and the Large Magellanic Cloud. Their mean values are log (M cl/M ?) = 4.25, 5.43, 2.72, and 4.18, respectively. The fraction of open to globular clusters is highest in the Milky Way and lowest in M31. Our comparisons of the cluster ages, masses, and metallicities show that our results are basically in agreement with previous studies (where objects in common are available); differences can be traced back to differences in the models adopted, the fitting methods used, and stochastic sampling effects.},
	language = {en},
	number = {2},
	urldate = {2019-07-16},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Fan, Zhou and Grijs, Richard de},
	month = mar,
	year = {2014},
	pages = {22},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/YAC6GMRL/Fan and Grijs - 2014 - STAR CLUSTERS IN M33 UPDATEDUBVRIPHOTOMETRY, AGES.pdf:application/pdf},
}

@article{weigel_stellar_2016,
	title = {Stellar mass functions: methods, systematics and results for the local {Universe}},
	volume = {459},
	issn = {0035-8711, 1365-2966},
	shorttitle = {Stellar mass functions},
	url = {http://arxiv.org/abs/1604.00008},
	doi = {10.1093/mnras/stw756},
	abstract = {We present a comprehensive method for determining stellar mass functions, and apply it to samples in the local Universe. We combine the classical 1/Vmax approach with STY, a parametric maximum likelihood method and SWML, a non-parametric maximum likelihood technique. In the parametric approach, we are assuming that the stellar mass function can be modelled by either a single or a double Schechter function and we use a likelihood ratio test to determine which model provides a better fit to the data. We discuss how the stellar mass completeness as a function of z biases the three estimators and how it can affect, especially the low mass end of the stellar mass function. We apply our method to SDSS DR7 data in the redshift range from 0.02 to 0.06. We find that the entire galaxy sample is best described by a double Schechter function with the following parameters: \${\textbackslash}log (M{\textasciicircum}\{*\}/M\_{\textbackslash}odot) = 10.79 {\textbackslash}pm 0.01\$, \${\textbackslash}log ({\textbackslash}Phi{\textasciicircum}\{*\}\_1/{\textbackslash}mathrm\{h{\textasciicircum}3{\textbackslash} Mpc{\textasciicircum}\{-3\}\}) = -3.31 {\textbackslash}pm 0.20\$, \${\textbackslash}alpha\_1 = -1.69 {\textbackslash}pm 0.10\$, \${\textbackslash}log ({\textbackslash}Phi{\textasciicircum}\{*\}\_2/{\textbackslash}mathrm\{h{\textasciicircum}3{\textbackslash} Mpc{\textasciicircum}\{-3\}\}) = -2.01 {\textbackslash}pm 0.28\$ and \${\textbackslash}alpha\_2 = -0.79 {\textbackslash}pm 0.04\$. We also use morphological classifications from Galaxy Zoo and halo mass, overdensity, central/satellite, colour and sSFR measurements to split the galaxy sample into over 130 subsamples. We determine and present the stellar mass functions and the best fit Schechter function parameters for each of these subsamples.},
	number = {2},
	urldate = {2020-05-29},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Weigel, Anna K. and Schawinski, Kevin and Bruderer, Claudio},
	month = jun,
	year = {2016},
	note = {arXiv: 1604.00008},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {2150--2187},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/Z5VDHR22/Weigel et al. - 2016 - Stellar mass functions methods, systematics and r.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/6KWFQT5P/1604.html:text/html},
}

@book{ivezic_statistics_2014,
	address = {Princeton, UNITED STATES},
	title = {Statistics, {Data} {Mining}, and {Machine} {Learning} in {Astronomy}: {A} {Practical} {Python} {Guide} for the {Analysis} of {Survey} {Data}},
	isbn = {978-1-4008-4891-1},
	shorttitle = {Statistics, {Data} {Mining}, and {Machine} {Learning} in {Astronomy}},
	url = {http://ebookcentral.proquest.com/lib/utah/detail.action?docID=1458117},
	urldate = {2020-06-02},
	publisher = {Princeton University Press},
	author = {Ivezi{\'c}, eljko and Connolly, Andrew J. and VanderPlas, Jacob T. and Gray, Alexander},
	year = {2014},
	keywords = {Astronomy -- Data processing., Statistical astronomy.},
	file = {ProQuest Ebook Snapshot:/Users/Tobin/Zotero/storage/U8PNSJLJ/reader.html:text/html},
}

@article{alstott_powerlaw_2014,
	title = {powerlaw: {A} {Python} {Package} for {Analysis} of {Heavy}-{Tailed} {Distributions}},
	volume = {9},
	issn = {1932-6203},
	shorttitle = {powerlaw},
	url = {https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0085777},
	doi = {10.1371/journal.pone.0085777},
	abstract = {Power laws are theoretically interesting probability distributions that are also frequently used to describe empirical data. In recent years, effective statistical methods for fitting power laws have been developed, but appropriate use of these techniques requires significant programming and statistical insight. In order to greatly decrease the barriers to using good statistical methods for fitting power law distributions, we developed the powerlaw Python package. This software package provides easy commands for basic fitting and statistical analysis of distributions. Notably, it also seeks to support a variety of user needs by being exhaustive in the options available to the user. The source code is publicly available and easily extensible.},
	language = {en},
	number = {1},
	urldate = {2020-06-04},
	journal = {PLOS ONE},
	author = {Alstott, Jeff and Bullmore, Ed and Plenz, Dietmar},
	month = jan,
	year = {2014},
	note = {Publisher: Public Library of Science},
	keywords = {Data visualization, Neurons, Probability distribution, Semantics, Simulation and modeling, Software tools, Source code, Statistical distributions},
	pages = {e85777},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/YZWK4KIH/Alstott et al. - 2014 - powerlaw A Python Package for Analysis of Heavy-T.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/3YRTIRDT/article.html:text/html},
}

@article{bastian_spectroscopic_2012,
	title = {Spectroscopic constraints on the form of the stellar cluster mass function},
	volume = {541},
	issn = {0004-6361, 1432-0746},
	url = {http://www.aanda.org/10.1051/0004-6361/201219079},
	doi = {10.1051/0004-6361/201219079},
	abstract = {This contribution addresses the question of whether the initial cluster mass function (ICMF) has a fundamental limit (or truncation) at high masses. The shape of the ICMF at high masses can be studied using the most massive young ({\textless}10 Myr) clusters, however this has proven difficult due to low-number statistics. In this contribution we use an alternative method based on the luminosities of the brightest clusters, combined with their ages. The advantages are that more clusters can be used and that the ICMF leaves a distinct pattern on the global relation between the cluster luminosity and median age within a population. If a truncation is present, a generic prediction (nearly independent of the cluster disruption law adopted) is that the median age of bright clusters should be younger than that of fainter clusters. In the case of an non-truncated ICMF, the median age should be independent of cluster luminosity. Here, we present optical spectroscopy of twelve young stellar clusters in the face-on spiral galaxy NGC 2997. The spectra are used to estimate the age of each cluster, and the brightness of the clusters is taken from the literature. The observations are compared with the model expectations of Larsen (2009, A\&A, 494, 539) for various ICMF forms and both mass dependent and mass independent cluster disruption. While there exists some degeneracy between the truncation mass and the amount of mass independent disruption, the observations favour a truncated ICMF. For low or modest amounts of mass independent disruption, a truncation mass of 5-6 {\texttimes} 105 M is estimated, consistent with previous determinations. Additionally, we investigate possible truncations in the ICMF in the spiral galaxy M 83, the interacting Antennae galaxies, and the collection of spiral and dwarf galaxies present in Larsen (2009, A\&A, 494, 539) based on photometric catalogues taken from the literature, and find that all catalogues are consistent with having a truncation in the cluster mass functions. However for the case of the Antennae, we find a truncation mass of a few {\texttimes}106 M , suggesting a dependence on the environment, as has been previously suggested.},
	language = {en},
	urldate = {2020-06-21},
	journal = {Astronomy \& Astrophysics},
	author = {Bastian, N. and Konstantopoulos, I. S. and Trancho, G. and Weisz, D. R. and Larsen, S. S. and Fouesneau, M. and Kaschinski, C. B. and Gieles, M.},
	month = may,
	year = {2012},
	pages = {A25},
	file = {Bastian et al. - 2012 - Spectroscopic constraints on the form of the stell.pdf:/Users/Tobin/Zotero/storage/D7SGQ9E9/Bastian et al. - 2012 - Spectroscopic constraints on the form of the stell.pdf:application/pdf},
}

@article{bastian_stellar_2012-1,
	title = {Stellar clusters in {M83}: formation, evolution, disruption and the influence of the environment: {M83} stellar cluster population},
	volume = {419},
	issn = {00358711},
	shorttitle = {Stellar clusters in {M83}},
	url = {https://academic.oup.com/mnras/article-lookup/doi/10.1111/j.1365-2966.2011.19909.x},
	doi = {10.1111/j.1365-2966.2011.19909.x},
	abstract = {We study the stellar cluster population in two adjacent fields in the nearby, face-on spiral galaxy M83 using multiwavelength Wide Field Camera 3/Hubble Space Telescope imaging. After automatic detection procedures, the clusters are selected through visual inspection to be centrally concentrated, symmetric, and resolved on the images, which allows us to differentiate between clusters and likely unbound associations. We compare our sample with previous studies and show that the differences between the catalogues are largely due to the inclusion of a large numbers of diffuse associations within previous catalogues as well as the inclusion of the central starburst region, where the completeness limit is significantly worse than in the surrounding regions. We derive the size distribution of the clusters, which is well described by a lognormal distribution with a peak at \~{}2.5 pc, and find evidence for an expansion in the halflight radius of clusters with age. The luminosity function of the clusters is well approximated by a power law with an index of -2 over most of the observed range; however, a steepening is seen at MV = -9.3 and -8.8 in the inner and outer fields, respectively. Additionally, we show that the cluster population is inconsistent with a pure power-law mass distribution, but instead exhibits a truncation at the high-mass end. If described as a Schechter function, the characteristic mass is 1.6 {\texttimes} 105 and 0.5 {\texttimes} 105 M for the inner and outer fields, respectively, in agreement with previous estimates of other cluster populations in spiral galaxies. Comparing the predictions of the mass-independent disruption (MID) and mass-dependent disruption (MDD) scenarios with the observed distributions, we find that both models can accurately fit the data. However, for the MID case, the fraction of clusters destroyed (or mass lost) per decade in age is dependent on the environment; hence, the age and mass distributions of clusters are not universal. In the MDD case, the disruption time-scale scales with galactocentric distance (being longer in the outer regions of the galaxy) in agreement with analytic and numerical predictions. Finally, we discuss the implications of our results on other extragalactic surveys, focusing on the fraction of stars that form in clusters and the need (or lack thereof) for infant mortality.},
	language = {en},
	number = {3},
	urldate = {2020-06-21},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Bastian, N. and Adamo, A. and Gieles, M. and Silva-Villa, E. and Lamers, H. J. G. L. M and Larsen, S. S. and Smith, L. J. and Konstantopoulos, I. S. and Zackrisson, E.},
	month = jan,
	year = {2012},
	pages = {2606--2622},
	file = {Bastian et al. - 2012 - Stellar clusters in M83 formation, evolution, dis.pdf:/Users/Tobin/Zotero/storage/I9XJ4CVI/Bastian et al. - 2012 - Stellar clusters in M83 formation, evolution, dis.pdf:application/pdf},
}

@article{schechter_analytic_1976,
	title = {An analytic expression for the luminosity function for galaxies.},
	volume = {203},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/1976ApJ...203..297S},
	doi = {10.1086/154079},
	abstract = {Abstract image available at: 
http://adsabs.harvard.edu/abs/1976ApJ...203..297S},
	urldate = {2020-06-21},
	journal = {The Astrophysical Journal},
	author = {Schechter, P.},
	month = jan,
	year = {1976},
	pages = {297--306},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/AYN3YZZ9/Schechter - 1976 - An analytic expression for the luminosity function.pdf:application/pdf},
}

@article{bik_clusters_2003,
	title = {Clusters in the inner spiral arms of {M} 51: {The} cluster {IMF} and the formation history},
	volume = {397},
	issn = {0004-6361},
	shorttitle = {Clusters in the inner spiral arms of {M} 51},
	url = {http://adsabs.harvard.edu/abs/2003A%26A...397..473B},
	doi = {10.1051/0004-6361:20021384},
	abstract = {We present the results of an analysis of the HST-WFPC2 observations of 
the interacting galaxy M 51. From the observations in 5 broadband
filters (UBVRI) and two narrowband filters (H$\alpha$ and [OIII]) we
study the cluster population in a region of 3.2 x 3.2 kpc2 in
the inner spiral arms of M 51, at a distance of about 1 to 3 kpc from
the nucleus. We found 877 cluster candidates and we derived their ages,
initial masses and extinctions by means of a comparison between the
observed spectral energy distribution and the predictions from cluster
synthesis models for instantaneous star formation and solar metallicity.
The lack of [OIII] emission in even the youngest clusters with strong
H$\alpha$ emission, indicates the absence of the most massive stars and
suggests a mass upper limit of about 25 to 30 Msun. The mass
versus age distribution of the clusters shows a drastic decrease in the
number of clusters with age, much more severe than can be expected on
the basis of evolutionary fading of the clusters. This indicates that
cluster dispersion is occurring on a timescale of 10 Myr or longer. The
cluster initial mass function has been derived from clusters younger
than 10 Myr by a linear regression fit of the cumulative mass
distribution. This results in an exponent alpha = -d log N(M) /d log (M)
= 2.1 +/- 0.3 in the range of 2.5x 103 {\textless} M {\textless} 5x
104 M{\textbackslash}odot but with an overabundance of clusters
with M {\textgreater} 2x 104 Msun. In the restricted range
of 2.5x 103 {\textless} M {\textless} 2x 104 Msun we
find alpha = 2.0 +/- 0.05. This exponent is very similar to the value
derived for clusters in the interacting Antennae galaxies, and to the
exponent of the mass distribution of the giant molecular clouds in our
Galaxy. To study the possible effects of the interaction of M 51 with
its companion NGC 5195 about 400 Myr ago, which triggered a huge
starburst in the nucleus, we determined the cluster formation rate as a
function of time for clusters with an initial mass larger than
104 Msun. There is no evidence for a peak in the
cluster formation rate at around 200 to 400 Myr ago within 2 sigma
accuracy, i.e. within a factor two. The formation rate of the detected
clusters decreases strongly with age by about a factor 102
between 10 Myr and 1 Gyr. For clusters older than about 150 Myr this is
due to the evolutionary fading of the clusters below the detection
limit. For clusters younger than 100 Myr this is due to the dispersion
of the clusters, unless one assumes that the cluster formation rate has
been steadily increasing with time from 1 Gyr ago to the present time.
Based on observations with the NASA/ESA Hubble Space Telescope, obtained
at the Space Telescope Science Institute, which is operated by AURA,
Inc., under NASA contract NAS 5-26555. The coordinates and the
photometry of the objects are available in electronic form at
http://astro.uu.nl/ {\textasciitilde} bastian/M51-bik/ and at http://www.edpsciences.org},
	urldate = {2020-06-21},
	journal = {Astronomy and Astrophysics},
	author = {Bik, A. and Lamers, H. J. G. L. M. and Bastian, N. and Panagia, N. and Romaniello, M.},
	month = jan,
	year = {2003},
	keywords = {galaxies: spiral, galaxies: star clusters, galaxies: starburst, galaxies: individual: M 51, galaxies: interactions},
	pages = {473--486},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/4VBM46II/Bik et al. - 2003 - Clusters in the inner spiral arms of M 51 The clu.pdf:application/pdf},
}

@article{allison_early_2010,
	title = {The early dynamical evolution of cool, clumpy star clusters},
	volume = {407},
	issn = {0035-8711},
	url = {https://academic.oup.com/mnras/article/407/2/1098/1122061},
	doi = {10.1111/j.1365-2966.2010.16939.x},
	abstract = {Abstract.  Observations and theory both suggest that star clusters form subvirial (cool) with highly substructured distributions. We perform a large ensemble of},
	language = {en},
	number = {2},
	urldate = {2020-06-21},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Allison, Richard J. and Goodwin, Simon P. and Parker, Richard J. and Portegies Zwart, Simon F. and de Grijs, Richard},
	month = sep,
	year = {2010},
	note = {Publisher: Oxford Academic},
	pages = {1098--1107},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/CIQZ2ZQA/Allison et al. - 2010 - The early dynamical evolution of cool, clumpy star.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/HRM92K9P/1122061.html:text/html},
}

@article{gieles_all_2012,
	title = {Do all stars in the solar neighbourhood form in clusters? {A} cautionary note on the use of the distribution of surface densities},
	volume = {426},
	issn = {1745-3925},
	shorttitle = {Do all stars in the solar neighbourhood form in clusters?},
	url = {https://academic.oup.com/mnrasl/article/426/1/L11/988361},
	doi = {10.1111/j.1745-3933.2012.01312.x},
	abstract = {Abstract.  Bressert et al. recently showed that the surface density distribution of low-mass, young stellar objects (YSOs) in the solar neighbourhood is approxi},
	language = {en},
	number = {1},
	urldate = {2020-06-21},
	journal = {Monthly Notices of the Royal Astronomical Society: Letters},
	author = {Gieles, Mark and Moeckel, Nickolas and Clarke, Cathie J.},
	month = oct,
	year = {2012},
	note = {Publisher: Oxford Academic},
	pages = {L11--L15},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/M8JN24WC/Gieles et al. - 2012 - Do all stars in the solar neighbourhood form in cl.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/TF5Y8U95/governor.html:text/html},
}

@article{li_multi-seeded_2005,
	title = {Multi-seeded multi-mode formation of embedded clusters in the {RMC}: {Clusters} formed in swept-up shells},
	volume = {431},
	copyright = {{\textcopyright} ESO, 2005},
	issn = {0004-6361, 1432-0746},
	shorttitle = {Multi-seeded multi-mode formation of embedded clusters in the {RMC}},
	url = {https://www.aanda.org/articles/aa/abs/2005/09/aa1429/aa1429.html},
	doi = {10.1051/0004-6361:20041429},
	abstract = {This is the first of a series of three papers on clustered star formation in the Rosette Molecular Complex. Here we investigate star formation in the interfacing layers between the expanding Rosette Nebula and its surrounding cloud, based on an analysis of the spatially complete and unbiased 2MASS data. Two medium-mass infrared clusters with ages of around 1 Myr are identified in the south and south-east arcs of the fragmented shell. The majority of the candidate cluster members in these radiation and pressure-confined regions are found to be almost uniformly distributed, roughly following the compression layers traced by the distribution of optical depth at 100 {\textless}i{\textgreater}$\mu${\textless}i/{\textgreater}m, and may well develop into gravitationally unbound systems upon their emergence from the parental cloud. These expanding shells are believed to be playing important roles in impeding the emerging young open cluster NGC 2244 from intruding immediately and deeply into the ambient molecular cloud, where sequential formation of massive clusters is taking place.},
	language = {en},
	number = {3},
	urldate = {2020-06-21},
	journal = {Astronomy \& Astrophysics},
	author = {Li, J. Z. and Smith, M. D.},
	month = mar,
	year = {2005},
	note = {Number: 3
Publisher: EDP Sciences},
	pages = {925--931},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/U55YNUS8/Li and Smith - 2005 - Multi-seeded multi-mode formation of embedded clus.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/4MFBTA62/aa1429.html:text/html},
}

@article{goodman_ensemble_2010,
	title = {Ensemble samplers with affine invariance},
	volume = {5},
	issn = {2157-5452},
	url = {https://msp.org/camcos/2010/5-1/p04.xhtml},
	doi = {10.2140/camcos.2010.5.65},
	number = {1},
	urldate = {2020-06-22},
	journal = {Communications in Applied Mathematics and Computational Science},
	author = {Goodman, Jonathan and Weare, Jonathan},
	month = jan,
	year = {2010},
	note = {Publisher: Mathematical Sciences Publishers},
	pages = {65--80},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/E2PINU2M/Goodman and Weare - 2010 - Ensemble samplers with affine invariance.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/JHCN5WWY/p04.html:application/xhtml+xml},
}

@article{whitmore_antennae_2010,
	title = {The {Antennae} {Galaxies} ({NGC} 4038/4039) {Revisited}: {Advanced} {Camera} for {Surveys} and {NICMOS} {Observations} of a {Prototypical} {Merger}},
	volume = {140},
	issn = {0004-6256},
	shorttitle = {The {Antennae} {Galaxies} ({NGC} 4038/4039) {Revisited}},
	url = {http://adsabs.harvard.edu/abs/2010AJ....140...75W},
	doi = {10.1088/0004-6256/140/1/75},
	abstract = {The Advanced Camera for Surveys and the Near Infrared Camera and 
Multi-Object Spectrometer (NICMOS) have been used to obtain new Hubble
Space Telescope images of NGC 4038/4039 ("The Antennae"). These new
observations allow us to better differentiate compact star clusters from
individual stars, based on both size and color. We use this ability to
extend the cluster luminosity function (LF) by approximately 2 mag over
our previous WFPC2 results, and find that it continues as a single power
law, dN/dL vprop L $\alpha$ with $\alpha$ = -2.13 {\textpm}
0.07, down to the observational limit of MV ? -7.
Similarly, the mass function (MF) is a single power law dN/dM vprop M
$\beta$ with $\beta$ = -2.10 {\textpm} 0.20 for clusters with
ages {\textless}3 {\texttimes} 108 yr, corresponding to lower mass limits
that range from 104 to 105 M sun,
depending on the age range of the subsample. Hence, the power-law
indices for the luminosity and MFs are essentially the same. The LF for
intermediate-age clusters (i.e., {\textasciitilde}100-300 Myr old objects found in the
loops, tails, and outer areas) shows no bend or turnover down to
MV ? -6, consistent with relaxation-driven cluster
disruption models which predict the turnover should not be observed
until MV ? -4. An analysis of individual {\textasciitilde}0.5 kpc sized
areas over diverse environments shows good agreement between values of
$\alpha$ and $\beta$, similar to the results for the total population of
clusters in the system. There is tentative evidence that the values of
both $\alpha$ and $\beta$ are flatter for the youngest clusters in some
areas, but it is possible that this is caused by observational biases.
Several of the areas studied show evidence for age gradients, with
somewhat older clusters appearing to have triggered the formation of
younger clusters. The area around Knot B is a particularly interesting
example, with a {\textasciitilde}10-50 Myr old cluster of estimated mass {\textasciitilde}106
M sun having apparently triggered the formation of several
younger, more massive (up to 5 {\texttimes} 106 M sun)
clusters along a dust lane. A comparison with new NICMOS observations
reveals that only 16\% {\textpm} 6\% of the IR-bright clusters in the
Antennae are still heavily obscured, with values of AV {\textgreater}3
mag.

Based on observations with the NASA/ESA Hubble Space Telescope, obtained
at the Space Telescope Science Institute, which is operated by the
Association of Universities for Research in Astronomy, Inc. under NASA
contract NAS5-26555. Also based on data obtained from the Hubble Legacy
Archive, which is a collaboration between the Space Telescope Science
Institute (STScI/NASA), the Space Telescope European Coordinating
Facility (ST-ECF/ESA), and the Canadian Astronomy Data Centre
(CADC/NRC/CSA).},
	urldate = {2020-06-26},
	journal = {The Astronomical Journal},
	author = {Whitmore, Bradley C. and Chandar, Rupali and Schweizer, Fran{\c c}ois and Rothberg, Barry and Leitherer, Claus and Rieke, Marcia and Rieke, George and Blair, W. P. and Mengel, S. and Alonso-Herrero, A.},
	month = jul,
	year = {2010},
	keywords = {galaxies: star clusters: general, galaxies: interactions, galaxies: individual: NGC 4038 NGC 4039},
	pages = {75--109},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/SCZZQJ8H/Whitmore et al. - 2010 - The Antennae Galaxies (NGC 40384039) Revisited A.pdf:application/pdf},
}

@article{adamo_star_2020,
	title = {Star clusters near and far; tracing star formation across cosmic time},
	volume = {216},
	issn = {0038-6308, 1572-9672},
	url = {http://arxiv.org/abs/2005.06188},
	doi = {10.1007/s11214-020-00690-x},
	abstract = {Star clusters are fundamental units of stellar feedback and unique tracers of their host galactic properties. In this review, we will first focus on their constituents, i.e.{\textbackslash} detailed insight into their stellar populations and their surrounding ionised, warm, neutral, and molecular gas. We, then, move beyond the Local Group to review star cluster populations at various evolutionary stages, and in diverse galactic environmental conditions accessible in the local Universe. At high redshift, where conditions for cluster formation and evolution are more extreme, we are only able to observe the integrated light of a handful of objects that we believe will become globular clusters. We therefore discuss how numerical and analytical methods, informed by the observed properties of cluster populations in the local Universe, are used to develop sophisticated simulations potentially capable of disentangling the genetic map of galaxy formation and assembly that is carried by globular cluster populations.},
	number = {4},
	urldate = {2020-07-16},
	journal = {Space Science Reviews},
	author = {Adamo, Angela and Zeidler, Peter and Kruijssen, J. M. Diederik and Chevance, M{\'e}lanie and Gieles, Mark and Calzetti, Daniela and Charbonnel, Corinne and Zinnecker, Hans and Krause, Martin G. H.},
	month = jun,
	year = {2020},
	note = {arXiv: 2005.06188},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {69},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/DSB8EU42/Adamo et al. - 2020 - Star clusters near and far\; tracing star formation.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/F2GBYTQW/2005.html:text/html},
}

@article{adamo_probing_2015-1,
	title = {Probing the role of the galactic environment in the formation of stellar clusters, using {M83} as a test bench},
	volume = {452},
	url = {http://adsabs.harvard.edu/abs/2015MNRAS.452..246A},
	doi = {10.1093/mnras/stv1203},
	abstract = {We present a study of the M83 cluster population, covering the disc of 
the galaxy between radii of 0.45 and 4.5 kpc. We aim to probe the
properties of the cluster population as a function of distance from the
galactic centre. We observe a net decline in cluster formation
efficiency ($\Gamma$, i.e. amount of star formation happening in bound
clusters) from about 26 per cent in the inner region to 8 per cent in
the outer part of the galaxy. The recovered $\Gamma$ values within
different regions of M83 follow the same $\Gamma$ versus star formation
rate density relation observed for entire galaxies. We also probe the
initial cluster mass function (ICMF) as a function of galactocentric
distance. We observe a significant steepening of the ICMF in the outer
regions (from -1.90 {\textpm} 0.11 to -2.70 {\textpm} 0.14) and for the
whole galactic cluster population (slope of -2.18 {\textpm} 0.07) of M83.
We show that this change of slope reflects a more fundamental change of
the `truncation mass' at the high-mass end of the distribution. This can
be modelled as a Schechter function of slope -2 with an exponential
cutoff mass (Mc) that decreases significantly from the inner
to the outer regions (from 4.00 to 0.25 {\texttimes} 105
M?) while the galactic Mc is ?1.60 {\texttimes}
105 M?. The trends in $\Gamma$ and ICMF are
consistent with the observed radial decrease of the
$\Sigma$(H2), hence in gas pressure. As gas pressure declines,
cluster formation becomes less efficient. We conclude that the host
galaxy environment appears to regulate (1) the fraction of stars locked
in clusters and (2) the upper mass limit of the ICMF, consistently
described by a near-universal slope -2 truncated at the high-mass end.},
	urldate = {2020-07-24},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Adamo, A. and Kruijssen, J. M. D. and Bastian, N. and Silva-Villa, E. and Ryon, J.},
	month = sep,
	year = {2015},
	keywords = {galaxies: spiral, galaxies: star clusters, galaxies: star formation},
	pages = {246--260},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/JAU6G5EF/Adamo et al. - 2015 - Probing the role of the galactic environment in th.pdf:application/pdf},
}

@article{adamo_legacy_2017-1,
	title = {Legacy {ExtraGalactic} {UV} {Survey} with {The} {Hubble} {Space} {Telescope}: {Stellar} {Cluster} {Catalogs} and {First} {Insights} {Into} {Cluster} {Formation} and {Evolution} in {NGC} 628},
	volume = {841},
	shorttitle = {Legacy {ExtraGalactic} {UV} {Survey} with {The} {Hubble} {Space} {Telescope}},
	url = {http://adsabs.harvard.edu/abs/2017ApJ...841..131A},
	doi = {10.3847/1538-4357/aa7132},
	abstract = {We report the large effort that is producing comprehensive high-level 
young star cluster (YSC) catalogs for a significant fraction of galaxies
observed with the Legacy ExtraGalactic UV Survey (LEGUS) Hubble treasury
program. We present the methodology developed to extract cluster
positions, verify their genuine nature, produce multiband photometry
(from NUV to NIR), and derive their physical properties via spectral
energy distribution fitting analyses. We use the nearby spiral galaxy
NGC 628 as a test case for demonstrating the impact that LEGUS will have
on our understanding of the formation and evolution of YSCs and compact
stellar associations within their host galaxy. Our analysis of the
cluster luminosity function from the UV to the NIR finds a steepening at
the bright end and at all wavelengths suggesting a dearth of luminous
clusters. The cluster mass function of NGC 628 is consistent with a
power-law distribution of slopes \~{} -2 and a truncation of a few
times 105 \{M\}? . After their formation, YSCs
and compact associations follow different evolutionary paths. YSCs
survive for a longer time frame, confirming their being potentially
bound systems. Associations disappear on timescales comparable to
hierarchically organized star-forming regions, suggesting that they are
expanding systems. We find mass-independent cluster disruption in the
inner region of NGC 628, while in the outer part of the galaxy there is
little or no disruption. We observe faster disruption rates for low mass
(<=104 \{M\}? ) clusters, suggesting that a
mass-dependent component is necessary to fully describe the YSC
disruption process in NGC 628.

Based on observations obtained with the NASA/ESA Hubble Space Telescope,
at the Space Telescope Science Institute, which is operated by the
Association of Universities for Research in Astronomy, Inc., under NASA
contract NAS 5-26555.},
	urldate = {2020-07-30},
	journal = {The Astrophysical Journal},
	author = {Adamo, A. and Ryon, J. E. and Messa, M. and Kim, H. and Grasha, K. and Cook, D. O. and Calzetti, D. and Lee, J. C. and Whitmore, B. C. and Elmegreen, B. G. and Ubeda, L. and Smith, L. J. and Bright, S. N. and Runnholm, A. and Andrews, J. E. and Fumagalli, M. and Gouliermis, D. A. and Kahre, L. and Nair, P. and Thilker, D. and Walterbos, R. and Wofford, A. and Aloisi, A. and Ashworth, G. and Brown, T. M. and Chandar, R. and Christian, C. and Cignoni, M. and Clayton, G. C. and Dale, D. A. and de Mink, S. E. and Dobbs, C. and Elmegreen, D. M. and Evans, A. S. and Gallagher, III, J. S. and Grebel, E. K. and Herrero, A. and Hunter, D. A. and Johnson, K. E. and Kennicutt, R. C. and Krumholz, M. R. and Lennon, D. and Levay, K. and Martin, C. and Nota, A. and {\"O}stlin, G. and Pellerin, A. and Prieto, J. and Regan, M. W. and Sabbi, E. and Sacchi, E. and Schaerer, D. and Schiminovich, D. and Shabani, F. and Tosi, M. and Van Dyk, S. D. and Zackrisson, E.},
	month = jun,
	year = {2017},
	keywords = {stars: formation, galaxies: individual: NGC 628, galaxies: star clusters: general, galaxies: star formation, M74},
	pages = {131},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/NW7SPFXB/Adamo et al. - 2017 - Legacy ExtraGalactic UV Survey with The Hubble Spa.pdf:application/pdf},
}

@article{freeman_varying_2017,
	title = {The varying mass distribution of molecular clouds across {M83}},
	volume = {468},
	url = {http://adsabs.harvard.edu/abs/2017MNRAS.468.1769F},
	doi = {10.1093/mnras/stx499},
	abstract = {The work of Adamo et al. showed that the mass distributions of young massive stellar clusters were truncated above a maximum-mass scale in the nearby galaxy M83 and that this truncation mass varies with the galactocentric radius. Here, we present a cloud-based analysis of Atacama Large Millimeter/submillimeter Array CO(1 {\textrightarrow} 0) observations of M83 to search for such a truncation mass in the molecular cloud population. We identify a population of 873 molecular clouds in M83 that is largely similar to those found in the Milky Way and Local Group galaxies, though clouds in the centre of the galaxy show high surface densities and enhanced turbulence, as is common for clouds in
high-density nuclear environments. Like the young massive clusters, we find a maximum-mass scale for the molecular clouds which decreases radially in the galaxy. We find that the most young massive cluster tracks the most massive molecular cloud with the cluster mass being 10-2 times that of the most massive molecular cloud. Outside the nuclear region of M83 (Rg {\textgreater} 0.5 kpc), there is no evidence for changing internal conditions in the population of molecular clouds, with the average internal pressures, densities and free-fall times remaining constant for the cloud population over the galaxy. This result is consistent with the bound cluster formation efficiency depending only on the large-scale properties of the interstellar medium rather than the internal conditions of individual clouds.},
	urldate = {2020-07-31},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Freeman, Pamela and Rosolowsky, Erik and Kruijssen, J. M. Diederik and Bastian, Nate and Adamo, Angela},
	month = jun,
	year = {2017},
	keywords = {stars: formation, galaxies: individual: M83, ISM: clouds},
	pages = {1769--1781},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/YRDN8XNF/Freeman et al. - 2017 - The varying mass distribution of molecular clouds .pdf:application/pdf},
}

@article{krumholz_slug_2019,
	title = {{SLUG} {IV}: a novel forward-modelling method to derive the demographics of star clusters},
	volume = {482},
	shorttitle = {{SLUG} {IV}},
	url = {http://adsabs.harvard.edu/abs/2019MNRAS.482.3550K},
	doi = {10.1093/mnras/sty2896},
	abstract = {We describe a novel method for determining the demographics of a 
population of star clusters, for example distributions of cluster mass
and age, from unresolved photometry. This method has a number of
desirable properties: it fully exploits all the information available in
a data set without any binning, correctly accounts for both measurement
error and sample incompleteness, naturally handles heterogenous data
(e.g. fields that have been imaged with different sets of filters or to
different depths), marginalizes over uncertain extinctions, and returns
the full posterior distributions of the parameters describing star
cluster demographics. We demonstrate the method using mock star cluster
catalogues and show that our method is robust and accurate, and that it
can recover the demographics of star cluster populations significantly
better than traditional fitting methods. For realistic sample sizes, our
method is sufficiently powerful that its accuracy is ultimately limited
by the accuracy of the underlying physical models for stellar evolution
and interstellar dust, rather than by statistical uncertainties. Our
method is implemented as part of the Stochastically Lighting Up Galaxies
(SLUG) stellar populations code, and is freely available.},
	urldate = {2020-07-31},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Krumholz, Mark R. and Adamo, Angela and Fumagalli, Michele and Calzetti, Daniela},
	month = jan,
	year = {2019},
	keywords = {galaxies: star clusters: general, methods: data analysis, methods: statistical, techniques: photometric},
	pages = {3550--3566},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/923DJIRT/Krumholz et al. - 2019 - SLUG IV a novel forward-modelling method to deriv.pdf:application/pdf},
}

@article{krumholz_slug_2015-1,
	title = {{SLUG} - stochastically lighting up galaxies - {III}. {A} suite of tools for simulated photometry, spectroscopy, and {Bayesian} inference with stochastic stellar populations},
	volume = {452},
	url = {http://adsabs.harvard.edu/abs/2015MNRAS.452.1447K},
	doi = {10.1093/mnras/stv1374},
	abstract = {Stellar population synthesis techniques for predicting the observable 
light emitted by a stellar population have extensive applications in
numerous areas of astronomy. However, accurate predictions for small
populations of young stars, such as those found in individual star
clusters, star-forming dwarf galaxies, and small segments of spiral
galaxies, require that the population be treated stochastically.
Conversely, accurate deductions of the properties of such objects also
require consideration of stochasticity. Here we describe a comprehensive
suite of modular, open-source software tools for tackling these related
problems. These include the following: a greatly-enhanced version of the
SLUG code introduced by da Silva et al., which computes spectra and
photometry for stochastically or deterministically sampled stellar
populations with nearly arbitrary star formation histories, clustering
properties, and initial mass functions; CLOUDY\_SLUG, a tool that
automatically couples SLUG-computed spectra with the CLOUDY radiative
transfer code in order to predict stochastic nebular emission;
BAYESPHOT, a general-purpose tool for performing Bayesian inference on
the physical properties of stellar systems based on unresolved
photometry; and CLUSTER\_SLUG and SFR\_SLUG, a pair of tools that use
BAYESPHOT on a library of SLUG models to compute the mass, age, and
extinction of mono-age star clusters, and the star formation rate of
galaxies, respectively. The latter two tools make use of an extensive
library of pre-computed stellar population models, which are included in
the software. The complete package is available at
http://www.slugsps.com.},
	urldate = {2020-08-05},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Krumholz, Mark R. and Fumagalli, Michele and da Silva, Robert L. and Rendahl, Theodore and Parra, Jonathan},
	month = sep,
	year = {2015},
	keywords = {stars: formation, galaxies: star clusters: general, galaxies: stellar content, methods: statistical, techniques: photometric, methods: numerical},
	pages = {1447--1467},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7DZWPYRL/Krumholz et al. - 2015 - SLUG - stochastically lighting up galaxies - III. .pdf:application/pdf},
}

@article{calzetti_legacy_2015,
	title = {Legacy {Extragalactic} {UV} {Survey} ({LEGUS}) {With} the {Hubble} {Space} {Telescope}. {I}. {Survey} {Description}},
	volume = {149},
	url = {http://adsabs.harvard.edu/abs/2015AJ....149...51C},
	doi = {10.1088/0004-6256/149/2/51},
	abstract = {The Legacy ExtraGalactic UV Survey (LEGUS) is a Cycle 21 Treasury 
program on the Hubble Space Telescope aimed at the investigation of star
formation and its relation with galactic environment in nearby galaxies,
from the scales of individual stars to those of \~{}kiloparsec-size
clustered structures. Five-band imaging from the near-ultraviolet to the
I band with the Wide-Field Camera 3 (WFC3), plus parallel optical
imaging with the Advanced Camera for Surveys (ACS), is being collected
for selected pointings of 50 galaxies within the local 12 Mpc. The
filters used for the observations with the WFC3 are F275W($\lambda$2704
{\r A}), F336W($\lambda$3355 {\r A}), F438W($\lambda$4325 {\r A}),
F555W($\lambda$5308 {\r A}), and F814W($\lambda$8024 {\r A}) the
parallel observations with the ACS use the filters F435W($\lambda$4328
{\r A}), F606W($\lambda$5921 {\r A}), and F814W($\lambda$8057 {\r A}).
The multiband images are yielding accurate recent (?50 Myr) star
formation histories from resolved massive stars and the
extinction-corrected ages and masses of star clusters and associations.
The extensive inventories of massive stars and clustered systems will be
used to investigate the spatial and temporal evolution of star formation
within galaxies. This will, in turn, inform theories of galaxy evolution
and improve the understanding of the physical underpinning of the
gas-star formation relation and the nature of star formation at high
redshift. This paper describes the survey, its goals and observational
strategy, and the initial scientific results. Because LEGUS will provide
a reference survey and a foundation for future observations with the
James Webb Space Telescope and with ALMA, a large number of data
products are planned for delivery to the community.

Based on observations obtained with the NASA/ESA Hubble Space Telescope
at the Space Telescope Science Institute, which is operated by the
Association of Universities for Research in Astronomy under NASA
Contract NAS 5-26555.},
	urldate = {2020-08-06},
	journal = {The Astronomical Journal},
	author = {Calzetti, D. and Lee, J. C. and Sabbi, E. and Adamo, A. and Smith, L. J. and Andrews, J. E. and Ubeda, L. and Bright, S. N. and Thilker, D. and Aloisi, A. and Brown, T. M. and Chandar, R. and Christian, C. and Cignoni, M. and Clayton, G. C. and da Silva, R. and de Mink, S. E. and Dobbs, C. and Elmegreen, B. G. and Elmegreen, D. M. and Evans, A. S. and Fumagalli, M. and Gallagher, III, J. S. and Gouliermis, D. A. and Grebel, E. K. and Herrero, A. and Hunter, D. A. and Johnson, K. E. and Kennicutt, R. C. and Kim, H. and Krumholz, M. R. and Lennon, D. and Levay, K. and Martin, C. and Nair, P. and Nota, A. and {\"O}stlin, G. and Pellerin, A. and Prieto, J. and Regan, M. W. and Ryon, J. E. and Schaerer, D. and Schiminovich, D. and Tosi, M. and Van Dyk, S. D. and Walterbos, R. and Whitmore, B. C. and Wofford, A.},
	month = feb,
	year = {2015},
	keywords = {galaxies: star clusters: general, galaxies: star formation, galaxies: stellar content, galaxies: general, ultraviolet: galaxies, ultraviolet: stars},
	pages = {51},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/AUAT4SG8/Calzetti et al. - 2015 - Legacy Extragalactic UV Survey (LEGUS) With the Hu.pdf:application/pdf},
}

@article{gieles_distinction_2011,
	title = {The distinction between star clusters and associations},
	volume = {410},
	issn = {1745-3925},
	url = {https://academic.oup.com/mnrasl/article/410/1/L6/989254},
	doi = {10.1111/j.1745-3933.2010.00967.x},
	abstract = {Abstract.  In Galactic studies a distinction is made between (open) star clusters and associations. For barely resolved objects at a distance of several Mpc, th},
	language = {en},
	number = {1},
	urldate = {2020-08-07},
	journal = {Monthly Notices of the Royal Astronomical Society: Letters},
	author = {Gieles, Mark and Portegies Zwart, Simon F.},
	month = jan,
	year = {2011},
	note = {Publisher: Oxford Academic},
	pages = {L6--L7},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/4FBSWLTE/Gieles and Portegies Zwart - 2011 - The distinction between star clusters and associat.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/JBNW6YZV/989254.html:text/html},
}

@article{silva_slugstochastically_2012,
	title = {{SLUG}{\textemdash}{STOCHASTICALLY} {LIGHTING} {UP} {GALAXIES}. {I}. {METHODS} {AND} {VALIDATING} {TESTS}},
	volume = {745},
	issn = {0004-637X},
	url = {https://doi.org/10.1088%2F0004-637x%2F745%2F2%2F145},
	doi = {10.1088/0004-637X/745/2/145},
	abstract = {The effects of stochasticity on the luminosities of stellar populations are an often neglected but crucial element for understanding populations in the low-mass or the low star formation rate regime. To address this issue, we present SLUG, a new code to {\textquotedblleft}Stochastically Light Up Galaxies.{\textquotedblright} SLUG synthesizes stellar populations using a Monte Carlo technique that properly treats stochastic sampling including the effects of clustering, the stellar initial mass function, star formation history, stellar evolution, and cluster disruption. This code produces many useful outputs, including (1) catalogs of star clusters and their properties such as their stellar initial mass distributions and their photometric properties in a variety of filters, (2) two dimensional histograms of color-magnitude diagrams of every star in the simulation, and (3) the photometric properties of field stars and the integrated photometry of the entire simulated galaxy. After presenting the SLUG algorithm in detail, we validate the code through comparisons with STARBURST99 in the well-sampled regime, and with observed photometry of Milky Way clusters. Finally, we demonstrate SLUG's capabilities by presenting outputs in the stochastic regime. SLUG is publicly distributed through the Web site http://sites.google.com/site/runslug/.},
	language = {en},
	number = {2},
	urldate = {2020-08-07},
	journal = {The Astrophysical Journal},
	author = {Silva, Robert L. da and Fumagalli, Michele and Krumholz, Mark},
	month = jan,
	year = {2012},
	note = {Publisher: IOP Publishing},
	pages = {145},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/IUVKW5BA/Silva et al. - 2012 - SLUG{\textemdash}STOCHASTICALLY LIGHTING UP GALAXIES. I. METHO.pdf:application/pdf},
}

@article{zackrisson_hubble_2011,
	title = {The {Hubble} {Space} {Telescope} colours of high-redshift {Population} {III} galaxies with strong {Ly$\alpha$} emission},
	volume = {418},
	url = {http://adsabs.harvard.edu/abs/2011MNRAS.418L.104Z},
	doi = {10.1111/j.1745-3933.2011.01153.x},
	abstract = {Population III (pop III) galaxies, made partly or exclusively of 
metal-free stars, are predicted to exist at high redshifts and may
produce very strong Ly$\alpha$ emission. A substantial fraction of these
Ly$\alpha$ photons are likely absorbed in the intergalactic medium at z
{\textgreater} 6, but recent simulations suggest that significant Ly$\alpha$
emission may be detectable up to z? 8.5, i.e. well into the
reionization epoch. Here, we argue that high-redshift pop III galaxies
with strong Ly$\alpha$ emission can be identified in Hubble Space
Telescope imaging data because of their unusual colours. We quantify
this effect in some of the filters used in Y-band dropout searches for
galaxies at z? 8 and find that pop III galaxies with high Ly$\alpha$
fluxes may exhibit much bluer J-H colours at z? 8-10 than any normal
type of galaxy at these redshifts. This colour signature can arise even
if pop III stars account for as little as \~{}10-3 to
10-2 of the stellar mass in these galaxies. Some of the
anomalously blue objects reported in current Y-band dropout samples do
in fact meet the colour criteria for Ly$\alpha$-emitting pop III
galaxies.},
	urldate = {2020-08-07},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Zackrisson, Erik and Inoue, Akio K. and Rydberg, Claes-Erik and Duval, Florent},
	month = nov,
	year = {2011},
	keywords = {dark ages, first stars, galaxies: high-redshift, reionization, stars: Population III},
	pages = {L104--L108},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/N6BKFX7B/Zackrisson et al. - 2011 - The Hubble Space Telescope colours of high-redshif.pdf:application/pdf},
}

@article{bertin_sextractor_1996,
	title = {{SExtractor}: {Software} for source extraction.},
	volume = {117},
	issn = {0365-0138},
	shorttitle = {{SExtractor}},
	url = {http://adsabs.harvard.edu/abs/1996A%26AS..117..393B},
	doi = {10.1051/aas:1996164},
	abstract = {We present the automated techniques we have developed for new software that optimally detects, de-blends, measures and classifies sources from astronomical images: SExtractor (Source Extractor). We show that a very reliable star/galaxy separation can be achieved on most images using a neural network trained with simulated images. Salient features of SExtractor include its ability to work on very large images, with minimal human intervention, and to deal with a wide variety of object shapes and magnitudes. It is therefore particularly suited to the analysis of large extragalactic surveys.},
	urldate = {2020-08-07},
	journal = {Astronomy and Astrophysics Supplement Series},
	author = {Bertin, E. and Arnouts, S.},
	month = jun,
	year = {1996},
	keywords = {GALAXIES: PHOTOMETRY, METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING},
	pages = {393--404},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/454L3NP8/Bertin and Arnouts - 1996 - SExtractor Software for source extraction..pdf:application/pdf},
}

@article{johnson_phat_2015,
	title = {{PHAT} {Stellar} {Cluster} {Survey}. {II}. {Andromeda} {Project} {Cluster} {Catalog}},
	volume = {802},
	url = {http://adsabs.harvard.edu/abs/2015ApJ...802..127J},
	doi = {10.1088/0004-637X/802/2/127},
	abstract = {We construct a stellar cluster catalog for the Panchromatic Hubble Andromeda Treasury (PHAT) survey using image classifications collected from the Andromeda Project citizen science website. We identify 2753 clusters and 2270 background galaxies within \~{}0.5 deg2 of PHAT imaging searched, or \~{}400 kpc2 in deprojected area at the distance of the Andromeda Galaxy (M31). These identifications result from 1.82 million classifications of \~{}20,000 individual
images (totaling \~{}7 gigapixels) by tens of thousands of volunteers. We show that our crowd-sourced approach, which collects {\textgreater}80
classifications per image, provides a robust, repeatable method of cluster identification. The high spatial resolution Hubble Space Telescope images resolve individual stars in each cluster and are instrumental in the factor of \~{}6 increase in the number of clusters known within the survey footprint. We measure integrated photometry in six filter passbands, ranging from the near-UV to the near-IR. PHAT clusters span a range of \~{}8 magnitudes in F475W (g-band) luminosity, equivalent to \~{}4 decades in cluster mass. We perform catalog
completeness analysis using {\textgreater}3000 synthetic cluster simulations to determine robust detection limits and demonstrate that the catalog is 50\% complete down to \~{}500 \{\{M\}? \} for ages {\textless}100
Myr. We include catalogs of clusters, background galaxies, remaining unselected candidates, and synthetic cluster simulations, making all information publicly available to the community. The catalog published here serves as the definitive base data product for PHAT cluster science, providing a census of star clusters in an \{\{L\}{\textbackslash}star \} spiral galaxy with unmatched sensitivity and quality.},
	urldate = {2020-08-10},
	journal = {The Astrophysical Journal},
	author = {Johnson, L. Clifton and Seth, Anil C. and Dalcanton, Julianne J. and Wallace, Matthew L. and Simpson, Robert J. and Lintott, Chris J. and Kapadia, Amit and Skillman, Evan D. and Caldwell, Nelson and Fouesneau, Morgan and Weisz, Daniel R. and Williams, Benjamin F. and Beerman, Lori C. and Gouliermis, Dimitrios A. and Sarajedini, Ata},
	month = apr,
	year = {2015},
	keywords = {galaxies: star clusters: general, galaxies: individual: M31, catalogs},
	pages = {127},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/R45L48WN/Johnson et al. - 2015 - PHAT Stellar Cluster Survey. II. Andromeda Project.pdf:application/pdf},
}

@article{zhang_mass_1999,
	title = {The {Mass} {Function} of {Young} {Star} {Clusters} in the ``{Antennae}'' {Galaxies}},
	volume = {527},
	url = {http://adsabs.harvard.edu/abs/1999ApJ...527L..81Z},
	doi = {10.1086/312412},
	abstract = {We determine the mass function of young star clusters in the merging galaxies known as the ``Antennae'' (NGC 4038/9) from deep images taken with the Wide Field Planetary Camera 2 on the refurbished Hubble Space Telescope. This is accomplished by means of reddening-free parameters and a comparison with stellar population synthesis tracks to estimate the intrinsic luminosity and age, and hence the mass, of each cluster. We find that the mass function of the young star clusters (with ages {\textless}{\textasciitilde}160 Myr) is well represented by a power law of the form
$\psi$(M){\textasciitilde}M-2 over the range
104{\textless}{\textasciitilde}M{\textless}{\textasciitilde}106 Msolar. This result may have important implications for our understanding of the origin of globular clusters during the early phases of galactic evolution.},
	urldate = {2020-08-17},
	journal = {The Astrophysical Journal Letters},
	author = {Zhang, Qing and Fall, S. Michael},
	month = dec,
	year = {1999},
	keywords = {Galaxies: Individual: NGC Number: NGC 4038/9, GALAXIES: INDIVIDUAL: NGC NUMBER: NGC 4038/9, Galaxies: Interactions, GALAXIES: INTERACTIONS, Galaxies: Star Clusters, GALAXIES: STAR CLUSTERS},
	pages = {L81--L84},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/AGEIZXBG/Zhang and Fall - 1999 - The Mass Function of Young Star Clusters in the ``.pdf:application/pdf},
}

@article{gieles_what_2009,
	title = {What determines the mass of the most massive star cluster in a galaxy: statistics, physics or disruption?},
	volume = {324},
	shorttitle = {What determines the mass of the most massive star cluster in a galaxy},
	url = {http://adsabs.harvard.edu/abs/2009Ap%26SS.324..299G},
	doi = {10.1007/s10509-009-0102-y},
	abstract = {In many different galactic environments the cluster initial mass 
function (CIMF) is well described by a power law with index -2. This
implies a linear relation between the mass of the most massive cluster (
M max ) and the number of clusters. Assuming a constant
cluster formation rate and no disruption of the most massive clusters it
also means that M max increases linearly with age when
determining M max in logarithmic age bins. We observe this
increase in five out of the seven galaxies in our sample, suggesting
that M max is determined by the size of the sample. It also
means that massive clusters are very stable against disruption, in
disagreement with the mass-independent disruption (MID) model. For the
clusters in M51 and the Antennae galaxies, the size-of-sample prediction
breaks down around 106 M?, suggesting that
this is a physical upper limit to the masses of star clusters in these
galaxies. In this method there is a degeneracy between MID and a CIMF
truncation. We show how the cluster luminosity function can serve as a
tool to distinguish between the two.},
	urldate = {2020-08-17},
	journal = {Astrophysics and Space Science},
	author = {Gieles, Mark},
	month = dec,
	year = {2009},
	keywords = {Galaxies: star clusters, Globular clusters: general},
	pages = {299--304},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/FFPEIVY8/Gieles - 2009 - What determines the mass of the most massive star .pdf:application/pdf},
}

@article{weisz_panchromatic_2013,
	title = {The {Panchromatic} {Hubble} {Andromeda} {Treasury}. {IV}. {A} {Probabilistic} {Approach} to {Inferring} the {High}-mass {Stellar} {Initial} {Mass} {Function} and {Other} {Power}-law {Functions}},
	volume = {762},
	url = {http://adsabs.harvard.edu/abs/2013ApJ...762..123W},
	doi = {10.1088/0004-637X/762/2/123},
	abstract = {We present a probabilistic approach for inferring the parameters of the 
present-day power-law stellar mass function (MF) of a resolved young
star cluster. This technique (1) fully exploits the information content
of a given data set; (2) can account for observational uncertainties in
a straightforward way; (3) assigns meaningful uncertainties to the
inferred parameters; (4) avoids the pitfalls associated with binning
data; and (5) can be applied to virtually any resolved young cluster,
laying the groundwork for a systematic study of the high-mass stellar MF
(M {\textgreater}{\textasciitilde} 1 M ?). Using simulated clusters and Markov
Chain Monte Carlo sampling of the probability distribution functions, we
show that estimates of the MF slope, $\alpha$, are unbiased and that the
uncertainty, $\Delta$$\alpha$, depends primarily on the number of observed
stars and on the range of stellar masses they span, assuming that the
uncertainties on individual masses and the completeness are both well
characterized. Using idealized mock data, we compute the theoretical
precision, i.e., lower limits, on $\alpha$, and provide an analytic
approximation for $\Delta$$\alpha$ as a function of the observed number of
stars and mass range. Comparison with literature studies shows that {\textasciitilde}3/4
of quoted uncertainties are smaller than the theoretical lower limit. By
correcting these uncertainties to the theoretical lower limits, we find
that the literature studies yield lang$\alpha$rang = 2.46, with a
1$\sigma$ dispersion of 0.35 dex. We verify that it is impossible for a
power-law MF to obtain meaningful constraints on the upper mass limit of
the initial mass function, beyond the lower bound of the most massive
star actually observed. We show that avoiding substantial biases in the
MF slope requires (1) including the MF as a prior when deriving
individual stellar mass estimates, (2) modeling the uncertainties in the
individual stellar masses, and (3) fully characterizing and then
explicitly modeling the completeness for stars of a given mass. The
precision on MF slope recovery in this paper are lower limits, as we do
not explicitly consider all possible sources of uncertainty, including
dynamical effects (e.g., mass segregation), unresolved binaries, and
non-coeval populations. We briefly discuss how each of these effects can
be incorporated into extensions of the present framework. Finally, we
emphasize that the technique and lessons learned are applicable to more
general problems involving power-law fitting.

Based on observations made with the NASA/ESA Hubble Space Telescope,
obtained from the Data Archive at the Space Telescope Science Institute,
which is operated by the Association of Universities for Research in
Astronomy, Inc., under NASA contract NAS 5-26555.},
	urldate = {2020-08-18},
	journal = {The Astrophysical Journal},
	author = {Weisz, Daniel R. and Fouesneau, Morgan and Hogg, David W. and Rix, Hans-Walter and Dolphin, Andrew E. and Dalcanton, Julianne J. and Foreman-Mackey, Daniel T. and Lang, Dustin and Johnson, L. Clifton and Beerman, Lori C. and Bell, Eric F. and Gordon, Karl D. and Gouliermis, Dimitrios and Kalirai, Jason S. and Skillman, Evan D. and Williams, Benjamin F.},
	month = jan,
	year = {2013},
	keywords = {galaxies: star clusters: general, methods: statistical, mass function, stars: luminosity function},
	pages = {123},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/9GWVJ4V7/Weisz et al. - 2013 - The Panchromatic Hubble Andromeda Treasury. IV. A .pdf:application/pdf},
}

@article{foreman-mackey_emcee_2013,
	title = {emcee: {The} {MCMC} {Hammer}},
	volume = {125},
	issn = {0004-6280},
	shorttitle = {emcee},
	url = {http://adsabs.harvard.edu/abs/2013PASP..125..306F},
	doi = {10.1086/670067},
	abstract = {We introduce a stable, well tested Python implementation of the affine-invariant ensemble sampler for Markov chain Monte Carlo (MCMC) proposed by Goodman \& Weare (2010). The code is open source and has already been used in several published projects in the astrophysics literature. The algorithm behind emcee has several advantages over traditional MCMC sampling methods and it has excellent performance as measured by the autocorrelation time (or function calls per independent sample). One major advantage of the algorithm is that it requires hand-tuning of only 1 or 2 parameters compared to \~{}N2 for a traditional algorithm in an N-dimensional parameter space. In this document, we describe the algorithm and the details of our
implementation. Exploiting the parallelism of the ensemble method, emcee permits any user to take advantage of multiple CPU cores without extra effort. The code is available online at http://dan.iel.fm/emcee under the GNU General Public License v2.},
	urldate = {2020-08-18},
	journal = {Publications of the Astronomical Society of the Pacific},
	author = {Foreman-Mackey, Daniel and Hogg, David W. and Lang, Dustin and Goodman, Jonathan},
	month = mar,
	year = {2013},
	pages = {306},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/ET49HNWE/Foreman-Mackey et al. - 2013 - emcee The MCMC Hammer.pdf:application/pdf},
}

@article{krumholz_star_2015,
	title = {Star {Cluster} {Properties} in {Two} {LEGUS} {Galaxies} {Computed} with {Stochastic} {Stellar} {Population} {Synthesis} {Models}},
	volume = {812},
	url = {http://adsabs.harvard.edu/abs/2015ApJ...812..147K},
	doi = {10.1088/0004-637X/812/2/147},
	abstract = {We investigate a novel Bayesian analysis method, based on the 
Stochastically Lighting Up Galaxies (slug) code, to derive the masses,
ages, and extinctions of star clusters from integrated light photometry.
Unlike many analysis methods, slug correctly accounts for incomplete
initial mass function (IMF) sampling, and returns full posterior
probability distributions rather than simply probability maxima. We
apply our technique to 621 visually confirmed clusters in two nearby
galaxies, NGC 628 and NGC 7793, that are part of the Legacy
Extragalactic UV Survey (LEGUS). LEGUS provides Hubble Space Telescope
photometry in the NUV, U, B, V, and I bands. We analyze the sensitivity
of the derived cluster properties to choices of prior probability
distribution, evolutionary tracks, IMF, metallicity, treatment of
nebular emission, and extinction curve. We find that slug's results for
individual clusters are insensitive to most of these choices, but that
the posterior probability distributions we derive are often quite broad,
and sometimes multi-peaked and quite sensitive to the choice of priors.
In contrast, the properties of the cluster population as a whole are
relatively robust against all of these choices. We also compare our
results from slug to those derived with a conventional non-stochastic
fitting code, Yggdrasil. We show that slug's stochastic models are
generally a better fit to the observations than the deterministic ones
used by Yggdrasil. However, the overall properties of the cluster
populations recovered by both codes are qualitatively similar.},
	urldate = {2020-09-04},
	journal = {The Astrophysical Journal},
	author = {Krumholz, Mark R. and Adamo, Angela and Fumagalli, Michele and Wofford, Aida and Calzetti, Daniela and Lee, Janice C. and Whitmore, Bradley C. and Bright, Stacey N. and Grasha, Kathryn and Gouliermis, Dimitrios A. and Kim, Hwihyun and Nair, Preethi and Ryon, Jenna E. and Smith, Linda J. and Thilker, David and Ubeda, Leonardo and Zackrisson, Erik},
	month = oct,
	year = {2015},
	keywords = {galaxies: individual: NGC 628, galaxies: star clusters: general, methods: data analysis, methods: statistical, techniques: photometric, NGC 7793},
	pages = {147},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/EHUX6Q27/Krumholz et al. - 2015 - Star Cluster Properties in Two LEGUS Galaxies Comp.pdf:application/pdf},
}

@article{webb_initial_2020,
	title = {The {Initial} {Properties} of {Young} {Star} {Clusters} in {M83}},
	url = {http://arxiv.org/abs/2012.07831},
	abstract = {The initial sizes and masses of massive star clusters provide information about the cluster formation process and also determine how cluster populations are modified and destroyed, which have implications for using clusters as tracers of galaxy assembly. Young massive cluster populations are often assumed to be unchanged since cluster formation, and therefore their distribution of masses and radii are used as the initial values. However, the first few hundred million years of cluster evolution does change both cluster mass and cluster radius, through both internal and external processes. In this paper, we use a large suite of \$N\$-body cluster simulations in an appropriate tidal field to determine the best initial mass and initial size distributions of young clusters in the nearby galaxy M83. We find that the initial masses follow a power-law distribution with a slope of -2.7 \${\textbackslash}pm\$ 0.4, and the half-mass radii follow a log-normal distribution with a mean of 2.57 \${\textbackslash}pm\$ 0.04 pc and a dispersion of 1.59 \${\textbackslash}pm\$ 0.01 pc. The corresponding initial projected half-light radius function has a mean of 2.7 \${\textbackslash}pm\$ 0.3 pc and a dispersion of 1.7 \${\textbackslash}pm\$ 0.2 pc. The evolution of the initial mass and size distribution functions are consistent with mass loss and expansion due to stellar evolution, independent of the external tidal field and the cluster's initial density profile. Observed cluster sizes and masses should not be used as the initial values, even when clusters are only a few hundred million years old.},
	urldate = {2020-12-17},
	journal = {arXiv:2012.07831 [astro-ph]},
	author = {Webb, Jeremy J. and Sills, Alison},
	month = dec,
	year = {2020},
	note = {arXiv: 2012.07831},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/ASS8J428/Webb and Sills - 2020 - The Initial Properties of Young Star Clusters in M.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/CCMPJJZF/2012.html:text/html},
}

@article{li_gibbs_2020,
	title = {Gibbs {Point} {Process} {Model} for {Young} {Star} {Clusters} in {M33}},
	url = {http://arxiv.org/abs/2012.05938},
	abstract = {We demonstrate the power of Gibbs point process models from the spatial statistics literature when applied to studies of resolved galaxies. We conduct a rigorous analysis of the spatial distributions of objects in the star formation complexes of M33, including giant molecular clouds (GMCs) and young stellar cluster candidates (YSCCs). We choose a hierarchical model structure from GMCs to YSCCs based on the natural formation hierarchy between them. This approach circumvents the limitations of the empirical two-point correlation function analysis by naturally accounting for the inhomogeneity present in the distribution of YSCCs. We also investigate the effects of GMCs' properties on their spatial distributions. We confirm that the distribution of GMCs and YSCCs are highly correlated. We found that the spatial distributions of YSCCs reaches a peak of clustering pattern at {\textasciitilde}250 pc scale compared to a Poisson process. This clustering mainly occurs in regions where the galactocentric distance {\textgreater}{\textasciitilde}4.5 kpc. Furthermore, the galactocentric distance of GMCs and their mass have strong positive effects on the correlation strength between GMCs and YSCCs. We outline some possible implications of these findings for our understanding of the cluster formation process.},
	urldate = {2020-12-17},
	journal = {arXiv:2012.05938 [astro-ph, stat]},
	author = {Li, Dayi and Barmby, Pauline},
	month = dec,
	year = {2020},
	note = {arXiv: 2012.05938},
	keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics, Statistics - Applications},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/F7AK8TXD/Li and Barmby - 2020 - Gibbs Point Process Model for Young Star Clusters .pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/PQDSRZVA/2012.html:text/html},
}

@article{li_star_2018,
	title = {Star {Cluster} {Formation} in {Cosmological} {Simulations}. {II}. {Effects} of {Star} {Formation} {Efficiency} and {Stellar} {Feedback}},
	volume = {861},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2018ApJ...861..107L},
	doi = {10.3847/1538-4357/aac9b8},
	abstract = {The implementation of star formation and stellar feedback in 
cosmological simulations plays a critical role in shaping galaxy
properties. In the first paper of the series, we presented a new method
to model star formation as a collection of star clusters. In this paper,
we improve the algorithm by eliminating accretion gaps, boosting
momentum feedback, and introducing a subgrid initial bound fraction, f
 i , that distinguishes cluster mass from stellar particle
mass. We perform a suite of simulations with different star formation
efficiency per freefall time \{? \vphantom{\{}\}ff\} and supernova
momentum feedback intensity \{f\vphantom{\{}\}boost\}. We find that the star
formation history of a Milky Way-sized galaxy is sensitive to
\{f\vphantom{\{}\}boost\}, which allows us to constrain its value,
\{f\vphantom{\{}\}boost\}? 5, in the current simulation setup. Changing
\{? \vphantom{\{}\}ff\} from a few percent to 200\% has little effect on
global galaxy properties. However, on smaller scales, the properties of
star clusters are very sensitive to \{? \vphantom{\{}\}ff\}. We find
that f i increases with \{? \vphantom{\{}\}ff\} and cluster
mass. Through the dependence on f i , the shape of the
cluster initial mass function varies strongly with \{\vphantom{\}}?
\vphantom{\{}\}ff\vphantom{\{}\}. The fraction of clustered star formation and maximum
cluster mass increase with the star formation rate surface density, with
the normalization of both relations dependent on \{\vphantom{\}}?
\vphantom{\{}\}ff\vphantom{\{}\}. The cluster formation timescale systematically
decreases with increasing \{? \vphantom{\{}\}ff\}. Local variations in
the gas accretion history lead to a 0.25 dex scatter for the integral
cluster formation efficiency. Joint constraints from all the observables
prefer the runs that produce a median integral efficiency of 16\%.},
	urldate = {2020-12-22},
	journal = {The Astrophysical Journal},
	author = {Li, Hui and Gnedin, Oleg Y. and Gnedin, Nickolay Y.},
	month = jul,
	year = {2018},
	keywords = {galaxies: star clusters: general, galaxies: star formation, galaxies: formation, methods: numerical, galaxies: high-redshift},
	pages = {107},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/QDJ6IG2C/Li et al. - 2018 - Star Cluster Formation in Cosmological Simulations.pdf:application/pdf},
}

@article{li_star_2017,
	title = {Star {Cluster} {Formation} in {Cosmological} {Simulations}. {I}. {Properties} of {Young} {Clusters}},
	volume = {834},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2017ApJ...834...69L},
	doi = {10.3847/1538-4357/834/1/69},
	abstract = {We present a new implementation of star formation in cosmological 
simulations by considering star clusters as a unit of star formation.
Cluster particles grow in mass over several million years at the rate
determined by local gas properties, with high time resolution. The
particle growth is terminated by its own energy and momentum feedback on
the interstellar medium. We test this implementation for Milky Way-sized
galaxies at high redshift by comparing the properties of model clusters
with observations of young star clusters. We find that the cluster
initial mass function is best described by a Schechter function rather
than a single power law. In agreement with observations, at low masses
the logarithmic slope is $\alpha$ ? 1.8\{--\}2, while the cutoff at high
mass scales with the star formation rate (SFR). A related trend is a
positive correlation between the surface density of the SFR and fraction
of stars contained in massive clusters. Both trends indicate that the
formation of massive star clusters is preferred during bursts of star
formation. These bursts are often associated with major-merger events.
We also find that the median timescale for cluster formation ranges from
0.5 to 4 Myr and decreases systematically with increasing star formation
efficiency. Local variations in the gas density and cluster accretion
rate naturally lead to the scatter of the overall formation efficiency
by an order of magnitude, even when the instantaneous efficiency is kept
constant. Comparison of the formation timescale with the observed age
spread of young star clusters provides an additional important
constraint on the modeling of star formation and feedback schemes.},
	urldate = {2020-12-22},
	journal = {The Astrophysical Journal},
	author = {Li, Hui and Gnedin, Oleg Y. and Gnedin, Nickolay Y. and Meng, Xi and Semenov, Vadim A. and Kravtsov, Andrey V.},
	month = jan,
	year = {2017},
	keywords = {galaxies: star clusters: general, galaxies: formation, cosmology: theory},
	pages = {69},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/R97SLB2Q/Li et al. - 2017 - Star Cluster Formation in Cosmological Simulations.pdf:application/pdf},
}

@article{weisz_high-mass_2015,
	title = {The {High}-mass {Stellar} {Initial} {Mass} {Function} in {M31} {Clusters}},
	volume = {806},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2015ApJ...806..198W},
	doi = {10.1088/0004-637X/806/2/198},
	abstract = {We have undertaken the largest systematic study of the high-mass stellar initial mass function (IMF) to date using the optical color-magnitude diagrams (CMDs) of 85 resolved, young (4 \{Myr\}{\textbackslash}lt t{\textbackslash}lt 25 \{Myr\}), intermediate mass star clusters (103-104
M?), observed as part of the Panchromatic Hubble
Andromeda Treasury program. We fit each cluster{\textquoteright}s CMD to measure its mass function (MF) slope for stars ?2 M?. By
modeling the ensemble of clusters, we find the distribution of MF slopes is best described by $\Gamma$ = +\{1.45\}-0.06+0.03 with a very small intrinsic scatter and no drastic outliers. This model allows the MF slope to depend on cluster mass, size, and age, but the data imply no significant dependencies within this regime of cluster properties. The lack of an age dependence suggests that the MF slope has not significantly evolved over the first \~{}25 Myr and provides direct observational evidence that the measured MF represents the IMF. Taken together, this analysis{\textemdash}based on an unprecedented large sample of young clusters, homogeneously constructed CMDs, well-defined selection criteria, and consistent principled modeling{\textemdash}implies that the
high-mass IMF slope in M31 clusters is universal. The IMF has a slope ($\Gamma$ = +\{1.45\}-0.06+0.03; statistical
uncertainties) that is slightly steeper than the canonical Kroupa (+1.30) and Salpeter (+1.35) values, and our measurement of it
represents a factor of \~{}20 improvement in precision over the Kroupa IMF (+1.30 {\textpm} 0.7). Using our inference model on select Milky Way (MW) and LMC high-mass IMF studies from the literature, we find \{$\Gamma$ \}\{MW\}\~{} +1.15+/- 0.1 and \{$\Gamma$ \}\{LMC\}\~{}
+1.3+/- 0.1, both with intrinsic scatter of \~{}0.3-0.4 dex. Thus,
while the high-mass IMF in the Local Group may be universal, systematics in the literature of IMF studies preclude any definitive conclusions; homogenous investigations of the high-mass IMF in the local universe are needed to overcome this limitation. Consequently, the present study represents the most robust measurement of the high-mass IMF slope to date. To facilitate practical use over the full stellar mass spectrum, we have grafted the M31 high-mass IMF slope onto widely used sub-solar mass Kroupa and Chabrier IMFs. The increased steepness in the M31 high-mass IMF slope implies that commonly used UV- and H$\alpha$-based
star formation rates should be increased by a factor of \~{}1.3-1.5 and the number of stars with masses {\textbackslash}gt 8 M? is \~{}25\%
fewer than expected for a Salpeter/Kroupa IMF.

Based on observations made with the NASA/ESA Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555. These observations are associated with program \#12055.},
	urldate = {2021-01-19},
	journal = {The Astrophysical Journal},
	author = {Weisz, Daniel R. and Johnson, L. Clifton and Foreman-Mackey, Daniel and Dolphin, Andrew E. and Beerman, Lori C. and Williams, Benjamin F. and Dalcanton, Julianne J. and Rix, Hans-Walter and Hogg, David W. and Fouesneau, Morgan and Johnson, Benjamin D. and Bell, Eric F. and Boyer, Martha L. and Gouliermis, Dimitrios and Guhathakurta, Puragra and Kalirai, Jason S. and Lewis, Alexia R. and Seth, Anil C. and Skillman, Evan D.},
	month = jun,
	year = {2015},
	keywords = {galaxies: star clusters: general, galaxies: star formation, mass function, stars: luminosity function, Hertzsprung{\textendash}Russell and C{\textendash}M diagrams, Local Group},
	pages = {198},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/SMJDH27B/Weisz et al. - 2015 - The High-mass Stellar Initial Mass Function in M31.pdf:application/pdf},
}

@article{bresolin_abundance_2011,
	title = {The {Abundance} {Scatter} in {M33} from {H} {II} {Regions}: {Is} {There} {Any} {Evidence} for {Azimuthal} {Metallicity} {Variations}?},
	volume = {730},
	issn = {0004-637X},
	shorttitle = {The {Abundance} {Scatter} in {M33} from {H} {II} {Regions}},
	url = {http://adsabs.harvard.edu/abs/2011ApJ...730..129B},
	doi = {10.1088/0004-637X/730/2/129},
	abstract = {Optical spectra of 25 H II regions in the inner 2 kpc of the M33 disk 
have been obtained with the Gemini Multi-Object Spectrograph at the
Gemini North telescope. The oxygen abundance gradient measured from the
detection of the [O III] $\lambda$4363 auroral line displays a scatter of
approximately 0.06 dex, a much smaller value than recently reported by
Rosolowsky \& Simon in this galaxy. The analysis of the abundances
for a large sample of H II regions derived from the R 23
strong-line indicator confirms that the scatter is small over the full
disk of M33, consistent with the measuring uncertainties, and comparable
to what is observed in other spiral galaxies. No evidence is therefore
found for significant azimuthal variations in the present-day
metallicity of the interstellar medium in this galaxy on spatial scales
from {\textasciitilde}100 pc to a few kpc. A considerable fraction of M33 H II regions
with auroral line detections show spectral features revealing sources of
hard ionizing radiation (such as He II emission and large [Ne III], [O
III] line fluxes). Since R 23 is shown to severely
underestimate the oxygen abundances in such cases, care must be taken in
chemical abundance studies of extragalactic H II regions based on this
strong-line indicator.

Based on observations obtained at the Gemini Observatory, which is
operated by the Association of Universities for Research in Astronomy,
Inc., under a cooperative agreement with the NSF on behalf of the Gemini
partnership: the National Science Foundation (United States), the
Science and Technology Facilities Council (United Kingdom), the National
Research Council (Canada), CONICYT (Chile), the Australian Research
Council (Australia), Minist{\'e}rio da Ci{\^e}ncia e Tecnologia
(Brazil) and Ministerio de Ciencia, Tecnolog{\'i}a e
Innovaci{\'o}n Productiva (Argentina).},
	urldate = {2021-01-19},
	journal = {The Astrophysical Journal},
	author = {Bresolin, Fabio},
	month = apr,
	year = {2011},
	keywords = {galaxies: ISM, galaxies: individual: M33, galaxies: abundances},
	pages = {129},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/SKUMKAMK/Bresolin - 2011 - The Abundance Scatter in M33 from H II Regions Is.pdf:application/pdf},
}

@article{plucinsky_chandra_2008,
	title = {Chandra {ACIS} {Survey} of {M33} ({ChASeM33}): {A} {First} {Look}},
	volume = {174},
	issn = {0067-0049},
	shorttitle = {Chandra {ACIS} {Survey} of {M33} ({ChASeM33})},
	url = {http://adsabs.harvard.edu/abs/2008ApJS..174..366P},
	doi = {10.1086/522942},
	abstract = {We present an overview of the Chandra ACIS Survey of M33 (ChASeM33): A Deep Survey of the Nearest Face-on Spiral Galaxy. The 1.4 Ms survey covers the galaxy out to R ? 18'(? 4 kpc) . These data provide the most intensive, high spatial resolution assessment of the X-ray source populations available for the confused inner regions of M33. Mosaic images of the ChASeM33 observations show several hundred individual X-ray sources as well as soft diffuse emission from the hot interstellar medium. Bright, extended emission surrounds the nucleus and is also seen from the giant H II regions NGC 604 and IC 131. Fainter extended emission and numerous individual sources appear to trace the inner spiral structure. The initial source catalog, arising from {\textasciitilde}2/3 of the expected survey data, includes 394 sources significant at the 3 $\sigma$ confidence level or greater, down to a limiting luminosity (absorbed) of {\textasciitilde}1.6 {\texttimes} 1035 ergs s-1 (0.35-8.0 keV). The
hardness ratios of the sources separate those with soft, thermal spectra such as supernova remnants from those with hard, nonthermal spectra such as X-ray binaries and background active galactic nuclei. Emission extended beyond the Chandra point-spread function is evident in 23 of the 394 sources. Cross-correlation of the ChASeM33 sources against previous catalogs of X-ray sources in M33 results in matches for the vast majority of the brighter sources and shows 28 ChASeM33 sources within 10'' of supernova remnants identified by prior optical and radio searches. This brings the total number of such associations to 31 out of 100 known supernova remnants in M33.},
	urldate = {2021-01-20},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Plucinsky, Paul P. and Williams, Benjamin and Long, Knox S. and Gaetz, Terrance J. and Sasaki, Manami and Pietsch, Wolfgang and T{\"u}llmann, Ralph and Smith, Randall K. and Blair, William P. and Helfand, David and Hughes, John P. and Winkler, P. Frank and de Avillez, Miguel and Bianchi, Luciana and Breitschwerdt, Dieter and Edgar, Richard J. and Ghavamian, Parviz and Grindlay, Jonathan and Haberl, Frank and Kirshner, Robert and Kuntz, Kip and Mazeh, Tsevi and Pannuti, Thomas G. and Shporer, Avi and Thilker, David A.},
	month = feb,
	year = {2008},
	keywords = {galaxies: individual: M33, supernova remnants, X-rays: galaxies},
	pages = {366--378},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/5G929H7N/Plucinsky et al. - 2008 - Chandra ACIS Survey of M33 (ChASeM33) A First Loo.pdf:application/pdf},
}

@article{kang_evolution_2012,
	title = {The evolution and star-formation history of {M33}},
	volume = {426},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1455K},
	doi = {10.1111/j.1365-2966.2012.21778.x},
	abstract = {We construct a parametrized model to explore the main properties of the star-formation history of M33. We assume that the disc originates and grows by primordial gas infall and adopt a simple form of gas accretion rate with one free parameter, the infall time-scale. We also include the contribution of the gas outflow process. A major update of the model is that we adopt a molecular-hydrogen-correlated star-formation law and calculate the evolution of the atomic and molecular gas separately. Comparisons between the model predictions and observational data show that the model predictions are very sensitive to the adopted infall time-scale, while the gas-outflow process mainly influences the
metallicity profile. A model adopting a moderate outflow rate and an inside-out formation scenario can be in good agreement with most of the observed constraints of the M33 disc. We also compare model predictions based on a molecular-hydrogen-correlated star-formation law and that based on the Kennicutt star-formation law. Our results imply that the molecular-hydrogen-correlated star-formation law should be preferred to describe the evolution of the M33 disc, especially the radial
distributions of both the cold gas and the stellar population.},
	urldate = {2021-01-28},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kang, Xiaoyu and Chang, Ruixiang and Yin, Jun and Hou, Jinliang and Zhang, Fenghui and Zhang, Yu and Han, Zhanwen},
	month = oct,
	year = {2012},
	keywords = {galaxies: spiral, galaxies: individual: M33, galaxies: evolution, galaxies: abundances},
	pages = {1455--1464},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/4ITZFAKQ/Kang et al. - 2012 - The evolution and star-formation history of M33.pdf:application/pdf},
}

@article{cautun_aftermath_2019,
	title = {The aftermath of the {Great} {Collision} between our {Galaxy} and the {Large} {Magellanic} {Cloud}},
	volume = {483},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2019MNRAS.483.2185C},
	doi = {10.1093/mnras/sty3084},
	abstract = {The Milky Way (MW) offers a uniquely detailed view of galactic structure 
and is often regarded as a prototypical spiral galaxy. But recent
observations indicate that the MW is atypical: it has an undersized
supermassive black hole at its centre; it is surrounded by a very low
mass, excessively metal-poor stellar halo; and it has an unusually large
nearby satellite galaxy, the Large Magellanic Cloud (LMC). Here, we show
that the LMC is on a collision course with the MW with which it will
merge in 2.4{\textasciicircum}\{+1.2\}\_\{-0.8\} \{Gyr\} (68 per cent confidence level). This
catastrophic and long-overdue event will restore the MW to normality.
Using the EAGLE galaxy formation simulation, we show that, as a result
of the merger, the central supermassive black hole will increase in mass
by up to a factor of 8. The Galactic stellar halo will undergo an
equally impressive transformation, becoming 5 times more massive. The
additional stars will come predominantly from the disrupted LMC, but a
sizeable number will be ejected on to the halo from the stellar disc.
The post-merger stellar halo will have the median metallicity of the
LMC, [Fe/H] = -0.5 dex, which is typical of other galaxies of similar
mass to the MW. At the end of this exceptional event, the MW will become
a true benchmark for spiral galaxies, at least temporarily.},
	urldate = {2021-02-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Cautun, Marius and Deason, Alis J. and Frenk, Carlos S. and McAlpine, Stuart},
	month = feb,
	year = {2019},
	keywords = {Magellanic Clouds, Galaxy: halo, galaxies: kinematics and dynamics, galaxies: dwarfs, galaxies: haloes},
	pages = {2185--2196},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/J5IDGVHE/Cautun et al. - 2019 - The aftermath of the Great Collision between our G.pdf:application/pdf},
}

@article{elmegreen_star_1993,
	title = {Star {Formation} at {Compressed} {Interfaces} in {Turbulent} {Self}-gravitating {Clouds}},
	volume = {419},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/1993ApJ...419L..29E},
	doi = {10.1086/187129},
	abstract = {Supersonic turbulence in both self-gravitating and diffuse clouds can produce self-similar, hierarchical density structures and broad
line-wings on a wide range of scales, making these two cloud types look similar and giving the clumps in each the same scaling laws.  We show here that the dense compressed regions that form between converging turbulent flows should collapse to form dense cores and ultimately stars in self-gravitating clouds, wheras they only disperse and reform intermittently in diffuse clouds.  Star formation in
turbulence-compressed regions should be as hierarchical as the
turbulence, leading to clusters and multiple star systems instead of single stars; some binary stars may form by gravitational capture of stars in nearby turbulent clumps.  Reasonable mass functions for clumps and stars are estimated from the theory.  The slope of the initial stellar mass function is steeper than that for the clumps because of the increasing lifetime for clumps with larger mass.},
	urldate = {2021-02-23},
	journal = {The Astrophysical Journal Letters},
	author = {Elmegreen, B. G.},
	month = dec,
	year = {1993},
	keywords = {INSTABILITIES, ISM: STRUCTURE, SHOCK WAVES, STARS: FORMATION, TURBULENCE},
	pages = {L29},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/3D3A7SZL/Elmegreen - 1993 - Star Formation at Compressed Interfaces in Turbule.pdf:application/pdf},
}

@article{whitworth_erosion_1979,
	title = {The erosion and dispersal of massive molecular clouds by young stars},
	volume = {186},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/1979MNRAS.186...59W},
	doi = {10.1093/mnras/186.1.59},
	abstract = {The paper evaluates the efficiency with which O stars disperse the molecular clouds from which they form. An O star near the surface of an extended molecular cloud ionizes a H II region which is
radiation-bounded on the inner side (towards the cloud center) and density-bounded on the outer side; consequently the ionized gas can stream away into space on the outer side, and this in turn enables the ionization front on the inner side to advance faster into the cloud, thus eroding a large cavity around the O star. This process may be very effective in destroying molecular clouds; if approximately 4 per cent of a cloud's material were converted into new stars with a Salpeter Initial Mass Function, the remaining 96 per cent could be broken up and
dispersed by the ionizing radiation from the O stars.},
	urldate = {2021-02-23},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Whitworth, A.},
	month = jan,
	year = {1979},
	keywords = {Early Stars, Galactic Structure, H Ii Regions, Interstellar Gas, Molecular Physics, O Stars, Protostars, Stellar Evolution, Stellar Winds},
	pages = {59--67},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/T9NJY54Z/Whitworth - 1979 - The erosion and dispersal of massive molecular clo.pdf:application/pdf},
}

@article{krumholz_big_2014,
	title = {The big problems in star formation: {The} star formation rate, stellar clustering, and the initial mass function},
	volume = {539},
	issn = {0370-1573},
	shorttitle = {The big problems in star formation},
	url = {http://adsabs.harvard.edu/abs/2014PhR...539...49K},
	doi = {10.1016/j.physrep.2014.02.001},
	abstract = {Star formation lies at the center of a web of processes that drive 
cosmic evolution: generation of radiant energy, synthesis of elements,
formation of planets, and development of life. Decades of observations
have yielded a variety of empirical rules about how it operates, but at
present we have no comprehensive, quantitative theory. In this review I
discuss the current state of the field of star formation, focusing on
three central questions: What controls the rate at which gas in a galaxy
converts to stars? What determines how those stars are clustered, and
what fraction of the stellar population ends up in gravitationally-bound
structures? What determines the stellar initial mass function, and does
it vary with star-forming environment? I use these three questions as a
lens to introduce the basics of star formation, beginning with a review
of the observational phenomenology and the basic physical processes. I
then review the status of current theories that attempt to solve each of
the three problems, pointing out links between them and opportunities
for theoretical and numerical work that crosses the scale between them.
I conclude with a discussion of prospects for theoretical progress in
the coming years.},
	urldate = {2021-02-23},
	journal = {Physics Reports},
	author = {Krumholz, Mark R.},
	month = jun,
	year = {2014},
	keywords = {ISM: clouds, mass function, Galaxies: star formation, ISM: molecules, Stars: formation, Stars: luminosity function, Turbulence},
	pages = {49--134},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7NEYJ6R7/Krumholz - 2014 - The big problems in star formation The star forma.pdf:application/pdf},
}

@article{hiltner_colors_1960,
	title = {Colors and {Magnitudes} of {Clusters} in {M31} and {M33}.},
	volume = {131},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/1960ApJ...131..163H},
	doi = {10.1086/146818},
	abstract = {Abstract image available at: 
http://adsabs.harvard.edu/abs/1960ApJ...131..163H},
	urldate = {2021-02-24},
	journal = {The Astrophysical Journal},
	author = {Hiltner, W. A.},
	month = jan,
	year = {1960},
	pages = {163},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/5HNTQ7LP/Hiltner - 1960 - Colors and Magnitudes of Clusters in M31 and M33..pdf:application/pdf},
}

@article{zloczewski_photometric_2008,
	title = {Photometric {Survey} for {Stellar} {Clusters} in the {Outer} {Part} of {M33}},
	volume = {58},
	issn = {0001-5237},
	url = {http://adsabs.harvard.edu/abs/2008AcA....58...23Z},
	abstract = {We present a catalog of 4780 extended sources from the outer field of M33. The catalog includes 73 previously identified clusters or planetary nebulae, 1153 likely background galaxies, and 3554 new candidate stellar clusters. The survey is based on deep ground-based images obtained with the MegaCam instrument on the CFHT telescope. We provide g'r'i'
photometry for detected objects as well as estimates of the FWHM and ellipticity of their profiles. The sample includes 122 new, relatively bright, likely globular clusters. Follow-up observations of fainter candidates from our list may extend the faint-end of the observed luminosity function of globular clusters in M33 by up to 3 magnitudes. The catalog includes several cluster candidates located in the outskirts of the galaxy. These objects are promising targets for deep photometry with the HST. We present a color-magnitude diagram for one detected object, showing that it is an extended and low-surface-brightness old cluster located at an angular distance of 27' from the center of M33.},
	urldate = {2021-02-24},
	journal = {Acta Astronomica},
	author = {Zloczewski, K. and Kaluzny, J. and Hartman, J.},
	month = mar,
	year = {2008},
	keywords = {Galaxies: star clusters, Catalogs, Galaxies: individual: M33},
	pages = {23--39},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/VBDZZH7S/Zloczewski et al. - 2008 - Photometric Survey for Stellar Clusters in the Out.pdf:application/pdf},
}

@article{williams_panchromatic_2021,
	title = {The {Panchromatic} {Hubble} {Andromeda} {Treasury}: {Triangulum} {Extended} {Region} ({PHATTER}) {I}. {Ultraviolet} to {Infrared} {Photometry} of 22 {Million} {Stars} in {M33}},
	volume = {2101},
	shorttitle = {The {Panchromatic} {Hubble} {Andromeda} {Treasury}},
	url = {http://adsabs.harvard.edu/abs/2021arXiv210101293W},
	abstract = {We present panchromatic resolved stellar photometry for 22 million stars 
in the Local Group dwarf spiral Triangulum (M33), derived from Hubble
Space Telescope (HST) observations with the Advanced Camera for Surveys
(ACS) in the optical (F475W, F814W), and the Wide Field Camera 3 (WFC3)
in the near ultraviolet (F275W, F336W) and near-infrared (F110W, F160W)
bands. The large, contiguous survey area covers \${\textbackslash}sim\$14 square kpc and
extends to 3.5 kpc (14 arcmin, or 1.5-2 scale lengths) from the center
of M33. The PHATTER observing strategy and photometry technique closely
mimic those of the Panchromatic Hubble Andromeda Treasury (PHAT), but
with updated photometry techniques that take full advantage of all
overlapping pointings (aligned to within \${\textless}\$5-10 milliarcseconds) and
improved treatment of spatially-varying point spread functions. The
photometry reaches a completeness-limited depth of F475W\${\textbackslash}sim\$28.5 in
the lowest surface density regions observed in M33 and F475W\${\textbackslash}sim\$26.5
in the most crowded regions found near the center of M33. We find the
young populations trace several relatively tight arms, while the old
populations show a clear, looser two-armed structure. We present
extensive analysis of the data quality including artificial star tests
to quantify completeness, photometric uncertainties, and flux biases.
This stellar catalog is the largest ever produced for M33, and is
publicly available for download by the community.},
	urldate = {2021-02-24},
	journal = {arXiv e-prints},
	author = {Williams, Benjamin F. and Durbin, Meredith J. and Dalcanton, Julianne J. and Lang, Dustin and Girardi, Leo and Smercina, Adam and Dolphin, Andrew and Weisz, Daniel R. and Choi, Yumi and Bell, Eric F. and Rosolowsky, Erik and Skillman, Evan and Koch, Eric W. and Lindberg, Christine W. and Hagen, Lea and Gordon, Karl D. and Seth, Anil and Gilbert, Karoline and Guhathakurta, Puragra and Lauer, Tod and Bianchi, Luciana},
	month = jan,
	year = {2021},
	keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
	pages = {arXiv:2101.01293},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/RVDNJWSI/Williams et al. - 2021 - The Panchromatic Hubble Andromeda Treasury Triang.pdf:application/pdf},
}

@article{bergh_he_1991,
	title = {{HE} {STELLAR} {POPULATIONS} {OF} {M33}},
	volume = {103},
	issn = {1538-3873},
	url = {https://iopscience.iop.org/article/10.1086/132860/meta},
	doi = {10.1086/132860},
	language = {en},
	number = {665},
	urldate = {2019-11-24},
	journal = {Publications of the Astronomical Society of the Pacific},
	author = {Bergh, Sidney van den},
	month = jul,
	year = {1991},
	pages = {609},
	file = {Snapshot:/Users/Tobin/Zotero/storage/IQEQKD84/132860.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/52E8YZD2/Bergh - 1991 - HE STELLAR POPULATIONS OF M33.pdf:application/pdf},
}

@article{blitz_role_2006,
	title = {The {Role} of {Pressure} in {GMC} {Formation} {II}: {The} {H} $_{\textrm{2}}$ -{Pressure} {Relation}},
	volume = {650},
	issn = {0004-637X, 1538-4357},
	shorttitle = {The {Role} of {Pressure} in {GMC} {Formation} {II}},
	url = {http://stacks.iop.org/0004-637X/650/i=2/a=933},
	doi = {10.1086/505417},
	abstract = {We show that the ratio of molecular to atomic gas in galaxies is determined by hydrostatic pressure and that the relation between the two is nearly linear. The pressure relation is shown to be good over 3 orders of magnitude for 14 galaxies, including dwarfs, H i{\textendash}rich, and H2-rich galaxies, as well as the Milky Way. The sample spans a factor of 5 in mean metallicity. The rms scatter of individual points of the relation is only about a factor of 2 for all the galaxies, although some show much more scatter than others. Using these results, we propose a modified star formation prescription based on pressure determining the degree to which the ISM is molecular. The formulation is different in high- and low-pressure regimes, defined by whether the gas is primarily atomic or primarily molecular. This formulation can be implemented in simulations and provides a more appropriate treatment of the outer regions of spiral galaxies and molecule-poor systems, such as dwarf irregulars and damped Ly  systems.},
	language = {en},
	number = {2},
	urldate = {2019-11-24},
	journal = {The Astrophysical Journal},
	author = {Blitz, Leo and Rosolowsky, Erik},
	month = oct,
	year = {2006},
	pages = {933--944},
	file = {Blitz and Rosolowsky - 2006 - The Role of Pressure in GMC Formation II The H s.pdf:/Users/Tobin/Zotero/storage/HE2QRLJ3/Blitz and Rosolowsky - 2006 - The Role of Pressure in GMC Formation II The H s.pdf:application/pdf},
}

@article{chomiuk_toward_2011,
	title = {{TOWARD} {A} {UNIFICATION} {OF} {STAR} {FORMATION} {RATE} {DETERMINATIONS} {IN} {THE} {MILKY} {WAY} {AND} {OTHER} {GALAXIES}},
	volume = {142},
	issn = {0004-6256, 1538-3881},
	url = {http://stacks.iop.org/1538-3881/142/i=6/a=197?key=crossref.6fbff35a49f2a07e05b1e15580cefe33},
	doi = {10.1088/0004-6256/142/6/197},
	abstract = {The star formation rate (SFR) of the Milky Way remains poorly known, with often-quoted values ranging from 1 to 10 M yr-1. This situation persists despite the potential for the Milky Way to serve as the ultimate SFR calibrator for external galaxies. We show that various estimates for the Galactic SFR are consistent with one another once they have been normalized to the same initial mass function (IMF) and massive star models, converging to 1.9 {\textpm} 0.4 M yr-1. However, standard SFR diagnostics are vulnerable to systematics founded in the use of indirect observational tracers sensitive only to high-mass stars. We find that absolute SFRs measured using resolved low/intermediate-mass stellar populations in Galactic H ii regions are systematically higher by factors of \~{}2{\textendash}3 compared with calibrations for SFRs measured from mid-IR and radio emission. We discuss some potential explanations for this discrepancy and conclude that it could be allayed if (1) the power-law slope of the IMF for intermediate-mass (1.5 M {\textless} m {\textless} 5M ) stars were steeper than the Salpeter slope or (2) a correction factor was applied to the extragalactic 24 $\mu$m SFR calibrations to account for the duration of star formation in individual mid-IR{\textendash}bright H ii regions relative to the lifetimes of O stars. Finally, we present some approaches for testing whether a Galactic SFR of \~{}2 M yr-1 is consistent with what we would measure if we could view the Milky Way as external observers. Using luminous radio supernova remnants and X-ray point sources, we find that the Milky Way deviates from expectations at the 1$\sigma$ {\textendash}3$\sigma$ level, hinting that perhaps the Galactic SFR is overestimated or extragalactic SFRs need to be revised upward.},
	language = {en},
	number = {6},
	urldate = {2019-11-11},
	journal = {The Astronomical Journal},
	author = {Chomiuk, Laura and Povich, Matthew S.},
	month = dec,
	year = {2011},
	pages = {197},
	file = {Chomiuk and Povich - 2011 - TOWARD A UNIFICATION OF STAR FORMATION RATE DETERM.pdf:/Users/Tobin/Zotero/storage/EJGZQIW7/Chomiuk and Povich - 2011 - TOWARD A UNIFICATION OF STAR FORMATION RATE DETERM.pdf:application/pdf},
}

@article{davidge_stellar_2011,
	title = {{THE} {STELLAR} {ARCHEOLOGY} {OF} {THE} {M33} {DISK}: {RECENT} {STAR}-{FORMING} {HISTORY} {AND} {CONSTRAINTS} {ON} {THE} {TIMING} {OF} {AN} {INTERACTION} {WITH} {M31},},
	volume = {738},
	issn = {0004-637X, 1538-4357},
	shorttitle = {{THE} {STELLAR} {ARCHEOLOGY} {OF} {THE} {M33} {DISK}},
	url = {http://stacks.iop.org/0004-637X/738/i=2/a=144?key=crossref.7586b290a170d1b93a265ebf414e6e32},
	doi = {10.1088/0004-637X/738/2/144},
	abstract = {Images recorded with MegaCam are used to investigate the recent (t 0.25 Gyr) star-forming history (SFH) of the Local Group Sc galaxy M33. The data sample the entire star-forming disk, as well as areas immediately to the north and south of the galaxy. The properties of the stellar disk change near RGC = 8 kpc. Within this radius the luminosity function of main-sequence stars indicates that the star formation rate (SFR) has been constant with time during at least the past 250 Myr, while at larger radii the SFR has declined during this same time period. That the recent SFR in the inner disk has been constant suggests that M33 has evolved in isolation for at least the past \~{}0.5 Gyr, thereby providing a constraint on the timing of any recent interaction with M31. The color of the main-sequence ridgeline changes with radius, suggesting a gradient in extinction of size $\Delta$AV /$\Delta$RGC = -0.05 mag kpc-1. The fractional contribution that young stars make to the total mass of the stellar disk changes with radius, peaking near 8 kpc. Evidence is also presented of systematic spatial variations in the SFH of the disk, such that the SFR during the past 100 Myr in the southern half of the galaxy has been \~{}0.4 dex higher than in the northern half. Finally, structures with sizes spanning many kpc that contain blue objects{\textemdash}presumably main-sequence stars that formed during intermediate epochs{\textemdash}are identified near the disk boundary. It is argued that these are tidal features that were pulled from the main body of M33 and{\textemdash}in some cases{\textemdash}are the fossil remnants of star formation that occurred in an extended disk during intermediate epochs.},
	language = {en},
	number = {2},
	urldate = {2019-11-11},
	journal = {The Astrophysical Journal},
	author = {Davidge, T. J. and Puzia, T. H.},
	month = sep,
	year = {2011},
	pages = {144},
	file = {Davidge and Puzia - 2011 - THE STELLAR ARCHEOLOGY OF THE M33 DISK RECENT STA.pdf:/Users/Tobin/Zotero/storage/WR48CDVZ/Davidge and Puzia - 2011 - THE STELLAR ARCHEOLOGY OF THE M33 DISK RECENT STA.pdf:application/pdf},
}

@article{elson_multi-scale_2019,
	title = {A {Multi}-{Scale} {Study} of {Star} {Formation} in {Messier} 33},
	volume = {483},
	issn = {0035-8711, 1365-2966},
	url = {http://arxiv.org/abs/1811.04590},
	doi = {10.1093/mnras/sty3091},
	abstract = {For the Local Group Scd galaxy M 33 this paper presents a multi-scale study of the relationship between the monochromatic star formation rate (SFR) estimator based on 12 \${\textbackslash}mu\$m emission and the total SFR estimator based on a combination of far-ultraviolet and 24 \${\textbackslash}mu\$m emission. We show the 12 \${\textbackslash}mu\$m emission to be a linear estimator of total SFR on spatial scales from 782 pc down to 49 pc, over almost four magnitudes in SFR. These results therefore extend to sub-kpc length scales the analogous results from other studies for global length scales. We use high-resolution HI and \${\textasciicircum}\{12\}{\textbackslash}mathrm\{CO\}(J=2-1)\$ image sets from the literature to compare the star formation to the neutral gas. For the full range of length scales we find well-defined power-law relationships between 12 \${\textbackslash}mu\$m-derived SFR surface densities and neutral gas surface densities. For the H\$\_{\textbackslash}mathrm\{2\}\$ gas component almost all correlations are consistent with being linear. No evidence is found for a breakdown in the star formation law at small length scales in M 33 reported by other authors. We show that the average star formation efficiency in M 33 is roughly \$10{\textasciicircum}\{-9\}\$ yr\${\textasciicircum}\{-1\}\$ and that it remains constant down to giant molecular cloud length scales. Toomre and shear-based models of the star formation threshold are shown to inaccurately account for the star formation activity in the inner disc of M 33. Finally, we clearly show that the HI saturation limit of \${\textbackslash}approx 9\$ M\$\_\{{\textbackslash}odot\}\$ pc\${\textasciicircum}\{-2\}\$ reported in the literature for other galaxies is not an intrinsic property of M 33 - it is systematically introduced as an artefact of spatially smoothing the data.},
	number = {1},
	urldate = {2019-12-03},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Elson, E. C. and Kam, S. Z. and Chemin, L. and Carignan, C. and Jarrett, T. H.},
	month = feb,
	year = {2019},
	note = {arXiv: 1811.04590},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {931--946},
	file = {arXiv.org Snapshot:/Users/Tobin/Zotero/storage/5FSK6X6I/1811.html:text/html;arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/76T27XWP/Elson et al. - 2019 - A Multi-Scale Study of Star Formation in Messier 3.pdf:application/pdf},
}

@article{ford_herschel_2013,
	title = {\textit{{HERSCHEL}} {EXPLOITATION} {OF} {LOCAL} {GALAXY} {ANDROMEDA} ({HELGA}). {III}. {THE} {STAR} {FORMATION} {LAW} {IN} {M31}},
	volume = {769},
	issn = {0004-637X, 1538-4357},
	url = {http://stacks.iop.org/0004-637X/769/i=1/a=55?key=crossref.9a5d8cced58917c669e60ab76c128c61},
	doi = {10.1088/0004-637X/769/1/55},
	abstract = {We present a detailed study of how the star formation rate (SFR) relates to the interstellar medium (ISM) of M31 at \~{}140 pc scales. The SFR is calculated using the far-ultraviolet and 24 $\mu$m emission, corrected for the old stellar population in M31. We find a global value for the SFR of 0.25+-00..0064 M yr-1 and compare this with the SFR found using the total far-infrared luminosity. There is general agreement in regions where young stars dominate the dust heating. Atomic hydrogen (H i) and molecular gas (traced by carbon monoxide, CO) or the dust mass is used to trace the total gas in the ISM. We show that the global surface densities of SFR and gas mass place M31 among a set of low-SFR galaxies in the plot of Kennicutt. The relationship between SFR and gas surface density is tested in six radial annuli across M31, assuming a power law relationship with index, N. The star formation (SF) law using total gas traced by H i and CO gives a global index of N = 2.03 {\textpm} 0.04, with a significant variation with radius; the highest values are observed in the 10 kpc ring. We suggest that this slope is due to H i turning molecular at $\Sigma$Gas \~{} 10 M pc-2. When looking at H2 regions, we measure a higher mean SFR suggesting a better spatial correlation between H2 and SF. We find N \~{} 0.6 with consistent results throughout the disk{\textemdash}this is at the low end of values found in previous work and argues against a superlinear SF law on small scales.},
	language = {en},
	number = {1},
	urldate = {2019-11-11},
	journal = {The Astrophysical Journal},
	author = {Ford, George P. and Gear, Walter K. and Smith, Matthew W. L. and Eales, Steve A. and Baes, Maarten and Bendo, George J. and Boquien, M{\'e}d{\'e}ric and Boselli, Alessandro and Cooray, Asantha R. and De Looze, Ilse and Fritz, Jacopo and Gentile, Gianfranco and Gomez, Haley L. and Gordon, Karl D. and Kirk, Jason and Lebouteiller, Vianney and O'Halloran, Brian and Spinoglio, Luigi and Verstappen, Joris and Wilson, Christine D.},
	month = may,
	year = {2013},
	pages = {55},
	file = {Ford et al. - 2013 - iHERSCHELi EXPLOITATION OF LOCAL GALAXY ANDRO.pdf:/Users/Tobin/Zotero/storage/2FAC8EUX/Ford et al. - 2013 - iHERSCHELi EXPLOITATION OF LOCAL GALAXY ANDRO.pdf:application/pdf},
}

@article{gao_star_2004,
	title = {The {Star} {Formation} {Rate} and {Dense} {Molecular} {Gas} in {Galaxies}},
	volume = {606},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2004ApJ...606..271G/abstract},
	doi = {10.1086/382999},
	abstract = {HCN luminosity is a tracer of dense molecular gas, n(H{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater})\&gt;{\textasciitilde}3{\texttimes}10{\textless}SUP{\textgreater}4{\textless}/SUP{\textgreater}cm{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater}, associated with star-forming giant molecular cloud (GMC) cores. We present the results and analysis of our survey of HCN emission from 65 infrared galaxies, including nine ultraluminous infrared galaxies (ULIGs, L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}\&gt;{\textasciitilde}10{\textless}SUP{\textgreater}12{\textless}/SUP{\textgreater}L{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}), 22 luminous infrared galaxies (LIGs, 10{\textless}SUP{\textgreater}11{\textless}/SUP{\textgreater}L{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}\&lt;L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}\&lt;{\textasciitilde}10{\textless}SUP{\textgreater}12{\textless}/SUP{\textgreater}L{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}), and 34 normal spiral galaxies with lower IR luminosity (most are large spiral galaxies). We have measured the global HCN line luminosity, and the observations are reported in Paper I. This paper analyzes the relationships between the total far-IR luminosity (a tracer of the star formation rate), the global HCN line luminosity (a measure of the total dense molecular gas content), and the CO luminosity (a measure of the total molecular content). We find a tight linear correlation between the IR and HCN luminosities L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater} and L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater} (in the log-log plot) with a correlation coefficient R=0.94, and an almost constant average ratio L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater}=900L{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}(Kkms{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}pc{\textless}SUP{\textgreater}2{\textless}/SUP{\textgreater}){\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}. The IR-HCN linear correlation is valid over 3 orders of magnitude including ULIGs, the most luminous objects in the local universe. The direct consequence of the linear IR-HCN correlation is that the star formation law in terms of dense molecular gas content has a power-law index of 1.0. The global star formation rate is linearly proportional to the mass of dense molecular gas in normal spiral galaxies, LIGs, and ULIGs. This is strong evidence in favor of star formation as the power source in ultraluminous galaxies since the star formation in these galaxies appears to be normal and expected given their high mass of dense star-forming molecular gas. {\textless}P /{\textgreater}The HCN-CO correlation is also much tighter than the IR-CO correlation. We suggest that the nonlinear correlation between L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater} and L{\textless}SUB{\textgreater}CO{\textless}/SUB{\textgreater} may be a consequence of the stronger and perhaps more physical correlations between L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater} and L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater} and between L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater} and L{\textless}SUB{\textgreater}CO{\textless}/SUB{\textgreater}. Thus, the star formation rate indicated by L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater} depends on the amount of dense molecular gas traced by HCN emission, not the total molecular gas traced by CO emission. One of the main arguments in favor of an active galactic nucleus (AGN) as the power source in ULIGs is the anomalously high ratio L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/L{\textless}SUB{\textgreater}CO{\textless}/SUB{\textgreater} or L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/M(H{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater}) or high star formation rate per M{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater} of gas, compared with that from normal spiral galaxies. This has been interpreted as indicating that a dust-enshrouded AGN is required to produce the very high luminosity. Viewed in terms of the dense gas mass the situation is completely different. The ratio L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater} or L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/M{\textless}SUB{\textgreater}dense{\textless}/SUB{\textgreater}, a measure of the star formation rate per solar mass of dense gas, is essentially the same in all galaxies including ULIGs. The ratio L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/M{\textless}SUB{\textgreater}dense{\textless}/SUB{\textgreater} is virtually independent of galaxy luminosity and on average L{\textless}SUB{\textgreater}IR{\textless}/SUB{\textgreater}/M{\textless}SUB{\textgreater}dense{\textless}/SUB{\textgreater}{\textasciitilde}90L{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}/M{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}, about the same as in GMC cores but much higher than in GMCs. We find that ULIGs simply have a large quantity of dense molecular gas and thus produce a prodigious starburst that heats the dust, produces the IR, and blocks all or most optical radiation. The HCN global luminosity may be used as an indicator of the star formation rate in high-redshift objects including hyperluminous galaxies. {\textless}P /{\textgreater}The HCN/CO ratio is an indicator of the dense molecular gas fraction and gauges the globally averaged molecular gas density. We find that the HCN/CO ratio is a powerful starburst indicator. All galaxies in our sample with a high dense gas mass fraction indicated by L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater}/L{\textless}SUB{\textgreater}CO{\textless}/SUB{\textgreater}\&gt;0.06 are LIGs or ULIGs. Normal spirals all have similar and low dense gas fractions L{\textless}SUB{\textgreater}HCN{\textless}/SUB{\textgreater}/L{\textless}SUB{\textgreater}CO{\textless}/SUB{\textgreater}=0.02-0.05. The global star formation efficiency depends on the fraction of the molecular gas in a dense phase.},
	language = {en},
	number = {1},
	urldate = {2019-12-03},
	journal = {ApJ},
	author = {Gao, Yu and Solomon, Philip M.},
	month = may,
	year = {2004},
	pages = {271--290},
	file = {Snapshot:/Users/Tobin/Zotero/storage/INH7VZQ2/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/4QARNW8Z/Gao and Solomon - 2004 - The Star Formation Rate and Dense Molecular Gas in.pdf:application/pdf},
}

@article{hammer_milky_2007,
	title = {The {Milky} {Way}, an {Exceptionally} {Quiet} {Galaxy}: {Implications} for the {Formation} of {Spiral} {Galaxies}},
	volume = {662},
	issn = {0004-637X, 1538-4357},
	shorttitle = {The {Milky} {Way}, an {Exceptionally} {Quiet} {Galaxy}},
	url = {http://stacks.iop.org/0004-637X/662/i=1/a=322},
	doi = {10.1086/516727},
	language = {en},
	number = {1},
	urldate = {2019-11-11},
	journal = {The Astrophysical Journal},
	author = {Hammer, F. and Puech, M. and Chemin, L. and Flores, H. and Lehnert, M. D.},
	month = jun,
	year = {2007},
	pages = {322--334},
	file = {Hammer et al. - 2007 - The Milky Way, an Exceptionally Quiet Galaxy Impl.pdf:/Users/Tobin/Zotero/storage/F4VNDM9A/Hammer et al. - 2007 - The Milky Way, an Exceptionally Quiet Galaxy Impl.pdf:application/pdf},
}

@article{heyer_molecular_2004,
	title = {The {Molecular} {Gas} {Distribution} and {Schmidt} {Law} in {M33}},
	volume = {602},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2004ApJ...602..723H/abstract},
	doi = {10.1086/381196},
	abstract = {The relationship between the star formation rate and surface density of neutral gas within the disk of M33 is examined with new imaging observations of {\textless}SUP{\textgreater}12{\textless}/SUP{\textgreater}CO J=1-0 emission gathered with the Five College Radio Astronomy Observatory (FCRAO) 14 m telescope and IRAS HiRes images of the 60 and 100 $\mu$m emission. The Schmidt law, $\Sigma${\textless}SUB{\textgreater}SFR{\textless}/SUB{\textgreater}{\textasciitilde}$\Sigma${\textless}SUP{\textgreater}n{\textless}/SUP{\textgreater}{\textless}SUB{\textgreater}gas{\textless}/SUB{\textgreater}, is constructed using radial profiles of the H I 21 cm, CO, and far-infrared emission. We identify a strong correlation between the star formation rate and molecular gas surface density. This suggests that the condensation of giant molecular clouds (GMCs) is the limiting step to star formation within the M33 disk. The corresponding molecular Schmidt index, n{\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater}, is 1.36+/-0.08. The star formation rate has a steep dependence on total mass gas surface density, ($\Sigma${\textless}SUB{\textgreater}HI{\textless}/SUB{\textgreater}+$\Sigma${\textless}SUB{\textgreater}H{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater}{\textless}/SUB{\textgreater}), owing to the shallow radial profile of the atomic gas that dominates the total gas surface density for most radii. The disk pressure of the gas is shown to play a prominent role in regulating the molecular gas fraction in M33.},
	language = {en},
	number = {2},
	urldate = {2019-12-03},
	journal = {ApJ},
	author = {Heyer, Mark H. and Corbelli, Edvige and Schneider, Stephen E. and Young, Judith S.},
	month = feb,
	year = {2004},
	pages = {723--729},
	file = {Snapshot:/Users/Tobin/Zotero/storage/JFQJ2ABG/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/WSGRYG9B/Heyer et al. - 2004 - The Molecular Gas Distribution and Schmidt Law in .pdf:application/pdf},
}

@article{kennicutt_rate_1983,
	title = {The rate of star formation in normal disk galaxies.},
	volume = {272},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/1983ApJ...272...54K/abstract},
	doi = {10.1086/161261},
	abstract = {Photometry of the integrated H$\alpha$ emission in a large sample of field spiral and irregular galaxies has been used to obtain quantitative estimates of the total star formation rate (SFR) in the galaxies. The photoionization properties of a stellar population have been modeled for a variety of choices for the initial mass function (IMF). Excellent agreement with the observed galaxy colors and H$\alpha$ emission is obtained with models using an IMF slope close to Salpeter's original value. The extinction-corrected star formation rates are large, as high as 20 M\_sun; yr{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} in giant Sc galaxies. The current rates in late-type galaxies are comparable to the past rates averaged over the age of the disk. Little evidence is found for a strong correlation between the SFR and average gas density. Comparison of the present SFRs with the remaining supply of interstellar gas yields consumption time scales of only a few times 10{\textless}SUP{\textgreater}9{\textless}/SUP{\textgreater} years in most cases.},
	language = {en},
	urldate = {2019-12-02},
	journal = {ApJ},
	author = {Kennicutt, R. C.},
	month = sep,
	year = {1983},
	pages = {54--67},
	file = {Snapshot:/Users/Tobin/Zotero/storage/JBNCJ97V/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/KQYMHAKF/Kennicutt - 1983 - The rate of star formation in normal disk galaxies.pdf:application/pdf},
}

@article{lewis_spatially-resolved_2015,
	title = {The spatially-resolved recent star formation history of {M31}},
	volume = {225},
	url = {https://ui.adsabs.harvard.edu/abs/2015AAS...22542902L/abstract},
	abstract = {We present the spatially-resolved star formation history (SFH) of the Andromeda Galaxy (M31) based on imaging of resolved stellar populations as part of the Panchromatic Hubble Andromeda Treasury (PHAT). We have gridded the survey into {\textasciitilde}9000 regions that are {\textasciitilde}100 pc x 100 pc in projected size. Treating each region independently, we model the optical color-magnitude diagrams and measure the SFHs over the past 400-600 Myr. We combine the individual SFHs to create maps of star formation (SF) across a contiguous 1/3 of M31's star forming disk, providing an unprecedented perspective on patterns of star formation in an Lstar galaxy. Our maps clearly recover M31's famous ringed structures and reveal that the 5 and 15 kpc rings formed within the last {\textasciitilde}250 Myr and are transient in nature. In contrast, the 10 kpc ring appears to be long-lived (\&gt;500 Myr), with some evidence for broadening of the ring and dispersion of stars into the stellar disk over the accessible lookback time. It also dominates the global recent SF; the majority of the total stellar mass budget within the last {\textasciitilde}500 Myr comes from the 10 kpc ring. Our global SFH of M31 is roughly constant over the last {\textasciitilde}500 Myr, with a notable peak 50 Myr ago and a shallow decline toward the present. Extrapolating our SFH to the entire disk, we find that the SFR of M31 over the most recent 100 Myr is {\textasciitilde}0.8 Msun/yr. {\textless}P /{\textgreater}},
	language = {en},
	urldate = {2019-12-03},
	journal = {AAS},
	author = {Lewis, Alexia and Dalcanton, Julianne and Collaboration, Phat},
	month = jan,
	year = {2015},
	pages = {429.02},
	file = {Snapshot:/Users/Tobin/Zotero/storage/TERW2AKL/abstract.html:text/html},
}

@article{miller_initial_1979,
	title = {The {Initial} {Mass} {Function} and {Stellar} {Birthrate} in the {Solar} {Neighborhood}},
	volume = {41},
	issn = {0067-0049},
	url = {https://ui.adsabs.harvard.edu/abs/1979ApJS...41..513M/abstract},
	doi = {10.1086/190629},
	abstract = {The paper examines the initial mass function (IMF) and time history of the stellar birthrate in the solar neighborhood under the assumption of a time-independent IMF over the lifetime of the galactic disk. All relevant observational quantities and the associated uncertainties are discussed. Also discussed are IMFs derived for a range of birthrate histories consistent with the continuity constraint. Finally, the study summarizes observational and theoretical arguments concerning the basic assumptions that the IMF is time independent and a continuous function of mass.},
	language = {en},
	urldate = {2019-12-03},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Miller, G. E. and Scalo, J. M.},
	month = nov,
	year = {1979},
	pages = {513},
	file = {Snapshot:/Users/Tobin/Zotero/storage/4NC9ZXNF/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/4MSCAI2S/Miller and Scalo - 1979 - The Initial Mass Function and Stellar Birthrate in.pdf:application/pdf},
}

@article{putman_disruption_2009,
	title = {{THE} {DISRUPTION} {AND} {FUELING} {OF} {M33}},
	volume = {703},
	issn = {0004-637X, 1538-4357},
	url = {http://stacks.iop.org/0004-637X/703/i=2/a=1486?key=crossref.cb7a565f78f38f08031d0a169c052de3},
	doi = {10.1088/0004-637X/703/2/1486},
	language = {en},
	number = {2},
	urldate = {2019-11-11},
	journal = {The Astrophysical Journal},
	author = {Putman, M. E. and Peek, J. E. G. and Muratov, A. and Gnedin, O. Y. and Hsu, W. and Douglas, K. A. and Heiles, C. and Stanimirovic, S. and Korpela, E. J. and Gibson, S. J.},
	month = oct,
	year = {2009},
	pages = {1486--1501},
	file = {Putman et al. - 2009 - THE DISRUPTION AND FUELING OF M33.pdf:/Users/Tobin/Zotero/storage/7XYX55UQ/Putman et al. - 2009 - THE DISRUPTION AND FUELING OF M33.pdf:application/pdf},
}

@book{schneider_extragalactic_2006,
	address = {Berlin ; New York},
	title = {Extragalactic astronomy and cosmology: an introduction},
	isbn = {978-3-540-33174-2},
	shorttitle = {Extragalactic astronomy and cosmology},
	language = {en},
	publisher = {Springer},
	author = {Schneider, P.},
	year = {2006},
	note = {OCLC: ocm74270145},
	keywords = {Astronomy, Cosmology, Evolution, Expanding universe, Galaxies},
	file = {Schneider - 2006 - Extragalactic astronomy and cosmology an introduc.pdf:/Users/Tobin/Zotero/storage/RC8Q6INM/Schneider - 2006 - Extragalactic astronomy and cosmology an introduc.pdf:application/pdf},
}

@article{tepper-garcia_andromeda_2019,
	title = {The {Andromeda} {System}: {A} new orbital history and its implications},
	shorttitle = {The {Andromeda} {System}},
	url = {https://ui.adsabs.harvard.edu/abs/2019arXiv191111911T/abstract},
	abstract = {We revisit the orbital history of the Triangulum galaxy (M33) around the Andromeda galaxy (M31) in view of the recent Gaia Data Release 2 proper motion measurements for both Local Group galaxies. Earlier studies consider highly idealized dynamical friction, but neglect the effects of dynamical mass loss. We show the latter process to be important using orbit integrations and N-body simulations, which are mutually consistent. Contrary to previous claims that only a `first infall' is supported by the data, we find an orbital solution that brings these galaxies to within {\textasciitilde}50 kpc of each other in the past, i.e. {\textasciitilde}6.5 Gyr ago. We explore the implications of this finding using a N-body/hydrodynamical simulation to model the infall of M33 into M31 with a focus on the origin of two prominent features of this system: 1) M31's metal-rich Giant Stellar Stream; and 2) the M31-M33 HI filament. We find that the tidal interaction does not produce a stellar structure reminiscent of the stellar stream that survives up to the present day. The observed, outer disc warp in M33 may well be a relic of this past interaction. Similarly, the HI filament is likely a fossil structure dating back to the time of the ancient encounter between these galaxies. Our model implies the existence of a much larger, diffuse gas stream, the `Triangulum stream', that extends from M33 away from M31. We anticipate upcoming observations with the recently commissioned, Five-hundred-meter Aperture Spherical radio Telescope (FAST) that will target the putative stream in its first years of operation.},
	language = {en},
	urldate = {2019-12-03},
	journal = {arXiv},
	author = {Tepper-Garc{\'i}a, Thor and Bland-Hawthorn, Joss and Li, Di},
	month = nov,
	year = {2019},
	pages = {arXiv:1911.11911},
	file = {Snapshot:/Users/Tobin/Zotero/storage/A9BQBX4B/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/SUBKA56N/Tepper-Garc{\'i}a et al. - 2019 - The Andromeda System A new orbital history and it.pdf:application/pdf},
}

@article{van_der_marel_first_2019,
	title = {First {Gaia} {Dynamics} of the {Andromeda} {System}: {DR2} {Proper} {Motions}, {Orbits}, and {Rotation} of {M31} and {M33}},
	volume = {872},
	issn = {0004-637X},
	shorttitle = {First {Gaia} {Dynamics} of the {Andromeda} {System}},
	url = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872...24V/abstract},
	doi = {10.3847/1538-4357/ab001b},
	abstract = {The 3D velocities of M31 and M33 are important for understanding the evolution and cosmological context of the Local Group. Their most massive stars are detected by Gaia, and we use Data Release 2 (DR2) to determine the galaxy proper motions (PMs). We select galaxy members based on, e.g., parallax, PM, color-magnitude diagram location, and local stellar density. The PM rotation of both galaxies is confidently detected, consistent with the known line-of-sight rotation curves: \{V\vphantom{\{}\}{\textless}SUB{\textgreater}rot{\textless}/SUB{\textgreater}\}=-206+/- 86 \{km\} \{\{\{s\}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} (counterclockwise) for M31, and \{V\vphantom{\{}\}{\textless}SUB{\textgreater}rot{\textless}/SUB{\textgreater}\}=80 +/- 52 \{km\} \{\{\{s\}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} (clockwise) for M33. We measure the center-of-mass PM of each galaxy relative to surrounding background quasars in DR2. This yields that (\{$\mu$ \}{\textless}SUB{\textgreater}$\alpha$ * {\textless}/SUB{\textgreater},\{$\mu$ \}{\textless}SUB{\textgreater}$\delta$ {\textless}/SUB{\textgreater}) equals (65+/- 18,-57+/- 15) $\mu$ \{as\} \{yr\vphantom{\{}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} for M31 and (31+/- 19,-29+/- 16) $\mu$ \{as\} \{yr\vphantom{\{}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} for M33. In addition to the listed random errors, each component has an additional residual systematic error of 16 $\mu$ \{as\} \{yr\vphantom{\{}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}. These results are consistent at 0.8$\sigma$ and 1.0$\sigma$ with the (2 and 3 times higher accuracy) measurements already available from Hubble Space Telescope (HST) optical imaging and Very Long Baseline Array water maser observations, respectively. This lends confidence that all these measurements are robust. The new results imply that the M31 orbit toward the Milky Way (MW) is somewhat less radial than previously inferred, \{V\}{\textless}SUB{\textgreater}{\textbackslash}tan ,\{DR{\textless}/SUB{\textgreater}2+\{HST\}\}=\{57\}{\textless}SUB{\textgreater}-31{\textless}/SUB{\textgreater}{\textless}SUP{\textgreater}+35{\textless}/SUP{\textgreater} \{km\} \{\{\{s\}\}\}{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}, and strengthen arguments that M33 may be on its first infall into M31. The results highlight the future potential of Gaia for PM studies beyond the MW satellite system.},
	language = {en},
	number = {1},
	urldate = {2019-12-04},
	journal = {ApJ},
	author = {van der Marel, Roeland P. and Fardal, Mark A. and Sohn, Sangmo Tony and Patel, Ekta and Besla, Gurtina and del Pino, Andr{\'e}s and Sahlmann, Johannes and Watkins, Laura L.},
	month = feb,
	year = {2019},
	pages = {24},
	file = {Snapshot:/Users/Tobin/Zotero/storage/XH5564TF/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/S74GM888/van der Marel et al. - 2019 - First Gaia Dynamics of the Andromeda System DR2 P.pdf:application/pdf},
}

@article{williams_recent_2003,
	title = {The {Recent} {Star} {Formation} {History} of the {M31} {Disk}},
	volume = {126},
	issn = {0004-6256, 1538-3881},
	url = {http://stacks.iop.org/1538-3881/126/i=3/a=1312},
	doi = {10.1086/377347},
	abstract = {The star formation history of the northern and southern M31 disk is measured using samples of BV photometry for 40 {\^A} 40 regions taken from the KPNO/CTIO Local Group Survey. The distances, mean reddening values, and age distributions of the stars in these regions were measured using the routines of Dolphin. Independent measurements of overlapping fields show that the results are stable for most samples. A slight distance gradient is seen across the major axis of the southern disk, and a mean distance of 24:47 {\AE} 0:03 is found by combining the results. Higher mean reddening values are seen to follow the spiral structure. The stellar age distributions are consistent with episodic star formation confined mainly to the gas-rich arm regions. If these episodes were caused by propagating density waves, the waves did not cause significant star formation episodes in the gas-poor interarm regions. A combination of all of the results provides the total star formation rate for 1.4 deg2 of the M31 disk for six epochs. These results suggest that star formation in the disk declined by \$50\% from \$250 to \$50 Myr ago. The lowest star formation rate occurred \$25 Myr ago, followed by a \$20\% increase to the present. The mean star formation rate for this large portion of M31 over the past 60 Myr is 0:63 {\AE} 0:07 M  yr{\`A}1, suggesting a total mean rate for the disk of \$1 M  yr{\`A}1.},
	language = {en},
	number = {3},
	urldate = {2019-11-11},
	journal = {The Astronomical Journal},
	author = {Williams, Benjamin F.},
	month = sep,
	year = {2003},
	pages = {1312--1325},
	file = {Williams - 2003 - The Recent Star Formation History of the M31 Disk.pdf:/Users/Tobin/Zotero/storage/FRUSAAAC/Williams - 2003 - The Recent Star Formation History of the M31 Disk.pdf:application/pdf},
}

@article{williams_star_2018,
	title = {The star formation law at {GMC} scales in {M33}, the {Triangulum} galaxy},
	volume = {479},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479..297W/abstract},
	doi = {10.1093/mnras/sty1476},
	abstract = {We present a high spatial resolution study, on scales of ?100 pc, of the relationship between star formation rate (SFR) and gas content within Local Group galaxy M33. Combining deep SCUBA-2 observations with archival GALEX, SDSS, WISE, Spitzer, and submillimetre Herschel data, we are able to model the entire SED from UV to sub-mm wavelengths. We calculate the SFR on a pixel-by-pixel basis using the total infrared luminosity, and find a total SFR of 0.17 {\textpm} 0.06 \{M\}\_? yr{\textless}SUP{\textgreater}-{\textless}/SUP{\textgreater}{\textless}SUP{\textgreater}1{\textless}/SUP{\textgreater}, somewhat lower than our other two measures of SFR - combined FUV and 24$\mu$m SFR (0.25{\textasciicircum}\{+0.10\}\_\{-0.07\} \{M\}\_? yr{\textless}SUP{\textgreater}-{\textless}/SUP{\textgreater}{\textless}SUP{\textgreater}1{\textless}/SUP{\textgreater}) and SED-fitting tool MAGPHYS (0.33{\textasciicircum}\{+0.05\}\_\{-0.06\} \{M\}\_? yr{\textless}SUP{\textgreater}-{\textless}/SUP{\textgreater}{\textless}SUP{\textgreater}1{\textless}/SUP{\textgreater}). We trace the total gas using a combination of the 21cm H I line for atomic hydrogen, and CO(J=2-1) data for molecular hydrogen. We have also traced the total gas using dust masses. We study the star formation law in terms of molecular gas, total gas, and gas from dust. We perform an analysis of the star formation law on a variety of pixel scales, from 25 arcsec to 500 arcsec (100 pc to 2 kpc). At kpc scales, we find that a linear Schmidt-type power law index is suitable for molecular gas, but the index appears to be much higher with total gas, and gas from dust. Whilst we find a strong scale dependence on the Schmidt index, the gas depletion time-scale is invariant with pixel scale. {\textless}P /{\textgreater}},
	language = {en},
	number = {1},
	urldate = {2019-12-03},
	journal = {MNRAS},
	author = {Williams, Thomas G. and Gear, Walter K. and Smith, Matthew W. L.},
	month = sep,
	year = {2018},
	pages = {297--314},
	file = {Snapshot:/Users/Tobin/Zotero/storage/EX99ZT6X/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/2CIHRDGJ/Williams et al. - 2018 - The star formation law at GMC scales in M33, the T.pdf:application/pdf},
}

@article{regan_near-infrared_1994,
	title = {The near-infrared structure of {M33}},
	volume = {434},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/1994ApJ...434..536R},
	doi = {10.1086/174755},
	abstract = {We present near-infrared mosaics of J, H, and K emission from the central 15 min x 30 min in M33 which map the stellar distribution of its disk and spheroidal components. Detailed examination of individual OB associations and population synthesis models show that recent massive star formation contributes significantly to near infrared emission, which must be considered in deriving the stellar mass distribution. The scale length of the exponential disk is less than 6 min, shorter than optical scale lengths in part because of a radial gradient in
extinction. We identify two grand-design spiral arms with an underlying stellar component in the inner 9 min; these terminate near the radius at which the rotation curve begins to flatten. A weak, bar-shaped excess in the stellar mass distribution is present in the inner 1.5 min; it is unclear whether this traces the inward extension of the spiral arms or a true bar. We find the spheroidal light is reasonably fitted by a single r1/4 distribution with a scale length much longer than previously reported for the central spheroidal component. Including a compact bulgelike component does not significantly improve the fit to the surface photometry indicating that the contribution of a compact bulge component to the spherodial light must be very low. In previous studies of M33, the ratio of the number of globular clusters to spheroid luminosity was anomalously high. Our more extended spheroid results in a ratio closer to that obtained for other spiral galaxies, although it is still high.},
	urldate = {2021-03-03},
	journal = {The Astrophysical Journal},
	author = {Regan, Michael W. and Vogel, Stuart N.},
	month = oct,
	year = {1994},
	keywords = {Galactic Structure, Astronomical Photometry, Error Analysis, Galactic Halos, Globular Clusters, Infrared Astronomy, Infrared Imagery, Luminosity, Mass Distribution, Spiral Galaxies, Star Formation, Supergiant Stars},
	pages = {536--545},
}

@article{regan_near-infrared_1994-1,
	title = {The near-infrared structure of {M33}},
	volume = {434},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/1994ApJ...434..536R},
	doi = {10.1086/174755},
	abstract = {We present near-infrared mosaics of J, H, and K emission from the central 15 min x 30 min in M33 which map the stellar distribution of its disk and spheroidal components. Detailed examination of individual OB associations and population synthesis models show that recent massive star formation contributes significantly to near infrared emission, which must be considered in deriving the stellar mass distribution. The scale length of the exponential disk is less than 6 min, shorter than optical scale lengths in part because of a radial gradient in
extinction. We identify two grand-design spiral arms with an underlying stellar component in the inner 9 min; these terminate near the radius at which the rotation curve begins to flatten. A weak, bar-shaped excess in the stellar mass distribution is present in the inner 1.5 min; it is unclear whether this traces the inward extension of the spiral arms or a true bar. We find the spheroidal light is reasonably fitted by a single r1/4 distribution with a scale length much longer than previously reported for the central spheroidal component. Including a compact bulgelike component does not significantly improve the fit to the surface photometry indicating that the contribution of a compact bulge component to the spherodial light must be very low. In previous studies of M33, the ratio of the number of globular clusters to spheroid luminosity was anomalously high. Our more extended spheroid results in a ratio closer to that obtained for other spiral galaxies, although it is still high.},
	urldate = {2021-03-03},
	journal = {The Astrophysical Journal},
	author = {Regan, Michael W. and Vogel, Stuart N.},
	month = oct,
	year = {1994},
	keywords = {Galactic Structure, Astronomical Photometry, Error Analysis, Galactic Halos, Globular Clusters, Infrared Astronomy, Infrared Imagery, Luminosity, Mass Distribution, Spiral Galaxies, Star Formation, Supergiant Stars},
	pages = {536--545},
}

@article{cook_star_2019,
	title = {Star {Cluster} {Catalogs} for the {LEGUS} {Dwarf} {Galaxies}},
	volume = {484},
	issn = {0035-8711, 1365-2966},
	url = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.4897C/abstract},
	doi = {10.1093/mnras/stz331},
	abstract = {We present the star cluster catalogs for 17 dwarf and irregular galaxies in the \$HST\$ Treasury Program "Legacy ExtraGalactic UV Survey" (LEGUS). Cluster identification and photometry in this subsample are similar to that of the entire LEGUS sample, but special methods were developed to provide robust catalogs with accurate fluxes due to low cluster statistics. The colors and ages are largely consistent for two widely used aperture corrections, but a significant fraction of the clusters are more compact than the average training cluster. However, the ensemble luminosity, mass, and age distributions are consistent suggesting that the systematics between the two methods are less than the random errors. When compared with the clusters from previous dwarf galaxy samples, we find that the LEGUS catalogs are more complete and provide more accurate total fluxes. Combining all clusters into a composite dwarf galaxy, we find that the luminosity and mass functions can be described by a power law with the canonical index of \$-2\$ independent of age and global SFR binning. The age distribution declines as a power law, with an index of \${\textbackslash}approx-0.80{\textbackslash}pm0.15\$, independent of cluster mass and global SFR binning. This decline of clusters is dominated by cluster disruption since the combined star formation histories and integrated-light SFRs are both approximately constant over the last few hundred Myr. Finally, we find little evidence for an upper-mass cutoff (\${\textless}2{\textbackslash}sigma\$) in the composite cluster mass function, and can rule out a truncation mass below \${\textbackslash}approx10{\textasciicircum}\{4.5\}\$M\$\_\{{\textbackslash}odot\}\$ but cannot rule out the existence of a truncation at higher masses.},
	number = {4},
	urldate = {2021-03-09},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Cook, D. O. and Lee, J. C. and Adamo, A. and Kim, H. and Chandar, R. and Whitmore, B. C. and Mok, A. and Ryon, J. E. and Dale, D. A. and Calzetti, D. and Andrews, J. E. and Aloisi, A. and Ashworth, G. and Bright, S. N. and Brown, T. M. and Christian, C. and Cignoni, M. and Clayton, G. C. and da Silva, R. and de Mink, S. E. and Dobbs, C. L. and Elmegreen, B. G. and Elmegreen, D. M. and Evans, A. S. and Fumagalli, M. and Gallagher III, J. S. and Gouliermis, D. A. and Grasha, K. and Grebel, E. K. and Herrero, A. and Hunter, D. A. and Jensen, E. I. and Johnson, K. E. and Kahre, L. and Kennicutt, R. C. and Krumholz, M. R. and Lee, N. J. and Lennon, D. and Linden, S. and Martin, C. and Messa, M. and Nair, P. and Nota, A. and Ostlin, G. and Parziale, R. C. and Pellerin, A. and Regan, M. W. and Sabbi, E. and Sacchi, E. and Schaerer, D. and Schiminovich, D. and Shabani, F. and Slane, F. A. and Small, J. and Smith, C. L. and Smith, L. J. and Taibi, S. and Thilker, D. A. and de la Torre, I. C. and Tosi, M. and Turner, J. A. and Ubeda, L. and Van Dyk, S. D. and Walterbos, R. A. M. and Wofford, A.},
	month = apr,
	year = {2019},
	note = {arXiv: 1902.00082},
	keywords = {Astrophysics - Astrophysics of Galaxies},
	pages = {4897--4919},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/QIJR744I/Cook et al. - 2019 - Star Cluster Catalogs for the LEGUS Dwarf Galaxies.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/2B9KMYCM/1902.html:text/html},
}

@article{kroupa_initial_2002,
	title = {The {Initial} {Mass} {Function} of {Stars}: {Evidence} for {Uniformity} in {Variable} {Systems}},
	volume = {295},
	issn = {00368075, 10959203},
	shorttitle = {The {Initial} {Mass} {Function} of {Stars}},
	url = {https://ui.adsabs.harvard.edu/abs/2002Sci...295...82K/abstract},
	doi = {10.1126/science.1067524},
	abstract = {The distribution of stellar masses that form in one star-formation event in a given volume of space is called the initial mass function (IMF). The IMF has been estimated from low-mass brown dwarfs to very massive stars. Combining IMF estimates for different populations in which the stars can be observed individually unveils an extraordinary uniformity of the IMF. This general insight appears to hold for populations including present-day star formation in small molecular clouds, rich and dense massive star-clusters forming in giant clouds, through to ancient and metal-poor exotic stellar populations that may be dominated by dark matter. This apparent universality of the IMF is a challenge for star formation theory because elementary considerations suggest that the IMF ought to systematically vary with star-forming conditions.},
	number = {5552},
	urldate = {2021-03-10},
	journal = {Science},
	author = {Kroupa, Pavel},
	month = jan,
	year = {2002},
	note = {arXiv: astro-ph/0201098},
	keywords = {Astrophysics},
	pages = {82--91},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/AY3U2CSV/Kroupa - 2002 - The Initial Mass Function of Stars Evidence for U.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/YRS4LP44/0201098.html:text/html},
}

@article{dalcanton_panchromatic_2012,
	title = {The {Panchromatic} {Hubble} {Andromeda} {Treasury}},
	volume = {200},
	issn = {0067-0049, 1538-4365},
	url = {https://ui.adsabs.harvard.edu/abs/2012ApJS..200...18D/abstract},
	doi = {10.1088/0067-0049/200/2/18},
	abstract = {The Panchromatic Hubble Andromeda Treasury (PHAT) is an on-going HST Multicycle Treasury program to image {\textasciitilde}1/3 of M31's star forming disk in 6 filters, from the UV to the NIR. The full survey will resolve the galaxy into more than 100 million stars with projected radii from 0-20 kpc over a contiguous 0.5 square degree area in 828 orbits, producing imaging in the F275W and F336W filters with WFC3/UVIS, F475W and F814W with ACS/WFC, and F110W and F160W with WFC3/IR. The resulting wavelength coverage gives excellent constraints on stellar temperature, bolometric luminosity, and extinction for most spectral types. The photometry reaches SNR=4 at F275W=25.1, F336W=24.9, F475W=27.9, F814W=27.1, F110W=25.5, and F160W=24.6 for single pointings in the uncrowded outer disk; however, the optical and NIR data are crowding limited, and the deepest reliable magnitudes are up to 5 magnitudes brighter in the inner bulge. All pointings are dithered and produce Nyquist-sampled images in F475W, F814W, and F160W. We describe the observing strategy, photometry, astrometry, and data products, along with extensive tests of photometric stability, crowding errors, spatially-dependent photometric biases, and telescope pointing control. We report on initial fits to the structure of M31's disk, derived from the density of RGB stars, in a way that is independent of the assumed M/L and is robust to variations in dust extinction. These fits also show that the 10 kpc ring is not just a region of enhanced recent star formation, but is instead a dynamical structure containing a significant overdensity of stars with ages {\textgreater}1 Gyr. (Abridged)},
	number = {2},
	urldate = {2021-03-12},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Dalcanton, J. J. and Williams, B. F. and Lang, D. and Lauer, T. R. and Kalirai, J. S. and Seth, A. C. and Dolphin, A. and Rosenfield, P. and Weisz, D. R. and Bell, E. F. and Bianchi, L. C. and Boyer, M. L. and Caldwell, N. and Dong, H. and Dorman, C. E. and Gilbert, K. M. and Girardi, L. and Gogarten, S. M. and Gordon, K. D. and Guhathakurta, P. and Hodge, P. W. and Holtzman, J. A. and Johnson, L. and Larsen, S. S. and Lewis, A. and Melbourne, J. L. and Olsen, K. A. G. and Rix, H.-W. and Rosema, K. and Saha, A. and Sarajedini, A. and Skillman, E. D. and Stanek, K. Z.},
	month = jun,
	year = {2012},
	note = {arXiv: 1204.0010},
	keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
	pages = {18},
	file = {arXiv Fulltext PDF:/Users/Tobin/Zotero/storage/JVBTAKQX/Dalcanton et al. - 2012 - The Panchromatic Hubble Andromeda Treasury.pdf:application/pdf;arXiv.org Snapshot:/Users/Tobin/Zotero/storage/LVQQGLY8/1204.html:text/html},
}

@article{king_structure_1962,
	title = {The structure of star clusters. {I}. an empirical density law},
	volume = {67},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/1962AJ.....67..471K},
	doi = {10.1086/108756},
	abstract = {Abstract image available at: 
http://adsabs.harvard.edu/abs/1962AJ.....67..471K},
	urldate = {2021-03-12},
	journal = {The Astronomical Journal},
	author = {King, Ivan},
	month = oct,
	year = {1962},
	pages = {471},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/IFVN8IGI/King - 1962 - The structure of star clusters. I. an empirical de.pdf:application/pdf},
}

@article{dolphin_wfpc2_2000,
	title = {{WFPC2} {Stellar} {Photometry} with {HSTPHOT}},
	volume = {112},
	issn = {0004-6280},
	url = {http://adsabs.harvard.edu/abs/2000PASP..112.1383D},
	doi = {10.1086/316630},
	abstract = {HSTphot, a photometry package designed to handle the undersampled point-spread functions (PSFs) found in WFPC2 images, is introduced and described, as well as some of the considerations that have to be made in order to obtain accurate PSF-fitting stellar photometry with WFPC2 data. Tests of HSTphot's internal reliability are made using multiple
observations of the same field, and tests of external reliability are made by comparisons with DoPHOT reductions of the same data.},
	urldate = {2021-03-12},
	journal = {Publications of the Astronomical Society of the Pacific},
	author = {Dolphin, Andrew E.},
	month = oct,
	year = {2000},
	keywords = {Techniques: Photometric},
	pages = {1383--1396},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/D6HV3WXX/Dolphin - 2000 - WFPC2 Stellar Photometry with HSTPHOT.pdf:application/pdf},
}

@article{kharchenko_global_2013,
	title = {Global survey of star clusters in the {Milky} {Way}. {II}. {The} catalogue of basic parameters},
	volume = {558},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2013A%26A...558A..53K},
	doi = {10.1051/0004-6361/201322302},
	abstract = {Context. Although they are the main constituents of the Galactic disk 
population, for half of the open clusters in the Milky Way reported in
the literature nothing is known except the raw position and an
approximate size. Aims: The main goal of this study is to
determine a full set of uniform spatial, structural, kinematic, and
astrophysical parameters for as many known open clusters as possible.
 Methods: On the basis of stellar data from PPMXL and 2MASS, we
used a dedicated data-processing pipeline to determine kinematic and
photometric membership probabilities for stars in a cluster region. Results: For an input list of 3784 targets from the literature, we
confirm that 3006 are real objects, the vast majority of them are open
clusters, but associations and globular clusters are also present. For
each confirmed object we determined the exact position of the cluster
centre, the apparent size, proper motion, distance, colour excess, and
age. For about 1500 clusters, these basic astrophysical parameters have
been determined for the first time. For the bulk of the clusters we also
derived the tidal radius. We estimated additionally average radial
velocities for more than 30\% of the confirmed clusters. The present
sample (called MWSC) reaches both the central parts of the Milky Way and
its outer regions. It is almost complete up to 1.8 kpc from the Sun and
also covers neighbouring spiral arms. However, for a small subset of the
oldest open clusters (log t ? 9) we found some evidence of
incompleteness within about 1 kpc from the Sun.

The MWSC survey is only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr
(ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/558/A53},
	urldate = {2021-03-13},
	journal = {Astronomy and Astrophysics},
	author = {Kharchenko, N. V. and Piskunov, A. E. and Schilbach, E. and R{\"o}ser, S. and Scholz, R.-D.},
	month = oct,
	year = {2013},
	keywords = {open clusters and associations: general, galaxies: star clusters: general, globular clusters: general, galaxies: fundamental parameters, galaxies: photometry, Galaxy: stellar content},
	pages = {A53},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/SCXJ8S78/Kharchenko et al. - 2013 - Global survey of star clusters in the Milky Way. I.pdf:application/pdf},
}

@article{kharchenko_global_2013-1,
	title = {Global survey of star clusters in the {Milky} {Way}. {II}. {The} catalogue of basic parameters},
	volume = {558},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2013A%26A...558A..53K},
	doi = {10.1051/0004-6361/201322302},
	abstract = {Context. Although they are the main constituents of the Galactic disk 
population, for half of the open clusters in the Milky Way reported in
the literature nothing is known except the raw position and an
approximate size. Aims: The main goal of this study is to
determine a full set of uniform spatial, structural, kinematic, and
astrophysical parameters for as many known open clusters as possible.
 Methods: On the basis of stellar data from PPMXL and 2MASS, we
used a dedicated data-processing pipeline to determine kinematic and
photometric membership probabilities for stars in a cluster region. Results: For an input list of 3784 targets from the literature, we
confirm that 3006 are real objects, the vast majority of them are open
clusters, but associations and globular clusters are also present. For
each confirmed object we determined the exact position of the cluster
centre, the apparent size, proper motion, distance, colour excess, and
age. For about 1500 clusters, these basic astrophysical parameters have
been determined for the first time. For the bulk of the clusters we also
derived the tidal radius. We estimated additionally average radial
velocities for more than 30\% of the confirmed clusters. The present
sample (called MWSC) reaches both the central parts of the Milky Way and
its outer regions. It is almost complete up to 1.8 kpc from the Sun and
also covers neighbouring spiral arms. However, for a small subset of the
oldest open clusters (log t ? 9) we found some evidence of
incompleteness within about 1 kpc from the Sun.

The MWSC survey is only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr
(ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/558/A53},
	urldate = {2021-03-18},
	journal = {Astronomy and Astrophysics},
	author = {Kharchenko, N. V. and Piskunov, A. E. and Schilbach, E. and R{\"o}ser, S. and Scholz, R.-D.},
	month = oct,
	year = {2013},
	keywords = {open clusters and associations: general, galaxies: star clusters: general, globular clusters: general, galaxies: fundamental parameters, galaxies: photometry, Galaxy: stellar content},
	pages = {A53},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/GC33JMMH/Kharchenko et al. - 2013 - Global survey of star clusters in the Milky Way. I.pdf:application/pdf},
}

@article{usher_sluggs_2019,
	title = {The {SLUGGS} survey: measuring globular cluster ages using both photometry and spectroscopy},
	volume = {490},
	issn = {0035-8711},
	shorttitle = {The {SLUGGS} survey},
	url = {http://adsabs.harvard.edu/abs/2019MNRAS.490..491U},
	doi = {10.1093/mnras/stz2596},
	abstract = {Globular cluster ages provide both an important test of models of 
globular cluster formation and a powerful method to constrain the
assembly history of galaxies. Unfortunately, measuring the ages of
unresolved old stellar populations has proven challenging. Here, we
present a novel technique that combines optical photometry with
metallicity constraints from near-infrared spectroscopy in order to
measure ages. After testing the method on globular clusters in the Milky
Way and its satellite galaxies, we apply our technique to three massive
early-type galaxies using data from the SAGES Legacy Unifying Globulars
and GalaxieS (SLUGGS) survey. The three SLUGGS galaxies and the Milky
Way show dramatically different globular cluster age and metallicity
distributions, with NGC 1407 and the Milky Way showing mostly old
globular clusters, while NGC 3115 and NGC 3377 show a range of globular
ages. This diversity implies different galaxy formation histories and
that the globular cluster optical colour-metallicity relation is not
universal as is commonly assumed in globular cluster studies. We find a
correlation between the median age of the metal-rich globular cluster
populations and the age of the field star populations, in line with
models where globular cluster formation is a natural outcome of
high-intensity star formation.},
	urldate = {2021-03-18},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Usher, Christopher and Brodie, Jean P. and Forbes, Duncan A. and Romanowsky, Aaron J. and Strader, Jay and Pfeffer, Joel and Bastian, Nate},
	month = nov,
	year = {2019},
	keywords = {galaxies: star clusters: general, galaxies: stellar content, galaxies: evolution, globular clusters: general},
	pages = {491--501},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/PNSFEU5N/Usher et al. - 2019 - The SLUGGS survey measuring globular cluster ages.pdf:application/pdf},
}

@article{schiavon_library_2005,
	title = {A {Library} of {Integrated} {Spectra} of {Galactic} {Globular} {Clusters}},
	volume = {160},
	issn = {0067-0049},
	url = {http://adsabs.harvard.edu/abs/2005ApJS..160..163S},
	doi = {10.1086/431148},
	abstract = {We present a new library of integrated spectra of 40 Galactic globular clusters, obtained with the Blanco 4 m telescope and the R-C
spectrograph at the Cerro Tololo Inter-American Observatory. The spectra cover the range {\textasciitilde}3350-6430 {\r A} with {\textasciitilde}3.1 {\r A} (FWHM) resolution.
The spectroscopic observations and data reduction were designed to integrate the full projected area within the cluster core radii in order to properly sample the light from stars in all relevant evolutionary stages. The S/N values of the flux-calibrated spectra range from 50 to 240 {\r A}-1 at 4000 {\r A} and from 125 to 500
{\r A}-1 at 5000 {\r A}. The selected targets span a wide
range of cluster parameters, including metallicity, horizontal-branch morphology, Galactic coordinates, Galactocentric distance, and
concentration. The total sample is thus fairly representative of the entire Galactic globular cluster population and should be valuable for comparison with similar integrated spectra of unresolved stellar populations in remote systems. For most of the library clusters, our spectra can be coupled with deep color-magnitude diagrams and reliable metal abundances from the literature to enable the calibration of stellar population synthesis models. In this paper we present a detailed account of the observations and data reduction. The spectral library is publicly available in electronic format from the National Optical Astronomical Observatory Web site.},
	urldate = {2021-03-18},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Schiavon, Ricardo P. and Rose, James A. and Courteau, St{\'e}phane and MacArthur, Lauren A.},
	month = sep,
	year = {2005},
	keywords = {Galaxies: Evolution, Galaxy: Globular Clusters: General},
	pages = {163--175},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/4XALJ46I/Schiavon et al. - 2005 - A Library of Integrated Spectra of Galactic Globul.pdf:application/pdf},
}

@article{harris_catalog_1996,
	title = {A {Catalog} of {Parameters} for {Globular} {Clusters} in the {Milky} {Way}},
	volume = {112},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/1996AJ....112.1487H},
	doi = {10.1086/118116},
	abstract = {A database of parameters for globular star clusters in the Milky Way is described which is available in electronic form through the
WorldWideWeb. The information in the catalog includes up-to-date measurements for cluster distance, reddening, luminosity, colors and spectral types, velocity, structural and dynamical parameters,
horizontal branch morphology, metallicity, and other quantities. This catalog will be updated regularly and maintained in electronic form for widest possible accessibility.},
	urldate = {2021-03-18},
	journal = {The Astronomical Journal},
	author = {Harris, William E.},
	month = oct,
	year = {1996},
	keywords = {CATALOGS, GLOBULAR CLUSTERS: GENERAL},
	pages = {1487},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/PGU79D8V/Harris - 1996 - A Catalog of Parameters for Globular Clusters in t.pdf:application/pdf},
}

@article{huang_tess_2018,
	title = {{TESS} {Discovery} of a {Transiting} {Super}-{Earth} in the pi {Mensae} {System}},
	volume = {868},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2018ApJ...868L..39H},
	doi = {10.3847/2041-8213/aaef91},
	abstract = {We report the detection of a transiting planet around $\pi$ Men (HD 39091), using data from the Transiting Exoplanet Survey Satellite (TESS). The solar-type host star is unusually bright (V = 5.7) and was already known to host a Jovian planet on a highly eccentric, 5.7 yr orbit. The newly discovered planet has a size of 2.04 {\textpm} 0.05 R
(+) and an orbital period of 6.27 days. Radial-velocity data from the High-Accuracy Radial-velocity Planet Searcher and
Anglo-Australian Telescope/University College London Echelle
Spectrograph archives also displays a 6.27 day periodicity, confirming the existence of the planet and leading to a mass determination of 4.82 {\textpm} 0.85 M (+). The star{\textquoteright}s proximity and
brightness will facilitate further investigations, such as atmospheric spectroscopy, asteroseismology, the Rossiter-McLaughlin effect,
astrometry, and direct imaging.},
	urldate = {2021-03-18},
	journal = {The Astrophysical Journal Letters},
	author = {Huang, Chelsea X. and Burt, Jennifer and Vanderburg, Andrew and G{\"u}nther, Maximilian N. and Shporer, Avi and Dittmann, Jason A. and Winn, Joshua N. and Wittenmyer, Rob and Sha, Lizhou and Kane, Stephen R. and Ricker, George R. and Vanderspek, Roland K. and Latham, David W. and Seager, Sara and Jenkins, Jon M. and Caldwell, Douglas A. and Collins, Karen A. and Guerrero, Natalia and Smith, Jeffrey C. and Quinn, Samuel N. and Udry, St{\'e}phane and Pepe, Francesco and Bouchy, Fran{\c c}ois and S{\'e}gransan, Damien and Lovis, Christophe and Ehrenreich, David and Marmier, Maxime and Mayor, Michel and Wohler, Bill and Haworth, Kari and Morgan, Edward H. and Fausnaugh, Michael and Ciardi, David R. and Christiansen, Jessie and Charbonneau, David and Dragomir, Diana and Deming, Drake and Glidden, Ana and Levine, Alan M. and McCullough, P. R. and Yu, Liang and Narita, Norio and Nguyen, Tam and Morton, Tim and Pepper, Joshua and P{\'a}l, Andr{\'a}s and Rodriguez, Joseph E. and Stassun, Keivan G. and Torres, Guillermo and Sozzetti, Alessandro and Doty, John P. and Christensen-Dalsgaard, J{\o}rgen and Laughlin, Gregory and Clampin, Mark and Bean, Jacob L. and Buchhave, Lars A. and Bakos, G. {\'A}. and Sato, Bun'ei and Ida, Shigeru and Kaltenegger, Lisa and Palle, Enric and Sasselov, Dimitar and Butler, R. P. and Lissauer, Jack and Ge, Jian and Rinehart, S. A.},
	month = dec,
	year = {2018},
	keywords = {planetary systems, planets and satellites: detection, stars: individual: HD 39091, TIC 261136679},
	pages = {L39},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/CMPD9UZD/Huang et al. - 2018 - TESS Discovery of a Transiting Super-Earth in the .pdf:application/pdf},
}

@article{conroy_complete_2018,
	title = {A {Complete} {Census} of {Luminous} {Stellar} {Variability} on {Day} to {Decade} {Timescales}},
	volume = {864},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2018ApJ...864..111C},
	doi = {10.3847/1538-4357/aad460},
	abstract = {Stellar photometric variability offers a novel probe of the interior structure and evolutionary state of stars. Here we present a census of stellar variability on day to decade timescales across the
color-magnitude diagram (CMD) for 73,000 stars brighter than M
I,814 = -5 in the Whirlpool Galaxy (M51). Our Cycle 24 Hubble Space Telescope (HST) program acquired V 606- and I 814-band images over 34 epochs spanning 1 year with
pseudo-random cadences enabling sensitivity to periods from days to months. We supplement these data with archival V- and I-band HST data obtained in 1995 and 2005, providing sensitivity to variability on decade timescales. At least 50\% of stars brighter than M
I,814 = -7 show strong evidence for variability within our Cycle 24 data; among stars with
\{V\}606-\{I\}814{\textgreater} 2 the variability fraction rises to ?100\%. Large amplitude variability ({\textgreater}0.3 mag) on decade
timescales is restricted to red supergiants (RSGs) and very luminous blue stars. Both populations display fairly smooth variability on month-year timescales. The Cepheid instability strip is clearly visible in our data, although the variability fraction within this region never exceeds ?10\%. The location of variable stars across the CMD broadly agrees with theoretical sources of variability, including the
instability strip, RSG pulsational instabilities, long-period
fundamental mode pulsations, and radiation-dominated envelopes in massive stars. Our data can be used to place stringent constraints on the precise onset of these various instabilities and their lifetimes and growth rates.},
	urldate = {2021-03-18},
	journal = {The Astrophysical Journal},
	author = {Conroy, Charlie and Strader, Jay and van Dokkum, Pieter and Dolphin, Andrew E. and Weisz, Daniel R. and Murphy, Jeremiah W. and Dotter, Aaron and Johnson, Benjamin D. and Cargile, Phillip},
	month = sep,
	year = {2018},
	keywords = {galaxies: individual: NGC 5194, stars: variables: general},
	pages = {111},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/UI7F2E57/Conroy et al. - 2018 - A Complete Census of Luminous Stellar Variability .pdf:application/pdf},
}

@article{poovelil_open_2020,
	title = {Open {Cluster} {Chemical} {Homogeneity} throughout the {Milky} {Way}},
	volume = {903},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2020ApJ...903...55P},
	doi = {10.3847/1538-4357/abb93e},
	abstract = {The chemical homogeneity of surviving stellar clusters contains important clues about interstellar medium (ISM) mixing efficiency, star formation, and the enrichment history of the Galaxy. Existing
measurements in a handful of open clusters suggest homogeneity in several elements at the 0.03 dex level. Here we present (i) a new cluster member catalog based only on APOGEE radial velocities and Gaia-DR2 proper motions, (ii) improved abundance uncertainties for APOGEE cluster members, and (iii) the dependence of cluster homogeneity on Galactic and cluster properties, using abundances of eight elements from the APOGEE survey for 10 high-quality clusters. We find that cluster homogeneity is uncorrelated with Galactocentric distance,   \${\textbar} Z{\textbar} \$ , age, and metallicity. However, velocity dispersion, which is a proxy for cluster mass, is positively correlated with intrinsic scatter at relatively high levels of significance for [Ca/Fe] and [Mg/Fe]. We also see a possible positive correlation at a low level of significance for [Ni/Fe], [Si/Fe], [Al/Fe], and [Fe/H], while [Cr/Fe] and [Mn/Fe] are uncorrelated. The elements that show a correlation with velocity dispersion are those that are predominantly produced by core-collapse supernovae (CCSNe). However, the small sample size and relatively low correlation significance highlight the need for follow-up studies. If borne out by future studies, these findings would suggest a quantitative difference between the correlation lengths of elements produced
predominantly by Type Ia SNe versus CCSNe, which would have implications for Galactic chemical evolution models and the feasibility of chemical tagging.},
	urldate = {2021-03-18},
	journal = {The Astrophysical Journal},
	author = {Poovelil, Vijith Jacob and Zasowski, G. and Hasselquist, S. and Seth, A. and Donor, John and Beaton, Rachael L. and Cunha, K. and Frinchaboy, Peter M. and Garc{\'i}a-Hern{\'a}ndez, D. A. and Hawkins, K. and Kratter, K. M. and Lane, Richard R. and Nitschelm, C.},
	month = nov,
	year = {2020},
	keywords = {1052, 1567, 224, 225, Chemical abundances, Chemical enrichment, Milky Way evolution, Star clusters},
	pages = {55},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/6IMEPZWR/Poovelil et al. - 2020 - Open Cluster Chemical Homogeneity throughout the M.pdf:application/pdf},
}

@article{dragomir_tess_2019,
	title = {{TESS} {Delivers} {Its} {First} {Earth}-sized {Planet} and a {Warm} {Sub}-{Neptune}},
	volume = {875},
	issn = {2041-8205},
	url = {https://doi.org/10.3847/2041-8213/ab12ed},
	doi = {10.3847/2041-8213/ab12ed},
	abstract = {The future of exoplanet science is bright, as Transiting Exoplanet Survey Satellite (TESS) once again demonstrates with the discovery of its longest-period confirmed planet to date. We hereby present HD 21749b (TOI 186.01), a sub-Neptune in a 36 day orbit around a bright (V = 8.1) nearby (16 pc) K4.5 dwarf. TESS measures HD 21749b to be R(+), and combined archival and follow-up precision radial velocity data put the mass of the planet at M(+). HD 21749b contributes to the TESS Level 1 Science Requirement of providing 50 transiting planets smaller than 4 R(+) with measured masses. Furthermore, we report the discovery of HD 21749c (TOI 186.02), the first Earth-sized () planet from TESS. The HD 21749 system is a prime target for comparative studies of planetary composition and architecture in multi-planet systems.},
	language = {en},
	number = {2},
	urldate = {2021-03-18},
	journal = {The Astrophysical Journal},
	author = {Dragomir, Diana and Teske, Johanna and G{\"u}nther, Maximilian N. and S{\'e}gransan, Damien and Burt, Jennifer A. and Huang, Chelsea X. and Vanderburg, Andrew and Matthews, Elisabeth and Dumusque, Xavier and Stassun, Keivan G. and Pepper, Joshua and Ricker, George R. and Vanderspek, Roland and Latham, David W. and Seager, Sara and Winn, Joshua N. and Jenkins, Jon M. and Beatty, Thomas and Bouchy, Fran{\c c}ois and Brown, Timothy M. and Butler, R. Paul and Ciardi, David R. and Crane, Jeffrey D. and Eastman, Jason D. and Fossati, Luca and Francis, Jim and Fulton, Benjamin J. and Gaudi, B. Scott and Goeke, Robert F. and James, David and Klaus, Todd C. and Kuhn, Rudolf B. and Lovis, Christophe and Lund, Michael B. and McDermott, Scott and Paegert, Martin and Pepe, Francesco and Rodriguez, Joseph E. and Sha, Lizhou and Shectman, Stephen A. and Shporer, Avi and Siverd, Robert J. and Soto, Aylin Garcia and Stevens, Daniel J. and Twicken, Joseph D. and Udry, St{\'e}phane and Villanueva, Steven and Wang, Sharon X. and Wohler, Bill and Yao, Xinyu and Zhan, Zhuchang},
	month = apr,
	year = {2019},
	note = {Publisher: American Astronomical Society},
	pages = {L7},
	file = {IOP Full Text PDF:/Users/Tobin/Zotero/storage/J3WJJJ3R/Dragomir et al. - 2019 - TESS Delivers Its First Earth-sized Planet and a W.pdf:application/pdf},
}

@article{noeske_star_2007,
	title = {Star {Formation} in {AEGIS} {Field} {Galaxies} since z=1.1: {The} {Dominance} of {Gradually} {Declining} {Star} {Formation}, and the {Main} {Sequence} of {Star}-forming {Galaxies}},
	volume = {660},
	issn = {0004-637X},
	shorttitle = {Star {Formation} in {AEGIS} {Field} {Galaxies} since z=1.1},
	url = {http://adsabs.harvard.edu/abs/2007ApJ...660L..43N},
	doi = {10.1086/517926},
	abstract = {We analyze star formation (SF) as a function of stellar mass 
(M*) and redshift z in the All-Wavelength Extended Groth
Strip International Survey. For 2905 field galaxies, complete to
1010(1010.8) Msolar at z{\textless}0.7(1),
with Keck spectroscopic redshifts out to z=1.1, we compile SF rates
(SFRs) from emission lines, GALEX, and Spitzer MIPS 24 $\mu$m photometry,
optical-NIR M* measurements, and HST morphologies. Galaxies
with reliable signs of SF form a distinct ``main sequence'' (MS), with a
limited range of SFRs at a given M* and z (1
$\sigma${\textless}{\textasciitilde}+/-0.3 dex), and log(SFR) approximately proportional to
logM*. The range of log(SFR) remains constant to z{\textgreater}1,
while the MS as a whole moves to higher SFR as z increases. The range of
the SFR along the MS constrains the amplitude of episodic variations of
SF and the effect of mergers on the SFR. Typical galaxies spend
{\textasciitilde}67\%(95\%) of their lifetime since z=1 within a factor of {\textless}{\textasciitilde}2(4) of
their average SFR at a given M* and z. The dominant mode of
the evolution of SF since z{\textasciitilde}1 is apparently a gradual decline of the
average SFR in most individual galaxies, not a decreasing frequency of
starburst episodes, or a decreasing factor by which SFRs are enhanced in
starbursts. LIRGs at z{\textasciitilde}1 seem to mostly reflect the high SFR typical for
massive galaxies at that epoch. The smooth MS may reflect that the same
set of few physical processes governs SF prior to additional quenching
processes. A gradual process like gas exhaustion may play a dominant
role.},
	urldate = {2021-03-23},
	journal = {The Astrophysical Journal Letters},
	author = {Noeske, K. G. and Weiner, B. J. and Faber, S. M. and Papovich, C. and Koo, D. C. and Somerville, R. S. and Bundy, K. and Conselice, C. J. and Newman, J. A. and Schiminovich, D. and Le Floc'h, E. and Coil, A. L. and Rieke, G. H. and Lotz, J. M. and Primack, J. R. and Barmby, P. and Cooper, M. C. and Davis, M. and Ellis, R. S. and Fazio, G. G. and Guhathakurta, P. and Huang, J. and Kassin, S. A. and Martin, D. C. and Phillips, A. C. and Rich, R. M. and Small, T. A. and Willmer, C. N. A. and Wilson, G.},
	month = may,
	year = {2007},
	keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: High-Redshift, Galaxies: Starburst},
	pages = {L43--L46},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/NYPTGPQ5/Noeske et al. - 2007 - Star Formation in AEGIS Field Galaxies since z=1.1.pdf:application/pdf},
}

@article{kennicutt_star_2012,
	title = {Star {Formation} in the {Milky} {Way} and {Nearby} {Galaxies}},
	volume = {50},
	issn = {0066-4146},
	url = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..531K},
	doi = {10.1146/annurev-astro-081811-125610},
	abstract = {We review progress over the past decade in observations of large-scale star formation, with a focus on the interface between extragalactic and Galactic studies. Methods of measuring gas contents and star-formation rates are discussed, and updated prescriptions for calculating
star-formation rates are provided. We review relations between star formation and gas on scales ranging from entire galaxies to individual molecular clouds.},
	urldate = {2021-03-23},
	journal = {Annual Review of Astronomy and Astrophysics},
	author = {Kennicutt, Robert C. and Evans, Neal J.},
	month = sep,
	year = {2012},
	pages = {531--608},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/J72MN5V4/Kennicutt and Evans - 2012 - Star Formation in the Milky Way and Nearby Galaxie.pdf:application/pdf},
}

@article{salim_uv_2007,
	title = {{UV} {Star} {Formation} {Rates} in the {Local} {Universe}},
	volume = {173},
	issn = {0067-0049},
	url = {http://adsabs.harvard.edu/abs/2007ApJS..173..267S},
	doi = {10.1086/519218},
	abstract = {We measure star formation rates (SFRs) of {\textasciitilde}50,000 optically selected galaxies in the local universe (z{\textasciitilde}0.1)-from gas-rich dwarfs to massive ellipticals. We obtain dust-corrected SFRs by fitting the GALEX
(ultraviolet) and SDSS photometry to a library of dust-attenuated population synthesis models. For star-forming galaxies, our UV-based SFRs compare remarkably well with those from SDSS-measured emission lines (H$\alpha$). Deviations from perfect agreement are shown to be due to differences in the dust attenuation estimates. In contrast to H$\alpha$ measurements, UV provides reliable SFRs for galaxies with weak H$\alpha$, and where H$\alpha$ is contaminated with AGN emission (1/2 of
the sample). Using full-SED SFRs, we calibrate a simple prescription that uses GALEX far- and near-UV magnitudes to produce dust-corrected SFRs for normal star-forming galaxies. The specific SFR is considered as a function of stellar mass for (1) star-forming galaxies with no AGNs, (2) those hosting an AGN, and (3) galaxies without H$\alpha$ emission. We find that the three have distinct star formation histories, with AGNs lying intermediate between the star-forming and the quiescent galaxies. Star-forming galaxies without an AGN lie on a relatively narrow linear sequence. Remarkably, galaxies hosting a strong AGN appear to represent the massive continuation of this sequence. On the other hand, weak AGNs, while also massive, have lower SFRs, sometimes extending to the realm of quiescent galaxies. We propose an evolutionary sequence for massive galaxies that smoothly connects normal star-forming galaxies to
quiescent galaxies via strong and weak AGNs. We confirm that some galaxies with no H$\alpha$ show signs of star formation in the UV. We
derive a cosmic star formation density at z=0.1 with significantly smaller total error than previous measurements.},
	urldate = {2021-03-23},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Salim, Samir and Rich, R. Michael and Charlot, St{\'e}phane and Brinchmann, Jarle and Johnson, Benjamin D. and Schiminovich, David and Seibert, Mark and Mallery, Ryan and Heckman, Timothy M. and Forster, Karl and Friedman, Peter G. and Martin, D. Christopher and Morrissey, Patrick and Neff, Susan G. and Small, Todd and Wyder, Ted K. and Bianchi, Luciana and Donas, Jos{\'e} and Lee, Young-Wook and Madore, Barry F. and Milliard, Bruno and Szalay, Alex S. and Welsh, Barry Y. and Yi, Sukyoung K.},
	month = dec,
	year = {2007},
	keywords = {Galaxies: Evolution, Galaxies: Active, Galaxies: Fundamental Parameters, Surveys, Ultraviolet: Galaxies},
	pages = {267--292},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/L8TF42WC/Salim et al. - 2007 - UV Star Formation Rates in the Local Universe.pdf:application/pdf},
}

@article{williams_detection_2009,
	title = {The {Detection} of {Inside}-{Out} {Disk} {Growth} in {M33}},
	volume = {695},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2009ApJ...695L..15W},
	doi = {10.1088/0004-637X/695/1/L15},
	abstract = {We present resolved stellar photometry of four fields along the major axis of the M33 disk from images taken with the Advanced Camera for Surveys aboard the Hubble Space Telescope. The photometry provides a detailed census of the red clump in all fields and reaches the ancient main sequence in the outermost field. Through detailed modeling of the color-magnitude diagrams, we find that the percentage of the stellar mass formed prior to z = 1 changes from 71 {\textpm} 9\% in the innermost field to 16 {\textpm} 6\% in the outermost field. The disk shows a clear
trend of increasing scale length with time, evolving from rs = 1.0 {\textpm} 0.1 kpc 10 Gyr ago to rs = 1.8 {\textpm} 0.1 at
times more recent than 5 Gyr ago, in agreement with analytical
predictions for disk growth. Beyond the disk truncation radius, however, the stellar density profile steepens with time and the age gradient reverses, in agreement with recent simulations. The late and slow growth of the stellar disk may be due in part to the low mass of M33.},
	urldate = {2021-03-23},
	journal = {The Astrophysical Journal Letters},
	author = {Williams, Benjamin F. and Dalcanton, Julianne J. and Dolphin, Andrew E. and Holtzman, Jon and Sarajedini, Ata},
	month = apr,
	year = {2009},
	keywords = {galaxies: spiral, galaxies: individual: M33, galaxies: evolution},
	pages = {L15--L19},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/YJKHU5UW/Williams et al. - 2009 - The Detection of Inside-Out Disk Growth in M33.pdf:application/pdf},
}

@article{lee_comparison_2009,
	title = {Comparison of {H$\alpha$} and {UV} {Star} {Formation} {Rates} in the {Local} {Volume}: {Systematic} {Discrepancies} for {Dwarf} {Galaxies}},
	volume = {706},
	issn = {0004-637X},
	shorttitle = {Comparison of {H$\alpha$} and {UV} {Star} {Formation} {Rates} in the {Local} {Volume}},
	url = {http://adsabs.harvard.edu/abs/2009ApJ...706..599L},
	doi = {10.1088/0004-637X/706/1/599},
	abstract = {Using a complete sample of {\textasciitilde}300 star-forming galaxies within 11 Mpc of 
the Milky Way, we evaluate the consistency between star formation rates
(SFRs) inferred from the far ultraviolet (FUV) non-ionizing continuum
and H$\alpha$ nebular emission, assuming standard conversion recipes in
which the SFR scales linearly with luminosity at a given wavelength. Our
analysis probes SFRs over 5 orders of magnitude, down to ultra-low
activities on the order of {\textasciitilde}10-4 M sun
yr-1. The data are drawn from the 11 Mpc H$\alpha$ and
Ultraviolet Galaxy Survey (11HUGS), which has obtained H$\alpha$ fluxes
from ground-based narrowband imaging, and UV fluxes from imaging with
GALEX. For normal spiral galaxies (SFR {\textasciitilde} 1 M sun
yr-1), our results are consistent with previous work which
has shown that FUV SFRs tend to be lower than H$\alpha$ SFRs before
accounting for internal dust attenuation, but that there is relative
consistency between the two tracers after proper corrections are
applied. However, a puzzle is encountered at the faint end of the
luminosity function. As lower luminosity dwarf galaxies, roughly less
active than the Small Magellanic Cloud, are examined, H$\alpha$ tends to
increasingly underpredict the total SFR relative to the FUV. The trend
is evident prior to corrections for dust attenuation, which affects the
FUV more than the nebular H$\alpha$ emission, so this general conclusion
is robust to the effects of dust. Although past studies have suggested
similar trends, this is the first time this effect is probed with a
statistical sample for galaxies with SFR {\textless}{\textasciitilde} 0.1 M sun
yr-1. By SFR {\textasciitilde} 0.003 M sun yr-1, the
average H$\alpha$-to-FUV flux ratio is lower than expected by a factor of
two, and at the lowest SFRs probed, the ratio exhibits an order of
magnitude discrepancy for the handful of galaxies that remain in the
sample. A range of standard explanations does not appear to be able to
fully account for the magnitude of the systematic. Some recent work has
argued for a stellar initial mass function which is deficient in
high-mass stars in dwarf and low surface brightness galaxies, and we
also consider this scenario. Under the assumption that the FUV traces
the SFR in dwarf galaxies more robustly, the prescription relating
H$\alpha$ luminosity to SFR is re-calibrated for use in the low SFR
regime when FUV data are not available.},
	urldate = {2021-03-23},
	journal = {The Astrophysical Journal},
	author = {Lee, Janice C. and Gil de Paz, Armando and Tremonti, Christy and Kennicutt, Jr., Robert C. and Salim, Samir and Bothwell, Matthew and Calzetti, Daniela and Dalcanton, Julianne and Dale, Daniel and Engelbracht, Chad and Funes, S. J. Jos{\'e} G. and Johnson, Benjamin and Sakai, Shoko and Skillman, Evan and van Zee, Liese and Walter, Fabian and Weisz, Daniel},
	month = nov,
	year = {2009},
	keywords = {stars: formation, galaxies: evolution, ultraviolet: galaxies, galaxies: photometry, galaxies: dwarf, surveys},
	pages = {599--613},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/CMCCZB24/Lee et al. - 2009 - Comparison of H$\alpha$ and UV Star Formation Rates in th.pdf:application/pdf},
}

@article{lintott_galaxy_2009,
	title = {Galaxy {Zoo}: `{Hanny}'s {Voorwerp}', a quasar light echo?},
	volume = {399},
	issn = {0035-8711},
	shorttitle = {Galaxy {Zoo}},
	url = {http://adsabs.harvard.edu/abs/2009MNRAS.399..129L},
	doi = {10.1111/j.1365-2966.2009.15299.x},
	abstract = {We report the discovery of an unusual object near the spiral galaxy IC2497, discovered by visual inspection of the Sloan Digital Sky Survey (SDSS) as part of the Galaxy Zoo project. The object, known as Hanny's Voorwerp, is bright in the SDSS g band due to unusually strong
[OIII]4959, 5007 emission lines. We present the results of the first targeted observations of the object in the optical, ultraviolet and X-ray, which show that the object contains highly ionized gas. Although the line ratios are similar to extended emission-line regions near luminous active galactic nucleus (AGN), the source of this ionization is not apparent. The emission-line properties, and lack of X-ray emission from IC2497, suggest either a highly obscured AGN with a novel geometry arranged to allow photoionization of the object but not the galaxy's own circumnuclear gas, or, as we argue, the first detection of a quasar light echo. In this case, either the luminosity of the central source has decreased dramatically or else the obscuration in the system has increased within 105yr. This object may thus represent the first direct probe of quasar history on these time-scales.

This publication has been made possible by the participation of more than 100000 volunteers in the Galaxy Zoo project. Their contributions are individually acknowledged at
http://www.galaxyzoo.org/Volunteers.aspx

E-mail: cjl@astro.ox.ac.uk {\textdaggerdbl}

Visiting Astronomer, Kitt Peak National Observatory, National Optical Astronomy Observatory, which is operated by the Association of
Universities for Research in Astronomy (AURA) under cooperative
agreement with the National Science Foundation.},
	urldate = {2021-03-26},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Lintott, Chris J. and Schawinski, Kevin and Keel, William and van Arkel, Hanny and Bennert, Nicola and Edmondson, Edward and Thomas, Daniel and Smith, Daniel J. B. and Herbert, Peter D. and Jarvis, Matt J. and Virani, Shanil and Andreescu, Dan and Bamford, Steven P. and Land, Kate and Murray, Phil and Nichol, Robert C. and Raddick, M. Jordan and Slosar, An{\v z}e and Szalay, Alex and Vandenberg, Jan},
	month = oct,
	year = {2009},
	keywords = {galaxies: active, galaxies: individual: IC2497, galaxies: peculiar, quasars: general},
	pages = {129--140},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/UXN95MX6/Lintott et al. - 2009 - Galaxy Zoo `Hanny's Voorwerp', a quasar light ech.pdf:application/pdf},
}

@article{girardi_acs_2010,
	title = {The {ACS} {Nearby} {Galaxy} {Survey} {Treasury}. {IX}. {Constraining} {Asymptotic} {Giant} {Branch} {Evolution} with {Old} {Metal}-poor {Galaxies}},
	volume = {724},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2010ApJ...724.1030G},
	doi = {10.1088/0004-637X/724/2/1030},
	abstract = {In an attempt to constrain evolutionary models of the asymptotic giant 
branch (AGB) phase at the limit of low masses and low metallicities, we
have examined the luminosity functions and number ratios between AGB and
red giant branch (RGB) stars from a sample of resolved galaxies from the
ACS Nearby Galaxy Survey Treasury. This database provides Hubble Space
Telescope optical photometry together with maps of completeness,
photometric errors, and star formation histories for dozens of galaxies
within 4 Mpc. We select 12 galaxies characterized by predominantly
metal-poor populations as indicated by a very steep and blue RGB, and
which do not present any indication of recent star formation in their
color-magnitude diagrams. Thousands of AGB stars brighter than the tip
of the RGB (TRGB) are present in the sample (between 60 and 400 per
galaxy), hence, the Poisson noise has little impact in our measurements
of the AGB/RGB ratio. We model the photometric data with a few sets of
thermally pulsing AGB (TP-AGB) evolutionary models with different
prescriptions for the mass loss. This technique allows us to set
stringent constraints on the TP-AGB models of low-mass, metal-poor stars
(with M {\textless} 1.5 M sun, [Fe/H]? -1.0). Indeed, those
which satisfactorily reproduce the observed AGB/RGB ratios have TP-AGB
lifetimes between 1.2 and 1.8 Myr, and finish their nuclear burning
lives with masses between 0.51 and 0.55 M sun. This is also
in good agreement with recent observations of white dwarf masses in the
M4 old globular cluster. These constraints can be added to those already
derived from Magellanic Cloud star clusters as important mileposts in
the arduous process of calibrating AGB evolutionary models.},
	urldate = {2021-03-30},
	journal = {The Astrophysical Journal},
	author = {Girardi, L{\'e}o and Williams, Benjamin F. and Gilbert, Karoline M. and Rosenfield, Philip and Dalcanton, Julianne J. and Marigo, Paola and Boyer, Martha L. and Dolphin, Andrew and Weisz, Daniel R. and Melbourne, Jason and Olsen, Knut A. G. and Seth, Anil C. and Skillman, Evan},
	month = dec,
	year = {2010},
	keywords = {stars: general},
	pages = {1030--1043},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/QZN6STR4/Girardi et al. - 2010 - The ACS Nearby Galaxy Survey Treasury. IX. Constra.pdf:application/pdf},
}

@article{dolphin_numerical_2002,
	title = {Numerical methods of star formation history measurement and applications to seven dwarf spheroidals},
	volume = {332},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2002MNRAS.332...91D},
	doi = {10.1046/j.1365-8711.2002.05271.x},
	abstract = {A comprehensive study of the measurement of star formation histories 
from colour-magnitude diagrams (CMDs) is presented, with an emphasis on
a variety of subtle issues involved in the generation of model CMDs and
maximum likelihood solution. Among these are the need for a complete
sampling of the synthetic CMD, the use of proper statistics for dealing
with Poisson-distributed data (and a demonstration of why $\chi$
2 must not be used), measuring full uncertainties in all
reported parameters, quantifying the goodness-of-fit, and questions of
binning the CMD and incorporating outside information. Several example
star formation history measurements are given. Two examples involve
synthetic data, in which the input and recovered parameters can be
compared to locate possible flaws in the methodology (none were
apparent) and measure the accuracy with which ages, metallicities and
star formation rates can be recovered. Solutions of the histories of
seven Galactic dwarf spheroidal companions (Carina, Draco, Leo I, Leo
II, Sagittarius, Sculptor and Ursa Minor) illustrate the ability to
measure star formation histories given a variety of conditions - numbers
of stars, complexity of star formation history and amount of foreground
contamination. Significant measurements of ancient {\textgreater}8Gyr star
formation are made in all seven galaxies. Sculptor, Draco and Ursa Minor
appear entirely ancient, while the other systems show varying amounts of
younger stars.},
	urldate = {2021-03-30},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Dolphin, A. E.},
	month = may,
	year = {2002},
	keywords = {galaxies: stellar content, methods: statistical, methods: numerical, Local Group},
	pages = {91--108},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7Z3NYRTQ/Dolphin - 2002 - Numerical methods of star formation history measur.pdf:application/pdf},
}

@article{chandar_star_1999,
	title = {Star {Clusters} in {M33}. {I}. {Detection}, {Morphology}, and {Photometry}},
	volume = {122},
	issn = {0067-0049},
	url = {http://adsabs.harvard.edu/abs/1999ApJS..122..431C},
	doi = {10.1086/313225},
	abstract = {In this paper we present the discovery of 60 star clusters in 20 multiband Hubble Space Telescope (HST) WFPC2 fields in M33. The fields sample a variety of environments, from outer regions to spiral arms and central regions, as well as a range of galactocentric distances. The HST spatial resolution allowed us to penetrate the crowded, spiral arm regions of M33 yielding the first unbiased, representative sample of star clusters for this galaxy. We discuss the separation of clusters from stellar sources, and from other extended sources such as
star-forming regions, H II regions, and supernova remnants. For the clusters we present multiband images and discuss morphology, location, and integrated photometry. Measured cluster colors and magnitudes are presented. The cluster density in our sample as a function of
galactocentric distance yields an estimate of 690 total clusters in M33.

Based on observations with the NASA/ESA Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555.},
	urldate = {2021-03-31},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Chandar, Rupali and Bianchi, Luciana and Ford, Holland C.},
	month = jun,
	year = {1999},
	keywords = {Galaxies: Star Clusters, GALAXIES: STAR CLUSTERS, Galaxies: Evolution, GALAXIES: EVOLUTION, Galaxies: Individual: Messier Number: M33, GALAXIES: INDIVIDUAL: MESSIER NUMBER: M33},
	pages = {431--464},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/RMWSDY43/Chandar et al. - 1999 - Star Clusters in M33. I. Detection, Morphology, an.pdf:application/pdf},
}

@article{ma_spectral_2002,
	title = {Spectral {Energy} {Distributions} and {Age} {Estimates} of 78 {Star} {Clusters} in {M33}},
	volume = {123},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/2002AJ....123.3141M},
	doi = {10.1086/340361},
	abstract = {In this third paper of our series, we present CCD spectrophotometry of 78 star clusters that were detected by Chandar, Bianchi, \& Ford in the nearby spiral galaxy M33. CCD images of M33 were obtained as a part of the BATC Multicolor Sky Survey of the sky in 13 intermediate-band filters from 3800 to 10000 {\r A}. By aperture photometry, we obtain
the spectral energy distributions of these 78 star clusters. As Chandar, Bianchi, \& Ford did, we estimate the ages of our sample clusters by comparing the photometry of each object with theoretical stellar population synthesis models for different values of metallicity. We find that the sample clusters formed continuously in M33 from
{\textasciitilde}3{\texttimes}106 to 1010 yr. This conclusion is
consistent with Chandar, Bianchi, \& Ford. The results also show that there are two peaks in cluster formation at {\textasciitilde}8{\texttimes}106 and {\textasciitilde}109 yr in these clusters.},
	urldate = {2021-03-31},
	journal = {The Astronomical Journal},
	author = {Ma, Jun and Zhou, Xu and Chen, Jiansheng and Wu, Hong and Jiang, Zhaoji and Xue, Suijian and Zhu, Jin},
	month = jun,
	year = {2002},
	keywords = {Galaxies: Star Clusters, Galaxies: Evolution, Galaxies: Individual: Messier Number: M33},
	pages = {3141--3153},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/LV4F83RC/Ma et al. - 2002 - Spectral Energy Distributions and Age Estimates of.pdf:application/pdf},
}

@article{stetson_center_1994,
	title = {The center of the core-cusp globular cluster {M15}: {CFHT} and {HST} {Observations}, {ALLFRAME} reductions},
	volume = {106},
	issn = {0004-6280},
	shorttitle = {The center of the core-cusp globular cluster {M15}},
	url = {http://adsabs.harvard.edu/abs/1994PASP..106..250S},
	doi = {10.1086/133378},
	abstract = {The central brightness cusps seen in some globular clusters are thought 
to be the relics of a gravothermal core collapse that occurred sometime
in the clusters' past. Recent observations show that the centers of such
clusters are bluer than their outskirts, indicating that the stellar
populations there are somehow different than those farther out,
presumably as a result of unusual physical processes that took place in
these extremely dense regions. Here I analyze a large body of digital
imagery from the Canada-France-Hawaii Telescope and the Hubble Space
Telescope to obtain color-magnitude and color-color diagrams for stars
in the central two arcminutes of the prototypical core-cusp globular
cluster M15 = NGC 7078 = C 2127 + 119. These data were reduced with a
new computer program, named ALLFRAME, that is described in detail here
for the first time. ALLFRAME makes simultaneous use of the geometric and
photometric information from all images of a given field to derive a
self-consistent set of positions and magnitudes for all detected
starlike objects in that area of sky, thereby extending the range of
magnitude and crowding conditions for which useful photometry is
obtainable. I tentatively conclude that the color gradient in M15 is due
to three distinct effects: (1) there is a deficiency of the brightest
red giants in the central regions of the cluster; (2) the giant branch
of the dominant cluster population shifts systematically toward the blue
as the center of the cluster is approached; and (3) the very center of
the cluster (radius approximately equal or less than 12 seconds)
contains a large population of blue and yellow stragglers that occupy
the area of the color-magnitude diagram between the main-sequence
turnoff and the horizontal branch and between the extended blue
horizontal branch and the subgiant branch; many of these appear to have
a significant ultraviolet excess.},
	urldate = {2021-03-31},
	journal = {Publications of the Astronomical Society of the Pacific},
	author = {Stetson, Peter B.},
	month = mar,
	year = {1994},
	keywords = {Astronomical Photometry, Globular Clusters, Calibrating, Color-Color Diagram, Color-Magnitude Diagram, Data Reduction, Hubble Space Telescope},
	pages = {250--280},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/ZJ8YLR8C/Stetson - 1994 - The center of the core-cusp globular cluster M15 .pdf:application/pdf},
}

@article{carrera_near-infrared_2013,
	title = {The near-infrared {Ca} {II} triplet as a metallicity indicator - {II}. {Extension} to extremely metal-poor metallicity regimes},
	volume = {434},
	issn = {0035-8711},
	url = {http://adsabs.harvard.edu/abs/2013MNRAS.434.1681C},
	doi = {10.1093/mnras/stt1126},
	abstract = {We extend our previous calibration of the infrared Ca II triplet (CaT) 
as a metallicity indicator to the metal-poor regime by including
observations of 55 field stars with [Fe/H] down to -4.0 dex. While we
previously solved the saturation at high metallicity using a combination
of a Lorentzian and a Gaussian to reproduce the line profiles, in this
paper we address the non-linearity at low metallicity following the
suggestion of Starkenburg et al. of adding two non-linear terms to the
relation among the [Fe/H], luminosity and strength of the calcium
triplet lines. Our calibration thus extends from -4.0 to +0.5 in
metallicity and is presented using four different luminosity indicators:
V - VHB, MV, MI and MK. The
calibration obtained in this paper results in a tight correlation
between [Fe/H] abundances measured from high-resolution spectra and
[Fe/H] values derived from the CaT, over the whole metallicity range
covered.},
	urldate = {2021-04-08},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Carrera, R. and Pancino, E. and Gallart, C. and del Pino, A.},
	month = sep,
	year = {2013},
	keywords = {stars: abundances, stars: late-type, techniques: spectroscopic},
	pages = {1681--1691},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/DFBIXWSS/Carrera et al. - 2013 - The near-infrared Ca II triplet as a metallicity i.pdf:application/pdf},
}

@article{castellani_rr_2003,
	title = {{RR} {Lyrae} variables in {Galactic} globular clusters. {I}. {The} observational scenario},
	volume = {410},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2003A%26A...410..871C},
	doi = {10.1051/0004-6361:20031381},
	abstract = {In this paper we revisit observational data concerning RR Lyrae stars in Galactic globular clusters, presenting frequency histograms of
fundamentalized periods for the 32 clusters having more than 12
pulsators with well recognized period and pulsation mode. One finds that the range of fundamentalized periods covered by the variables in a given cluster remains fairly constant in varying the cluster metallicity all over the metallicity range spanned by the cluster sample, with the only two exceptions given by M 15 and NGC 6441. We conclude that the width in temperature of the RR Lyrae instability strip appears largely
independent of the cluster metallicity. At the same time, it appears that the fundamentalized periods are not affected by the predicted variation of pulsators luminosity with metal abundance, indicating the occurrence of a correlated variation in the pulsator mass. We discuss mean periods in a selected sample of statistically significant ``RR rich" clusters with no less than 10 RRab and 5 RRc variables. One finds a clear evidence for the well known Oosterhoff dichotomy in the mean period of ab-type variables, together with a similarly
clear evidence for a constancy of the mean fundamentalized period in passing from Oosterhoff type II to type I clusters. On
this basis, the origin of the Oosterhoff dichotomy is discussed, presenting evidence against a strong dependence of the RR Lyrae
luminosity on the metal content. On the contrary, i) the continuity of the mean fundamentalized period, ii) the period frequency histograms in the two prototypes M 3 (type I) and M 15 (type II), iii) the relative abundance of first overtone pulsators, and iv) the observed difference between mean fundamental and fundamentalized periods
, all agree in suggesting the dominant occurrence of a
variation in the pulsation mode in a middle region of the instability strip (the ``OR" zone), where variables of Oosterhoff type I and type II clusters are pulsating in the fundamental or first overtone mode, respectively.},
	urldate = {2021-04-15},
	journal = {Astronomy and Astrophysics},
	author = {Castellani, M. and Caputo, F. and Castellani, V.},
	month = nov,
	year = {2003},
	keywords = {stars: evolution, stars: horizontal-branch, stars: variables: RR Lyr},
	pages = {871--878},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/HMHJ9PHP/Castellani et al. - 2003 - RR Lyrae variables in Galactic globular clusters. .pdf:application/pdf},
}

@article{macleod_modeling_2010,
	title = {Modeling the {Time} {Variability} of {SDSS} {Stripe} 82 {Quasars} as a {Damped} {Random} {Walk}},
	volume = {721},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2010ApJ...721.1014M},
	doi = {10.1088/0004-637X/721/2/1014},
	abstract = {We model the time variability of {\textasciitilde}9000 spectroscopically confirmed quasars in SDSS Stripe 82 as a damped random walk (DRW). Using 2.7 million photometric measurements collected over 10 yr, we confirm the results of Kelly et al. and Koz{\l }owski et al. that this model can explain quasar light curves at an impressive fidelity level (0.01-0.02 mag). The DRW model provides a simple, fast (O(N) for N data points), and powerful statistical description of quasar light curves by a characteristic timescale ($\tau$) and an asymptotic rms variability on long timescales (SF$\infty$). We searched for correlations
between these two variability parameters and physical parameters such as luminosity and black hole mass, and rest-frame wavelength. Our analysis shows SF$\infty$ to increase with decreasing luminosity and
rest-frame wavelength as observed previously, and without a correlation with redshift. We find a correlation between SF$\infty$ and
black hole mass with a power-law index of 0.18 {\textpm} 0.03,
independent of the anti-correlation with luminosity. We find that $\tau$ increases with increasing wavelength with a power-law index of 0.17, remains nearly constant with redshift and luminosity, and increases with increasing black hole mass with a power-law index of 0.21 {\textpm} 0.07. The amplitude of variability is anti-correlated with the Eddington ratio, which suggests a scenario where optical fluctuations are tied to variations in the accretion rate. However, we find an additional dependence on luminosity and/or black hole mass that cannot be explained by the trend with Eddington ratio. The radio-loudest quasars have systematically larger variability amplitudes by about 30\%, when
corrected for the other observed trends, while the distribution of their characteristic timescale is indistinguishable from that of the full sample. We do not detect any statistically robust differences in the characteristic timescale and variability amplitude between the full sample and the small subsample of quasars detected by ROSAT. Our results provide a simple quantitative framework for generating mock quasar light curves, such as currently used in LSST image simulations.},
	urldate = {2021-04-15},
	journal = {The Astrophysical Journal},
	author = {MacLeod, C. L. and Ivezi{\'c}, {\v Z}. and Kochanek, C. S. and Koz{\l }owski, S. and Kelly, B. and Bullock, E. and Kimball, A. and Sesar, B. and Westman, D. and Brooks, K. and Gibson, R. and Becker, A. C. and de Vries, W. H.},
	month = oct,
	year = {2010},
	keywords = {quasars: general},
	pages = {1014--1033},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/5NT4F7W3/MacLeod et al. - 2010 - Modeling the Time Variability of SDSS Stripe 82 Qu.pdf:application/pdf},
}

@article{de_marchi_variable_2007,
	title = {Variable stars in the open cluster {NGC} 6791 and its surrounding field},
	volume = {471},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2007A%26A...471..515D},
	doi = {10.1051/0004-6361:20077386},
	abstract = {Aims:This work presents a high-precision variability survey in the field of the old, super metal-rich open cluster NGC 6791. Methods: The data sample consists of more than 75 000 high-precision CCD time series measurements in the V band obtained mainly at the Canada-France-Hawaii Telescope, with additional data from S. Pedro M{\'a}rtir and Loiano
observatories, over a time span of ten nights. The field covers an area of 42 {\texttimes} 28 arcmin{\textasciicircum}2. Results: We have discovered 260 new
variables and re-determined periods and amplitudes of 70 known variable stars. By means of a photometric evaluation of the membership in NGC 6791, and a preliminary membership based on the proper motions, we give a full description of the variable content of the cluster and
surrounding field in the range 16? V{\textless} 23.5. Accurate periods can be given for the variables with P? 4.0 d, while for ones with longer periods the limited time-baseline hampered precise determinations. We categorized the entire sample as follows: 6 pulsating, 3 irregular, 3 cataclysmic, 89 rotational variables and 61 eclipsing systems; moreover, we detected 168 candidate variables for which we cannot give a
variability class since their periods are much longer than our time baseline. Conclusions: On the basis of photometric
considerations, and of the positions of the stars with respect to the center of the cluster, we inferred that 11 new variable stars are likely members of the cluster, for 22 stars the membership is doubtful and 137 are likely non-members. We also detected an outburst of about 3 mag in the light curve of a very faint blue star belonging to the cluster and we suggest that this star could be a new U Gem (dwarf nova) cataclysmic variable.

Appendix A is only available in electronic form at http://www.aanda.org},
	urldate = {2021-04-15},
	journal = {Astronomy and Astrophysics},
	author = {de Marchi, F. and Poretti, E. and Montalto, M. and Piotto, G. and Desidera, S. and Bedin, L. R. and Claudi, R. and Arellano Ferro, A. and Bruntt, H. and Stetson, P. B.},
	month = aug,
	year = {2007},
	keywords = {stars: variables: general, cataclysmic variables, open clusters and associations: individual: NGC 6791, stars: binaries: eclipsing, stars: novae, stars: starspots, stars: statistics},
	pages = {515--526},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/7I5ZM9ZM/de Marchi et al. - 2007 - Variable stars in the open cluster NGC 6791 and it.pdf:application/pdf},
}

@article{cantat-gaudin_gaia_2018,
	title = {A {Gaia} {DR2} view of the open cluster population in the {Milky} {Way}},
	volume = {618},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2018A%26A...618A..93C},
	doi = {10.1051/0004-6361/201833476},
	abstract = {Context. Open clusters are convenient probes of the structure and history of the Galactic disk. They are also fundamental to stellar evolution studies. The second Gaia data release contains precise astrometry at the submilliarcsecond level and homogeneous photometry at the mmag level, that can be used to characterise a large number of clusters over the entire sky. Aims: In this study we aim to establish a list of members and derive mean parameters, in particular distances, for as many clusters as possible, making use of Gaia data alone. Methods: We compiled a list of thousands of known or putative clusters from the literature. We then applied an unsupervised membership assignment code, UPMASK, to the Gaia DR2 data contained within the fields of those clusters. Results: We obtained a list of members and cluster parameters for 1229 clusters. As expected, the youngest clusters are seen to be tightly distributed near the Galactic plane and to trace the spiral arms of the Milky Way, while older objects are more uniformly distributed, deviate further from the plane, and tend to be located at larger Galactocentric distances. Thanks to the quality of Gaia DR2 astrometry, the fully homogeneous parameters derived in this study are the most precise to date. Furthermore, we report on the serendipitous discovery of 60 new open clusters in the fields analysed during this study.

Full Table 1 is only available in electronic form at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr
(ftp://130.79.128.5) or via http://cdsweb.u-strasbg.fr/cgi-bin/qcat?J/A+A/618/A93},
	urldate = {2021-05-24},
	journal = {Astronomy and Astrophysics},
	author = {Cantat-Gaudin, T. and Jordi, C. and Vallenari, A. and Bragaglia, A. and Balaguer-N{\'u}{\~n}ez, L. and Soubiran, C. and Bossini, D. and Moitinho, A. and Castro-Ginard, A. and Krone-Martins, A. and Casamiquela, L. and Sordo, R. and Carrera, R.},
	month = oct,
	year = {2018},
	keywords = {open clusters and associations: general, Galaxy: disk, Galaxy: structure, stars: distances},
	pages = {A93},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/Y23EZCWZ/Cantat-Gaudin et al. - 2018 - A Gaia DR2 view of the open cluster population in .pdf:application/pdf},
}

@article{conroy_ubiquitous_2015,
	title = {Ubiquitous time variability of integrated stellar populations},
	volume = {527},
	issn = {0028-0836},
	url = {http://adsabs.harvard.edu/abs/2015Natur.527..488C},
	doi = {10.1038/nature15731},
	abstract = {Long-period variable stars arise in the final stages of the asymptotic giant branch phase of stellar evolution. They have periods of up to about 1,000 days and amplitudes that can exceed a factor of three in the I-band flux. These stars pulsate predominantly in their fundamental mode, which is a function of mass and radius, and so the pulsation periods are sensitive to the age of the underlying stellar population. The overall number of long-period variables in a population is directly related to their lifetimes, which is difficult to predict from first principles because of uncertainties associated with stellar mass-loss and convective mixing. The time variability of these stars has not previously been taken into account when modelling the spectral energy distributions of galaxies. Here we construct time-dependent stellar population models that include the effects of long-period variable stars, and report the ubiquitous detection of this expected {\textquoteleft}pixel shimmer{\textquoteright} in the massive metal-rich galaxy M87. The pixel light
curves display a variety of behaviours. The observed variation of 0.1 to 1 per cent is very well matched to the predictions of our models. The data provide a strong constraint on the properties of variable stars in an old and metal-rich stellar population, and we infer that the lifetime of long-period variables in M87 is shorter by approximately 30 per cent compared to predictions from the latest stellar evolution models.},
	urldate = {2021-05-25},
	journal = {Nature},
	author = {Conroy, Charlie and van Dokkum, Pieter G. and Choi, Jieun},
	month = nov,
	year = {2015},
	pages = {488--491},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/T8CNBGVL/Conroy et al. - 2015 - Ubiquitous time variability of integrated stellar .pdf:application/pdf},
}

@article{ciardi_characterizing_2011,
	title = {Characterizing the {Variability} of {Stars} with {Early}-release {Kepler} {Data}},
	volume = {141},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/2011AJ....141..108C},
	doi = {10.1088/0004-6256/141/4/108},
	abstract = {We present a variability analysis of the early-release first quarter of data publicly released by the Kepler project. Using the stellar
parameters from the Kepler Input Catalog, we have separated the sample into 129,000 dwarfs and 17,000 giants and further sub-divided the luminosity classes into temperature bins corresponding approximately to the spectral classes A, F, G, K, and M. Utilizing the inherent sampling and time baseline of the public data set (30 minute sampling and 33.5 day baseline), we have explored the variability of the stellar sample. The overall variability rate of the dwarfs is 25\% for the entire sample, but can reach 100\% for the brightest groups of stars in the sample. G dwarfs are found to be the most stable with a dispersion floor of $\sigma$ {\textasciitilde} 0.04 mmag. At the precision of Kepler, {\textgreater}95\% of the giant
stars are variable with a noise floor of {\textasciitilde}0.1 mmag, 0.3 mmag, and 10 mmag for the G giants, K giants, and M giants, respectively. The photometric dispersion of the giants is consistent with acoustic variations of the photosphere; the photometrically derived predicted radial velocity distribution for the K giants is in agreement with the measured radial velocity distribution. We have also briefly explored the variability fraction as a function of data set baseline (1-33 days), at the native 30 minute sampling of the public Kepler data. To within the limitations of the data, we find that the overall variability fractions increase as the data set baseline is increased from 1 day to 33 days, in particular for the most variable stars. The lower mass M dwarf, K dwarf, and G dwarf stars increase their variability more significantly than the higher mass F dwarf and A dwarf stars as the time baseline is increased, indicating that the variability of the lower mass stars is mostly characterized by timescales of weeks while the variability of the higher mass stars is mostly characterized by timescales of days. A study of the distribution of the variability as a function of galactic latitude suggests that sources closer to the galactic plane are more variable. This may be the result of sampling differing populations (i.e., ages) as a function of latitude or may be the result of higher background contamination that is inflating the variability fractions at lower latitudes. A comparison of the M dwarf statistics to the variability of 29 known bright M dwarfs indicates that the M dwarfs are primarily variable on timescales of weeks or longer presumably dominated by spots and binarity. On shorter timescales of hours, which are relevant for planetary transit detection, the stars are significantly less variable, with {\textasciitilde}80\% having 12 hr dispersions of 0.5 mmag or less.},
	urldate = {2021-05-26},
	journal = {The Astronomical Journal},
	author = {Ciardi, David R. and von Braun, Kaspar and Bryden, Geoff and van Eyken, Julian and Howell, Steve B. and Kane, Stephen R. and Plavchan, Peter and Ram{\'i}rez, Solange V. and Stauffer, John R.},
	month = apr,
	year = {2011},
	keywords = {stars: variables: general, stars: statistics},
	pages = {108},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/57AWGI6L/Ciardi et al. - 2011 - Characterizing the Variability of Stars with Early.pdf:application/pdf},
}

@article{basri_photometric_2011,
	title = {Photometric {Variability} in {Kepler} {Target} {Stars}. {II}. {An} {Overview} of {Amplitude}, {Periodicity}, and {Rotation} in {First} {Quarter} {Data}},
	volume = {141},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/2011AJ....141...20B},
	doi = {10.1088/0004-6256/141/1/20},
	abstract = {We provide an overview of stellar variability in the first quarter data 
from the Kepler mission. The intent of this paper is to examine the
entire sample of over 150,000 target stars for periodic behavior in
their light curves and relate this to stellar characteristics. This data
set constitutes an unprecedented study of stellar variability given its
great precision and complete time coverage (with a half hour cadence).
Because the full Kepler pipeline is not currently suitable for a study
of stellar variability of this sort, we describe our procedures for
treating the "raw" pipeline data. About half of the total sample
exhibits convincing periodic variability up to two weeks, with
amplitudes ranging from differential intensity changes of less than
10-4 up to more than 10\%. K and M dwarfs have a greater
fraction of period behavior than G dwarfs. The giants in the sample have
distinctive quasi-periodic behavior, but are not periodic in the way we
define it. Not all periodicities are due to rotation, and the most
significant period is not necessarily the rotation period. We discuss
properties of the light curves, and in particular look at a sample of
very clearly periodic G dwarfs. It is clear that a large number of them
do vary because of rotation and starspots, but it will take further
analysis to fully exploit this.},
	urldate = {2021-05-26},
	journal = {The Astronomical Journal},
	author = {Basri, Gibor and Walkowicz, Lucianne M. and Batalha, Natalie and Gilliland, Ronald L. and Jenkins, Jon and Borucki, William J. and Koch, David and Caldwell, Doug and Dupree, Andrea K. and Latham, David W. and Marcy, Geoffrey W. and Meibom, Soeren and Brown, Tim},
	month = jan,
	year = {2011},
	keywords = {stars: variables: general, stars: statistics, stars: activity, stars: rotation, stars: solar-type, starspots},
	pages = {20},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/JASYST8Y/Basri et al. - 2011 - Photometric Variability in Kepler Target Stars. II.pdf:application/pdf},
}

@article{marigo_new_2017,
	title = {A {New} {Generation} of {PARSEC}-{COLIBRI} {Stellar} {Isochrones} {Including} the {TP}-{AGB} {Phase}},
	volume = {835},
	issn = {0004-637X},
	url = {http://adsabs.harvard.edu/abs/2017ApJ...835...77M},
	doi = {10.3847/1538-4357/835/1/77},
	abstract = {We introduce a new generation of PARSEC-COLIBRI stellar isochrones that 
includes a detailed treatment of the thermally pulsing asymptotic giant
branch (TP-AGB) phase, covering a wide range of initial metallicities
(0.0001 {\textless} ZI {\textless} 0.06). Compared to previous releases,
the main novelties and improvements are use of new TP-AGB tracks and
related atmosphere models and spectra for M and C-type stars; inclusion
of the surface H+He+CNO abundances in the isochrone tables, accounting
for the effects of diffusion, dredge-up episodes and hot-bottom burning;
inclusion of complete thermal pulse cycles, with a complete description
of the in-cycle changes in the stellar parameters; new pulsation models
to describe the long-period variability in the fundamental and
first-overtone modes; and new dust models that follow the growth of the
grains during the AGB evolution, in combination with radiative transfer
calculations for the reprocessing of the photospheric emission. Overall,
these improvements are expected to lead to a more consistent and
detailed description of properties of TP-AGB stars expected in resolved
stellar populations, especially in regard to their mean photometric
properties from optical to mid-infrared wavelengths. We illustrate the
expected numbers of TP-AGB stars of different types in stellar
populations covering a wide range of ages and initial metallicities,
providing further details on the {\textquotedblleft}C-star island{\textquotedblright} that
appears at intermediate values of age and metallicity, and about the
AGB-boosting effect that occurs at ages close to 1.6-Gyr for populations
of all metallicities. The isochrones are available through a new
dedicated web server.},
	urldate = {2021-06-04},
	journal = {The Astrophysical Journal},
	author = {Marigo, Paola and Girardi, L{\'e}o and Bressan, Alessandro and Rosenfield, Philip and Aringer, Bernhard and Chen, Yang and Dussin, Marco and Nanni, Ambra and Pastorelli, Giada and Rodrigues, Tha{\'i}se S. and Trabucchi, Michele and Bladh, Sara and Dalcanton, Julianne and Groenewegen, Martin A. T. and Montalb{\'a}n, Josefina and Wood, Peter R.},
	month = jan,
	year = {2017},
	keywords = {stars: general, stars: abundances, stars: evolution, stars: AGB and post-AGB, stars: carbon, stars: mass loss},
	pages = {77},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/DWCCVMGU/Marigo et al. - 2017 - A New Generation of PARSEC-COLIBRI Stellar Isochro.pdf:application/pdf},
}

@article{cantat-gaudin_painting_2020,
	title = {Painting a portrait of the {Galactic} disc with its stellar clusters},
	volume = {640},
	issn = {0004-6361},
	url = {http://adsabs.harvard.edu/abs/2020A%26A...640A...1C},
	doi = {10.1051/0004-6361/202038192},
	abstract = {Context. The large astrometric and photometric survey performed by the Gaia mission allows for a panoptic view of the Galactic disc and its stellar cluster population. Hundreds of stellar clusters were only discovered after the latest Gaia data release (DR2) and have yet to be characterised. Aims: Here we make use of the deep and homogeneous Gaia photometry down to G = 18 to estimate the distance, age, and interstellar reddening for about 2000 stellar clusters identified with Gaia DR2 astrometry. We use these objects to study the structure and evolution of the Galactic disc. Methods: We relied on a set of objects with well-determined parameters in the literature to train an artificial neural network to estimate parameters from the Gaia
photometry of cluster members and their mean parallax. Results: We obtain reliable parameters for 1867 clusters. Our catalogue confirms the relative lack of old stellar clusters in the inner disc (with a few notable exceptions). We also quantify and discuss the variation of scale height with cluster age, and we detect the Galactic warp in the
distribution of old clusters. Conclusions: This work results in a large and homogeneous cluster catalogue, allowing one to trace the structure of the disc out to distances of \~{}4 kpc. However, the
present sample is still unable to trace the outer spiral arm of the Milky Way, which indicates that the outer disc cluster census might still be incomplete.

List of cluster parameters and complete list of their members are only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/cat/J/A+A/640/A1},
	urldate = {2021-06-07},
	journal = {Astronomy and Astrophysics},
	author = {Cantat-Gaudin, T. and Anders, F. and Castro-Ginard, A. and Jordi, C. and Romero-G{\'o}mez, M. and Soubiran, C. and Casamiquela, L. and Tarricq, Y. and Moitinho, A. and Vallenari, A. and Bragaglia, A. and Krone-Martins, A. and Kounkel, M.},
	month = aug,
	year = {2020},
	keywords = {open clusters and associations: general, Galaxy: disk},
	pages = {A1},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/VG7ZLQ6C/Cantat-Gaudin et al. - 2020 - Painting a portrait of the Galactic disc with its .pdf:application/pdf},
}

@article{clement_variable_2001,
	title = {Variable {Stars} in {Galactic} {Globular} {Clusters}},
	volume = {122},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/2001AJ....122.2587C},
	doi = {10.1086/323719},
	abstract = {Based on a search of the literature up to 2001 May, the number of known variable stars in Galactic globular clusters is approximately 3000. Of these, more than 2200 have known periods and the majority (approximately 1800) are of the RR Lyrae type. In addition to the RR Lyrae population, there are approximately 100 eclipsing binaries, 120 SX Phoenicis variables, 60 Cepheids (including Population II Cepheids, anomalous Cepheids and RV Tauri), and 120 SR/red variables. The mean period of the fundamental mode RR Lyrae variables is 0.585 days, for the overtone variables it is 0.342 days (0.349 days for the first-overtone pulsators and 0.296 days for the second-overtone pulsators) and approximately 30\% are overtone pulsators. These numbers indicate that about 65\% of RR Lyrae variables in Galactic globular clusters belong to Oosterhoff type I systems. The mean period of the RR Lyrae variables in the Oosterhoff type I clusters seems to be correlated with metal abundance in the sense that the periods are longer in the more metal poor clusters. Such a correlation does not exist for the Oosterhoff type II clusters. Most of the Cepheids are in clusters with blue horizontal branches.},
	urldate = {2021-06-08},
	journal = {The Astronomical Journal},
	author = {Clement, Christine M. and Muzzin, Adam and Dufton, Quentin and Ponnampalam, Thivya and Wang, John and Burford, Jay and Richardson, Alan and Rosebery, Tara and Rowe, Jason and Hogg, Helen Sawyer},
	month = nov,
	year = {2001},
	keywords = {Galaxy: Globular Clusters: General, Stars: Binaries: Eclipsing, Stars: Horizontal-Branch, Stars: Oscillations, Stars: Variables: Cepheids, Stars: Variables: RR Lyrae Variable},
	pages = {2587--2599},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/UEWJVWX6/Clement et al. - 2001 - Variable Stars in Galactic Globular Clusters.pdf:application/pdf},
}

@article{clement_vizier_2017,
	title = {{VizieR} {Online} {Data} {Catalog}: {Updated} catalog of variable stars in globular clusters ({Clement}+ 2017)},
	volume = {5150},
	shorttitle = {{VizieR} {Online} {Data} {Catalog}},
	url = {http://adsabs.harvard.edu/abs/2017yCat.5150....0C},
	abstract = {This Catalogue is an update to Helen Sawyer Hogg's Third Catalogue on 
Variable Stars in Globular Clusters (1973, David Dunlap Observatory
Publications, Volume 3, Number 6: 1973PDDO....3....6S; see Cat V/97; see
also Clement+, 2001AJ....122.2587C).

This catalogue is based on the individual cluster files downloaded on
http://www.astro.utoronto.ca/{\textasciitilde}cclement/cat/listngc.html on the
01-Feb-2017. Later updates are indicated in clusters.dat; column
"Update".

(7 data files).},
	urldate = {2021-06-08},
	journal = {VizieR Online Data Catalog},
	author = {Clement, C. M.},
	month = feb,
	year = {2017},
	keywords = {Clusters: globular, References, Stars: variable},
}

@article{vanderplas_understanding_2018,
	title = {Understanding the {Lomb}-{Scargle} {Periodogram}},
	volume = {236},
	issn = {0067-0049},
	url = {http://adsabs.harvard.edu/abs/2018ApJS..236...16V},
	doi = {10.3847/1538-4365/aab766},
	abstract = {The Lomb-Scargle periodogram is a well-known algorithm for detecting and characterizing periodic signals in unevenly sampled data. This paper presents a conceptual introduction to the Lomb-Scargle periodogram and important practical considerations for its use. Rather than a rigorous mathematical treatment, the goal of this paper is to build intuition about what assumptions are implicit in the use of the Lomb-Scargle periodogram and related estimators of periodicity, so as to motivate important practical considerations required in its proper application and interpretation.},
	urldate = {2021-06-08},
	journal = {The Astrophysical Journal Supplement Series},
	author = {VanderPlas, Jacob T.},
	month = may,
	year = {2018},
	keywords = {methods: data analysis, methods: statistical},
	pages = {16},
	file = {Submitted Version:/Users/Tobin/Zotero/storage/J4KP8NB3/VanderPlas - 2018 - Understanding the Lomb-Scargle Periodogram.pdf:application/pdf},
}

@article{welch_robust_1993,
	title = {Robust variable star detection techniques suitable for automated searches - {New} results for {NGC} 1866},
	volume = {105},
	issn = {00046256},
	url = {http://adsabs.harvard.edu/cgi-bin/bib_query?1993AJ....105.1813W},
	doi = {10.1086/116556},
	abstract = {We describe sensitive techniques for identifying variable stars in multiepoch photometry lists made in two or more bandpasses or pairwise in a single bandpass. Our search strategy employs the correlation in brightness change between paired frames, which allows the extraction of information on variability in the presence of random photometric noise. A statistic for assessing the type of variable or degree of contamination by an unresolved source (depending on circumstance) is also described, as well as a bootstrap scheme for predicting confidence intervals for detection of real variability. These detection schemes are manifestly more robust than existing search techniques. To illustrate the power of this technique, we give a two-epoch example for photometry in the field of NGC 3201, a globular cluster rich in RR Lyr variables. Even this simple application has allowed us to rediscover 34 of 57 previously known (actual) variables, to verify the misidentification of several of them, and to discover four probable new variables (three of which may be RR Lyr stars). We then apply the variability statistics to 27 V and 29 B frames centered on the young, rich, Cepheid-bearing LMC cluster NGC 1866, which have been reduced with ALLFRAME. This application has resulted in the discovery of 12 new variables, as well as the recovery of all 15 of the previously known variables that lie within this field. Specific results are: (1) the discovery of four new Cepheid variables in NGC 1866, bringing the total number of probable member Cepheids to 23, (2) periods for all but one of the 23 NGC 1866 Cepheids, (3) good evidence for photometric contamination of several variables by unresolved companions, (4) the discovery of a RRab variable in the NGC 1866 field with a peak-to-peak V light-curve amplitude of 1.0 mag, an intensity-weighted mean V mag = 19.28{\textpm}0.01 mag, and a period of 0.5565 days, (5) (re)discovery of three longer-period red variables, and (6) the detection of several main-sequence or main-sequence-tumoff variable stars.},
	language = {en},
	urldate = {2021-06-14},
	journal = {The Astronomical Journal},
	author = {Welch, Douglas L. and Stetson, Peter B.},
	month = may,
	year = {1993},
	pages = {1813},
	file = {Welch and Stetson - 1993 - Robust variable star detection techniques suitable.pdf:/Users/Tobin/Zotero/storage/LYKXJEUQ/Welch and Stetson - 1993 - Robust variable star detection techniques suitable.pdf:application/pdf},
}

@article{bica_updated_2020,
	title = {An {Updated} {Small} {Magellanic} {Cloud} and {Magellanic} {Bridge} {Catalog} of {Star} {Clusters}, {Associations}, and {Related} {Objects}},
	volume = {159},
	issn = {0004-6256},
	url = {http://adsabs.harvard.edu/abs/2020AJ....159...82B},
	doi = {10.3847/1538-3881/ab6595},
	abstract = {We present a catalog of star clusters, associations, and related 
extended objects in the Small Magellanic Cloud (SMC) and the Magellanic
Bridge with 2741 entries, a factor 2 more than a previous version from a
decade ago. Literature data up until 2018 December are included. The
identification of star clusters was carried out with digital atlases in
various bands currently available in the Digitized Sky Survey and the
Machine Automatique {\`a} M{\'e}surer pour l'Astronomie. imaging
surveys. In particular, we cross-identified recent cluster samples from
the Visible and Infrared Survey Telescope for Astronomy near-infrared
YJKs survey of the Magellanic System, Optical Gravitational
Lensing Experiment IV, and Survey of the MAgellanic Stellar History
surveys, confirming new clusters and pointing out equivalencies. A major
contribution of the present catalog consists of the accurate central
positions for clusters and small associations, including a new sample of
45 clusters or candidates in the SMC and 19 in the Magellanic Bridge, as
well as a compilation of the most reliable age and metallicity values
from the literature. A general catalog must also deal with the recent
discoveries of 27 faint and ultra-faint star clusters and galaxies
projected on the far surroundings of the Clouds, most of them from the
Dark Energy Survey. The information on these objects has been
complemented with photometric, spectroscopic, and kinematical follow-up
data from the literature. The underluminous galaxies around the
Magellanic System, still very few as compared to the predictions from
$\Lambda$ Cold Dark Matter simulations, can bring constraints to galaxy
formation and hierarchical evolution. Furthermore, we provide
diagnostics, when possible, of the nature of the ultra-faint clusters,
searching for borders of the Magellanic System extensions into the Milky
Way gravitational potential.},
	urldate = {2021-06-15},
	journal = {The Astronomical Journal},
	author = {Bica, Eduardo and Westera, Pieter and Kerber, Leandro de O. and Dias, Bruno and Maia, Francisco and Santos, Jr., Jo{\~a}o F. C. and Barbuy, Beatriz and Oliveira, Raphael A. P.},
	month = mar,
	year = {2020},
	keywords = {1567, 1468, 212, 600},
	pages = {82},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/63RGAKNR/Bica et al. - 2020 - An Updated Small Magellanic Cloud and Magellanic B.pdf:application/pdf},
}

@article{hargis_time-series_2005,
	title = {Time-{Series} {Ensemble} {Photometry} and the {Search} for {Variable} {Stars} in the {Open} {Cluster} {M11}},
	volume = {130},
	issn = {0004-6256},
	url = {https://ui.adsabs.harvard.edu/abs/2005AJ....130.2824H},
	doi = {10.1086/497034},
	abstract = {This work presents the first large-scale photometric variability survey of the intermediate-age ({\textasciitilde}200 Myr) open cluster M11. Thirteen nights of data over two observing seasons were analyzed (using crowded field and ensemble photometry techniques) to obtain high relative precision photometry. In this study we focus on the detection of candidate member variable stars for follow-up studies. A total of 39 variable stars were detected and can be categorized as follows: one irregular (probably pulsating) variable, six $\delta$ Scuti variables, 14 detached eclipsing binary systems, 17 W UMa variables, and one unidentified/candidate variable. While previous proper-motion studies allow for cluster membership determination for the brightest stars, we find that membership determination is significantly hampered below V=15, R=15.5 by the large population of field stars overlapping the cluster main sequence. Of the brightest detected variables that have a high likelihood of cluster membership, we find five systems in which further work could help constrain theoretical stellar models, including one potential W UMa member of this young cluster.},
	urldate = {2021-06-18},
	journal = {The Astronomical Journal},
	author = {Hargis, Jonathan R. and Sandquist, Eric L. and Bradstreet, David H.},
	month = dec,
	year = {2005},
	keywords = {Astrophysics, Stars: Binaries: Eclipsing, open clusters and associations: individual (M11), Stars: Variables: $\delta$ Scuti},
	pages = {2824--2837},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/VESZIA2F/Hargis et al. - 2005 - Time-Series Ensemble Photometry and the Search for.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/NZYZYQW2/abstract.html:text/html},
}

@article{stetson_automatic_1996,
	title = {On the {Automatic} {Determination} of {Light}-{Curve} {Parameters} for {Cepheid} {Variables}},
	volume = {108},
	issn = {0004-6280},
	url = {https://ui.adsabs.harvard.edu/abs/1996PASP..108..851S},
	doi = {10.1086/133808},
	abstract = {A computerized algorithm for the automatic detection of Cepheid variables and for the estimation of their periods, amplitudes, and mean magnitudes from sparse data sets is presented. It is intended to be suitable for use in such programs as the measurement of Cepheid distances to external galaxies, for example with the Hubble Space Telescope. The reliability of the algorithm is tested by application to new photometric reductions of pre-repair HST images of the nearby Sdm galaxy IC 4182, with comparison to published analyses of the same data (Saha et al. 1994, ApJ, 425, 14). (SECTION: Stars)},
	urldate = {2021-06-18},
	journal = {Publications of the Astronomical Society of the Pacific},
	author = {Stetson, Peter B.},
	month = oct,
	year = {1996},
	keywords = {CEPHEIDS, METHODS: NUMERICAL},
	pages = {851},
	file = {Snapshot:/Users/Tobin/Zotero/storage/639MS27N/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/CLVI4E4U/Stetson - 1996 - On the Automatic Determination of Light-Curve Para.pdf:application/pdf},
}

@article{messa_young_2018-1,
	title = {The young star cluster population of {M51} with {LEGUS} - {II}. {Testing} environmental dependences},
	volume = {477},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.1683M},
	doi = {10.1093/mnras/sty577},
	abstract = {It has recently been established that the properties of young star clusters (YSCs) can vary as a function of the galactic environment in which they are found. We use the cluster catalogue produced by the Legacy Extragalactic UV Survey (LEGUS) collaboration to investigate cluster properties in the spiral galaxy M51. We analyse the cluster population as a function of galactocentric distance and in arm and inter-arm regions. The cluster mass function exhibits a similar shape at all radial bins, described by a power law with a slope close to -2 and an exponential truncation around 105 M?. While the mass functions of the YSCs in the spiral arm and inter-arm regions have similar truncation masses, the inter-arm region mass function has a significantly steeper slope than the one in the arm region, a trend that is also observed in the giant molecular cloud mass function and predicted by simulations. The age distribution of clusters is dependent on the region considered, and is consistent with rapid disruption only in dense regions, while little disruption is observed at large galactocentric distances and in the inter-arm region. The fraction of stars forming in clusters does not show radial variations, despite the drop in the H2 surface density measured as a function of galactocentric distance. We suggest that the higher disruption rate observed in the inner part of the galaxy is likely at the origin of the observed flat cluster formation efficiency radial profile.},
	urldate = {2021-06-21},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Messa, Matteo and Adamo, A. and Calzetti, D. and Reina-Campos, M. and Colombo, D. and Schinnerer, E. and Chandar, R. and Dale, D. A. and Gouliermis, D. A. and Grasha, K. and Grebel, E. K. and Elmegreen, B. G. and Fumagalli, M. and Johnson, K. E. and Kruijssen, J. M. D. and {\"O}stlin, G. and Shabani, F. and Smith, L. J. and Whitmore, B. C.},
	month = jun,
	year = {2018},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: individual: M51, galaxies: star clusters: general, galaxies: star formation, galaxies: individual: NGC 5194},
	pages = {1683--1707},
	file = {Snapshot:/Users/Tobin/Zotero/storage/2T9JJCZ9/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/DU4QMLIW/Messa et al. - 2018 - The young star cluster population of M51 with LEGU.pdf:application/pdf},
}

@article{pakstiene_search_2019,
	title = {Search for variable stars in the northern sky: analysis of photometric time series for 3598 stars},
	volume = {364},
	issn = {0004-640X},
	shorttitle = {Search for variable stars in the northern sky},
	url = {https://ui.adsabs.harvard.edu/abs/2019Ap&SS.364...31P/abstract},
	doi = {10.1007/s10509-019-3522-3},
	abstract = {As extensive ground-based observations and characterisation of different variable stars are of the utmost importance in preparing optimal input catalogues for space missions, our aim was to search for new variable stars in selected fields of the northern sky. We obtained 24 470 CCD images and analysed photometric time series of stars using the DAOPHOT based package Muniwin as the first step, and the Period04 package was used to further analyse the suspected new variable stars. The light curves and other observational results are presented for 3598 stars online. We found 81 new variable stars, among them is an eclipsing binary with a variable component and possibly eccentric orbits TYC4038-693-1 which we also observed spectroscopically, four $\delta$ Scuti candidates, six other variable stars with periods falling into the interval of 35 minutes to 20 days. Furthermore, we identified 70 slowly varying stars with so far undefined periodicity. Additional photometric and spectral observations were carried out for TYC2764-1997-1, and its previous candidacy for eclipsing binaries was approved.},
	language = {en},
	number = {2},
	urldate = {2021-06-22},
	journal = {Astrophysics and Space Science},
	author = {Pak{\v s}tien{\.e}, E. and Janulis, R. and Drazdauskas, A. and Mikolaitis, {\v S} and Tautvai{\v s}ien{\.e}, G. and Minkevi{\v c}i{\=u}t{\.e}, R. and Bagdonas, V. and Klebonas, L. and Qvam, J. K. T.},
	month = feb,
	year = {2019},
	pages = {31},
	file = {Snapshot:/Users/Tobin/Zotero/storage/JSPWXWKW/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/RUZBUA47/Pak{\v s}tien{\.e} et al. - 2019 - Search for variable stars in the northern sky ana.pdf:application/pdf},
}

@article{luger_update_2018,
	title = {An {Update} to the {EVEREST} {K2} {Pipeline}: {Short} {Cadence}, {Saturated} {Stars}, and {Kepler}-like {Photometry} {Down} to {Kp} = 15},
	volume = {156},
	issn = {0004-6256},
	shorttitle = {An {Update} to the {EVEREST} {K2} {Pipeline}},
	url = {https://ui.adsabs.harvard.edu/abs/2018AJ....156...99L},
	doi = {10.3847/1538-3881/aad230},
	abstract = {We present an update to the EVEREST K2 pipeline that addresses various limitations in the previous version and improves the photometric precision of the light curves. We develop a fast regularization scheme for pixel-level decorrelation (PLD) and adapt the algorithm to include the PLD vectors of other stars to enhance the predictive power of the model and minimize overfitting, particularly for faint stars. We also modify PLD to work for saturated stars and improve its performance on variable stars, although some high-frequency variables may still suffer from overfitting. On average, EVEREST 2.0 light curves have 10-20\% higher photometric precision than those in version 1, yielding the highest-precision light curves at all \{Kp\} magnitudes of any publicly available K2 catalog. For most K2 campaigns, we recover the original Kepler precision to at least \{Kp\} = 14, and to at least \{Kp\} = 15 for campaigns 1, 5, 6, and 13. We also detrend most short-cadence targets observed by K2, obtaining even higher photometric precision for these stars. Like all aggressive, flexible models, EVEREST is prone to overfitting, and may cause a decrease in transit depths by \~{}10\% we urge users to mask signals of interest using our open-source software, which we show removes this bias. Light curves for campaigns 0-8 and 10-13 are available online in the EVEREST catalog, which will be updated with future campaigns. EVEREST 2.0 is open source and is coded in a framework that can be adapted to other photometric surveys, including Kepler and the upcoming TESS mission.},
	urldate = {2021-06-22},
	journal = {The Astronomical Journal},
	author = {Luger, Rodrigo and Kruse, Ethan and Foreman-Mackey, Daniel and Agol, Eric and Saunders, Nicholas},
	month = sep,
	year = {2018},
	keywords = {techniques: photometric, catalogs, Astrophysics - Instrumentation and Methods for Astrophysics, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics},
	pages = {99},
	file = {Snapshot:/Users/Tobin/Zotero/storage/WY6GRMIC/abstract.html:text/html;Submitted Version:/Users/Tobin/Zotero/storage/9K7CEIQG/Luger et al. - 2018 - An Update to the EVEREST K2 Pipeline Short Cadenc.pdf:application/pdf},
}

@article{gillen_ngts_2020,
	title = {{NGTS} clusters survey - {I}. {Rotation} in the young benchmark open cluster {Blanco} 1},
	volume = {492},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492.1008G},
	doi = {10.1093/mnras/stz3251},
	abstract = {We determine rotation periods for 127 stars in the \~{}115-Myr-old Blanco 1 open cluster using \~{}200 d of photometric monitoring with the Next Generation Transit Survey. These stars span F5-M3 spectral types (1.2 M? ? M ? 0.3 M?) and increase the number of known rotation periods in Blanco 1 by a factor of four. We determine rotation periods using three methods: Gaussian process (GP) regression, generalized autocorrelation function (G-ACF), and Lomb-Scargle (LS) periodogram, and find that the GP and G-ACF methods are more applicable to evolving spot modulation patterns. Between mid-F and mid-K spectral types, single stars follow a well-defined rotation sequence from \~{}2 to 10 d, whereas stars in photometric multiple systems typically rotate faster. This may suggest that the presence of a moderate-to-high mass ratio companion inhibits angular momentum loss mechanisms during the early pre-main sequence, and this signature has not been erased at \~{}100 Myr. The majority of mid-F to mid-K stars display evolving modulation patterns, whereas most M stars show stable modulation signals. This morphological change coincides with the shift from a well-defined rotation sequence (mid-F to mid-K stars) to a broad rotation period distribution (late-K and M stars). Finally, we compare our rotation results for Blanco 1 to the similarly aged Pleiades: the single-star populations in both clusters possess consistent rotation period distributions, which suggests that the angular momentum evolution of stars follows a well-defined pathway that is, at least for mid-F to mid-K stars, strongly imprinted by \~{}100 Myr.},
	urldate = {2021-06-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Gillen, Edward and Briegal, Joshua T. and Hodgkin, Simon T. and Foreman-Mackey, Daniel and Van Leeuwen, Floor and Jackman, James A. G. and McCormac, James and West, Richard G. and Queloz, Didier and Bayliss, Daniel and Goad, Michael R. and Watson, Christopher A. and Wheatley, Peter J. and Belardi, Claudia and Burleigh, Matthew R. and Casewell, Sarah L. and Jenkins, James S. and Raynard, Liam and Smith, Alexis M. S. and Tilbrook, Rosanna H. and Vines, Jose I.},
	month = feb,
	year = {2020},
	keywords = {Astrophysics - Solar and Stellar Astrophysics, stars: variables: general, stars: rotation, binaries: general, open clusters and associations: individual: Blanco 1},
	pages = {1008--1024},
	file = {Snapshot:/Users/Tobin/Zotero/storage/6WWIL747/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/BTAFPVB6/Gillen et al. - 2020 - NGTS clusters survey - I. Rotation in the young be.pdf:application/pdf},
}

@article{giacobbe_photometric_2020,
	title = {Photometric rotation periods for 107 {M} dwarfs from the {APACHE} survey},
	volume = {491},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5216G},
	doi = {10.1093/mnras/stz3364},
	abstract = {We present rotation period measurements for 107 M dwarfs in the mass range 0.15-0.70 M\_? observed within the context of the APACHE photometric survey. We measure rotation periods in the range 0.5-190 d, with the distribution peaking at \~{}30 d. We revise the stellar masses and radii for our sample of rotators by exploiting the Gaia DR2 data. For \~{}20 per cent of the sample, we compare the photometric rotation periods with those derived from different spectroscopic indicators, finding good correspondence in most cases. We compare our rotation periods distribution to the one obtained by the Kepler survey in the same mass range, and to that derived by the MEarth survey for stars in the mass range 0.07-0.25 M\_?. The APACHE and Kepler periods distributions are in good agreement, confirming the reliability of our results, while the APACHE distribution is consistent with the MEarth result only for the older/slow rotators, and in the overlapping mass range of the two surveys. Combining the APACHE/Kepler distribution with the MEarth distribution, we highlight that the rotation period increases with decreasing stellar mass, in agreement with previous work. Our findings also suggest that the spin-down time scale, from fast to slow rotators, changes crossing the fully convective limit at \{?\}0.3 M\_? for M dwarfs. The catalogue of 107 rotating M dwarfs presented here is particularly timely, as the stars are prime targets for the potential identification of transiting small planets with TESS and amenable to high-precision mass determination and further atmospheric characterization measurements.},
	urldate = {2021-06-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Giacobbe, P. and Benedetto, M. and Damasso, M. and Sozzetti, A. and Christille, J. M. and Lattanzi, M. G. and Calcidese, P. and Carbognani, A. and Barbato, D. and Pinamonti, M. and Poggio, E. and Lanza, A. F. and Bernagozzi, A. and Cenadelli, D. and Lanteri, L. and Bertolini, E.},
	month = feb,
	year = {2020},
	keywords = {techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, stars: statistics, stars: rotation, stars: low-mass},
	pages = {5216--5237},
	file = {Snapshot:/Users/Tobin/Zotero/storage/KNFWUPCM/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/RC8NC2MK/Giacobbe et al. - 2020 - Photometric rotation periods for 107 M dwarfs from.pdf:application/pdf},
}

@article{andronov_variable_2020,
	title = {Variable stars: a net of complementary methods for time series analysis. {Application} to {RY} {UMa}},
	volume = {31},
	issn = {1055-6796},
	shorttitle = {Variable stars},
	url = {https://ui.adsabs.harvard.edu/abs/2020A&AT...31..411A/abstract},
	abstract = {The expert system for time series analysis of irregularly spaced signals is reviewed. It consists of a number of complementary algorithms and programs, which may be effective for different types of variability. Obviously, for a pure sine signal, all the methods should produce the same results. However, for irregularly spaced signals with a complicated structure, e.g. a sum of different components, different methods may produce significantly different results. The basic approach is based on the classical method of least squares (1994OAP.....7...49A). However, contrary to common "step-by-step" methods of removal of important components (e.g. mean, trend ("detrending"), sine wave ("prewhitening"), where covariations between different components are ignored, i.e. erroneously assumed to be zero, we use complete mathematical models. Some of the methods are illustrated in the observations of the semi-regular pulsating variable RY UMa. The star shows a drastic cyclic change of semi-amplitude of pulsations between 0.01 to 0.37 mag, which is interpreted as a bias between the waves with close periods and a beat period of 4000 d (11 yr). The dominating period has changed from 307.35(8) d before 1993 to 285.26(6) d after 1993. The initial epoch of the maximum brightness for the recent interval is 2454008.8(5). It is suggested that the apparent period switch is due to variability of amplitudes of these two waves and an occasional swap of the dominating wave. Keywords: Time series analysis, data analysis, pulsating stars, stars: individual: RY UMa},
	language = {en},
	number = {4},
	urldate = {2021-06-22},
	journal = {Astronomical and Astrophysical Transactions},
	author = {Andronov, I. L. and Chinarova, L. L.},
	year = {2020},
	pages = {411--422},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/B4HACN89/Andronov and Chinarova - 2020 - Variable stars a net of complementary methods for.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/E2MAD5TE/abstract.html:text/html},
}

@article{andronov_autocorrelation_1994,
	title = {Autocorrelation function bias owed to a limited number of de-trended observations. {Applications} to autoregressive models with noise.},
	volume = {315},
	issn = {0004-6337},
	url = {https://ui.adsabs.harvard.edu/abs/1994AN....315..353A},
	doi = {10.1002/asna.2103150506},
	abstract = {Analytical expressions were derived for the expectation of the autocorrelation function (ACF) corresponding to low-frequency least squares fits and deviations from them in the case of a limited number of observations N. A vector of values of the autocorrelation function may be obtained by multiplication of a N N matrix Z (dependent on concrete basic functions used for trend determination) by a vector of the unbiased ACF. Because much computational time is needed to obtain such a matrix, its components are to be computed once for concrete N and basic functions, and then stored as a file. An algorithm is proposed for determining the contribution of the correlated signal to the 'signal noise'. The expressions are written for general form of the ACF, and illustrated by the application to autoregressive models. The statistical properties of the model parameters are studied. The method is applied to cataclysmic binaries AM Her and TT Ari. The precise expressions allow us to obtain reliable results and to avoid misinterpretation being possible when using the approximate methods.},
	urldate = {2021-06-22},
	journal = {Astronomische Nachrichten},
	author = {Andronov, I. L.},
	month = aug,
	year = {1994},
	keywords = {Astrophysics, Autocorrelation, Autoregressive Processes, Bias, Cataclysmic Variables, Covariance, Data Processing, Least Squares Method},
	pages = {353--370},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/6YX8W669/Andronov - 1994 - Autocorrelation function bias owed to a limited nu.pdf:application/pdf},
}

@article{pepper_survey_2006,
	title = {Survey for {Transiting} {Extrasolar} {Planets} in {Stellar} {Systems}. {IV}. {Variables} in the {Field} of {NGC} 1245},
	volume = {132},
	issn = {0004-6256},
	url = {https://ui.adsabs.harvard.edu/abs/2006AJ....132.1177P},
	doi = {10.1086/505942},
	abstract = {The Survey for Transiting Extrasolar Planets in Stellar Systems (STEPSS) project is a search for planetary transits in open clusters. In this paper we analyze the STEPSS observations of the open cluster NGC 1245 to determine the variable-star content of the cluster. Out of 6787 stars observed with V{\textless}22, of which {\textasciitilde}870 are cluster members, we find 14 stars with clear intrinsic variability that are potential cluster members and 29 clear variables that are not cluster members. None of these variables have been previously identified. We present light curves, finder charts, and stellar/photometric data on these variable objects. Several of the interacting binaries have estimated distances consistent with the cluster distance determined from isochrone fits to the color-magnitude diagram. Four stars at the main-sequence turnoff of the cluster have light curves consistent with $\gamma$ Doradus variability. If these $\gamma$ Doradus candidates are confirmed, they represent the oldest and coolest members of this class of variable discovered to date.},
	urldate = {2021-06-22},
	journal = {The Astronomical Journal},
	author = {Pepper, Joshua and Burke, Christopher J.},
	month = sep,
	year = {2006},
	keywords = {Astrophysics, Techniques: Photometric, Surveys, Stars: Binaries: General, Stars: Variables: Other},
	pages = {1177--1188},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/RWCSNURK/Pepper and Burke - 2006 - Survey for Transiting Extrasolar Planets in Stella.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/ZYJHQFQF/abstract.html:text/html},
}

@article{sullivan_transiting_2015,
	title = {The {Transiting} {Exoplanet} {Survey} {Satellite}: {Simulations} of {Planet} {Detections} and {Astrophysical} {False} {Positives}},
	volume = {809},
	issn = {0004-637X},
	shorttitle = {The {Transiting} {Exoplanet} {Survey} {Satellite}},
	url = {https://ui.adsabs.harvard.edu/abs/2015ApJ...809...77S},
	doi = {10.1088/0004-637X/809/1/77},
	abstract = {The Transiting Exoplanet Survey Satellite (TESS) is a NASA-sponsored Explorer mission that will perform a wide-field survey for planets that transit bright host stars. Here, we predict the properties of the transiting planets that TESS will detect along with the EB stars that produce false-positive photometric signals. The predictions are based on Monte Carlo simulations of the nearby population of stars, occurrence rates of planets derived from Kepler, and models for the photometric performance and sky coverage of the TESS cameras. We expect that TESS will find approximately 1700 transiting planets from 2{\texttimes} \{10\}5 pre-selected target stars. This includes 556 planets smaller than twice the size of Earth, of which 419 are hosted by M dwarf stars and 137 are hosted by FGK dwarfs. Approximately 130 of the R{\textless} 2 \{R\}{\textbackslash}oplus planets will have host stars brighter than \{K\}s=9. Approximately 48 of the planets with R{\textless} 2 \{R\}{\textbackslash}oplus lie within or near the habitable zone (0.2{\textless} S/\{S\}{\textbackslash}oplus {\textless} 2); between 2 and 7 such planets have host stars brighter than \{K\}s=9. We also expect approximately 1100 detections of planets with radii 2-4 \{R\}{\textbackslash}oplus , and 67 planets larger than 4 \{R\}{\textbackslash}oplus . Additional planets larger than 2 \{R\}{\textbackslash}oplus can be detected around stars that are not among the pre-selected target stars, because TESS will also deliver full-frame images at a 30-minute cadence. The planet detections are accompanied by over 1000 astrophysical false positives. We discuss how TESS data and ground-based observations can be used to distinguish the false positives from genuine planets. We also discuss the prospects for follow-up observations to measure the masses and atmospheres of the TESS planets.},
	urldate = {2021-06-23},
	journal = {The Astrophysical Journal},
	author = {Sullivan, Peter W. and Winn, Joshua N. and Berta-Thompson, Zachory K. and Charbonneau, David and Deming, Drake and Dressing, Courtney D. and Latham, David W. and Levine, Alan M. and McCullough, Peter R. and Morton, Timothy and Ricker, George R. and Vanderspek, Roland and Woods, Deborah},
	month = aug,
	year = {2015},
	keywords = {planets and satellites: detection, surveys, Astrophysics - Earth and Planetary Astrophysics, space vehicles: instruments},
	pages = {77},
	file = {Snapshot:/Users/Tobin/Zotero/storage/FMBJXEHP/abstract.html:text/html;Full Text:/Users/Tobin/Zotero/storage/Q93XH2NU/Sullivan et al. - 2015 - The Transiting Exoplanet Survey Satellite Simulat.pdf:application/pdf},
}

@article{maiz_apellaniz_numerical_2005,
	title = {Numerical {Biases} on {Initial} {Mass} {Function} {Determinations} {Created} by {Binning}},
	volume = {629},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2005ApJ...629..873M},
	doi = {10.1086/431458},
	abstract = {We detect and quantify significant numerical biases in the determination of the slope of power laws with Salpeter (or similar) indices from uniformly binned data using $\chi$2 minimization. The biases are caused by the correlation between the number of stars per bin and the assigned weights and are especially important when the number of stars per bin is small. This result implies the existence of systematic errors in the values of IMFs calculated in this way. We propose as an alternative using variable-size bins and dividing the stars evenly among them. Such variable-size bins yield very small biases that are only weakly dependent on the number of stars per bin. Furthermore, we show that they allow for the calculation of reliable IMFs with only a small total number of stars. Therefore, they are a preferred alternative to the standard uniform-size binning.},
	urldate = {2021-06-24},
	journal = {The Astrophysical Journal},
	author = {Ma{\'i}z Apell{\'a}niz, J. and {\'U}beda, L.},
	month = aug,
	year = {2005},
	keywords = {Astrophysics, Mass Function, Methods: Numerical, Methods: Statistical, Stars: Luminosity Function},
	pages = {873--880},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/24Z3ZM5T/Ma{\'i}z Apell{\'a}niz and {\'U}beda - 2005 - Numerical Biases on Initial Mass Function Determin.pdf:application/pdf;Snapshot:/Users/Tobin/Zotero/storage/Q3VDV4Z7/abstract.html:text/html},
}

@article{grudic_model_2021,
	title = {A model for the formation of stellar associations and clusters from giant molecular clouds},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.tmp.1646G},
	doi = {10.1093/mnras/stab1894},
	abstract = {We present a large suite of MHD simulations of turbulent, star-forming giant molecular clouds (GMCs) with stellar feedback, extending previous work by simulating 10 different random realizations for each point in the parameter space of cloud mass and size. It is found that once the clouds disperse due to stellar feedback, both self-gravitating star clusters and unbound stars generally remain, which arise from the same underlying continuum of substructured stellar density, ie. the hierarchical cluster formation scenario. The fraction of stars that are born within gravitationally-bound star clusters is related to the overall cloud star formation efficiency set by stellar feedback, but has significant scatter due to stochastic variations in the small-scale details of the star-forming gas flow. We use our numerical results to calibrate a model for mapping the bulk properties (mass, size, and metallicity) of self-gravitating GMCs onto the star cluster populations they form, expressed statistically in terms of cloud-level distributions. Synthesizing cluster catalogues from an observed GMC catalogue in M83, we find that this model predicts initial star cluster masses and sizes that are in good agreement with observations, using only standard IMF and stellar evolution models as inputs for feedback. Within our model, the ratio of the strength of gravity to stellar feedback is the key parameter setting the masses of star clusters, and of the various feedback channels direct stellar radiation (photon momentum and photoionization) is the most important on GMC scales.},
	urldate = {2021-07-16},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Grudi{\'c}, Michael Y. and Kruijssen, J. M. Diederik and Faucher-Gigu{\'e}re, Claude-Andr{\'e} and Hopkins, Philip F. and Ma, Xiangcheng and Quataert, Eliot and Boylan-Kolchin, Michael},
	month = jul,
	year = {2021},
	keywords = {Astrophysics - Astrophysics of Galaxies, stars: formation, galaxies: star clusters: general, galaxies: star formation, Astrophysics - Solar and Stellar Astrophysics},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/NIY8K2SP/Grudi{\'c} et al. - 2021 - A model for the formation of stellar associations .pdf:application/pdf},
}

@article{lee_phangs-hst_2021,
	title = {The {PHANGS}-{HST} {Survey}: {A} {Census} of {Star} {Clusters} and {Multi}-{Scale} {Stellar} {Associations} in {Nearby} {Spiral} {Galaxies}},
	volume = {53},
	shorttitle = {The {PHANGS}-{HST} {Survey}},
	url = {https://ui.adsabs.harvard.edu/abs/2021AAS...23833104L},
	abstract = {The PHANGS program is building the first dataset to enable the multi-phase, multi-scale study of star formation across the nearby spiral galaxy population. This effort is enabled by large Treasury programs with ALMA, VLT/MUSE, and HST, with which we have obtained CO(2-1) imaging, optical spectroscopic mapping, and high resolution UV-optical imaging, respectively. Here, we present PHANGS-HST, which is obtaining five band NUV-U-B-V-I imaging of the disks of 38 spiral galaxies at distances of 4-23 Mpc, and parallel V and I band imaging of their halos, to provide a census of tens of thousands of compact star clusters and associations. The combination of HST, ALMA, and VLT/MUSE observations will yield an unprecedented joint catalog of the observed and physical properties of \~{}100,000 star clusters, associations, HII regions, and molecular clouds. With these basic units of star formation, PHANGS will systematically chart the evolutionary cycling between gas and stars, across a diversity of galactic environments found in nearby galaxies. We discuss the design of the PHANGS-HST survey, and provide an overview of the HST data processing pipeline and first results, highlighting new methods for selecting star cluster candidates, morphological classification of candidates with convolutional neural networks, and identification of stellar associations over a range of physical scales with a watershed algorithm. We describe the cross-observatory imaging, catalogs, and software products being released at MAST, which will seed a broad range of community science, in particular, upcoming JWST study of dust embedded star formation and ISM physics.},
	urldate = {2021-07-16},
	author = {Lee, J. and Whitmore, B. and Thilker, D. and Deger, S. and Chandar, R. and Larson, K. and Dale, D. and Turner, J. and Ubeda, L. and Anand, G. and Boquien, M. and Schinnerer, E. and Leroy, A. and {Phangs Team}},
	month = jun,
	year = {2021},
	note = {Conference Name: American Astronomical Society Meeting Abstracts},
	pages = {331.04},
}

@article{eisner_planet_2021,
	title = {Planet {Hunters} {TESS} {III}: two transiting planets around the bright {G} dwarf {HD} 152843},
	volume = {505},
	issn = {0035-8711},
	shorttitle = {Planet {Hunters} {TESS} {III}},
	url = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505.1827E},
	doi = {10.1093/mnras/stab1253},
	abstract = {We report on the discovery and validation of a two-planet system around a bright (V = 8.85 mag) early G dwarf (1.43 R?, 1.15 M?, TOI 2319) using data from NASA's Transiting Exoplanet Survey Satellite (TESS). Three transit events from two planets were detected by citizen scientists in the month-long TESS light curve (sector 25), as part of the Planet Hunters TESS project. Modelling of the transits yields an orbital period of \$11.6264 \_\{ - 0.0025 \} {\textasciicircum} \{ + 0.0022 \}\$ d and radius of \$3.41 \_\{ - 0.12 \} {\textasciicircum} \{ + 0.14 \}\$ R(+) for the inner planet, and a period in the range 19.26-35 d and a radius of \$5.83 \_\{ - 0.14 \} {\textasciicircum} \{ + 0.14 \}\$ R(+) for the outer planet, which was only seen to transit once. Each signal was independently statistically validated, taking into consideration the TESS light curve as well as the ground-based spectroscopic follow-up observations. Radial velocities from HARPS-N and EXPRES yield a tentative detection of planet b, whose mass we estimate to be \$11.56 \_\{ - 6.14 \} {\textasciicircum} \{ + 6.58 \}\$ M(+), and allow us to place an upper limit of 27.5 M(+) (99 per cent confidence) on the mass of planet c. Due to the brightness of the host star and the strong likelihood of an extended H/He atmosphere on both planets, this system offers excellent prospects for atmospheric characterization and comparative planetology.},
	urldate = {2021-07-16},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Eisner, N. L. and Nicholson, B. A. and Barrag{\'a}n, O. and Aigrain, S. and Lintott, C. and Kaye, L. and Klein, B. and Miller, G. and Taylor, J. and Zicher, N. and Buchhave, L. A. and Caldwell, D. A. and Horner, J. and Llama, J. and Mortier, A. and Rajpaul, V. M. and Stassun, K. and Sporer, A. and Tkachenko, A. and Jenkins, J. M. and Latham, D. and Ricker, G. and Seager, S. and Winn, J. and Alhassan, S. and Baeten, E. M. L. and Bean, S. J. and Bundy, D. M. and Efremov, V. and Ferstenou, R. and Goodwin, B. L. and Hof, M. and Hoffman, T. and Hubert, A. and Lau, L. and Lee, S. and Maetschke, D. and Peltsch, K. and Rubio-Alfaro, C. and Wilson, G. M.},
	month = aug,
	year = {2021},
	keywords = {methods: statistical, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics, HD 152843, stars: fundamental parameters, stars: individual: TIC 349488688},
	pages = {1827--1840},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/3B93SZBZ/Eisner et al. - 2021 - Planet Hunters TESS III two transiting planets ar.pdf:application/pdf},
}

@article{2021ApJS..253...11P,
	title = {{TESS} {Observations} of {Cepheid} {Stars}: {First} {Light} {Results}},
	volume = {253},
	issn = {0067-0049},
	shorttitle = {{TESS} {Observations} of {Cepheid} {Stars}},
	url = {https://ui.adsabs.harvard.edu/abs/2021ApJS..253...11P},
	doi = {10.3847/1538-4365/abd4e3},
	abstract = {We present the first analysis of Cepheid stars observed by the TESS space mission in Sectors 1{\textendash}5. Our sample consists of 25 pulsators: ten fundamental mode, three overtone and two double-mode classical Cepheids, plus three type II and seven anomalous Cepheids. The targets were chosen from fields with different stellar densities, both from the Galactic field and from the Magellanic System. Three targets have 2 minutes cadence light curves available by the TESS Science Processing Operations Center: for the rest, we prepared custom light curves from the full-frame images with our own differential photometric FITSH pipeline. Our main goal was to explore the potential and the limitations of TESS concerning the various subtypes of Cepheids. We detected many low-amplitude features: weak modulation, period jitter, and timing variations due to light-time effect. We also report signs of nonradial modes and the first discovery of such a mode in an anomalous Cepheid, the overtone star XZ Cet, which we then confirmed with ground-based multicolor photometric measurements. We prepared a custom photometric solution to minimize saturation effects in the bright fundamental-mode classical Cepheid, $\beta$ Dor with the lightkurve software, and we revealed strong evidence of cycle-to-cycle variations in the star. In several cases, however, fluctuations in the pulsation could not be distinguished from instrumental effects, such as contamination from nearby sources, which also varies between sectors. Finally, we discuss how precise light-curve shapes will be crucial not only for classification purposes but also to determine physical properties of these stars.},
	urldate = {2021-08-23},
	journal = {The Astrophysical Journal Supplement Series},
	author = {Plachy, E. and P{\'a}l, A. and B{\'o}di, A. and Szab{\'o}, P. and Moln{\'a}r, L. and Szabados, L. and Benk{\H o}, J. M. and Anderson, R. I. and Bellinger, E. P. and Bhardwaj, A. and Ebadi, M. and Gazeas, K. and Hambsch, F. -J. and Hasanzadeh, A. and Jurkovic, M. I. and Kalaee, M. J. and Kervella, P. and Kolenberg, K. and Miko{\l }ajczyk, P. and Nardetto, N. and Nemec, J. M. and Netzel, H. and Ngeow, C. -C. and Ozuyar, D. and Pascual-Granado, J. and Pilecki, B. and Ripepi, V. and Skarka, M. and Smolec, R. and S{\'o}dor, {\'A}. and Szab{\'o}, R. and Christensen-Dalsgaard, J. and Jenkins, J. M. and Kjeldsen, H. and Ricker, G. R. and Vanderspek, R.},
	month = mar,
	year = {2021},
	note = {ADS Bibcode: 2021ApJS..253...11P},
	keywords = {Astrophysics - Solar and Stellar Astrophysics, Cepheid variable stars, Stellar photometry, Stellar pulsations},
	pages = {11},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/SV2MAI85/Plachy et al. - 2021 - TESS Observations of Cepheid Stars First Light Re.pdf:application/pdf},
}

@article{2019MNRAS.489L..80B,
	title = {Multiple populations in integrated light spectroscopy of intermediate-age clusters},
	volume = {489},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489L..80B},
	doi = {10.1093/mnrasl/slz130},
	abstract = {The presence of star-to-star light-element abundance variations (also known as multiple populations, MPs) appears to be ubiquitous within old and massive clusters in the Milky Way and all studied nearby galaxies. Most previous studies have focused on resolved images or spectroscopy of individual stars, although there has been significant effort in the past few years to look for multiple population signatures in integrated light spectroscopy. If proven feasible, integrated light studies offer a potential way to vastly open parameter space, as clusters out to 10s of Mpc can be studied. We use the Na D lines in the integrated spectra of two clusters with similar ages (2-3 Gyr) but very different masses: NGC 1978 (\~{}3 {\texttimes} 105 M?) in the Large Magellanic Cloud and G114 (1.7 {\texttimes} 107 M?) in NGC 1316. For NGC 1978, our findings agree with resolved studies of individual stars that did not find evidence for Na spreads. However, for G114, we find clear evidence for the presence of multiple populations. The fact that the same anomalous abundance patterns are found in both the intermediate age and ancient globular clusters lends further support to the notion that young massive clusters are effectively the same as the ancient globular clusters, only separated in age.},
	urldate = {2021-09-11},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Bastian, Nate and Usher, Christopher and Kamann, Sebastian and Lardo, Carmela and Larsen, S{\o}ren S. and Cabrera-Ziri, Ivan and Chantereau, William and Martocchia, Silvia and Salaris, Maurizio and Schiavon, Ricardo P. and Asa'd, Randa and Hilker, Michael},
	month = oct,
	year = {2019},
	note = {ADS Bibcode: 2019MNRAS.489L..80B},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star clusters: general},
	pages = {L80--L85},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/MC4HW2UE/Bastian et al. - 2019 - Multiple populations in integrated light spectrosc.pdf:application/pdf},
}

@article{2020IAUS..351..317L,
	title = {Chemical composition of globular clusters in dwarf galaxies},
	volume = {351},
	url = {https://ui.adsabs.harvard.edu/abs/2020IAUS..351..317L},
	doi = {10.1017/S1743921319006604},
	abstract = {This contribution gives an update on on-going efforts to characterise the detailed chemical abundances of Local Group globular clusters (GCs) from integrated-light spectroscopy. Observations of a sample of 20 GCs so far, located primarily within dwarf galaxies, show that at low metallicities the [$\alpha$/Fe] ratios are generally indistinguishable from those in Milky Way GCs. However, the "knee" above which [$\alpha$/Fe] decreases towards Solar-scaled values occurs at lower metallicities in the dwarfs, implying that GCs follow the same trends seen in field stars. Efforts are underway to establish NLTE corrections for integrated-light abundance measurements, and preliminary results for Mn are discussed.},
	urldate = {2021-09-11},
	author = {Larsen, S{\o}ren S.},
	month = jan,
	year = {2020},
	note = {Conference Name: Star Clusters: From the Milky Way to the Early Universe
ADS Bibcode: 2020IAUS..351..317L},
	keywords = {galaxies: star clusters: general, galaxies: abundances, techniques: spectroscopic},
	pages = {317--320},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/MQFFP29T/Larsen - 2020 - Chemical composition of globular clusters in dwarf.pdf:application/pdf},
}

@article{2008AJ....136.2782L,
	title = {The {Star} {Formation} {Efficiency} in {Nearby} {Galaxies}: {Measuring} {Where} {Gas} {Forms} {Stars} {Effectively}},
	volume = {136},
	issn = {0004-6256},
	shorttitle = {The {Star} {Formation} {Efficiency} in {Nearby} {Galaxies}},
	url = {https://ui.adsabs.harvard.edu/abs/2008AJ....136.2782L},
	doi = {10.1088/0004-6256/136/6/2782},
	abstract = {We measure the star formation efficiency (SFE), the star formation rate (SFR) per unit of gas, in 23 nearby galaxies and compare it with expectations from proposed star formation laws and thresholds. We use H I maps from The H I Nearby Galaxy Survey (THINGS) and derive H2 maps of CO measured by HERA CO-Line Extragalactic Survey and Berkeley-Illinois-Maryland Association Survey of Nearby Galaxies. We estimate the SFR by combining Galaxy Evolution Explorer (GALEX) far-ultraviolet maps and the Spitzer Infrared Nearby Galaxies Survey (SINGS) 24 $\mu$m maps, infer stellar surface density profiles from SINGS 3.6 $\mu$m data, and use kinematics from THINGS. We measure the SFE as a function of the free fall and orbital timescales, midplane gas pressure, stability of the gas disk to collapse (including the effects of stars), the ability of perturbations to grow despite shear, and the ability of a cold phase to form. In spirals, the SFE of H2 alone is nearly constant at (5.25 {\textpm} 2.5) {\texttimes} 10-10 yr-1 (equivalent to an H2 depletion time of 1.9 {\texttimes} 109 yr) as a function of all of these variables at our 800 pc resolution. Where the interstellar medium (ISM) is mostly H I, however, the SFE decreases with increasing radius in both spiral and dwarf galaxies, a decline reasonably described by an exponential with scale length 0.2r 25-0.25r 25. We interpret this decline as a strong dependence of giant molecular cloud (GMC) formation on environment. The ratio of molecular-to-atomic gas appears to be a smooth function of radius, stellar surface density, and pressure spanning from the H2-dominated to H I-dominated ISM. The radial decline in SFE is too steep to be reproduced only by increases in the free-fall time or orbital time. Thresholds for large-scale instability suggest that our disks are stable or marginally stable and do not show a clear link to the declining SFE. We suggest that ISM physics below the scales that we observe{\textemdash}phase balance in the H I, H2 formation and destruction, and stellar feedback{\textemdash}governs the formation of GMCs from H I.},
	urldate = {2021-09-17},
	journal = {The Astronomical Journal},
	author = {Leroy, Adam K. and Walter, Fabian and Brinks, Elias and Bigiel, Frank and de Blok, W. J. G. and Madore, Barry and Thornley, M. D.},
	month = dec,
	year = {2008},
	note = {ADS Bibcode: 2008AJ....136.2782L},
	keywords = {Astrophysics, galaxies: ISM, stars: formation, galaxies: evolution, radio lines: galaxies},
	pages = {2782--2845},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/C7VTPVZM/Leroy et al. - 2008 - The Star Formation Efficiency in Nearby Galaxies .pdf:application/pdf},
}

@article{berta_molecular_2013,
	title = {Molecular gas mass functions of normal star-forming galaxies since z {\textasciitilde} 3},
	volume = {555},
	issn = {0004-6361},
	url = {https://ui.adsabs.harvard.edu/abs/2013A%26A...555L...8B/abstract},
	doi = {10.1051/0004-6361/201321776},
	abstract = {We used deep far-infrared data from the PEP/GOODS-Herschel surveys and restframe ultraviolet photometry to study the evolution of the molecular gas mass function of normal star-forming galaxies. Computing the molecular gas mass, M{\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater}, by scaling star formation rates through depletion timescales, or combining infrared (IR) luminosity and obscuration properties as described in the literature, we obtained M{\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater} for roughly 700, z = 0.2-3.0 galaxies near the star-forming main sequence. The number density of galaxies follows a Schechter function of M{\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater}. The characteristic mass M{\textless}SUP{\textgreater} * {\textless}/SUP{\textgreater} is found to strongly evolve up to z {\textasciitilde} 1 and then flatten at earlier epochs, resembling the IR luminosity evolution of similar objects. At z {\textasciitilde} 1, our result is supported by an estimate based on the stellar mass function of star-forming galaxies and gas fraction scalings from the PHIBSS survey. We compared our measurements with results from current models, finding better agreement with those that are treating star formation laws directly rather than in post-processing. Integrating the mass function, we studied the evolution of the M{\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater} density and its density parameter $\Omega${\textless}SUB{\textgreater}mol{\textless}/SUB{\textgreater}. {\textless}P /{\textgreater}Herschel is an ESA space observatory with science instruments provided by European-led Principal Investigator consortia and with important participation from NASA.},
	language = {en},
	urldate = {2021-09-20},
	journal = {Astronomy \&amp; Astrophysics, Volume 555, id.L8, {\textless}NUMPAGES{\textgreater}5{\textless}/NUMPAGES{\textgreater} pp.},
	author = {Berta, S. and Lutz, D. and Nordon, R. and Genzel, R. and Magnelli, B. and Popesso, P. and Rosario, D. and Saintonge, A. and Wuyts, S. and Tacconi, L. J.},
	month = jul,
	year = {2013},
	pages = {L8},
	file = {Snapshot:/Users/Tobin/Zotero/storage/E8YKWW2Q/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/8UX6K7L2/Berta et al. - 2013 - Molecular gas mass functions of normal star-formin.pdf:application/pdf},
}

@article{2019MNRAS.486.3134K,
	title = {The {E}-{MOSAICS} project: tracing galaxy formation and assembly with the age-metallicity distribution of globular clusters},
	volume = {486},
	issn = {0035-8711},
	shorttitle = {The {E}-{MOSAICS} project},
	url = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.3134K},
	doi = {10.1093/mnras/stz968},
	abstract = {We present 25 cosmological zoom-in simulations of Milky-Way-mass galaxies in the `MOdelling Star cluster population Assembly In Cosmological Simulations within EAGLE' (E-MOSAICS) project. E-MOSAICS couples a detailed physical model for the formation, evolution, and disruption of star clusters to the EAGLE galaxy formation simulations. This enables following the co-formation and co-evolution of galaxies and their star cluster populations, thus realizing the long-standing promise of using globular clusters (GCs) as tracers of galaxy formation and assembly. The simulations show that the age-metallicity distributions of GC populations exhibit strong galaxy-to-galaxy variations, resulting from differences in their evolutionary histories. We develop a formalism for systematically constraining the assembly histories of galaxies using GC age-metallicity distributions. These distributions are characterized through 13 metrics that we correlate with 30 quantities describing galaxy formation and assembly (e.g. halo properties, formation/assembly redshifts, stellar mass assembly time-scales, galaxy merger statistics), resulting in 20 statistically (highly) significant correlations. The GC age-metallicity distribution is a sensitive probe of the mass growth, metal enrichment, and minor merger history of the host galaxy. No such relation is found between GCs and major mergers, which play a sub-dominant role in GC formation for Milky-Way-mass galaxies. Finally, we show how the GC age-metallicity distribution enables the reconstruction of the host galaxy's merger tree, allowing us to identify all progenitors with masses M\_*? 10{\textasciicircum}8 M\_? for redshifts 1 <= z <= 2.5. These results demonstrate that cosmological simulations of the co-formation and co-evolution of GCs and their host galaxies successfully unlock the potential of GCs as quantitative tracers of galaxy formation and assembly.},
	urldate = {2021-09-20},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kruijssen, J. M. Diederik and Pfeffer, Joel L. and Crain, Robert A. and Bastian, Nate},
	month = jul,
	year = {2019},
	note = {ADS Bibcode: 2019MNRAS.486.3134K},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star formation, galaxies: evolution, galaxies: formation, globular clusters: general, galaxies: haloes},
	pages = {3134--3179},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/G9KB2CF2/Kruijssen et al. - 2019 - The E-MOSAICS project tracing galaxy formation an.pdf:application/pdf},
}

@article{2019MNRAS.486.3180K,
	title = {The formation and assembly history of the {Milky} {Way} revealed by its globular cluster population},
	volume = {486},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.3180K},
	doi = {10.1093/mnras/sty1609},
	abstract = {We use the age-metallicity distribution of 96 Galactic globular clusters (GCs) to infer the formation and assembly history of the Milky Way (MW), culminating in the reconstruction of its merger tree. Based on a quantitative comparison of the Galactic GC population to the 25 cosmological zoom-in simulations of MW-mass galaxies in the E-MOSAICS project, which self-consistently model the formation and evolution of GC populations in a cosmological context, we find that the MW assembled quickly for its mass, reaching \{25, 50\} per cent of its present-day halo mass already at z = \{3, 1.5\} and half of its present-day stellar mass at z = 1.2. We reconstruct the MW's merger tree from its GC age-metallicity distribution, inferring the number of mergers as a function of mass ratio and redshift. These statistics place the MW's assembly rate among the 72th-94th percentile of the E-MOSAICS galaxies, whereas its integrated properties (e.g. number of mergers, halo concentration) match the median of the simulations. We conclude that the MW has experienced no major mergers (mass ratios {\textgreater}1:4) since z \~{} 4, sharpening previous limits of z \~{} 2. We identify three massive satellite progenitors and constrain their mass growth and enrichment histories. Two are proposed to correspond to Sagittarius (a few 108 M?) and the GCs formerly associated with Canis Major (\~{} 10{\textasciicircum}9 M\_?). The third satellite has no known associated relic and was likely accreted between z = 0.6 and 1.3. We name this enigmatic galaxy Kraken and propose that it is the most massive satellite (M\_*\~{} 2{\texttimes} 10{\textasciicircum}9 M\_?) ever accreted by the MW. We predict that \~{}40 per cent of the Galactic GCs formed ex situ (in galaxies with masses M* = 2 {\texttimes} 107-2{\texttimes} 10{\textasciicircum}9 M\_?), with 6 {\textpm} 1 being former nuclear clusters.},
	urldate = {2021-09-20},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kruijssen, J. M. Diederik and Pfeffer, Joel L. and Reina-Campos, Marta and Crain, Robert A. and Bastian, Nate},
	month = jul,
	year = {2019},
	note = {ADS Bibcode: 2019MNRAS.486.3180K},
	keywords = {Astrophysics - Astrophysics of Galaxies, Galaxy: halo, galaxies: star formation, globular clusters: general, Galaxy: stellar content, Galaxy: evolution, Galaxy: formation},
	pages = {3180--3202},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/3UC8BBWK/Kruijssen et al. - 2019 - The formation and assembly history of the Milky Wa.pdf:application/pdf},
}

@article{2020MNRAS.499.3267A,
	title = {Star cluster formation in the most extreme environments: insights from the {HiPEEC} survey},
	volume = {499},
	issn = {0035-8711},
	shorttitle = {Star cluster formation in the most extreme environments},
	url = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.3267A},
	doi = {10.1093/mnras/staa2380},
	abstract = {We present the Hubble imaging Probe of Extreme Environments and Clusters (HiPEEC) survey. We fit HST NUV to NIR broad-band and H $\alpha$ fluxes to derive star cluster ages, masses, and extinctions and determine the star formation rate (SFR) of six merging galaxies. These systems are excellent laboratories to trace cluster formation under extreme gas physical conditions, rare in the local Universe, but typical for star-forming galaxies at cosmic noon. We detect clusters with ages of 1-500 Myr and masses that exceed 107 M?. The recent cluster formation history and their distribution within the host galaxies suggest that systems such as NGC 34, NGC 1614, and NGC 4194 are close to their final coalescing phase, while NGC 3256, NGC 3690, and NGC 6052 are at an earlier/intermediate stage. A Bayesian analysis of the cluster mass function in the age interval 1-100 Myr provides strong evidence in four of the six galaxies that an exponentially truncated power law better describes the observed mass distributions. For two galaxies, the fits are inconclusive due to low number statistics. We determine power-law slopes $\beta$ \~{} -1.5 to -2.0 and truncation masses, Mc, between 106 and a few times 107 M?, among the highest values reported in the literature. Advanced mergers have higher Mc than early/intermediate merger stage galaxies, suggesting rapid changes in the dense gas conditions during the merger. We compare the total stellar mass in clusters to the SFR of the galaxy, finding that these systems are among the most efficient environments to form star clusters in the local Universe.},
	urldate = {2021-09-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Adamo, A. and Hollyhead, K. and Messa, M. and Ryon, J. E. and Bajaj, V. and Runnholm, A. and Aalto, S. and Calzetti, D. and Gallagher, J. S. and Hayes, M. J. and Kruijssen, J. M. D. and K{\"o}nig, S. and Larsen, S. S. and Melinder, J. and Sabbi, E. and Smith, L. J. and {\"O}stlin, G.},
	month = dec,
	year = {2020},
	note = {ADS Bibcode: 2020MNRAS.499.3267A},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star clusters: general, galaxies: starburst, galaxies: interactions, star clusters: statistics},
	pages = {3267--3294},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/DAW8WVE3/Adamo et al. - 2020 - Star cluster formation in the most extreme environ.pdf:application/pdf},
}

@article{beasley_evidence_2015,
	title = {Evidence for temporal evolution in the {M33} disc as traced by its star clusters},
	volume = {451},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.3400B},
	doi = {10.1093/mnras/stv943},
	abstract = {We present precision radial velocities and stellar population parameters for 77 star clusters in the Local Group galaxy M33. Our Gran Telescopio de Canarias and William Herschel Telescope observations sample both young, massive clusters and known/candidate globular clusters (GCs), spanning ages \~{}106-1010 yr, and metallicities, [M/H] \~{} -1.7 to solar. The cluster system exhibits an age-metallicity relation; the youngest clusters are the most metal rich. When compared to H I data, clusters with [M/H] \~{} -1.0 and younger than \~{}4 Gyr are clearly identified as a disc population. The clusters show evidence for strong time evolution in the disc radial metallicity gradient (d[M/H]dt/dR = 0.03 dex kpc-1 Gyr-1). The oldest clusters have stronger, more negative gradients than the youngest clusters in M33. The clusters also show a clear age-velocity dispersion relation. The line-of-sight velocity dispersions of the clusters increases with age similar to Milky Way open clusters and stars. The general shape of the relation is reproduced by disc heating simulations, and the similarity between the relations in M33 and the Milky Way suggests that heating by substructure and cooling of the interstellar medium both play a role in shaping this relation. We identify 12 `classical' GCs, six of which are newly identified GC candidates. The GCs are more metal rich than Milky Way halo clusters, and show weak rotation. The inner (R {\textless} 4.5 kpc) GCs exhibit a steep radial metallicity gradient (d[M/H]/dR = -0.29 {\textpm} 0.11 dex kpc-1) and an exponential-like surface density profile. We argue that these inner GCs are thick disc rather than halo objects.},
	urldate = {2021-09-23},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Beasley, Michael A. and San Roman, Izaskun and Gallart, Carme and Sarajedini, Ata and Aparicio, Antonio},
	month = aug,
	year = {2015},
	note = {ADS Bibcode: 2015MNRAS.451.3400B},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: star clusters: general, Local Group},
	pages = {3400--3418},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/99TDE8EY/Beasley et al. - 2015 - Evidence for temporal evolution in the M33 disc as.pdf:application/pdf},
}

@article{rosolowsky_high-resolution_2007,
	title = {High-{Resolution} {Molecular} {Gas} {Maps} of {M33}},
	volume = {661},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2007ApJ...661..830R},
	doi = {10.1086/516621},
	abstract = {New observations of CO (J=1--{\textgreater}0) line emission from M33, using the 25 element BEARS focal plane array at the Nobeyama Radio Observatory 45 m telescope, in conjunction with existing maps from the BIMA interferometer and the FCRAO 14 m telescope, give the highest resolution (13") and most sensitive ($\sigma$rms{\textasciitilde}60 mK) maps to date of the distribution of molecular gas in the central 5.5 kpc of the galaxy. A new catalog of giant molecular clouds (GMCs) has a completeness limit of 1.3{\texttimes}105 Msolar. The fraction of molecular gas found in GMCs is a strong function of radius in the galaxy, declining from 60\% in the center to 20\% at galactocentric radius Rgal{\textasciitilde}4 kpc. Beyond that radius, GMCs are nearly absent, although molecular gas exists. Most (90\%) of the emission from low-mass clouds is found within 100 pc projected separation of a GMC. In an annulus 2.1 kpcgal{\textless}4.1 kpc, GMC masses follow a power-law distribution with index -2.1. Inside that radius, the mass distribution is truncated, and clouds more massive than 8{\texttimes}105 Msolar are absent. The cloud mass distribution shows no significant difference in the grand-design spiral arms versus the interarm region. The CO surface brightness ratio for the arm to interarm regions is 1.5, typical of other flocculent galaxies.},
	urldate = {2021-09-23},
	journal = {The Astrophysical Journal},
	author = {Rosolowsky, Erik and Keto, Eric and Matsushita, Satoki and Willner, S. P.},
	month = jun,
	year = {2007},
	note = {ADS Bibcode: 2007ApJ...661..830R},
	keywords = {Astrophysics, Catalogs, Galaxies: Individual: Messier Number: M33, ISM: Clouds, Radio Lines: ISM},
	pages = {830--844},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/6T2ELCT6/Rosolowsky et al. - 2007 - High-Resolution Molecular Gas Maps of M33.pdf:application/pdf},
}

@article{utomo_origin_2019,
	title = {The {Origin} of {Interstellar} {Turbulence} in {M33}},
	volume = {871},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2019ApJ...871...17U},
	doi = {10.3847/1538-4357/aaf582},
	abstract = {We utilize the multi-wavelength data of M33 to study the origin of turbulence in its interstellar medium. We find that the H I turbulent energy surface density inside 8 kpc is \~{}1-3 {\texttimes} 1046 erg pc-2, and has no strong dependence on galactocentric radius because of the lack of variation in H I surface density and H I velocity dispersion. Then, we consider the energies injected by supernovae (SNe), the magneto-rotational instability (MRI), and the gravity-driven turbulence from accreted materials as the sources of turbulent energy. For a constant dissipation time of turbulence, the SNe energy can maintain turbulence inside \~{}4 kpc radius (equivalent to \~{}0.5 R 25), while the MRI energy is always smaller than the turbulent energy within 8 kpc radius. However, when we let the dissipation time to be equal to the crossing time of turbulence across the H I scale height, the SNe energy is enough to maintain turbulence out to 7 kpc radius, and the sum of SNe and MRI energies is able to maintain turbulence out to 8 kpc radius. Due to lack of constraint in the mass accretion rate through the disk of M33, we cannot rule out the accretion driven turbulence as a possible source of energy. Furthermore, by resolving individual giant molecular clouds in M33, we also show that the SNe energy can maintain turbulence within individual molecular clouds with \~{}1\% of coupling efficiency. This result strengthens the proposition that stellar feedback is an important source of energy to maintain turbulence in nearby galaxies.},
	urldate = {2021-09-23},
	journal = {The Astrophysical Journal},
	author = {Utomo, Dyas and Blitz, Leo and Falgarone, Edith},
	month = jan,
	year = {2019},
	note = {ADS Bibcode: 2019ApJ...871...17U},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: individual: M33, ISM: kinematics and dynamics, ISM: structure},
	pages = {17},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/5W5MSWXX/Utomo et al. - 2019 - The Origin of Interstellar Turbulence in M33.pdf:application/pdf},
}

@article{koch_kinematics_2018,
	title = {Kinematics of the atomic {ISM} ifigun {M33} on 80 pc scales},
	volume = {479},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479.2505K},
	doi = {10.1093/mnras/sty1674},
	abstract = {We present new L-band (1-2 GHz) observations of the nearby spiral galaxy M33 with 80 pc resolution obtained with the Karl G. Jansky Very Large Array. The H I observations, combined with H I measurements from the Green Bank Telescope, improve the spectral resolution and sensitivity (2.8 K rms noise in a 0.2 \{km s{\textasciicircum}\{-1\}\} channel) compared to previous observations. We find individual profiles are usually non-Gaussian, harbouring line wings, multiple components, and asymmetries. Given this spectral complexity, we quantify the motions in the atomic interstellar medium through moment analysis of the spectra and fits to aligned, stacked profiles. The measured value of the H I line width depends strongly on the method used, with the velocity stacked profiles aligned to the peak velocity giving the minimum value of $\sigma$ = 7 \{km s{\textasciicircum}\{-1\}\} and all other methods giving higher values ($\sigma$ \~{} 10 \{km s{\textasciicircum}\{-1\}\}). All measurements of the line width show a shallow radial trend, with $\sigma$ decreasing by \~{}2 \{km s{\textasciicircum}\{-1\}\} from Rgal = 0 to Rgal = 8 kpc. We consider a number of energy sources that might maintain the line width against turbulent dissipation, but no single source is adequate. We find excess emission relative to a Gaussian in the stacked profile line wings, ranging from 9 per cent to 26 per cent depending on how the spectra are aligned. By splitting the line wings into symmetric and asymmetric components, we find that the lagging rotational disc accounts for one-third of the line wing flux. We also find emission far from the rotation-axis of the galaxy in multiple discrete H I clouds, including a filament with a projected length of \~{}8 kpc.},
	urldate = {2021-09-23},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Koch, Eric W. and Rosolowsky, Erik W. and Lockman, Felix J. and Kepley, Amanda A. and Leroy, Adam and Schruba, Andreas and Braine, Jonathan and Dalcanton, Julianne and Johnson, Megan C. and Stanimirovi{\'c}, Sne{\v z}ana},
	month = sep,
	year = {2018},
	note = {ADS Bibcode: 2018MNRAS.479.2505K},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: ISM, galaxies: individual: M33, ISM: kinematics and dynamics, radio lines: ISM},
	pages = {2505--2533},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/79IJJJ6H/Koch et al. - 2018 - Kinematics of the atomic ISM ifigun M33 on 80 pc s.pdf:application/pdf},
}

@article{kruijssen_fraction_2012,
	title = {On the fraction of star formation occurring in bound stellar clusters},
	volume = {426},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.426.3008K},
	doi = {10.1111/j.1365-2966.2012.21923.x},
	abstract = {We present a theoretical framework in which bound stellar clusters arise naturally at the high-density end of the hierarchy of the interstellar medium (ISM). Due to short free-fall times, these high-density regions achieve high local star formation efficiencies, enabling them to form bound clusters. Star-forming regions of lower density remain substructured and gas-rich, ending up unbound when the residual gas is expelled. Additionally, the tidal perturbation of star-forming regions by nearby, dense giant molecular clouds imposes a minimum density contrast required for the collapse to a bound cluster. The fraction of all star formation that occurs in bound stellar clusters (the cluster formation efficiency, hereafter CFE) follows by integration of these local clustering and survival properties over the full density spectrum of the ISM, and hence is set by galaxy-scale physics. We derive the CFE as a function of observable galaxy properties, and find that it increases with the gas surface density, from $\Gamma$ \~{} 1 per cent in low-density galaxies to a peak value of $\Gamma$ \~{} 70 per cent at densities of $\Sigma$g \~{} 103 M? pc-2. This explains the observation that the CFE increases with the star formation rate density in nearby dwarf, spiral and starburst galaxies. Indeed, comparing our model results with observed galaxies yields excellent agreement. The model is applied further by calculating the spatial variation of the CFE within single galaxies. We also consider the variation of the CFE with cosmic time and show that it increases with redshift, peaking in high-redshift, gas-rich disc galaxies. It is estimated that up to 30-35 per cent of all stars in the Universe once formed in bound stellar clusters. We discuss how our theory can be verified with Gaia and ALMA, and provide possible implementations for theoretical work and for simulations of galaxy formation and evolution.},
	urldate = {2021-09-23},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kruijssen, J. M. Diederik},
	month = nov,
	year = {2012},
	note = {ADS Bibcode: 2012MNRAS.426.3008K},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: ISM, stars: formation, galaxies: star clusters: general, galaxies: stellar content, galaxies: starburst, Astrophysics - Cosmology and Nongalactic Astrophysics},
	pages = {3008--3040},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/F9KKYI6F/Kruijssen - 2012 - On the fraction of star formation occurring in bou.pdf:application/pdf},
}

@article{de_grijs_clustering_2014,
	title = {Clustering of {Local} {Group} {Distances}: {Publication} {Bias} or {Correlated} {Measurements}? {II}. {M31} and {Beyond}},
	volume = {148},
	issn = {0004-6256},
	shorttitle = {Clustering of {Local} {Group} {Distances}},
	url = {https://ui.adsabs.harvard.edu/abs/2014AJ....148...17D},
	doi = {10.1088/0004-6256/148/1/17},
	abstract = {The accuracy of extragalactic distance measurements ultimately depends on robust, high-precision determinations of the distances to the galaxies in the local volume. Following our detailed study addressing possible publication bias in the published distance determinations to the Large Magellanic Cloud (LMC), here we extend our distance range of interest to include published distance moduli to M31 and M33, as well as to a number of their well-known dwarf galaxy companions. We aim at reaching consensus on the best, most homogeneous, and internally most consistent set of Local Group distance moduli to adopt for future, more general use based on the largest set of distance determinations to individual Local Group galaxies available to date. Based on a careful, statistically weighted combination of the main stellar population tracers (Cepheids, RR Lyrae variables, and the magnitude of the tip of the red-giant branch), we derive a recommended distance modulus to M31 of (m-M)\_0{\textasciicircum}M31 = 24.46 +/- 0.10 mag{\textemdash}adopting as our calibration an LMC distance modulus of (m-M)\_0{\textasciicircum}LMC = 18.50 mag{\textemdash}and a fully internally consistent set of benchmark distances to key galaxies in the local volume, enabling us to establish a robust and unbiased, near-field extragalactic distance ladder.},
	urldate = {2021-09-30},
	journal = {The Astronomical Journal},
	author = {de Grijs, Richard and Bono, Giuseppe},
	month = jul,
	year = {2014},
	note = {ADS Bibcode: 2014AJ....148...17D},
	keywords = {astronomical databases: miscellaneous, Astrophysics - Astrophysics of Galaxies, distance scale, galaxies: distances and redshifts, galaxies: individual: M31 M32 M33 NGC 147 NGC 185 NGC 205 IC 10 IC 1613},
	pages = {17},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/V8DGVGTR/de Grijs and Bono - 2014 - Clustering of Local Group Distances Publication B.pdf:application/pdf},
}

@article{kelly_aspects_2007,
	title = {Some {Aspects} of {Measurement} {Error} in {Linear} {Regression} of {Astronomical} {Data}},
	volume = {665},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2007ApJ...665.1489K},
	doi = {10.1086/519947},
	abstract = {I describe a Bayesian method to account for measurement errors in linear regression of astronomical data. The method allows for heteroscedastic and possibly correlated measurement errors and intrinsic scatter in the regression relationship. The method is based on deriving a likelihood function for the measured data, and I focus on the case when the intrinsic distribution of the independent variables can be approximated using a mixture of Gaussian functions. I generalize the method to incorporate multiple independent variables, nondetections, and selection effects (e.g., Malmquist bias). A Gibbs sampler is described for simulating random draws from the probability distribution of the parameters, given the observed data. I use simulation to compare the method with other common estimators. The simulations illustrate that the Gaussian mixture model outperforms other common estimators and can effectively give constraints on the regression parameters, even when the measurement errors dominate the observed scatter, source detection fraction is low, or the intrinsic distribution of the independent variables is not a mixture of Gaussian functions. I conclude by using this method to fit the X-ray spectral slope as a function of Eddington ratio using a sample of 39 z{\textless}{\textasciitilde}0.8 radio-quiet quasars. I confirm the correlation seen by other authors between the radio-quiet quasar X-ray spectral slope and the Eddington ratio, where the X-ray spectral slope softens as the Eddington ratio increases. IDL routines are made available for performing the regression.},
	urldate = {2021-09-30},
	journal = {The Astrophysical Journal},
	author = {Kelly, Brandon C.},
	month = aug,
	year = {2007},
	note = {ADS Bibcode: 2007ApJ...665.1489K},
	keywords = {Astrophysics, Methods: Data Analysis, Methods: Numerical, Methods: Statistical},
	pages = {1489--1506},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/ZD2F5NFW/Kelly - 2007 - Some Aspects of Measurement Error in Linear Regres.pdf:application/pdf},
}

@article{marigo_evolution_2008,
	title = {Evolution of asymptotic giant branch stars. {II}. {Optical} to far-infrared isochrones with improved {TP}-{AGB} models},
	volume = {482},
	issn = {0004-6361},
	url = {https://ui.adsabs.harvard.edu/abs/2008A%26A...482..883M/abstract},
	doi = {10.1051/0004-6361:20078467},
	abstract = {We present a large set of theoretical isochrones, whose distinctive features mostly reside on the greatly-improved treatment of the thermally-pulsing asymptotic giant branch (TP-AGB) phase. Essentially, we have coupled the TP-AGB tracks described in Paper I, at their stages of pre-flash quiescent H-shell burning, with the evolutionary tracks for the previous evolutionary phases from Girardi et al. (2000, A\&amp;AS, 141, 371). Theoretical isochrones for any intermediate value of age and metallicity are then derived by interpolation in the grids. We take care that the isochrones keep, to a good level of detail, the several peculiarities present in these TP-AGB tracks - e.g., the cool tails of C-type stars owing to the use of proper molecular opacities as convective dredge-up occurs along the TP-AGB; the bell-shaped sequences in the Hertzsprung-Russell (HR) diagram for stars with hot-bottom burning; the changes of pulsation mode between fundamental and first overtone; the sudden changes of mean mass-loss rates as the surface chemistry changes from M- to C-type; etc. Theoretical isochrones are then converted to about 20 different photometric systems - including traditional ground-based systems, and those of recent major wide-field surveys such as SDSS, OGLE, DENIS, 2MASS, UKIDSS, etc., - by means of synthetic photometry applied to an updated library of stellar spectra, suitably extended to include C-type stars. Finally, we correct the predicted photometry for the effect of circumstellar dust during the mass-losing stages of the AGB evolution, which allows us to improve the results for the optical-to-infrared systems, and to simulate mid- and far-IR systems such as those of Spitzer and AKARI. We illustrate the most striking properties of these isochrones by means of basic comparisons with observational data for the Milky Way disc and the Magellanic Clouds. Access to the data is provided both via a web repository of static tables (http://stev.oapd.inaf.it/dustyAGB07 and CDS), and via an interactive web interface (http://stev.oapd.inaf.it/cmd), which provides tables for any intermediate value of age and metallicity, for several photometric systems, and for different choices of dust properties.},
	language = {en},
	number = {3},
	urldate = {2021-09-30},
	journal = {Astronomy and Astrophysics, Volume 482, Issue 3, 2008, pp.883-905},
	author = {Marigo, P. and Girardi, L. and Bressan, A. and Groenewegen, M. a. T. and Silva, L. and Granato, G. L.},
	month = may,
	year = {2008},
	pages = {883},
	file = {Snapshot:/Users/Tobin/Zotero/storage/7WHMWZ76/abstract.html:text/html;Full Text PDF:/Users/Tobin/Zotero/storage/W342E5WH/Marigo et al. - 2008 - Evolution of asymptotic giant branch stars. II. Op.pdf:application/pdf},
}

@article{rosolowsky_m33_2008,
	title = {The {M33} {Metallicity} {Project}: {Resolving} the {Abundance} {Gradient} {Discrepancies} in {M33}},
	volume = {675},
	issn = {0004-637X},
	shorttitle = {The {M33} {Metallicity} {Project}},
	url = {https://ui.adsabs.harvard.edu/abs/2008ApJ...675.1213R},
	doi = {10.1086/527407},
	abstract = {We present a new determination of the metallicity gradient in M33, based on Keck LRIS measurements of oxygen abundances using the temperature-sensitive emission line [O III] $\lambda$4363 in 61 H II regions. These data approximately triple the sample of direct oxygen abundances in M33. We find a central abundance of 12 + log (O/H) = 8.36 +/- 0.04 and a slope of -0.027 +/- 0.012 dex kpc-1, in agreement with infrared measurements of the neon abundance gradient but much shallower than most previous oxygen gradient measurements. There is substantial intrinsic scatter of 0.11 dex in the metallicity at any given radius in M33, which imposes a fundamental limit on the accuracy of gradient measurements that rely on small samples of objects. We also show that the ionization state of neon does not follow the ionization state of oxygen as is commonly assumed, suggesting that neon abundance measurements from optical emission lines require careful treatment of the ionization corrections. Data presented herein were obtained at the W. M. Keck Observatory, which is operated as a scientific partnership among the California Institute of Technology, the University of California, and the National Aeronautics and Space Administration. The Observatory was made possible by the generous financial support of the W. M. Keck Foundation.},
	urldate = {2021-09-30},
	journal = {The Astrophysical Journal},
	author = {Rosolowsky, Erik and Simon, Joshua D.},
	month = mar,
	year = {2008},
	note = {ADS Bibcode: 2008ApJ...675.1213R},
	keywords = {Astrophysics, galaxies: abundances, galaxies: individual: M33, galaxies: spiral, H II regions, ISM: abundances, ISM: evolution},
	pages = {1213--1222},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/JHSVT7IR/Rosolowsky and Simon - 2008 - The M33 Metallicity Project Resolving the Abundan.pdf:application/pdf},
}

@article{elmegreen_pressure_2009,
	title = {A pressure dependence for bound and unbound clusters},
	volume = {324},
	issn = {0004-640X},
	url = {https://ui.adsabs.harvard.edu/abs/2009Ap&SS.324...83E/abstract},
	doi = {10.1007/s10509-009-0131-6},
	abstract = {Hierarchical structure in gas and young stars produces clusters in high-density regions where the individual stellar orbits rapidly mix. For a fixed density at the onset of gas collapse (e.g. determined by changes in the ionization equilibrium and grain properties), the efficiency of star formation is automatically high in the high-density regions of giant molecular clouds. Thus, bound cluster formation follows somewhat trivially from hierarchical structure. The density where the efficiency is high enough to produce a bound cluster depends on the dispersion of the density probability distribution function (pdf), decreasing for higher dispersions and making bound cluster formation more likely. Similarly, the mass fraction of star formation in the form of bound clusters increases with the pdf dispersion. Because this dispersion is related to the turbulent Mach number, and also to the interstellar medium pressure and star-formation rate per unit volume, it follows that high-pressure or highly active regions tend to produce bound clusters, while low-pressure and inactive regions tend to produce stars in unbound associations.},
	language = {en},
	number = {2-4},
	urldate = {2021-10-08},
	journal = {Astrophysics and Space Science},
	author = {Elmegreen, Bruce G.},
	month = dec,
	year = {2009},
	pages = {83--89},
	file = {Snapshot:/Users/Tobin/Zotero/storage/LX7GEFIT/abstract.html:text/html},
}

@article{elmegreen_two_2018,
	title = {Two {Thresholds} for {Globular} {Cluster} {Formation} and the {Common} {Occurrence} of {Massive} {Clusters} in the {Early} {Universe}},
	volume = {869},
	issn = {0004-637X},
	url = {https://ui.adsabs.harvard.edu/abs/2018ApJ...869..119E},
	doi = {10.3847/1538-4357/aaed45},
	abstract = {Young massive clusters (YMCs) are usually accompanied by lower-mass clusters and unbound stars with a total mass equal to several tens times the mass of the YMC. If this was also true when globular clusters (GCs) formed, then their cosmic density implies that most star formation before redshift \~{}2 made a GC that lasted until today. Star-forming regions had to change after this time for the modern universe to be making very few YMCs. Here we consider the conditions needed for the formation of a \~{}106 M ? cluster. These include a star formation rate (SFR) inside each independent region that exceeds \~{}1 M ? yr-1 to sample the cluster mass function up to such a high mass, and an SFR per unit area of $\Sigma$SFR \~{} 1 M ? kpc-2 yr-1 to get the required high gas surface density from the Kennicutt-Schmidt relation, and therefore the required high pressure from the weight of the gas. High pressures are implied by the virial theorem at cluster densities. The ratio of these two quantities gives the area of a GC-forming region, \~{}1 kpc2, and the young stellar mass converted to a cloud mass gives a typical gas surface density of 500-1000 M ? pc-2. Observations of star-forming clumps in young galaxies are consistent with these numbers, suggesting that they formed today{\textquoteright}s GCs. Observations of the cluster cutoff mass in local galaxies agree with the maximum mass calculated from $\Sigma$SFR. Metal-poor stellar populations in local dwarf irregular galaxies confirm the dominant role of GC formation in building their young disks.},
	urldate = {2021-10-08},
	journal = {The Astrophysical Journal},
	author = {Elmegreen, Bruce G.},
	month = dec,
	year = {2018},
	note = {ADS Bibcode: 2018ApJ...869..119E},
	keywords = {Astrophysics - Astrophysics of Galaxies, galaxies: clusters: general, galaxies: star clusters: general, galaxies: star formation, globular clusters: general},
	pages = {119},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/IXGT8KDJ/Elmegreen - 2018 - Two Thresholds for Globular Cluster Formation and .pdf:application/pdf},
}

@article{kroupa_variation_2001,
	title = {On the variation of the initial mass function},
	volume = {322},
	issn = {0035-8711},
	url = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.322..231K},
	doi = {10.1046/j.1365-8711.2001.04022.x},
	abstract = {A universal initial mass function (IMF) is not intuitive, but so far no convincing evidence for a variable IMF exists. The detection of systematic variations of the IMF with star-forming conditions would be the Rosetta Stone for star formation. In this contribution an average or Galactic-field IMF is defined, stressing that there is evidence for a change in the power-law index at only two masses: near 0.5Msolar and near 0.08Msolar. Using this supposed universal IMF, the uncertainty inherent in any observational estimate of the IMF is investigated by studying the scatter introduced by Poisson noise and the dynamical evolution of star clusters. It is found that this apparent scatter reproduces quite well the observed scatter in power-law index determinations, thus defining the fundamental limit within which any true variation becomes undetectable. The absence of evidence for a variable IMF means that any true variation of the IMF in well-studied populations must be smaller than this scatter. Determinations of the power-law indices $\alpha$ are subject to systematic errors arising mostly from unresolved binaries. The systematic bias is quantified here, with the result that the single-star IMFs for young star clusters are systematically steeper by $\Delta$$\alpha${\textasciitilde}0.5 between 0.1 and 1Msolar than the Galactic-field IMF, which is populated by, on average, about 5-Gyr-old stars. The MFs in globular clusters appear to be, on average, systematically flatter than the Galactic-field IMF (Piotto \& Zoccali; Paresce \& De Marchi), and the recent detection of ancient white-dwarf candidates in the Galactic halo and the absence of associated low-mass stars (Ibata et al.; M{\'e}ndez \& Minniti) suggest a radically different IMF for this ancient population. Star formation in higher metallicity environments thus appears to produce relatively more low-mass stars. While still tentative, this is an interesting trend, being consistent with a systematic variation of the IMF as expected from theoretical arguments.},
	urldate = {2021-10-08},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Kroupa, Pavel},
	month = apr,
	year = {2001},
	note = {ADS Bibcode: 2001MNRAS.322..231K},
	keywords = {Astrophysics, BINARIES: GENERAL, GLOBULAR CLUSTERS: GENERAL, MASS FUNCTION, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION},
	pages = {231--246},
	file = {Full Text PDF:/Users/Tobin/Zotero/storage/PM6IXB3I/Kroupa - 2001 - On the variation of the initial mass function.pdf:application/pdf},
}

%%%%%%%%%%%%%%%%%%%
% Cliff's additions

@article{Kroupa01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.322..231K},
	Author = {{Kroupa}, P.},
	Date-Added = {2011-11-06 21:30:29 -0800},
	Date-Modified = {2011-11-06 21:30:29 -0800},
	Doi = {10.1046/j.1365-8711.2001.04022.x},
	Eprint = {arXiv:astro-ph/0009005},
	Journal = {\mnras},
	Keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GLOBULAR CLUSTERS: GENERAL, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL},
	Month = apr,
	Pages = {231-246},
	Title = {{On the variation of the initial mass function}},
	Volume = 322,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04022.x}
}

@ARTICLE{Elmegreen18,
       author = {{Elmegreen}, Bruce G.},
        title = "{Two Thresholds for Globular Cluster Formation and the Common Occurrence of Massive Clusters in the Early Universe}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: star clusters: general, galaxies: star formation, globular clusters: general, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = dec,
       volume = {869},
       number = {2},
          eid = {119},
        pages = {119},
          doi = {10.3847/1538-4357/aaed45},
archivePrefix = {arXiv},
       eprint = {1810.12940},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...869..119E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Elmegreen09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009Ap%26SS.324...83E},
	Author = {{Elmegreen}, B.~G.},
	Date-Added = {2015-07-12 01:52:44 +0000},
	Date-Modified = {2015-07-12 01:52:55 +0000},
	Doi = {10.1007/s10509-009-0131-6},
	Journal = {\apss},
	Keywords = {Star clusters, Molecular clouds, Turbulence, Star formation efficiency},
	Month = dec,
	Pages = {83-89},
	Title = {{A pressure dependence for bound and unbound clusters}},
	Volume = 324,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-009-0131-6}
}

@ARTICLE{emcee2013,
       author = {{Foreman-Mackey}, Daniel and {Hogg}, David W. and {Lang}, Dustin and {Goodman}, Jonathan},
        title = "{emcee: The MCMC Hammer}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Computational Physics, Statistics - Computation},
         year = 2013,
        month = mar,
       volume = {125},
       number = {925},
        pages = {306},
          doi = {10.1086/670067},
archivePrefix = {arXiv},
       eprint = {1202.3665},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PASP..125..306F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{corner2016,
      doi = {10.21105/joss.00024},
      url = {https://doi.org/10.21105/joss.00024},
      year  = {2016},
      month = {jun},
      publisher = {The Open Journal},
      volume = {1},
      number = {2},
      pages = {24},
      author = {Daniel Foreman-Mackey},
      title = {corner.py: Scatterplot matrices in Python},
      journal = {The Journal of Open Source Software}
}

